Contributing Components of Metabolic Energy Models to Metabolic Cost Estimations in Gait

Objective: As metabolic cost is a primary factor influencing humans' gait, we want to deepen our understanding of metabolic energy expenditure models. Therefore, this paper identifies the parameters and input variables, such as muscle or joint states, that contribute to accurate metabolic cost estimations. Methods: We explored the parameters of four metabolic energy expenditure models in a Monte Carlo sensitivity analysis. Then, we analysed the model parameters by their calculated sensitivity indices, physiological context, and the resulting metabolic rates during the gait cycle. The parameter combination with the highest accuracy in the Monte Carlo simulations represented a quasi-optimized model. In the second step, we investigated the importance of input parameters and variables by analysing the accuracy of neural networks trained with different input features. Results: Power-related parameters were most influential in the sensitivity analysis and the neural network-based feature selection. We observed that the quasi-optimized models produced negative metabolic rates, contradicting muscle physiology. Neural network-based models showed promising abilities but have been unable to match the accuracy of traditional metabolic energy expenditure models. Conclusion: We showed that power-related metabolic energy expenditure model parameters and inputs are most influential during gait. Furthermore, our results suggest that neural network-based metabolic energy expenditure models are viable. However, bigger datasets are required to achieve better accuracy. Significance: As there is a need for more accurate metabolic energy expenditure models, we explored which musculoskeletal parameters are essential when developing a model to estimate metabolic energy.

==> plots/all/GastrocnemiusFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 0.844753671125167
1 0.780335636891916
2 0.682885563141999
3 0.472000428911296
4 0.289589154979955
5 0.172900509750404
6 0.100857177308073
7 0.0573791701749404
8 0.0317191868869399
9 0.016928565255424
10 0.00862687824527201
11 0.00409280244677169
12 -0.0034384616528089
13 -0.014424782996813
14 -0.0189347466812424
15 -0.0163018449593193
16 -0.0121532372419504
17 -0.00871332556575995
18 -0.00623903858233853
19 -0.00445823570264854
20 -0.00318435012925675
21 -0.00242533393845148
22 -0.0021372701481374
23 -0.0022274495347292
24 -0.00230527082435992
25 0.0158665472536293
26 0.26502824001677
27 0.829499359314652
28 1.45892585720535
29 1.95055444358517
30 1.9709471116978
31 1.50024063643477
32 0.773108373043768
33 0.0610607427425379
34 -0.416539409997163
35 -0.638025331110662
36 -0.811756599208411
37 -1.19781514352547
38 -1.94541302226667
39 -3.06135603210735
40 -4.38522791880938
41 -5.7630052433869
42 -7.18227802082709
43 -8.73620536941587
44 -10.4840724030962
45 -12.3220418503314
46 -13.9060582192875
47 -14.7058143511542
48 -14.215750631503
49 -12.0043332532902
50 -7.82279832867811
51 -1.73186588029257
52 7.27273013955952
53 20.1652017054656
54 33.5196678085323
55 45.6347433570328
56 57.9400062522837
57 68.4251326905794
58 75.2284607877938
59 77.9305296600302
60 74.9692489177309
61 66.3088887589238
62 56.9197169184507
63 44.1429018194206
64 29.0577361881774
65 20.0705087966184
66 13.5273200433949
67 8.78676852615611
68 5.3603905020841
69 2.89755986632119
70 1.1785522223868
71 0.0642204890538483
72 -0.559541783667726
73 -0.787332449201799
74 -0.773025088921619
75 -0.677835787075488
76 -0.564252455079604
77 -0.454797559492304
78 -0.360026177273006
79 -0.279802856454854
80 -0.213769090634424
81 -0.161539853939668
82 -0.119933548146572
83 -0.0872095419206725
84 -0.0627369918527558
85 -0.0439804621132342
86 -0.104850466712002
87 -0.727313540932754
88 -1.83924899345851
89 -2.90143056257755
90 -3.62590617094353
91 -3.77469496158761
92 -3.89302607394487
93 -3.87537081752489
94 -3.0748244593844
95 -2.14063779519554
96 -2.12198911453445
97 -2.24784616507294
98 -2.03109349585919
99 -1.486322208431
};
\addplot [semithick, color1]
table {%
0 1.03664496750001
1 0.911185471281044
2 0.775405822870654
3 0.538620017611708
4 0.338507006725227
5 0.209312807756492
6 0.128116701471925
7 0.077787427750457
8 0.0469460293325769
9 0.0282292590296796
10 0.0169616826546827
11 0.0102137649443775
12 0.00168652213852069
13 -0.00915491831360002
14 -0.0140078514092139
15 -0.012423140536453
16 -0.00933825300918748
17 -0.00672916165040059
18 -0.00486280077575104
19 -0.00354584970288316
20 -0.00266654484172778
21 -0.00229780787465913
22 -0.00263020335719822
23 -0.0042935069978168
24 -0.00863375136704217
25 -0.0172252508389188
26 0.0200762284907159
27 0.226536006880878
28 0.537287271899314
29 0.770995506372714
30 0.72488187816985
31 0.346830672974738
32 -0.247073052436049
33 -0.857871826903356
34 -1.3184112807437
35 -1.61806641627684
36 -1.89921611229621
37 -2.33938737333833
38 -3.03754472283558
39 -3.96261357845971
40 -5.00936652762284
41 -6.08514462763103
42 -7.18019046262947
43 -8.36028641831312
44 -9.66981512496934
45 -11.0228942908485
46 -12.1314547343736
47 -12.5647142536968
48 -11.9088952953988
49 -9.80791552396465
50 -6.08300793140226
51 -0.81291355805839
52 7.04891349088926
53 18.6579738282325
54 31.5239450145998
55 43.9928638818552
56 56.7352214019156
57 68.0385218391212
58 76.1062145030913
59 80.3105276292354
60 79.0464202721651
61 71.7971236541499
62 62.3961496781258
63 49.7430644392581
64 34.7410801686859
65 23.6425656484777
66 15.5957221464161
67 9.89888952967671
68 5.94291061985658
69 3.23347395942757
70 1.42686483218628
71 0.298224787622668
72 -0.31721449087225
73 -0.560152091002177
74 -0.580530317704674
75 -0.52185706499841
76 -0.440823841843958
77 -0.358744323817521
78 -0.286018076639237
79 -0.223432608280989
80 -0.171331419926587
81 -0.129847745609366
82 -0.0965724134379303
83 -0.0702569926547063
84 -0.0505477492479257
85 -0.0353993952600936
86 -0.154565749029429
87 -1.0913106409835
88 -2.00971529608493
89 -2.88679250851705
90 -3.42966765723746
91 -3.54867685816315
92 -3.76452564418365
93 -3.65991076721174
94 -2.99258074902777
95 -2.38878341893154
96 -2.31396670348002
97 -2.01581332529108
98 -1.6987576903056
99 -0.782625595031585
};
\addplot [semithick, color2]
table {%
0 1.62469141093767
1 1.3388596780281
2 1.08751759355295
3 0.761202532310655
4 0.495586060161672
5 0.32036386685607
6 0.206812302745842
7 0.133685733339471
8 0.0867458819333469
9 0.0566386160849176
10 0.0372979103842422
11 0.0248124989741332
12 0.00506770538023192
13 -0.00324176944396418
14 -0.00622425158127442
15 -0.00568808713624014
16 -0.00428496038842472
17 -0.00306955193535271
18 -0.00219567004686788
19 -0.00157076199768742
20 -0.00113669277644113
21 -0.000920894985311651
22 -0.000973672585237522
23 -0.00145153189438735
24 -0.00258598880335419
25 -0.00159073194730821
26 0.0639099792188987
27 0.666616654125679
28 1.67438375193941
29 2.20047525318072
30 1.58604525925063
31 0.996731980434157
32 0.671707081340468
33 0.429406143885951
34 0.284768499578778
35 0.236828630856583
36 0.20933269741665
37 0.102831651381623
38 -0.142866655304085
39 -0.530262527233881
40 -1.00057623571979
41 -1.49558004142619
42 -2.00885086108492
43 -2.57615939744862
44 -3.22354440150407
45 -3.90903574654455
46 -4.48478820272512
47 -4.72559358438085
48 -4.41337053307316
49 -3.35831473806268
50 -1.45431008861493
51 1.7821713701362
52 12.3150183894586
53 29.0162648670572
54 44.0122016443433
55 58.2298154124639
56 72.5786806872549
57 85.081936909608
58 93.7221469822575
59 97.9210267260702
60 95.8712280600073
61 86.9128008052531
62 75.5084811316196
63 60.9052417820448
64 43.7764424923076
65 29.9302166765472
66 19.8915423302614
67 12.7989220301679
68 7.89318484279402
69 4.54906540486136
70 2.32180328402664
71 0.840268803340696
72 -0.0693495958013546
73 -0.224823798639971
74 -0.255092474003186
75 -0.238189021804553
76 -0.20560679019965
77 -0.169687111142643
78 -0.136671920692628
79 -0.107552833278691
80 -0.0829096920565336
81 -0.0630887262361209
82 -0.0470428783948696
83 -0.0342633319021284
84 -0.0246598458961465
85 -0.017244080194815
86 -0.0728983225802954
87 -0.514248534535736
88 -0.953847946814798
89 -1.37801563275505
90 -1.63851635767055
91 -1.68044782022259
92 -1.75933023837476
93 -1.68198914132763
94 -1.30712274278591
95 -0.937631474643335
96 -0.855076829571789
97 -0.711201049647264
98 -0.573600768174922
99 -0.182306617914913
};
\addplot [semithick, color3]
table {%
0 1.46398411501418
1 1.25338339834025
2 1.04891697279798
3 0.801735506112992
4 0.592773629802389
5 0.441971919396825
6 0.333841818171695
7 0.255843790054544
8 0.198957836252516
9 0.156885514133191
10 0.125296218509245
11 0.10109967944921
12 0.0788946965949076
13 0.0575080069395181
14 0.0429284197027211
15 0.0355074198558233
16 0.0311584218220846
17 0.0281249119658166
18 0.0262223667265488
19 0.0259857845378089
20 0.0284573004528105
21 0.0372726418732944
22 0.0580289164793598
23 0.101352374634031
24 0.183646757343952
25 0.444258045706827
26 1.34468216066657
27 2.33985962036595
28 3.14945600174372
29 3.77882782327264
30 4.12729777457593
31 4.171023862839
32 4.03042436568033
33 3.85819416926933
34 3.79503244556248
35 3.87560871379345
36 3.97918775182653
37 3.95348673999564
38 3.70921057864631
39 3.28374142965673
40 2.76049135359325
41 2.20759261529739
42 1.63342470982819
43 0.974179245117077
44 0.179382047117807
45 -0.721732069159926
46 -1.58067841785124
47 -2.10975181090692
48 -1.94562104850531
49 -0.854719372141076
50 1.24941231358775
51 4.2623886236798
52 9.87220798434324
53 19.5470902623999
54 29.4631869614346
55 37.6439990431698
56 45.397906258026
57 50.9797358479737
58 53.1644913968595
59 52.0469601339939
60 47.2664724576128
61 39.5468164516452
62 32.6068675871023
63 25.383353339533
64 17.768853655711
65 13.2366019544844
66 9.89835743660303
67 7.28048334326332
68 5.13801853863154
69 3.38011749611823
70 1.99406370564864
71 1.00550186299723
72 0.415781947484749
73 0.119759040563324
74 0.00728944460821773
75 -0.0288148492377475
76 -0.0336430432116033
77 -0.0256003921839839
78 -0.0147136389894075
79 -0.00329120637286663
80 0.0069165269093835
81 0.0144901018083087
82 0.0202504935645583
83 0.0243157332974966
84 0.0263014667377017
85 0.0274262397748876
86 0.3238015608159
87 2.04143070130774
88 1.42455637905543
89 0.832830233715755
90 0.207829931483237
91 0.144356450032463
92 0.565639506539418
93 0.295398562264516
94 0.787056639063526
95 1.76391315672323
96 1.68294485773807
97 0.859098170827483
98 0.7803389379165
99 0.300431085888196
};
\addplot [semithick, color4]
table {%
0 2.4276549216962
1 2.20607865510656
2 1.89224776971734
3 1.31354529881035
4 0.817650035335976
5 0.493895645249056
6 0.290543157073069
7 0.166160473820465
8 0.0919796028429693
9 0.0488718934957426
10 0.0245242660011322
11 0.0112137758199464
12 0.00415242339367766
13 0.010572867411937
14 0.0138000769522679
15 0.0118938284008071
16 0.00890780730032141
17 0.00644284277654295
18 0.00468958386450974
19 0.00346824114917647
20 0.00268233475518535
21 0.00240858953683166
22 0.00288812360646262
23 0.00493509322232673
24 0.0104528848515767
25 0.0266930304176907
26 0.0574235460997527
27 0.0275233861336561
28 0.125429756799069
29 0.0880289968626618
30 0.317089689613741
31 0.860167546591051
32 1.5580459112708
33 2.25472016201946
34 2.8268971151292
35 3.2829720348295
36 3.74640370797087
37 4.35569366436971
38 5.17580438008646
39 6.17015767562553
40 7.24825057302425
41 8.33435746796173
42 9.42185581554001
43 10.5608135940797
44 11.7787908462131
45 12.9927479684959
46 13.9504280938177
47 14.2888949359929
48 13.6670270403796
49 11.7990497680587
50 8.57055202374962
51 4.10995268868147
52 12.6356659161724
53 41.9341773816067
54 75.3749829222209
55 105.298006861363
56 132.947889263778
57 153.701596296454
58 163.03719637687
59 160.114305128649
60 144.905620769962
61 120.56082528012
62 97.8920373459971
63 76.5797591448011
64 55.0521577633916
65 40.0196762179242
66 29.1184061192497
67 20.6070395249682
68 13.6161443704182
69 7.86351962936489
70 3.35909777543454
71 0.693242999059023
72 0.403092306075826
73 0.567145829098798
74 0.55682890486946
75 0.488263323381161
76 0.406450516043683
77 0.327614906933469
78 0.259359826600969
79 0.201587922886256
80 0.154039764976999
81 0.116434337091344
82 0.0864763528152116
83 0.0629129347661307
84 0.0452949962576791
85 0.0318056250916965
86 0.144433910847333
87 1.020937570824
88 1.86569422969864
89 2.66225442231622
90 3.1584275138983
91 3.29839153633701
92 3.54605377302905
93 3.50223255187458
94 2.99543509861712
95 2.59299255397171
96 2.61102892897319
97 2.33267595788884
98 2.00853998847143
99 1.07085255765231
};
\addplot [semithick, color5]
table {%
0 1.32871251497389
1 1.1436512529841
2 0.981462300552534
3 0.672672984146803
4 0.416245362461717
5 0.258603104956525
6 0.162945647173715
7 0.104400358194274
8 0.0680568190306824
9 0.0451174283810069
10 0.0303883948133359
11 0.0207628757668599
12 0.0121334346651599
13 0.00562411084966396
14 0.00307901043584332
15 0.00212781625485023
16 0.00156549545240042
17 0.00117657593708614
18 0.000914682590083962
19 0.000762527254713417
20 0.000732464367103962
21 0.000864331070218825
22 0.00133549250858593
23 0.00280446303633076
24 0.0072047714116933
25 0.0321983252183818
26 0.244850637014271
27 0.801584245313701
28 1.60291543738354
29 2.48734679099665
30 3.21356325942362
31 3.70143117310129
32 4.03638982850254
33 4.34285443759168
34 4.72569066201041
35 5.22679673503916
36 5.79937122008293
37 6.34873226542909
38 6.79434183989533
39 7.12800615212001
40 7.38755610416855
41 7.61148663824804
42 7.8078919807229
43 7.94730452653143
44 7.99886198177803
45 7.96260499899835
46 7.87816858979987
47 7.82334512021604
48 7.89108917629645
49 8.23147338414032
50 9.15512183983629
51 11.2614287680707
52 16.4795211864478
53 28.2988256364053
54 44.9782807514151
55 63.2357490829129
56 82.6980351123926
57 99.4870080036866
58 109.804469927807
59 112.398517468383
60 106.26944757586
61 92.8115796866995
62 78.574528489754
63 62.37791977654
64 44.3795895328893
65 31.3673477797512
66 21.8093647530231
67 14.5770661436787
68 8.95677452243475
69 4.76716310248917
70 2.15126107551769
71 0.89565179110471
72 0.384489300967011
73 0.197447684942518
74 0.125112884544593
75 0.0880638290517436
76 0.065094145576806
77 0.0490992157514622
78 0.0373408480404687
79 0.028317497988962
80 0.0212884425539974
81 0.0159012000397383
82 0.0116955564055131
83 0.00843238289004237
84 0.00602474828895599
85 0.00421261626992712
86 0.0213334803791861
87 0.15113892760798
88 0.265002732477991
89 0.367577202207872
90 0.43549010177463
91 0.476770689271608
92 0.556653537705907
93 0.617988885757391
94 0.73527803656539
95 1.02835245992229
96 1.24091386821982
97 1.23654173084958
98 1.16166805121053
99 0.9387180302467
};
\addplot [semithick, black]
table {%
0 0.606913730424049
1 0.551519663776641
2 0.473061942429336
3 0.328386324702587
4 0.204412508833994
5 0.123473911312264
6 0.0726357892682672
7 0.0415401184551162
8 0.0229949007107423
9 0.0122179733739356
10 0.00613106650028305
11 0.00280344395498661
12 -0.00326861934546164
13 -0.0126874408943244
14 -0.0165600923427215
15 -0.0142725940809685
16 -0.0106893687603857
17 -0.00773141133185154
18 -0.00562750063741168
19 -0.00416188937901176
20 -0.00321880170622242
21 -0.00289030744419799
22 -0.00346574832775514
23 -0.00592211186679207
24 -0.012543461821892
25 -0.0320316365012288
26 -0.0689082553197033
27 -0.0330280633603874
28 0.0260361164599118
29 -0.0345236446526237
30 -0.380507627536489
31 -1.03220105590926
32 -1.86965509352496
33 -2.70566419442335
34 -3.39227653815503
35 -3.9395664417954
36 -4.49568444956504
37 -5.22683239724365
38 -6.21096525610375
39 -7.40418921075063
40 -8.6979006876291
41 -10.0012289615541
42 -11.306226978648
43 -12.6729763128957
44 -14.1345490154557
45 -15.591297562195
46 -16.7405137125812
47 -17.1466739231915
48 -16.4004324484555
49 -14.1588597216704
50 -10.2846624284995
51 -4.93194322641776
52 2.01447792810318
53 10.4835443454017
54 18.8437457305552
55 26.3245017153408
56 33.2369723159446
57 38.4253990741134
58 40.7592990942176
59 40.0285762821621
60 36.2264051924906
61 30.1402063200301
62 24.4730093364993
63 19.1449397862003
64 13.7630394408479
65 10.0049190544811
66 7.27960152981243
67 5.15175988124206
68 3.40403609260456
69 1.96587990734122
70 0.839774443858635
71 0.0302445539531225
72 -0.483710767290991
73 -0.680574994918557
74 -0.668194685843352
75 -0.585915988057394
76 -0.487740619252419
77 -0.393137888320162
78 -0.311231791921163
79 -0.241905507463507
80 -0.184847717972398
81 -0.139721204509613
82 -0.103771623378254
83 -0.0754955217193569
84 -0.0543539955092149
85 -0.0381667501100358
86 -0.1733206930168
87 -1.2251250849888
88 -2.23883307563837
89 -3.19470530677946
90 -3.79011301667797
91 -3.95806984360441
92 -4.25526452763485
93 -4.20267906224949
94 -3.59452211834055
95 -3.11159106476605
96 -3.13323471476783
97 -2.79921114946661
98 -2.41024798616572
99 -1.28502306918277
};


==> plots/all/GastrocnemiusTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 1.22379602882288
1 1.11654209509586
2 0.962523734653257
3 0.667966043599958
4 0.414531121125094
5 0.249892860165182
6 0.146911159697263
7 0.0841191088869386
8 0.0467574399030685
9 0.0250821210039153
10 0.0128531311372429
11 0.00614266423141303
12 -0.00456505089741036
13 -0.0196491262853633
14 -0.0258222668904299
15 -0.0222176696562325
16 -0.0165327147613866
17 -0.0118096858276465
18 -0.00839434736677945
19 -0.0058990229417692
20 -0.00403254902548257
21 -0.00273473304039449
22 -0.00167629000627155
23 0.000165445129759553
24 0.00564463377748228
25 0.0610990425208379
26 0.620781673927084
27 1.77805804536149
28 3.04284618706419
29 4.10752568375375
30 4.42798315448268
31 3.98894265408687
32 3.1816443900391
33 2.41627044964057
34 2.02531061510563
35 2.06008914036019
36 2.20965603155735
37 2.07247586753297
38 1.40603967721751
39 0.29555604732491
40 -1.03742674373629
41 -2.41293653783573
42 -3.81422293395807
43 -5.40136783942655
44 -7.29766744345854
45 -9.4071997990301
46 -11.313316777706
47 -12.2979608849643
48 -11.6644931746077
49 -8.79497017561616
50 -3.16726549028949
51 5.44889484994616
52 19.7333221126653
53 43.3205595573029
54 66.4701197592206
55 83.7391800814908
56 100.344597435614
57 111.467885251026
58 114.390675882879
59 110.186618531437
60 98.1732084365808
61 79.9532826218347
62 65.054886400936
63 48.6865793851438
64 31.2242397097206
65 22.3290624660789
66 15.8692590040923
67 10.9546927649255
68 7.08201955279189
69 4.0204756904495
70 1.69674110537783
71 0.110448838957324
72 -0.765430154823481
73 -1.07704382169438
74 -1.05747294786213
75 -0.927256658491837
76 -0.771877634968442
77 -0.622145708461326
78 -0.492499764587398
79 -0.382754390767731
80 -0.292419270129641
81 -0.220968257989401
82 -0.164049663917447
83 -0.119282280012347
84 -0.0858021944548757
85 -0.0601391521571383
86 -0.129731504245551
87 -0.893294629644194
88 -2.38311438717544
89 -3.7999724701669
90 -4.76730535594234
91 -4.92478951928842
92 -4.98223644991044
93 -4.933571752159
94 -3.76495889760891
95 -2.30202496459446
96 -2.22776402582728
97 -2.6028217638718
98 -2.4013179243378
99 -2.03301559162246
};
\addplot [semithick, color1]
table {%
0 1.60428182426596
1 1.32171980198979
2 1.07503532372369
3 0.755906634790639
4 0.494949111222899
5 0.321694470717536
6 0.208756884457034
7 0.135628963605131
8 0.0884437621515421
9 0.0580253842393468
10 0.0383869728446671
11 0.025646731523992
12 0.0128202572653366
13 -0.00111858124811494
14 -0.00822083107964275
15 -0.00825045779797847
16 -0.00630828066991644
17 -0.00449687271695182
18 -0.00317224953479477
19 -0.00219473467707566
20 -0.00146487697527681
21 -0.00101806429870936
22 -0.000837780816058947
23 -0.000821797796305921
24 -0.000347771823367739
25 0.0139936210137152
26 0.207728776724756
27 0.776775564358461
28 1.61508773649831
29 2.50095794350667
30 3.12600664473841
31 3.36156529889808
32 3.31709240300703
33 3.21576956481896
34 3.26839097021041
35 3.5347359273475
36 3.88755381154538
37 4.12349762822262
38 4.09282815058144
39 3.79397126768123
40 3.32198064952179
41 2.7723648488227
42 2.15824226739123
43 1.3985528200933
44 0.419306790313286
45 -0.729447015052529
46 -1.79675364102541
47 -2.36211683019428
48 -1.99635130196005
49 -0.304099250625576
50 3.00305230593757
51 8.0363572188907
52 16.303923441955
53 30.1355751827899
54 46.3836992846883
55 62.036297184152
56 77.96350064673
57 91.799963429905
58 101.098327541841
59 105.262176409043
60 102.494794074937
61 92.206618997282
62 79.546852064858
63 62.9818906502329
64 43.589688327739
65 29.4264093644329
66 19.2997049869014
67 12.2453761108747
68 7.43516261491065
69 4.20026316168794
70 2.07191630053805
71 0.74323818879987
72 0.000586128080309639
73 -0.327752311218636
74 -0.408531034083025
75 -0.393735902719927
76 -0.345065258012236
77 -0.287121002228902
78 -0.232495791798725
79 -0.183517304196292
80 -0.141660248508925
81 -0.107874447586523
82 -0.0803660381500477
83 -0.0583574213802312
84 -0.0418441846138915
85 -0.029043684382826
86 -0.111281573585265
87 -0.782289167136921
88 -1.4799201360776
89 -2.17481899232056
90 -2.59769363896877
91 -2.60648450890767
92 -2.63813926947073
93 -2.41889739611844
94 -1.62127201984264
95 -0.744096013397644
96 -0.451834205990363
97 -0.243019579943196
98 -0.0964480326249768
99 0.338915127112474
};
\addplot [semithick, color2]
table {%
0 2.09460252106024
1 1.66864964778379
2 1.31880985701267
3 0.92912363975269
4 0.61893438609913
5 0.410532420512711
6 0.272449750084074
7 0.181323103317499
8 0.1212524003935
9 0.0816093232776815
10 0.0553677228040764
11 0.0378955220488819
12 0.00516611304783371
13 -0.00951098654915367
14 -0.0136499640134468
15 -0.0118896128465368
16 -0.00891477522907838
17 -0.00643719978853879
18 -0.00467134024493486
19 -0.0034350684422541
20 -0.00262736091890915
21 -0.00232112575773965
22 -0.00273182090141584
23 -0.00458039888719246
24 -0.00948583205625147
25 -0.0213390978696531
26 0.0550822109168461
27 1.09307811318094
28 2.65993117720134
29 3.6583562941098
30 2.54476592939936
31 0.866103222783688
32 -0.405504475030962
33 -1.30720408150085
34 -1.90606012016608
35 -2.30196244917477
36 -2.68144483953994
37 -3.23455722127901
38 -4.04557632465966
39 -5.05945683866263
40 -6.16164133262408
41 -7.26591323581558
42 -8.36819908895923
43 -9.52832559445477
44 -10.7808388824197
45 -12.0410092518685
46 -13.0449129953
47 -13.4092635674259
48 -12.7701060588684
49 -10.8065494180505
50 -7.25936680101919
51 0.574409237973525
52 18.139746117679
53 39.5128444715146
54 56.4442780073305
55 72.1768900807714
56 87.7814596495961
57 100.961863501253
58 109.412162501498
59 112.659910801361
60 109.00521762296
61 97.927092235654
62 84.6256771065353
63 67.4681911607652
64 47.3614450166611
65 32.5394564473611
66 21.8292022984206
67 14.2591580125433
68 9.00045826012224
69 5.38853530120867
70 2.95509890489012
71 1.12935066084225
72 -0.347642583007187
73 -0.550665029292085
74 -0.553349764284244
75 -0.490483487735718
76 -0.410950059368731
77 -0.332671142109281
78 -0.264206420923412
79 -0.205831948594235
80 -0.157542710300765
81 -0.119232313771038
82 -0.0886195762830731
83 -0.064483174112353
84 -0.0464199974994817
85 -0.0325667051846334
86 -0.145803394553613
87 -1.03021886637192
88 -1.88805868884189
89 -2.70069722763788
90 -3.20553811360012
91 -3.33598667128577
92 -3.56862162772073
93 -3.50361565238892
94 -2.94679880536021
95 -2.47569490577222
96 -2.45688070911183
97 -2.1730092229515
98 -1.85433394076697
99 -0.928020035885876
};
\addplot [semithick, color3]
table {%
0 0.700493277657715
1 0.610063384855314
2 0.509752663188075
3 0.351463357256912
4 0.218886731963192
5 0.13255594949158
6 0.0783403495732268
7 0.0451290403272443
8 0.0252581062893918
9 0.0136499333936834
10 0.00704132091401353
11 0.0033840960569439
12 -0.00288998773643002
13 -0.0124270368585182
14 -0.0163785737198747
15 -0.0141475709455553
16 -0.0106024169193377
17 -0.00766865893111175
18 -0.00557879692310532
19 -0.00411884583892225
20 -0.00317135356674525
21 -0.00281029197210663
22 -0.00325650362672316
23 -0.00518459481291425
24 -0.00967466744946731
25 -0.00923605114895475
26 0.243393667021364
27 1.01896712158091
28 2.03481967619782
29 3.07087867625404
30 3.60098980238074
31 3.57131108118095
32 3.29307377919628
33 3.07085645396413
34 3.16426805379183
35 3.64788851057557
36 4.29440218634597
37 4.77686703848641
38 4.86876772666564
39 4.62558113541689
40 4.21111780835123
41 3.7580422186786
42 3.27780316512334
43 2.62748457512129
44 1.68287107983638
45 0.463605045473169
46 -0.807508228951309
47 -1.65805799132359
48 -1.48391550901931
49 0.112775004884825
50 3.41702628958659
51 8.71360800121699
52 18.0586206556264
53 35.818743994492
54 52.7756520288932
55 63.3883621428244
56 73.9389469829575
57 79.5720917161359
58 79.0288231692025
59 74.3867982550655
60 64.6080677186401
61 50.5365917713061
62 39.4264483959909
63 28.0125229914631
64 17.0612845565734
65 12.0613743444063
66 8.53922623771021
67 5.92510477461715
68 3.88032323226821
69 2.26018287494854
70 1.02216659696271
71 0.143796516492853
72 -0.412231907972331
73 -0.635402921748744
74 -0.639663696405228
75 -0.567879219670997
76 -0.476319315737189
77 -0.385890300030541
78 -0.306618537110686
79 -0.238959248827337
80 -0.182958809642577
81 -0.138504116568152
82 -0.102984281847748
83 -0.0749844076641057
84 -0.0540197430586765
85 -0.0379458135547098
86 -0.109287552421443
87 -0.758930394633964
88 -1.69800763261079
89 -2.58706681097999
90 -3.1948051029146
91 -3.2861325238714
92 -3.28650422969196
93 -3.25784943180929
94 -2.4915229487615
95 -1.4402146595133
96 -1.36282805315128
97 -1.69852495976041
98 -1.53298862776457
99 -1.04078186515815
};
\addplot [semithick, color4]
table {%
0 2.36470883760201
1 2.14887776905736
2 1.84318412966901
3 1.2794866967819
4 0.796449383042316
5 0.481089543137196
6 0.283009733012398
7 0.161852138618143
8 0.089594685710077
9 0.0476047058529141
10 0.0238883821709143
11 0.0109230165075469
12 -0.000406227878875452
13 -0.0055454503110026
14 -0.00723811602332331
15 -0.00623829201998703
16 -0.00467212921899952
17 -0.0033792596735473
18 -0.00245967846627465
19 -0.00181908636607117
20 -0.00140687984846588
21 -0.00126330096422289
22 -0.00151481573802673
23 -0.00258844769146356
24 -0.0054825196696977
25 -0.0140004473776207
26 -0.0301185486558
27 -0.0144359674862097
28 0.116677951843863
29 0.0273220506198385
30 -0.166312982975552
31 -0.451156361175233
32 -0.81719233265502
33 -1.18259674850155
34 -1.48270255130284
35 -1.72191304234116
36 -1.96498213758478
37 -2.28455364515783
38 -2.71470026918467
39 -3.23623681902998
40 -3.80169464236555
41 -4.37135579327652
42 -4.9417467586436
43 -5.53912810479488
44 -6.17795502548541
45 -6.81467339515932
46 -7.31697493190335
47 -7.49450019369615
48 -7.16833157918785
49 -6.18858079426432
50 -4.49523942122898
51 -2.15566293680393
52 11.1252658733535
53 40.8468761213275
54 73.4206030096487
55 102.56776001466
56 129.500715226417
57 149.716304350954
58 158.809843888713
59 155.962739588902
60 141.148397571068
61 117.434832463462
62 95.3538181123397
63 74.594140877575
64 53.6247235258601
65 38.9820156006255
66 28.3634019282132
67 20.072724523574
68 13.2630946181989
69 7.65962830879761
70 3.27200053226236
71 0.527409698783994
72 -0.211421203633672
73 -0.297466987130559
74 -0.292055778567442
75 -0.256093252000706
76 -0.213182578839195
77 -0.171833440897227
78 -0.136033771639101
79 -0.105732510028626
80 -0.0807935850622731
81 -0.061069604458067
82 -0.045356694539843
83 -0.0329977233301
84 -0.023757145653829
85 -0.0166819942674442
86 -0.0757553315123745
87 -0.53547995534761
88 -0.978553333094589
89 -1.39634774929017
90 -1.6565896607624
91 -1.73000054368765
92 -1.85989895004966
93 -1.83691479683828
94 -1.57110042640469
95 -1.36002002149534
96 -1.36948006837424
97 -1.22348442595036
98 -1.05347568164477
99 -0.561660277907807
};
\addplot [semithick, color5]
table {%
0 1.68306146868475
1 1.44387422208733
2 1.21696502196947
3 0.838343808269522
4 0.52550357700818
5 0.327798859156587
6 0.205036170143873
7 0.128975380686964
8 0.0817845804699398
9 0.0523898694653926
10 0.033968551104545
11 0.0223189895833499
12 0.00975905700550415
13 -0.00416981617331956
14 -0.010985097063636
15 -0.0104642813818763
16 -0.00796714023441097
17 -0.00571778067048183
18 -0.00408050869692784
19 -0.00288609671339812
20 -0.00202258594768751
21 -0.00154333548604572
22 -0.00149167749528436
23 -0.00196212461616306
24 -0.00278759791010219
25 0.00736965249934901
26 0.191360839016886
27 0.767091077123858
28 1.59999818630836
29 2.42946969721603
30 2.89719219970156
31 2.90090338742333
32 2.60163958245001
33 2.25990806308732
34 2.10062590401828
35 2.16537319882797
36 2.29185455823597
37 2.24911225597397
38 1.88567685825653
39 1.2190225988815
40 0.369176719414527
41 -0.551821755685257
42 -1.53110148721623
43 -2.65770550632403
44 -4.00441827978988
45 -5.49108347628098
46 -6.78990871037563
47 -7.37310146531298
48 -6.70303617766444
49 -4.28246838626878
50 0.231513231521808
51 7.02133385389584
52 17.7414706858981
53 35.2872065433299
54 56.4060730103708
55 77.4834075082839
56 98.9816534641023
57 117.267561215329
58 128.576177700622
59 131.299028391172
60 123.487601254017
61 106.483747584431
62 88.8189021906379
63 70.1359443615015
64 50.2322082625779
65 35.985279503449
66 25.3539929664109
67 17.0505468946692
68 10.5629118687191
69 5.79826619478932
70 2.68140864527227
71 0.898730489666408
72 -0.0353825700135153
73 -0.43496816602027
74 -0.526913396570674
75 -0.501271536879606
76 -0.434694871580427
77 -0.358006096779065
78 -0.286876824084913
79 -0.224097963184888
80 -0.171269264563379
81 -0.129218921739157
82 -0.0954996118242951
83 -0.0689166061296098
84 -0.0491981566030387
85 -0.0340979974875141
86 -0.135593427635901
87 -0.954859661610181
88 -1.79134516212042
89 -2.61705335040792
90 -3.12829336902453
91 -3.18147937184331
92 -3.28808807542737
93 -3.09726337273033
94 -2.28000163181427
95 -1.43749132107976
96 -1.20646874520206
97 -0.93732807463048
98 -0.703261477787094
99 -0.030218953943336
};
\addplot [semithick, black]
table {%
0 0.606913730424049
1 0.551519663776641
2 0.473061942429336
3 0.328386324702587
4 0.204412508833994
5 0.123473911312264
6 0.0726357892682672
7 0.0415401184551162
8 0.0229949007107423
9 0.0122179733739356
10 0.00613106650028305
11 0.00280344395498661
12 -0.00326861934546164
13 -0.0126874408943244
14 -0.0165600923427215
15 -0.0142725940809685
16 -0.0106893687603857
17 -0.00773141133185154
18 -0.00562750063741168
19 -0.00416188937901176
20 -0.00321880170622242
21 -0.00289030744419799
22 -0.00346574832775514
23 -0.00592211186679207
24 -0.012543461821892
25 -0.0320316365012288
26 -0.0689082553197033
27 -0.0330280633603874
28 0.0260361164599118
29 -0.0345236446526237
30 -0.380507627536489
31 -1.03220105590926
32 -1.86965509352496
33 -2.70566419442335
34 -3.39227653815503
35 -3.9395664417954
36 -4.49568444956504
37 -5.22683239724365
38 -6.21096525610375
39 -7.40418921075063
40 -8.6979006876291
41 -10.0012289615541
42 -11.306226978648
43 -12.6729763128957
44 -14.1345490154557
45 -15.591297562195
46 -16.7405137125812
47 -17.1466739231915
48 -16.4004324484555
49 -14.1588597216704
50 -10.2846624284995
51 -4.93194322641776
52 2.01447792810318
53 10.4835443454017
54 18.8437457305552
55 26.3245017153408
56 33.2369723159446
57 38.4253990741134
58 40.7592990942176
59 40.0285762821621
60 36.2264051924906
61 30.1402063200301
62 24.4730093364993
63 19.1449397862003
64 13.7630394408479
65 10.0049190544811
66 7.27960152981243
67 5.15175988124206
68 3.40403609260456
69 1.96587990734122
70 0.839774443858635
71 0.0302445539531225
72 -0.483710767290991
73 -0.680574994918557
74 -0.668194685843352
75 -0.585915988057394
76 -0.487740619252419
77 -0.393137888320162
78 -0.311231791921163
79 -0.241905507463507
80 -0.184847717972398
81 -0.139721204509613
82 -0.103771623378254
83 -0.0754955217193569
84 -0.0543539955092149
85 -0.0381667501100358
86 -0.1733206930168
87 -1.2251250849888
88 -2.23883307563837
89 -3.19470530677946
90 -3.79011301667797
91 -3.95806984360441
92 -4.25526452763485
93 -4.20267906224949
94 -3.59452211834055
95 -3.11159106476605
96 -3.13323471476783
97 -2.79921114946661
98 -2.41024798616572
99 -1.28502306918277
};


==> plots/all/GlutealsFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 75.4552915765271
1 91.6855504248945
2 82.7397690593801
3 84.0685056799989
4 88.6146189662493
5 88.0188390485033
6 77.4200489668944
7 62.7062848964068
8 51.5495328216187
9 48.4401501752169
10 53.0163797484152
11 62.3281026253104
12 73.6448653984488
13 84.0904959656628
14 92.4472960325368
15 93.3301831623582
16 86.0383689860541
17 76.027397592003
18 65.8757360685227
19 57.9684759395622
20 52.1334901667763
21 47.6971758958281
22 43.9377174134057
23 40.0026083960155
24 36.1870315525843
25 35.3071136007987
26 33.3504263304274
27 31.4766715541238
28 30.2965423548003
29 29.8383757112878
30 28.8154403049233
31 26.9177031297912
32 24.7398713363562
33 22.5098893531562
34 20.6217155776109
35 19.464744748649
36 18.9932728437143
37 18.6654812108846
38 17.931791440867
39 16.7155410181401
40 15.038477998813
41 13.1278357096843
42 11.2603277070409
43 9.72876469514166
44 8.55669550334487
45 7.810947983407
46 7.5069877217159
47 7.56658580520308
48 8.01140016228758
49 8.87729284379471
50 10.2605478362364
51 12.2790183549233
52 14.6285686641433
53 16.3147412847667
54 15.2691093342367
55 12.7692018738256
56 7.36200131110735
57 0.999341589939634
58 0.00906608634891126
59 -0.611274833724055
60 -0.959444619210899
61 -1.10308090421362
62 -1.10038981916211
63 -1.0092932489981
64 -0.876512230102612
65 -0.729272903403724
66 -0.589415914396025
67 -0.468118564069929
68 -0.366605913948177
69 -0.281100111946902
70 -0.211266431325273
71 -0.156630097884055
72 -0.113181186173547
73 -0.0799616330993877
74 -0.0570517481971714
75 -0.0413416742809696
76 -0.029929634695949
77 -0.0216359352812504
78 -0.0156816335576843
79 -0.0114580151914064
80 -0.00850710922293468
81 -0.00649093569737314
82 -0.00515995248907987
83 -0.00432820080277627
84 -0.00384398098319825
85 -0.00351795075059169
86 -0.00288593580410647
87 -1.19060684384371e-05
88 0.0252726307971598
89 0.345504982800476
90 2.10245482246506
91 3.39307571869667
92 3.91723050333312
93 4.00379859639592
94 4.00664073447946
95 8.04741530338915
96 14.6561493165769
97 19.4174957443705
98 25.9057524266751
99 34.425855458866
};
\addplot [semithick, color1]
table {%
0 33.0294769203037
1 41.795374983964
2 43.9608042257808
3 48.2393315689727
4 52.7497110655766
5 53.2516980183486
6 47.429834491212
7 38.4025837758865
8 31.2975371178053
9 29.7019452983846
10 33.9860510893882
11 42.3547653383178
12 52.5275915983749
13 62.104478428302
14 69.556600311879
15 71.8854565700315
16 68.270260266009
17 61.4283902185848
18 53.6231272826264
19 46.7400274710776
20 41.1909443649422
21 36.8907015725281
22 33.4597663263045
23 30.3766961492581
24 27.5971884632173
25 25.1526418546936
26 23.1218514593792
27 21.4654387126882
28 20.1525312875557
29 19.1752737000785
30 18.0904465006113
31 16.7598067824714
32 15.3386404923627
33 13.8993648732427
34 12.6008251076026
35 11.6215238856209
36 10.9690567827941
37 10.4712209681218
38 9.94062860289246
39 9.29475764774744
40 8.49957072859405
41 7.59022887569438
42 6.65323027125678
43 5.79018932572636
44 5.05553542120292
45 4.48836755936018
46 4.11215883059461
47 3.92851567034072
48 3.94136559899383
49 4.16562485947103
50 4.63767515379587
51 5.37975639087608
52 6.2894328831106
53 7.00759009244079
54 6.95914600035643
55 6.03261361235098
56 4.1607022157789
57 2.03847323803451
58 0.807500721027603
59 0.0317322921793637
60 -0.4276316768014
61 -0.661617177289043
62 -0.736565497991344
63 -0.713091636581408
64 -0.63844284345961
65 -0.540704608563184
66 -0.441818561352808
67 -0.353484276767779
68 -0.278198586235058
69 -0.213722931795891
70 -0.160542032451576
71 -0.118782569517615
72 -0.0853950410625775
73 -0.059883104441255
74 -0.0425706209454988
75 -0.0308988596717316
76 -0.0223896495066653
77 -0.0162549921832372
78 -0.0119116957472377
79 -0.00890653213362707
80 -0.00690486130944302
81 -0.00566920096553
82 -0.00504165967514758
83 -0.00493891529334024
84 -0.00536205412529336
85 -0.00644802290147664
86 -0.00860710890213565
87 -0.0124385801924584
88 -0.0106188147515065
89 0.129639326585294
90 1.02160951521785
91 2.14478119629093
92 2.82976545727452
93 2.81942719611717
94 2.21387916720757
95 2.93295398079837
96 5.19975901452838
97 7.39387743117
98 10.0196615611125
99 13.9458100098335
};
\addplot [semithick, color2]
table {%
0 73.2269145608992
1 93.1243134997138
2 99.1968604862519
3 105.653901958272
4 112.211531587538
5 114.200327965524
6 107.87010360101
7 96.471958886869
8 86.2213045415147
9 81.7983306882047
10 84.0795744004726
11 91.2216310798173
12 100.805353769343
13 110.163557823138
14 117.781225906434
15 119.358040068464
16 113.174048718999
17 102.719410214312
18 90.9593391087462
19 80.5201258941292
20 72.0825406941479
21 65.4895646212173
22 60.1308233991554
23 55.1371336369412
24 50.3663402545939
25 50.2126330760988
26 47.5732964590236
27 44.2027616253108
28 41.6212981020798
29 39.8678760194397
30 38.1993718336728
31 36.1938403391765
32 33.9633050634012
33 31.6014022920908
34 29.3757094094221
35 27.6284946079026
36 26.4675469777262
37 25.6478899600981
38 24.7844129459025
39 23.650641306408
40 22.1254972027715
41 20.2557784233481
42 18.2118830935397
43 16.2369813748404
44 14.4791867218105
45 13.0630543745722
46 12.0736458328815
47 11.5265107398503
48 11.4430268087618
49 11.8587973596401
50 12.8484922663054
51 14.4985768643661
52 16.6628194379784
53 18.6833421689166
54 19.1604390860631
55 17.9743799383599
56 14.4549431310209
57 9.37746102844032
58 5.01917946201129
59 1.51236155138326
60 0.532958096520401
61 0.172731085585383
62 -0.0170977790162789
63 -0.111061274331615
64 -0.147642547882294
65 -0.150337831840545
66 -0.13689545823436
67 -0.117917009975257
68 -0.0978976626489308
69 -0.0779363189499249
70 -0.0599026149056747
71 -0.0450132706963275
72 -0.0324886658457677
73 -0.0226469092653077
74 -0.0160662233587678
75 -0.0117036470537337
76 -0.0084860400573422
77 -0.006146342200832
78 -0.00448166433462223
79 -0.00332609095943455
80 -0.00255315550726882
81 -0.00207039891230672
82 -0.00181338562645899
83 -0.00174349236979636
84 -0.00184900377225165
85 -0.00215495186197998
86 -0.00273991507820336
87 -0.00353197037144417
88 0.00924866195655734
89 0.250256297158742
90 1.60422869768471
91 3.1758448230044
92 4.13374624517753
93 4.34561553392808
94 4.17717318887821
95 6.75515106378517
96 12.406735587533
97 18.3434079357644
98 25.4910463909529
99 34.7546276714303
};
\addplot [semithick, color3]
table {%
0 52.6501194707552
1 60.3551498023471
2 57.7263597656383
3 60.0090818850204
4 63.6764140095923
5 63.848203148775
6 57.8031646226804
7 49.5838189680289
8 43.3604459996153
9 42.1002160138164
10 45.9454567531335
11 53.1534182713929
12 61.7621343181304
13 69.7626783145424
14 76.3184513424133
15 77.8052294449283
16 74.0340356189189
17 67.8344389175073
18 61.0036272524268
19 55.2663549518114
20 50.8134320912693
21 47.3844168006131
22 44.534442208274
23 41.6535456511602
24 38.8214161713176
25 36.2275873822438
26 34.1237599008711
27 32.5661142818881
28 31.4536129632322
29 30.8239362936573
30 29.9866386020557
31 28.7064893771356
32 27.2379159882042
33 25.6886868951871
34 24.2971041842907
35 23.3360544896815
36 22.830558445446
37 22.4837754171506
38 21.9470449298631
39 21.1120896956089
40 19.932134929166
41 18.5001664063683
42 16.9784066164721
43 15.5924259568928
44 14.4150801709491
45 13.5543074232184
46 13.0709377612203
47 12.9402122875825
48 13.2100159494659
49 14.0305898638383
50 15.4315900092808
51 17.3500296801808
52 19.4612916173469
53 20.9244890223709
54 20.084009320412
55 18.0721896339367
56 13.7865019960524
57 8.09343878548703
58 6.06096256381379
59 4.61542432368953
60 3.53996085769455
61 2.72106692626744
62 2.10856211031454
63 1.65325802699024
64 1.31289771081105
65 1.05728545457314
66 0.860911301130588
67 0.705939292316304
68 0.58204647869809
69 0.483515871746972
70 0.404032843247082
71 0.338495028464818
72 0.285038759831478
73 0.240952273274962
74 0.203856400531154
75 0.173192411701004
76 0.147322587657682
77 0.126761024455529
78 0.111126363883994
79 0.100291091431553
80 0.0943246512228972
81 0.0934095081233537
82 0.0978718624527087
83 0.109855890944648
84 0.136320960120714
85 0.174925193593227
86 0.238282581849132
87 0.353011863777049
88 0.598600814441118
89 1.5169420731177
90 4.7975890144107
91 6.02950790088495
92 6.26789502889792
93 6.57782425967353
94 7.38992303444115
95 12.4814516442801
96 18.2187768194621
97 21.6881427357175
98 25.8783467016616
99 30.9122425182486
};
\addplot [semithick, color4]
table {%
0 56.6152544261717
1 67.1436268073342
2 66.8398555970822
3 76.1543133945859
4 86.2975830554611
5 84.2829936183686
6 65.3050616161134
7 39.23643169782
8 20.8498275433093
9 20.0912513139678
10 37.2826343692406
11 66.3726878239357
12 99.8676032779865
13 130.41833297686
14 153.331751027991
15 161.77995834071
16 154.829118692141
17 139.479815101555
18 121.453549151101
19 105.444489011369
20 92.4192911980323
21 82.3084896289866
22 74.3180384097947
23 67.3195981782619
24 61.3125232338008
25 56.2891674129595
26 52.2678403652316
27 48.9631883834741
28 46.2771636331226
29 44.1801910833802
30 41.561798501595
31 38.2194933413046
32 34.6636257543801
33 31.0970631118905
34 27.9324164111397
35 25.6148363682666
36 24.1080724761501
37 22.9351858721065
38 21.6535106709909
39 20.1037991028156
40 18.2320673056854
41 16.1311324814572
42 14.008859685745
43 12.0908191955603
44 10.4921976468287
45 9.29179313218613
46 8.53638662248555
47 8.2337776713245
48 8.39570321649889
49 9.06556342067562
50 10.3438390779372
51 12.2703078386295
52 14.5487772144754
53 16.2117429219927
54 15.8901035486174
55 13.2049386798783
56 8.18360906985005
57 2.95882274210875
58 0.692727665176914
59 0.440374710986686
60 0.691118804668227
61 0.794556225512167
62 0.792607162328462
63 0.726987758666446
64 0.631347511018008
65 0.525295495246654
66 0.424562141310586
67 0.337197672162493
68 0.264084548138046
69 0.202502320995085
70 0.152211245667886
71 0.112871192373115
72 0.0815997960183536
73 0.0577238043719316
74 0.0413304954965425
75 0.0301467333015444
76 0.0219724408084975
77 0.0160615451653532
78 0.011861512912056
79 0.00894603949906402
80 0.00700207467374505
81 0.00580963305203719
82 0.00522650703418184
83 0.00518606930432508
84 0.00571288309908167
85 0.0069905117773419
86 0.00955401490311049
87 0.0144448655280278
88 0.0217428472095306
89 0.267711203418131
90 2.51633574132493
91 5.3815668058837
92 7.10955341830121
93 7.05803110087803
94 4.99133044102281
95 5.36929718696121
96 8.99553298846378
97 11.8995293727315
98 15.1723574030307
99 21.4929617107211
};
\addplot [semithick, color5]
table {%
0 67.9428360394658
1 87.6024688757278
2 94.555982949639
3 101.007450952872
4 107.622599489776
5 110.837437144196
6 107.244969950952
7 99.2715157763012
8 91.529357984054
9 87.4068391578526
10 87.9327316942245
11 92.5534851637744
12 100.260422284398
13 109.178818738522
14 117.662688372975
15 120.698319433944
16 115.866757677049
17 106.429052619041
18 95.3624511997893
19 85.4345217680478
20 77.4197197632656
21 71.2066384380734
22 66.1831231731891
23 61.4161857005
24 56.7439759133814
25 52.3126851987736
26 48.462531586715
27 45.3719954323126
28 43.0534616916614
29 41.5585736869757
30 40.1081148622549
31 38.2629926662407
32 36.147323336298
33 33.8590852047582
34 31.6821333433236
35 29.987753083147
36 28.9048331115453
37 28.1806162195796
38 27.3976306987538
39 26.3027924542992
40 24.7547432523009
41 22.798174995475
42 20.6172963721497
43 18.4846816657481
44 16.5703987626792
45 15.0220425276119
46 13.9439288850801
47 13.3615828380285
48 13.3087395857088
49 13.8366701735212
50 15.0448758639226
51 17.0534355965252
52 19.7081470942878
53 22.2355740109442
54 22.948574787261
55 21.7097074611153
56 17.6878318141649
57 11.7326596349533
58 7.78222187281695
59 5.06280750503943
60 3.24881602050754
61 2.07541438207523
62 1.33142105123441
63 0.863322283807849
64 0.567367796819735
65 0.37915342025555
66 0.256978172623649
67 0.175905343972365
68 0.12141882741574
69 0.0847785779458658
70 0.0597853290701755
71 0.0424256150972211
72 0.0304530147382052
73 0.0220945510162242
74 0.0160109432124307
75 0.0116005504551592
76 0.00847893082969518
77 0.00627508823176655
78 0.00472918338215133
79 0.00366523074393999
80 0.00296603400418142
81 0.00255813061665794
82 0.00240487579967415
83 0.00250780831949601
84 0.00292342186348075
85 0.00382726123475385
86 0.00572754684596192
87 0.0102249000115131
88 0.0281179451196022
89 0.221574398666327
90 1.41792538027368
91 3.01496267146195
92 4.09361678838104
93 4.14569751212532
94 3.70337435159011
95 6.10491382605371
96 11.3149304097387
97 16.8975332754193
98 23.6649229985977
99 32.2378385366986
};
\addplot [semithick, black]
table {%
0 14.1538136065429
1 16.7859067018335
2 16.7099638992705
3 19.0385783486465
4 21.5743957638653
5 21.0707484045922
6 16.3262654040283
7 9.80910792445499
8 5.21245688582733
9 5.02281282849195
10 9.32065859231016
11 16.5931719559839
12 24.9669008194966
13 32.6045832442151
14 38.3329377569979
15 40.4449895851775
16 38.7072796730353
17 34.8699537753887
18 30.3633872877751
19 26.3611222528424
20 23.1048227995081
21 20.5771224072467
22 18.5795096024487
23 16.8298995445655
24 15.3281308084502
25 14.0722918532399
26 13.0669600913079
27 12.2407970958685
28 11.5692909082806
29 11.0450477708451
30 10.3904496253988
31 9.55487333532615
32 8.66590643859503
33 7.77426577797263
34 6.98310410278493
35 6.40370909206665
36 6.02701811903753
37 5.73379646802663
38 5.41337766774772
39 5.0259497757039
40 4.55801682642135
41 4.03278312036429
42 3.50221492143625
43 3.02270479889008
44 2.62304941170717
45 2.32294828304653
46 2.13409665562139
47 2.05844441783112
48 2.09892580412472
49 2.2663908551689
50 2.58595976948429
51 3.06757695965738
52 3.63719430361885
53 4.05293573049817
54 3.97252588715434
55 3.30123466996957
56 2.04590226746251
57 0.739705685527187
58 -0.0148632593168147
59 -0.528449653184023
60 -0.829342565601872
61 -0.9534674706146
62 -0.951128594794154
63 -0.872385310399736
64 -0.75761701322161
65 -0.630354594295985
66 -0.509474569572703
67 -0.404637206594991
68 -0.316901457765655
69 -0.243002785194102
70 -0.182653494801463
71 -0.135445430847738
72 -0.0979197552220243
73 -0.0692685652463179
74 -0.0495965945958509
75 -0.0361760799618532
76 -0.026366928970197
77 -0.0192738541984238
78 -0.0142338154944672
79 -0.0107352473988768
80 -0.00840248960849406
81 -0.00697155966244462
82 -0.00627180844101821
83 -0.00622328316519009
84 -0.006855459718898
85 -0.00838861413281028
86 -0.0114648178837326
87 -0.0173338386336333
88 -0.021427430586839
89 0.0669278008545328
90 0.629083935331232
91 1.34539170147093
92 1.7773883545753
93 1.76450777521951
94 1.2478326102557
95 1.3423242967403
96 2.24888324711595
97 2.97488234318287
98 3.79308935075768
99 5.37324042768028
};


==> plots/all/GlutealsTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 113.884696433841
1 142.615725377702
2 130.332466638676
3 134.434788007485
4 144.387619121921
5 146.545801666361
6 131.302425834269
7 108.244475333638
8 90.4630660829427
9 85.6125811621704
10 93.0590694562154
11 107.837086118808
12 125.739662147035
13 142.262770494358
14 156.227789348998
15 156.705475097692
16 142.245168803214
17 124.102329415579
18 106.580108157467
19 93.6712843565823
20 84.6069495918161
21 77.8454520915319
22 71.9635520349518
23 65.3360564906242
24 58.6782696542717
25 52.8396089792325
26 48.553208206609
27 45.8048353643806
28 44.0625276111826
29 43.366755856969
30 41.865545429254
31 39.1086445114939
32 35.9478888284288
33 32.7107279360162
34 29.9652596736901
35 28.2740426072449
36 27.5724659696158
37 27.0809868388019
38 26.008681502812
39 24.2435972306325
40 21.8156107859159
41 19.0502002838673
42 16.3454514915786
43 14.1234444658217
44 12.4199200082583
45 11.3318599061423
46 10.8820548475629
47 10.9583818546073
48 11.5912826590101
49 12.8314775885516
50 14.8160178651679
51 17.711291650053
52 21.0792033782359
53 23.4942885209839
54 22.0020130847569
55 18.4081866454222
56 10.6317583561963
57 1.48426941888471
58 0.0353202757614789
59 -0.836201280247655
60 -1.31249134748
61 -1.50898368750301
62 -1.50530314853262
63 -1.38068567825533
64 -1.19904466263024
65 -0.997624863054732
66 -0.806303787840902
67 -0.640371732682698
68 -0.501504529589927
69 -0.38453409058893
70 -0.289002349045322
71 -0.214259574791557
72 -0.154819534208655
73 -0.109369432261485
74 -0.078015139506568
75 -0.0565063234445415
76 -0.0408876565683452
77 -0.0295321814161634
78 -0.021372995402329
79 -0.0155754605419568
80 -0.01151035536787
81 -0.00871146640286614
82 -0.00683123868954651
83 -0.00560422965825521
84 -0.00480098116299327
85 -0.00411015592286966
86 -0.00275437488197723
87 0.00231603130957421
88 0.0405693298147366
89 0.509525603728961
90 3.07906459195733
91 4.90345963908246
92 5.61144881811951
93 5.78676508875171
94 5.88633519104582
95 11.8410381791909
96 21.5203524970031
97 28.4754095837771
98 37.920065825749
99 50.3127364232582
};
\addplot [semithick, color1]
table {%
0 76.211858607035
1 102.126728167694
2 111.470748487193
3 120.108123974611
4 128.879039484663
5 132.970144267819
6 127.29697955693
7 114.978285611569
8 103.067983748167
9 97.0724657956697
10 98.1660040164203
11 104.397389080933
12 113.244783361433
13 121.913441649117
14 129.043762678338
15 129.481022960495
16 120.986114269891
17 107.809585138154
18 93.5236801049323
19 81.121872991305
20 71.2801391316783
21 63.6769150022222
22 57.5379136251063
23 51.8793905532036
24 46.5360506633079
25 41.6375516689843
26 37.4534065988203
27 34.065581526584
28 31.4254634508096
29 29.5060252413601
30 27.6484529831323
31 25.5383847099612
32 23.3103759248009
33 21.0577661475862
34 18.9998614486389
35 17.3859637797933
36 16.2515542470926
37 15.3758382372283
38 14.4812067837162
39 13.4297067431629
40 12.1656169805638
41 10.7441079434427
42 9.29449920820022
43 7.96730137578048
44 6.83976463753647
45 5.96065146132996
46 5.35282697110777
47 5.00436536208965
48 4.90782406302617
49 5.06897058214541
50 5.51895075010449
51 6.28039984695079
52 7.23922769011905
53 7.99035895378565
54 7.84081989434991
55 6.70021997926709
56 4.52607725016786
57 2.0908859210994
58 0.749993655885794
59 -0.0404747113546468
60 -0.475939562837896
61 -0.676658913930398
62 -0.721879052817344
63 -0.677041202539796
64 -0.589703656863801
65 -0.486544825538628
66 -0.387636187447059
67 -0.302674945044309
68 -0.232634721095235
69 -0.174179543209486
70 -0.127176894673446
71 -0.0912421126614528
72 -0.0630788353105231
73 -0.0421021860379248
74 -0.0285690190501707
75 -0.0199144845866754
76 -0.0137935519552242
77 -0.00951377411767223
78 -0.00657677839879468
79 -0.00459943178418363
80 -0.0032997603913227
81 -0.00247334871437286
82 -0.00197139156315514
83 -0.00168496617056465
84 -0.00152811839331022
85 -0.00140739115475594
86 -0.00110713191226359
87 0.000525115653707265
88 0.017756157591265
89 0.246407294109491
90 1.56482358928782
91 3.06041484661495
92 3.93060741362579
93 4.06310552974974
94 3.82413963522177
95 6.12059116674446
96 11.3188307801536
97 16.9020766663225
98 23.8463753457839
99 33.1883066922937
};
\addplot [semithick, color2]
table {%
0 104.544120475885
1 134.624745090663
2 145.136861698737
3 154.41126704634
4 163.729359721402
5 168.258403490414
6 162.865332551887
7 150.635995724616
8 138.563085466371
9 132.256077315266
10 133.090681164655
11 139.245095003658
12 148.267456849805
13 157.356612101301
14 165.180912141329
15 166.182321767957
16 157.653243107645
17 143.816867499523
18 128.324697186368
19 114.540630739416
20 103.428400548051
21 94.7492098180372
22 87.6457381567183
23 80.876241190107
24 74.182383663992
25 67.7705715234811
26 62.1236201846228
27 57.5388183971742
28 54.0398625925188
29 51.6840090952028
30 49.5558507902617
31 47.0628679087543
32 44.2831640072923
33 41.3218069271712
34 38.5043188837329
35 36.2578922566151
36 34.7431400261669
37 33.6769022535967
38 32.5684038704862
39 31.1145301051124
40 29.1502966190536
41 26.7311466051543
42 24.0725559531811
43 21.4904016064217
44 19.17933154306
45 17.3043664824322
46 15.9781037783646
47 15.2189450135249
48 15.0527420621731
49 15.5205254937295
50 16.7095731949672
51 18.7316377864924
52 21.4184407545122
53 23.9802093586735
54 24.6498831795143
55 23.3201298250945
56 19.063288826777
57 12.6726725569107
58 6.98946695156099
59 1.91808304661114
60 -0.0120222084537866
61 -0.526767537588775
62 -0.65540839881325
63 -0.646782312572192
64 -0.58193218533096
65 -0.494012924092591
66 -0.404483227433868
67 -0.324255967053668
68 -0.255718356664409
69 -0.196964108412059
70 -0.148422871896205
71 -0.110208200250682
72 -0.0796123916566736
73 -0.0561689166287633
74 -0.0401436919028887
75 -0.0292616553704278
76 -0.0213015125153748
77 -0.0155433920213696
78 -0.0114527273153577
79 -0.00861401508252056
80 -0.00672058992057119
81 -0.00555563702381925
82 -0.00497711806182464
83 -0.00491490045504652
84 -0.00538366811651201
85 -0.00654148575117403
86 -0.00885075233809026
87 -0.013098399087045
88 0.00294457242878415
89 0.341960388350177
90 2.01681649618987
91 3.8617791388894
92 4.96802617993999
93 5.34687588100429
94 5.56296634383648
95 9.53361935704443
96 17.6643834556296
97 26.3680585805195
98 36.8803717812956
99 50.1102104478042
};
\addplot [semithick, color3]
table {%
0 127.608955264791
1 167.54334414671
2 148.336349458735
3 150.110613630223
4 160.797000723134
5 165.624997023451
6 151.722900847035
7 133.474380040076
8 117.882836336568
9 110.471840975113
10 111.432050339618
11 117.651463227202
12 126.728437702103
13 135.86647723992
14 146.176099392296
15 144.068000762863
16 130.164293704185
17 113.230410797631
18 96.8553723756488
19 84.6165440524295
20 76.0186476007748
21 69.6516890086324
22 64.1641457010582
23 57.9964410570574
24 51.5981778909362
25 45.7490580890978
26 41.2161051341624
27 38.1650334217455
28 36.2036457259658
29 35.3752487958347
30 34.2059851363483
31 32.1427512812961
32 29.7028485830382
33 27.1251536629483
34 24.8577180537165
35 23.3709640328016
36 22.693902065501
37 22.2774686585253
38 21.4660649540854
39 20.0892539467925
40 18.1227129453806
41 15.8121703521803
42 13.4895305919879
43 11.5080732990827
44 9.93219071161385
45 8.83994225385686
46 8.25651645498695
47 8.10859525780467
48 8.45400741394978
49 9.54207750668851
50 11.5315570156925
51 14.5389235228445
52 18.1767997205702
53 20.8857571025452
54 19.207708483921
55 15.6443107660352
56 10.1593575040865
57 3.19847314243138
58 1.51535855553836
59 0.426127418693613
60 -0.233125576478591
61 -0.580781813639231
62 -0.717983719426116
63 -0.72641888659435
64 -0.666155675272028
65 -0.57300278845452
66 -0.473480996537858
67 -0.382023142254687
68 -0.302675820089343
69 -0.234046103917663
70 -0.177009316592088
71 -0.131883638984855
72 -0.0956693872619843
73 -0.0678410426432264
74 -0.0486770899625865
75 -0.0355696996093652
76 -0.0259638563898267
77 -0.0189982677065157
78 -0.014036876104253
79 -0.0105847230456788
80 -0.00827595870026421
81 -0.00685166662476938
82 -0.00614214245990955
83 -0.00605808653460635
84 -0.00659317808564492
85 -0.00793345177077526
86 -0.010549672203072
87 -0.015084036750108
88 -0.0132103095095796
89 0.162166292345975
90 1.27589431464372
91 2.1938893611918
92 2.54664156919488
93 2.67267756021305
94 2.9419804380931
95 7.8293978711664
96 17.0802266033478
97 24.4288769651661
98 35.3240757499814
99 49.5819576313709
};
\addplot [semithick, color4]
table {%
0 55.1472910289548
1 65.402675759625
2 65.1067809604622
3 74.1797264085074
4 84.0599936552597
5 82.0976400260612
6 63.6117822857084
7 38.2190796404356
8 20.3092173494299
9 19.570310061789
10 36.3159418557019
11 64.6517262688216
12 97.2781600675697
13 127.036747199731
14 149.356048712041
15 157.585204477029
16 150.814591487997
17 135.863276320709
18 118.304409110612
19 102.710444064017
20 90.0229734908962
21 80.1743324785825
22 72.3910637588053
23 65.5740844109448
24 59.7227654766295
25 54.8296590479517
26 50.9126000278805
27 47.6936335773271
28 45.0772541205895
29 43.0346534707739
30 40.4841525642725
31 37.2285092354507
32 33.7648408890995
33 30.290754796722
34 27.2081634637146
35 24.9506753997179
36 23.4829800283436
37 22.3405049206586
38 21.0920619694274
39 19.5825325020195
40 17.7593323911891
41 15.7128722037556
42 13.6456273119995
43 11.777319235146
44 10.2201479623749
45 9.05086844941625
46 8.31504869451346
47 8.02028601850346
48 8.17801303492797
49 8.8305045940116
50 10.0756361473486
51 11.9521539600988
52 14.1715454482035
53 15.7913925154497
54 15.4780928524935
55 12.8625509817035
56 7.97141822670303
57 2.88210413458341
58 0.480422122619915
59 -0.23097575925729
60 -0.36249059417506
61 -0.416743338983032
62 -0.415721058780592
63 -0.381303797287793
64 -0.331140656069584
65 -0.275516560833345
66 -0.222682094349596
67 -0.17685958435946
68 -0.138511879752667
69 -0.106212110224053
70 -0.0798345299094634
71 -0.0592007413374017
72 -0.0427989491003016
73 -0.0302760335900153
74 -0.0216777719964998
75 -0.0158119084491701
76 -0.0115245064529421
77 -0.00842425211270786
78 -0.00622134260312944
79 -0.00469218193981282
80 -0.00367257581735523
81 -0.00304714228978763
82 -0.0027412937218373
83 -0.00272008420384436
84 -0.00299639711009296
85 -0.00366651109858438
86 -0.00501106396699543
87 -0.00757630649414502
88 -0.00658387318741008
89 0.260769783625429
90 2.45109027345918
91 5.24202944672519
92 6.92521150737269
93 6.87502509980072
94 4.86191142727642
95 5.23007796381849
96 8.76228996413467
97 11.5909893204024
98 14.7789569751268
99 20.9356758447666
};
\addplot [semithick, color5]
table {%
0 77.983831112979
1 99.4977402595976
2 106.364738825506
3 114.570619597583
4 123.10969788058
5 125.973270351012
6 118.792802786819
7 105.803387354972
8 94.5013014985386
9 90.2848680528614
10 94.241958263325
11 104.551532376254
12 118.648235775221
13 133.240599323022
14 145.935956179408
15 150.646373726305
16 144.786746147803
17 132.801933167817
18 118.637650598833
19 105.910728108453
20 95.5956744479349
21 87.5863332523008
22 81.1352166677286
23 75.0981913178619
24 69.3216529690946
25 63.9610322929752
26 59.3708831641535
27 55.6820914290881
28 52.8908042205322
29 51.047519249327
30 49.1369912201293
31 46.6631515511107
32 43.8509986180106
33 40.8416025013395
34 38.0133611652596
35 35.8443165894876
36 34.4627882405065
37 33.5109609168241
38 32.4692825770424
39 31.0462310814101
40 29.0860821071763
41 26.6545175667333
42 23.9855437561352
43 21.4073580054352
44 19.1198324454888
45 17.2919606622731
46 16.0416955247168
47 15.3988189772276
48 15.4021727861528
49 16.1162904831763
50 17.6689572033198
51 20.1938089375784
52 23.4644828745496
53 26.4584530134971
54 27.1214799618796
55 25.1915469941004
56 19.8210774334933
57 12.4429153397871
58 7.65913414431897
59 4.36112243585628
60 2.19825710461424
61 0.873283796103024
62 0.126966980773151
63 -0.246894303266644
64 -0.398865501418231
65 -0.42286308686811
66 -0.386992672534311
67 -0.330588150856816
68 -0.270305797098814
69 -0.210596111863065
70 -0.157745831747668
71 -0.115278211607961
72 -0.0805476634673394
73 -0.0541298687663173
74 -0.0371630580797973
75 -0.0263239694384655
76 -0.0185456194841219
77 -0.0130388777700901
78 -0.00922036851239346
79 -0.00662905478496368
80 -0.00492261968996618
81 -0.00385462120651084
82 -0.00325165727568654
83 -0.00299945788108176
84 -0.00303303751520458
85 -0.00333100960908085
86 -0.00387539157647724
87 -0.00397951518014698
88 0.0107743355747778
89 0.261664162175518
90 1.79327143813602
91 3.76691667126034
92 5.07053793151041
93 5.21062260750719
94 4.56410069837956
95 7.04232367601655
96 12.8825130954056
97 18.959384703341
98 26.2790065954435
99 35.9643732272503
};
\addplot [semithick, black]
table {%
0 14.1538136065429
1 16.7859067018335
2 16.7099638992705
3 19.0385783486465
4 21.5743957638653
5 21.0707484045922
6 16.3262654040283
7 9.80910792445499
8 5.21245688582733
9 5.02281282849195
10 9.32065859231016
11 16.5931719559839
12 24.9669008194966
13 32.6045832442151
14 38.3329377569979
15 40.4449895851775
16 38.7072796730353
17 34.8699537753887
18 30.3633872877751
19 26.3611222528424
20 23.1048227995081
21 20.5771224072467
22 18.5795096024487
23 16.8298995445655
24 15.3281308084502
25 14.0722918532399
26 13.0669600913079
27 12.2407970958685
28 11.5692909082806
29 11.0450477708451
30 10.3904496253988
31 9.55487333532615
32 8.66590643859503
33 7.77426577797263
34 6.98310410278493
35 6.40370909206665
36 6.02701811903753
37 5.73379646802663
38 5.41337766774772
39 5.0259497757039
40 4.55801682642135
41 4.03278312036429
42 3.50221492143625
43 3.02270479889008
44 2.62304941170717
45 2.32294828304653
46 2.13409665562139
47 2.05844441783112
48 2.09892580412472
49 2.2663908551689
50 2.58595976948429
51 3.06757695965738
52 3.63719430361885
53 4.05293573049817
54 3.97252588715434
55 3.30123466996957
56 2.04590226746251
57 0.739705685527187
58 -0.0148632593168147
59 -0.528449653184023
60 -0.829342565601872
61 -0.9534674706146
62 -0.951128594794154
63 -0.872385310399736
64 -0.75761701322161
65 -0.630354594295985
66 -0.509474569572703
67 -0.404637206594991
68 -0.316901457765655
69 -0.243002785194102
70 -0.182653494801463
71 -0.135445430847738
72 -0.0979197552220243
73 -0.0692685652463179
74 -0.0495965945958509
75 -0.0361760799618532
76 -0.026366928970197
77 -0.0192738541984238
78 -0.0142338154944672
79 -0.0107352473988768
80 -0.00840248960849406
81 -0.00697155966244462
82 -0.00627180844101821
83 -0.00622328316519009
84 -0.006855459718898
85 -0.00838861413281028
86 -0.0114648178837326
87 -0.0173338386336333
88 -0.021427430586839
89 0.0669278008545328
90 0.629083935331232
91 1.34539170147093
92 1.7773883545753
93 1.76450777521951
94 1.2478326102557
95 1.3423242967403
96 2.24888324711595
97 2.97488234318287
98 3.79308935075768
99 5.37324042768028
};


==> plots/all/HamstringsFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 52.6209488918741
1 59.6415344352113
2 72.1063105499025
3 76.6967042776192
4 79.1408850206407
5 77.7104084079539
6 71.2130172294894
7 62.4432291663755
8 54.8352784041614
9 50.4068420152462
10 49.055111449221
11 49.3611306975421
12 49.8225534197148
13 47.5750771606917
14 40.7598181616922
15 34.1288514747658
16 28.5173657339192
17 21.8701598272433
18 16.4587892693878
19 13.7259777718251
20 12.6918223111422
21 12.1779427263679
22 11.2825005680213
23 9.38326531966965
24 7.13081416421745
25 5.40074146767538
26 4.69870846554851
27 5.21785545970255
28 6.55574282870195
29 8.25423515837458
30 9.31961637614079
31 9.40965110393236
32 8.98154493408331
33 8.42916045412818
34 8.18024675978574
35 8.46405604326099
36 9.1422643626572
37 9.72734045517865
38 9.80802331851765
39 9.34840255296422
40 8.45249986183206
41 7.38726621236428
42 6.37556098220649
43 5.56642459488156
44 5.10560639791421
45 4.93840047504951
46 4.9205687275593
47 5.12369176785086
48 5.67097873018596
49 6.65304388899348
50 8.20694477337527
51 10.373806231818
52 12.8626923433548
53 15.2411794101105
54 17.1664948533001
55 14.3841881677573
56 7.859233954351
57 4.53445106558909
58 3.14180053381177
59 2.12298987000732
60 1.37759199472421
61 0.850590396906223
62 0.483359328274714
63 0.227846843454006
64 0.0514639112297367
65 -0.0573830508036528
66 -0.107094108487654
67 -0.118094461392858
68 -0.10856387286018
69 -0.0952160859062248
70 -0.0902993453048952
71 -0.0861152843336843
72 -0.0744831455836803
73 -0.0598622164772711
74 -0.0466858676478104
75 -0.0357504700306772
76 -0.0269336759289835
77 -0.0202229950019455
78 -0.0152244276210612
79 -0.0114186746711922
80 -0.00857055506286555
81 -0.00650435956924539
82 -0.00494934804814101
83 -0.0037705461753032
84 -0.00292178049530517
85 -0.00233375710820798
86 -0.00210083852574302
87 -0.160686190336096
88 -1.63109362448518
89 -5.32282753804808
90 -11.1842423244662
91 -16.2982231137428
92 -18.8909363452756
93 -17.6924754801089
94 -12.6693596811755
95 -3.51998986138112
96 10.5265790957192
97 28.5001731551601
98 47.7007123063412
99 62.5301196603813
};
\addplot [semithick, color1]
table {%
0 41.7867751372297
1 45.8100782910323
2 55.4012444411054
3 60.5170045299517
4 63.2246090915784
5 62.8168438812417
6 58.5863263288058
7 52.2531809255341
8 46.2632241317058
9 42.2623335149123
10 40.5275185858979
11 40.3432943966288
12 40.5978722412862
13 39.0714155984474
14 34.525247895551
15 29.5005705887593
16 24.390244174647
17 19.3103148066001
18 15.009092039457
19 12.1587138199402
20 10.4831827129798
21 9.42100920888593
22 8.40978827974444
23 7.07556179957061
24 5.64584307234039
25 4.50798442421399
26 3.9032187574888
27 3.90358495543585
28 4.41077115509253
29 5.21722331396866
30 5.82930215128516
31 5.98613410165545
32 5.81789476129662
33 5.52966418240887
34 5.35134997187997
35 5.42581516422271
36 5.7122251876153
37 5.99834542265679
38 6.08044001656645
39 5.89563822952347
40 5.48066686477423
41 4.94972777105036
42 4.41340234204093
43 3.95979418264656
44 3.65486956737981
45 3.48867262178706
46 3.42719782238424
47 3.50123163235253
48 3.76780057139518
49 4.29341920049705
50 5.17004163793377
51 6.44169015608699
52 7.99091149233016
53 9.60066725105796
54 10.8524477337132
55 9.95260911102121
56 7.06150053974446
57 4.79004875440819
58 3.31395996552807
59 2.24308572684757
60 1.46617491259526
61 0.919617489593743
62 0.540257819375487
63 0.277542722634246
64 0.0974926341367476
65 -0.0134092165622086
66 -0.0665267528621394
67 -0.0832041867931946
68 -0.0800913633172544
69 -0.072252844382115
70 -0.0706768788974097
71 -0.0689759774647632
72 -0.0603136286995312
73 -0.0487052006262902
74 -0.0380836933806602
75 -0.0292064303926262
76 -0.0220172734337858
77 -0.0165415317642178
78 -0.0124651014390226
79 -0.00935921719984334
80 -0.00703583431799949
81 -0.00535400309538801
82 -0.00408855261771265
83 -0.00313056049955602
84 -0.00244707907542136
85 -0.00198612016642162
86 -0.00196925797018756
87 -0.358782331039759
88 -3.37406741617367
89 -8.7730615756988
90 -15.2694530979822
91 -21.1617099487201
92 -24.989873574657
93 -26.103563682523
94 -23.8323819080068
95 -17.6491026445442
96 -7.02913174465304
97 6.77811300515525
98 22.8408819886721
99 36.7407067479013
};
\addplot [semithick, color2]
table {%
0 75.8408564018024
1 77.886506586954
2 87.5216023156436
3 92.3011772823977
4 94.6640614580429
5 93.4859831192378
6 87.4698585220323
7 78.5777583561237
8 69.9407909022416
9 63.8454029308015
10 60.845781887479
11 60.0814987436096
12 60.1059427894119
13 57.9959156731748
14 51.6989412875546
15 44.5337713549445
16 39.6130364952176
17 32.3282576729965
18 25.5180099463771
19 20.8495979207247
20 18.0948133495557
21 16.4603040232863
22 15.0613614481826
23 13.1769153345328
24 10.9722589448938
25 8.99422034719792
26 7.71333155168037
27 7.433149049412
28 8.09795251169509
29 9.41713076383044
30 10.5989986037854
31 11.1356860742806
32 11.1301483655123
33 10.8477147938333
34 10.6462788762568
35 10.7970596170017
36 11.3085893266023
37 11.8836046345633
38 12.1686485788854
39 12.0068135601007
40 11.3958584146336
41 10.4860507044318
42 9.45955828316979
43 8.4821082361503
44 7.71143574959566
45 7.18704083955422
46 6.86655227787023
47 6.79405010075275
48 7.06428174467054
49 7.78158899122651
50 9.08390161642893
51 11.0425460028712
52 13.4769914734876
53 16.0289499601725
54 18.192838763476
55 17.1008806575065
56 12.5671486050658
57 8.70011611895998
58 6.09382798652116
59 4.21534834561605
60 2.86224747576712
61 1.90624781811349
62 1.23656442879544
63 0.768244804975966
64 0.383808001371045
65 0.0845934159052277
66 0.0128498474589732
67 -0.00974212836167946
68 -0.0178362582392736
69 -0.0206520667072604
70 -0.0247519611556537
71 -0.027346756153752
72 -0.0252864659212585
73 -0.0209838810437186
74 -0.016697170866721
75 -0.0129642352662588
76 -0.00985741064372824
77 -0.0074610518441899
78 -0.00566312325637935
79 -0.0042778430426645
80 -0.00323348441907286
81 -0.00247532909323075
82 -0.00190000945377983
83 -0.00146031838781891
84 -0.00114539855939008
85 -0.000932355664472978
86 -0.000922001617817205
87 -0.159064008898763
88 -1.48969762415941
89 -3.83868891314031
90 -6.68748582690857
91 -9.17031262979089
92 -10.5321433141116
93 -10.3851356368499
94 -8.42175356159492
95 -4.37875564752625
96 2.20388849318387
97 15.4780588873369
98 56.9753649976332
99 74.898382527483
};
\addplot [semithick, color3]
table {%
0 41.9266808329699
1 45.9457922821717
2 54.0806701589015
3 57.8341900534891
4 59.8790819218949
5 59.4233232856798
6 55.7001154613553
7 50.2473699758462
8 45.2097773092467
9 42.0257849697614
10 40.8681479903195
11 40.9802344746973
12 41.3762626292106
13 40.0752462436628
14 35.6531899183442
15 31.0016534077495
16 26.27467210073
17 21.4420664115092
18 17.3171610287404
19 14.8590548786116
20 13.6753668456611
21 13.0291921159508
22 12.2659541147032
23 10.8711200798333
24 9.14465546523684
25 7.65454091860427
26 6.86703027247526
27 7.07615948439308
28 8.18700110000802
29 9.71234286668837
30 10.6436894128428
31 10.7199384777437
32 10.3643442684863
33 9.90969924602015
34 9.70912196245908
35 9.97030983108578
36 10.5638634101356
37 11.0626763013975
38 11.1302824927518
39 10.7595872204711
40 10.1178340405153
41 9.34139500234616
42 8.5270492594843
43 7.7975830061219
44 7.29308120505146
45 7.01589067679016
46 6.88002636429052
47 6.94380773768089
48 7.34439159060677
49 8.2036839185343
50 9.56596540549589
51 11.3602832028729
52 13.3143785233286
53 15.0981302745485
54 16.5303672960544
55 14.6802172305051
56 9.86183163622307
57 6.82538569588995
58 5.17537672855101
59 3.91395305260447
60 2.94582344581476
61 2.21213510320981
62 1.65637408402214
63 1.23255969681783
64 0.911080107667373
65 0.681008196029249
66 0.52357987170594
67 0.40991863757157
68 0.327232119181707
69 0.262849622892481
70 0.206709005138519
71 0.160857708215885
72 0.12837368330011
73 0.105089629091349
74 0.0869718602824052
75 0.0724162795408096
76 0.0605717524570353
77 0.050693074077314
78 0.0424200972632916
79 0.0355963803238924
80 0.0299789885469514
81 0.0253587069236499
82 0.0216682349394996
83 0.0188441473045028
84 0.0168570108776349
85 0.0158433057472957
86 0.0216653174816828
87 0.857765047048898
88 6.5817561139163
89 9.09703109246663
90 7.6482741434178
91 5.64631315754847
92 4.15025450488658
93 4.36679469605236
94 5.93607757716727
95 8.86608110248428
96 13.6657851218515
97 19.8811723941977
98 30.7374545747759
99 41.7925773553948
};
\addplot [semithick, color4]
table {%
0 91.5501008910868
1 106.798430678567
2 135.902368663778
3 151.218274189009
4 159.203781197788
5 158.593012705333
6 147.979035300688
7 131.971700816902
8 116.941806755747
9 107.116964696001
10 103.105737745249
11 102.985208132093
12 103.854496381398
13 99.9507425229877
14 88.2695831873757
15 75.4339846437794
16 62.3592690627868
17 49.3097126693655
18 38.2876243868894
19 31.0399415276955
20 26.7786771191202
21 24.0113534959053
22 21.2621016224755
23 17.6089526410385
24 13.7806031621607
25 10.8770207616539
26 9.50171384705105
27 9.71562625802472
28 11.1841434725931
29 13.3379998783302
30 14.8758458906121
31 15.1506356309197
32 14.5630073425312
33 13.6995050652834
34 13.1903236456852
35 13.3981078445355
36 14.1659424051195
37 14.8932501994997
38 15.0463138533612
39 14.4883017259292
40 13.3543943619755
41 11.9738123085441
42 10.6435889355898
43 9.58839241764595
44 8.95496242905292
45 8.68021795740104
46 8.66313646451648
47 8.99088009614752
48 9.81583458518417
49 11.3165862673641
50 13.7408289631858
51 17.2034475374339
52 21.3899546663437
53 25.7276716435652
54 29.1129395229502
55 26.733568238438
56 18.9993461964514
57 12.9186954769191
58 8.96200092818134
59 6.07135108887866
60 3.9574840351093
61 2.45824948476106
62 1.40716059883062
63 0.668790978787702
64 0.197732952140436
65 0.0413591392187195
66 0.0771608772109056
67 0.0850823211942541
68 0.0782170874604576
69 0.0686030913738805
70 0.0650621659258575
71 0.0620496633234014
72 0.0536731071354202
73 0.043143069528633
74 0.0336523749589718
75 0.0257758103955668
76 0.0194251003487798
77 0.0145917300280341
78 0.010992189744185
79 0.00825259299235243
80 0.00620349981838075
81 0.00471812553711053
82 0.00360170739420567
83 0.00275812637758177
84 0.00215623232770484
85 0.00175047552861759
86 0.00174168752096228
87 0.327934831230141
88 3.09312464412336
89 8.1006588392507
90 14.1359660090594
91 19.7679141426583
92 23.777525427619
93 25.6901869374197
94 24.9569052016339
95 21.0943285870213
96 13.663689542673
97 4.94368823210746
98 30.8167583393428
99 69.6267997855808
};
\addplot [semithick, color5]
table {%
0 63.5658286164311
1 65.5714649150243
2 75.4037530449548
3 81.5846878108783
4 85.4275839384395
5 85.3906130333919
6 80.2616766742084
7 72.2521157133209
8 64.5785078695477
9 59.4617933223951
10 57.3913474031807
11 57.5008888345674
12 58.2857770082789
13 56.5779678770093
14 50.5288796694958
15 43.6763412077967
16 36.5718914485948
17 29.383642102903
18 23.1745486086765
19 18.9884070332969
20 16.5405340325414
21 15.063880516971
22 13.7428762594159
23 11.967156017831
24 9.94372293018476
25 8.16183500962506
26 7.02926868537639
27 6.83480373437683
28 7.54335299733777
29 8.86701026086349
30 10.0140196087964
31 10.5113770307748
32 10.4952710194848
33 10.2351946547431
34 10.0709588122515
35 10.257021174221
36 10.7969791412416
37 11.3960517097125
38 11.7076311217438
39 11.58197348103
40 11.0208883493757
41 10.1705822497386
42 9.2049187759819
43 8.28396468447109
44 7.56580594725123
45 7.09500458787161
46 6.83656672242785
47 6.84726190286801
48 7.24188114222255
49 8.15849803124925
50 9.78954794885229
51 12.2553729857653
52 15.3699342677566
53 18.734865358365
54 21.5121604266856
55 20.0632673404429
56 14.5437930908204
57 10.0686411787958
58 7.09135985985143
59 4.90688198031746
60 3.30998301743231
61 2.18122267484465
62 1.40051356359222
63 0.870988014828431
64 0.521314856787639
65 0.303704005019865
66 0.178871186604067
67 0.109683940730181
68 0.070182631356505
69 0.0456692319350303
70 0.0287062570880884
71 0.0185403307289089
72 0.0130509499524654
73 0.00949483332268169
74 0.00695169601675556
75 0.00508545133481216
76 0.00370101681722552
77 0.00269408489309393
78 0.00196894627352205
79 0.0014384004024756
80 0.00105406669167144
81 0.000781686054539688
82 0.000583042036313105
83 0.000437212944412414
84 0.000335095449159282
85 0.000266994093771869
86 0.000262562694063713
87 0.0591155980937463
88 0.570087435456667
89 1.56687400965418
90 2.73589666351135
91 4.07469861299573
92 5.70104829113979
93 8.04509475610731
94 11.6095227737409
95 16.9124981262766
96 24.834916211148
97 36.1933403590009
98 50.1915776526819
99 63.3116860430272
};
\addplot [semithick, black]
table {%
0 22.8875252227717
1 26.6996076696418
2 33.9755921659446
3 37.8045685472521
4 39.8009452994471
5 39.6482531763332
6 36.994758825172
7 32.9929252042254
8 29.2354516889368
9 26.7792411740002
10 25.7764344363122
11 25.7463020330233
12 25.9636240953495
13 24.9876856307469
14 22.0673957968439
15 18.8584961609449
16 15.5898172656967
17 12.3274281673414
18 9.57190609672236
19 7.75998538192388
20 6.69466927978005
21 6.00283837397631
22 5.31552540561888
23 4.40223816025963
24 3.44515079054018
25 2.71925519041348
26 2.37542846176276
27 2.42890656450618
28 2.79603586814828
29 3.33449996958254
30 3.71896147265301
31 3.78765890772994
32 3.64075183563279
33 3.42487626632086
34 3.2975809114213
35 3.34952696113389
36 3.54148560127988
37 3.72331254987493
38 3.76157846334029
39 3.6220754314823
40 3.33859859049387
41 2.99345307713601
42 2.66089723389746
43 2.39709810441149
44 2.23874060726323
45 2.17005448935026
46 2.16578411612912
47 2.24772002403688
48 2.45395864629604
49 2.82914656684103
50 3.43520724079644
51 4.30086188435849
52 5.34748866658591
53 6.43191791089129
54 7.27823488073754
55 6.68339205960951
56 4.74983654911286
57 3.22967386922976
58 2.24050023204534
59 1.51783777221967
60 0.989371008777324
61 0.614562371190264
62 0.351790149707654
63 0.167197744696925
64 0.0365448469033149
65 -0.0496309670624634
66 -0.0925930526530868
67 -0.102098785433105
68 -0.0938605049525491
69 -0.0823237096486566
70 -0.0780745991110289
71 -0.0744595959880817
72 -0.0644077285625043
73 -0.0517716834343596
74 -0.0403828499507661
75 -0.0309309724746801
76 -0.0233101204185358
77 -0.017510076033641
78 -0.013190627693022
79 -0.00990311159082292
80 -0.0074441997820569
81 -0.00566175064453264
82 -0.0043220488730468
83 -0.00330975165309812
84 -0.00258747879324581
85 -0.00210057063434111
86 -0.00209002502515474
87 -0.39352179747617
88 -3.71174957294804
89 -9.72079060710084
90 -16.9631592108713
91 -23.72149697119
92 -28.5330305131429
93 -30.8282243249037
94 -29.9482862419607
95 -25.3131943044255
96 -16.3964274512076
97 -4.62624874354812
98 7.7041895848357
99 17.4066999463952
};


==> plots/all/HamstringsTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 81.7667200063883
1 93.3012079006605
2 113.03671367112
3 119.434583602717
4 123.184202718073
5 120.924197250307
6 110.208069582714
7 95.9059929684752
8 83.7982218881649
9 77.0884179082974
10 75.4721332859134
11 76.4884598876353
12 77.6601551791467
13 74.1252542702037
14 62.3980062908536
15 51.560259397326
16 41.3625120603538
17 31.4805214153302
18 23.7244815789395
19 19.7816909055437
20 18.2748428073771
21 17.5330944696055
22 16.2617445614058
23 13.555278233484
24 10.3291440155173
25 7.83895690806437
26 6.81782051851332
27 7.54682446651714
28 9.45208085758687
29 11.8820562127095
30 13.4197240303724
31 13.5677634869835
32 12.9697588174156
33 12.1863868751883
34 11.8325831565178
35 12.2407653441969
36 13.21583886886
37 14.0604680207676
38 14.1835640607728
39 13.5300415986486
40 12.2461348251525
41 10.714035301787
42 9.25485589049314
43 8.0845590535597
44 7.41408526919997
45 7.1658487173086
46 7.13254396140431
47 7.41600631716653
48 8.19191973348145
49 9.58799934429033
50 11.7967133856867
51 14.8741131567876
52 18.4051554187859
53 21.7730832623918
54 24.5290354918626
55 20.6016003491907
56 11.2947501944353
57 6.52630387194554
58 4.52571802380246
59 3.0640744755477
60 1.99508426754851
61 1.23749762890126
62 0.707152098383432
63 0.335457694636496
64 0.0776871383186818
65 -0.0784954198962189
66 -0.146499293462891
67 -0.161547709406135
68 -0.148510198604897
69 -0.130250788814674
70 -0.123524792197041
71 -0.117801019451203
72 -0.10188841831046
73 -0.0818873160942742
74 -0.0638624858386655
75 -0.0489032175001907
76 -0.0368421566454157
77 -0.0276621709761375
78 -0.020824257465224
79 -0.0156180205691026
80 -0.0117217484699986
81 -0.00889510143505864
82 -0.0067677007058622
83 -0.00515479473214238
84 -0.00399284019875208
85 -0.00318633658126291
86 -0.00285049186336767
87 -0.196562983940229
88 -2.02023886094669
89 -6.80499175759696
90 -14.6056496895576
91 -21.3621993914805
92 -24.6452265815923
93 -22.636152532149
94 -14.8332546580422
95 -0.981131534228404
96 20.0992366251722
97 47.4905002657461
98 78.272127116167
99 102.937069927768
};
\addplot [semithick, color1]
table {%
0 104.770766106655
1 103.813256978982
2 112.499912951192
3 116.263827713577
4 117.912276576845
5 115.867851568102
6 108.085594563631
7 96.6916591228874
8 85.4962398563104
9 77.3795893001728
10 73.1133174795274
11 71.6884348466755
12 71.3955020379926
13 68.8073948799177
14 61.1291006577808
15 52.3076715123821
16 43.3121674649045
17 34.4430897542277
18 26.8347458680504
19 21.6569723077918
20 18.6115939682438
21 16.8141803028559
22 15.31535720352
23 13.3460996485642
24 11.0542190439261
25 8.99337811535815
26 7.64082556884874
27 7.29583876996341
28 7.89077949384285
29 9.13178326876805
30 10.2426726270454
31 10.7231227868293
32 10.6702070411486
33 10.3432969998574
34 10.0920155449422
35 10.1786891573466
36 10.6099452777242
37 11.0989651926786
38 11.3067382808727
39 11.0853043016763
40 10.4383272344362
41 9.51674861154035
42 8.50021318007038
43 7.54734580215146
44 6.80117837016398
45 6.28995800496143
46 5.96815175352428
47 5.86944967663516
48 6.07102794887596
49 6.65650604130892
50 7.73730283847741
51 9.36336958397415
52 11.3654479632418
53 13.4253497286826
54 15.0823820083379
55 13.9045882605443
56 9.89741542587656
57 6.64228977324757
58 4.52825431035762
59 3.04210808066294
60 1.99510192746713
61 1.27266756068973
62 0.778601319111344
63 0.440912912665364
64 0.2116489484871
65 0.0680972755928851
66 -0.0071099239922125
67 -0.0391046385193925
68 -0.046963837353762
69 -0.0471909284383239
70 -0.0515689416357394
71 -0.0541561075246651
72 -0.0486921352125964
73 -0.0395762666965382
74 -0.03093134719723
75 -0.0236219269012135
76 -0.0176774602217197
77 -0.0131844690973424
78 -0.00987701263416217
79 -0.00736810814812521
80 -0.00550581263240332
81 -0.00417654358520596
82 -0.00317797102801759
83 -0.00241964346470379
84 -0.00188139798044171
85 -0.00151851776868118
86 -0.00146883500769076
87 -0.212164994439695
88 -1.94345814564084
89 -4.71489710687655
90 -7.93113854374929
91 -9.94158815057917
92 -9.28641775207812
93 -4.93412457725059
94 3.86254329293414
95 17.4014895679789
96 36.205847035903
97 59.6649695245528
98 86.1694818520636
99 109.511320545253
};
\addplot [semithick, color2]
table {%
0 107.22083187545
1 107.275440154162
2 116.470439620061
3 120.746985651754
4 122.826943809706
5 121.218572672159
6 113.984814997359
7 103.135983698183
8 92.3312466716925
9 84.4499521330142
10 80.3695232737369
11 79.1574253528873
12 79.1070255518939
13 76.6944095223178
14 68.9443656461822
15 59.8379335105501
16 50.3356247574523
17 40.7324818361532
18 32.2803923849334
19 26.4088160490366
20 22.9351770974159
21 20.9256623544789
22 19.2931070089244
23 17.0855756074089
24 14.4050226815032
25 11.8872906587267
26 10.1506955862208
27 9.655511075499
28 10.3785094971814
29 11.9823121972147
30 13.5018100809406
31 14.2754434095087
32 14.3779062224187
33 14.1026539959474
34 13.8803092748039
35 14.0596682924898
36 14.6847226289955
37 15.4148873483419
38 15.8102593525778
39 15.656205886546
40 14.9236349577831
41 13.7808202973501
42 12.4512792288319
43 11.1464233633477
44 10.078911842528
45 9.31979070060588
46 8.82221974621344
47 8.63483397065983
48 8.86993816390022
49 9.64744073385418
50 11.1222532273796
51 13.3732827708697
52 16.1849151810807
53 19.1257917579935
54 21.6764367844679
55 20.4915643350512
56 15.1827697666233
57 10.5412464379823
58 7.38638095071129
59 5.12519868550136
60 3.50558759656397
61 2.36322687971498
62 1.56284942473442
63 1.00264266437446
64 0.523802684500057
65 0.0975566012625562
66 -0.0520736593675992
67 -0.0737508070890399
68 -0.0717033218399517
69 -0.0647613409085045
70 -0.0632353931750718
71 -0.0615763961209768
72 -0.0538061967059767
73 -0.0434642948773463
74 -0.0340079308135862
75 -0.0261025574082243
76 -0.019697210824011
77 -0.0148126361793272
78 -0.0111713089470629
79 -0.0083946827173593
80 -0.00631548982017188
81 -0.00480824387547525
82 -0.00367365579056916
83 -0.00281471340150796
84 -0.00220151840578905
85 -0.00178790630428895
86 -0.00177652900555201
87 -0.328994518880577
88 -3.09905976343191
89 -8.09200653313773
90 -14.115147183931
91 -19.6687337640496
92 -23.4684871856102
93 -24.9740232713647
94 -23.5754730669257
95 -18.5926264555213
96 -7.57394992422925
97 25.7224269017241
98 88.0458078103975
99 109.797623561087
};
\addplot [semithick, color3]
table {%
0 74.5354416231359
1 79.0951164980312
2 90.690222242856
3 93.462641825377
4 95.3849644399009
5 93.3685306619475
6 84.7891545196056
7 73.2343294805441
8 63.2622166357103
9 57.4571859844517
10 55.7303881526031
11 56.2868244287808
12 57.269984945832
13 54.8781872856231
14 45.8145792848505
15 37.3072016611432
16 29.396586098447
17 21.9367264520492
18 16.1662150613889
19 13.1170621973264
20 11.8402256698058
21 11.2265663366673
22 10.4080990795024
23 8.7190327066304
24 6.66950421492763
25 5.02475706485894
26 4.21667142872533
27 4.4231082952565
28 5.63746602792319
29 7.53771305645643
30 8.7717768062189
31 8.84889153558423
32 8.35479208851748
33 7.7575419770241
34 7.51465980246682
35 7.8979615914874
36 8.76225492493471
37 9.50287435457128
38 9.59291054710206
39 9.03959257127825
40 8.14573785005907
41 7.12066847769962
42 6.09657446147605
43 5.22949472216468
44 4.66213666536854
45 4.36540809353801
46 4.22464587545165
47 4.28861044875057
48 4.70210247179064
49 5.64396959365133
50 7.27104795449047
51 9.6264415115881
52 12.3712727296599
53 14.9408295370643
54 17.168858287589
55 14.2375511804208
56 7.40933133957732
57 4.34222956773759
58 2.93239087431328
59 1.94829973875753
60 1.25721499697405
61 0.781250472071879
62 0.455544166617945
63 0.231789361011903
64 0.0767952646054198
65 -0.0244388033306666
66 -0.0767328607341304
67 -0.0921059165174973
68 -0.0875612267218722
69 -0.0783428353083483
70 -0.0755336226202631
71 -0.0728202356921263
72 -0.0633483579168147
73 -0.0510876948202121
74 -0.0399403166076473
75 -0.0306437354960041
76 -0.0231231034352404
77 -0.0173875386982105
78 -0.0131095854949908
79 -0.00984898870787826
80 -0.00740754818800779
81 -0.00563639620559082
82 -0.00430408160042663
83 -0.00329657944971898
84 -0.00257723381587286
85 -0.00209178041831174
86 -0.00206929655624204
87 -0.142520227775567
88 -1.22505327821811
89 -2.71501452741361
90 -5.9605176752055
91 -8.15765635406139
92 -7.72115360311252
93 -2.81692829543449
94 6.61067850986453
95 20.2539567668171
96 39.1695617891815
97 63.9590912106057
98 89.5509297887751
99 108.560091038501
};
\addplot [semithick, color4]
table {%
0 89.1763202116255
1 104.029279701408
2 132.378588636371
3 147.297371708755
4 155.075824415369
5 154.480892393141
6 144.142122271176
7 128.549838136406
8 113.909650605222
9 104.339554526454
10 100.432333720359
11 100.314929290728
12 101.161677972835
13 97.359143614963
14 85.9808622671926
15 73.4780748896742
16 60.7423704832573
17 48.0311729178519
18 37.2948737274424
19 30.2351143044278
20 26.0843392019777
21 23.3887688514153
22 20.7108016725583
23 17.1523743177161
24 13.4232891972468
25 10.5949930906541
26 9.25534618025041
27 9.46371210745919
28 10.894152490244
29 12.9921620681512
30 14.4901336388278
31 14.757798421652
32 14.1854066066709
33 13.3442938735357
34 12.8483148972381
35 13.0507115092706
36 13.7986370710966
37 14.5070866755511
38 14.6561815785239
39 14.1126380141422
40 13.0081314631494
41 11.6633461917308
42 10.3676138626023
43 9.33977728291028
44 8.72277134905972
45 8.45515066113115
46 8.43851207019199
47 8.75775771555092
48 9.56132215686015
49 11.023161207452
50 13.3845462939684
51 16.7573834590003
52 20.8353396454173
53 25.0605849961383
54 28.3580770739822
55 26.0403999386787
56 18.506716691027
57 12.5837297103227
58 8.7296273486269
59 5.91392847795055
60 3.854871377664
61 2.39451012155529
62 1.37067466806821
63 0.651450057384098
64 0.179285878566241
65 -0.021692795578265
66 -0.0404707440143771
67 -0.0446255274131979
68 -0.0410247244275097
69 -0.0359822004355703
70 -0.0341249912829419
71 -0.0325449389808743
72 -0.0281514500333702
73 -0.022628463879633
74 -0.0176506113158585
75 -0.0135193670936476
76 -0.0101884308743699
77 -0.00765333666538467
78 -0.00576538413473996
79 -0.00432847047002121
80 -0.00325372471410211
81 -0.002474648523217
82 -0.00188908917620476
83 -0.00144663242074491
84 -0.001130940053099
85 -0.00091812132758
86 -0.000913512033063525
87 -0.172001240626606
88 -1.62233842073513
89 -4.248781274674
90 -7.41428924122861
91 -10.3682361046647
92 -12.4712701521815
93 -13.474457740857
94 -13.0898527636703
95 -11.0639381414372
96 -7.16658106752686
97 -1.243026666519
98 30.0177179796103
99 67.8214631393617
};
\addplot [semithick, color5]
table {%
0 77.7944321390962
1 81.9411960483328
2 95.5317349880608
3 103.410480402099
4 108.065854961868
5 107.925039937445
6 101.514820692778
7 91.4839005279082
8 81.8161041246792
9 75.3269147201836
10 72.6500095827666
11 72.7011204658176
12 73.6223683198082
13 71.5178431807312
14 63.9637350884087
15 55.339664748432
16 46.3666995407469
17 37.2629052501389
18 29.3832413237546
19 24.0711465055584
20 20.9639551684508
21 19.0787321080979
22 17.3613233835411
23 15.0246766903552
24 12.3764351684091
25 10.1008663813893
26 8.72607705896734
27 8.55992374291548
28 9.51333755187358
29 11.2124786989347
30 12.6541965940603
31 13.2410377044657
32 13.1585665523332
33 12.7709414965785
34 12.5325315420106
35 12.7693038271681
36 13.4629101464831
37 14.2133703683192
38 14.5747286536378
39 14.3661841177493
40 13.6086519790226
41 12.5077443922424
42 11.2945975224299
43 10.1742605932717
44 9.33489499766781
45 8.81034915081309
46 8.54602612068919
47 8.61387988701784
48 9.15590927198194
49 10.3408597148536
50 12.4032620969427
51 15.4862468681142
52 19.3568037325871
53 23.5196682379595
54 27.0096783238353
55 25.2932604557244
56 18.4149798787733
57 12.7625362332063
58 8.99085038766849
59 6.22195802058634
60 4.19156809827093
61 2.7458283650092
62 1.73312671967568
63 1.03156299615647
64 0.552707529366258
65 0.244915369951075
66 0.0717031560536847
67 -0.0106101779955775
68 -0.0422541374774986
69 -0.0547563247846043
70 -0.0700213552004541
71 -0.079456597577306
72 -0.073514334503622
73 -0.0603034491956719
74 -0.0472138261899978
75 -0.0359732639124179
76 -0.0267896985273015
77 -0.0198577076646437
78 -0.0147698054224127
79 -0.0109297906520462
80 -0.00809667546676361
81 -0.00608323355517249
82 -0.00458257767588151
83 -0.00345507256822816
84 -0.00266031567106633
85 -0.00212680113484686
86 -0.00205028868772687
87 -0.324937236414933
88 -3.02130032109476
89 -7.63898020612224
90 -13.1680590049825
91 -17.6873308668923
92 -19.60190464604
93 -18.1150336563802
94 -12.58527746898
95 -2.57853418749132
96 12.6608243452334
97 32.4945841432368
98 54.77007639552
99 74.1539273442522
};
\addplot [semithick, black]
table {%
0 22.8875252227717
1 26.6996076696418
2 33.9755921659446
3 37.8045685472521
4 39.8009452994471
5 39.6482531763332
6 36.994758825172
7 32.9929252042254
8 29.2354516889368
9 26.7792411740002
10 25.7764344363122
11 25.7463020330233
12 25.9636240953495
13 24.9876856307469
14 22.0673957968439
15 18.8584961609449
16 15.5898172656967
17 12.3274281673414
18 9.57190609672236
19 7.75998538192388
20 6.69466927978005
21 6.00283837397631
22 5.31552540561888
23 4.40223816025963
24 3.44515079054018
25 2.71925519041348
26 2.37542846176276
27 2.42890656450618
28 2.79603586814828
29 3.33449996958254
30 3.71896147265301
31 3.78765890772994
32 3.64075183563279
33 3.42487626632086
34 3.2975809114213
35 3.34952696113389
36 3.54148560127988
37 3.72331254987493
38 3.76157846334029
39 3.6220754314823
40 3.33859859049387
41 2.99345307713601
42 2.66089723389746
43 2.39709810441149
44 2.23874060726323
45 2.17005448935026
46 2.16578411612912
47 2.24772002403688
48 2.45395864629604
49 2.82914656684103
50 3.43520724079644
51 4.30086188435849
52 5.34748866658591
53 6.43191791089129
54 7.27823488073754
55 6.68339205960951
56 4.74983654911286
57 3.22967386922976
58 2.24050023204534
59 1.51783777221967
60 0.989371008777324
61 0.614562371190264
62 0.351790149707654
63 0.167197744696925
64 0.0365448469033149
65 -0.0496309670624634
66 -0.0925930526530868
67 -0.102098785433105
68 -0.0938605049525491
69 -0.0823237096486566
70 -0.0780745991110289
71 -0.0744595959880817
72 -0.0644077285625043
73 -0.0517716834343596
74 -0.0403828499507661
75 -0.0309309724746801
76 -0.0233101204185358
77 -0.017510076033641
78 -0.013190627693022
79 -0.00990311159082292
80 -0.0074441997820569
81 -0.00566175064453264
82 -0.0043220488730468
83 -0.00330975165309812
84 -0.00258747879324581
85 -0.00210057063434111
86 -0.00209002502515474
87 -0.39352179747617
88 -3.71174957294804
89 -9.72079060710084
90 -16.9631592108713
91 -23.72149697119
92 -28.5330305131429
93 -30.8282243249037
94 -29.9482862419607
95 -25.3131943044255
96 -16.3964274512076
97 -4.62624874354812
98 7.7041895848357
99 17.4066999463952
};


==> plots/all/IliopsoasFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 -0.0552623438987708
1 -0.0473844606796558
2 -0.0458926382613352
3 -0.0412948003730184
4 -0.033168378105482
5 -0.0231007469070847
6 -0.0141120258073932
7 -0.00944927862944951
8 -0.00757749349581299
9 -0.00606199515657963
10 -0.00467267532838745
11 -0.00351924507854558
12 -0.00261823028259554
13 -0.00227343665848069
14 -0.00256968998111465
15 -0.00261440314187851
16 -0.0021700731770428
17 -0.00166389569820546
18 -0.00125398055979122
19 -0.000959109766264536
20 -0.000756294539773122
21 -0.000626764599872511
22 -0.000553718757123175
23 -0.000521625222924628
24 -0.000524048952884134
25 -0.000551611101381692
26 -0.000593063198812673
27 -0.000631129474105602
28 -0.000656989507038512
29 -0.000667593367183888
30 -0.00064906349385579
31 -0.000609655480681116
32 -0.000565200391446915
33 -0.000516649755604067
34 -0.000469686514917096
35 -0.000438433014854556
36 -0.000421925774129646
37 -0.000407913581884673
38 -0.000390279181920124
39 -0.000369843563352322
40 -0.000345498121541328
41 -0.000315813211707424
42 -0.000282486384597256
43 -0.00025221297714874
44 -0.000233355179170077
45 -0.000234868468926556
46 -0.000265145109045054
47 -0.000326190488287754
48 -0.000407680332242476
49 -0.00049435994157054
50 -0.000571936756861733
51 -0.000621910611248881
52 -0.000628975847221152
53 -0.000590441990173536
54 -0.00050965508210323
55 -0.000393291960417979
56 -0.000151928870913814
57 0.9876874832663
58 5.33658186446976
59 14.0535734756967
60 26.1872510878756
61 40.1979650680122
62 53.6048827463998
63 65.4656920524998
64 75.8040207973457
65 83.1360572256946
66 87.0048178473417
67 88.3524503687817
68 86.9799893090132
69 82.4384306293307
70 73.0473150501132
71 62.4122151563036
72 50.8080243820095
73 40.9703133238113
74 37.231739608511
75 38.7011454737614
76 40.0271846097556
77 40.3228200497435
78 38.8742412653286
79 35.5702888736097
80 31.4617825483302
81 28.2915339655854
82 25.9394839042967
83 23.0736617922628
84 19.4167969374602
85 14.7703401774838
86 8.41263133705302
87 3.25905680081421
88 3.73128612308471
89 4.8392497492365
90 2.54557254836993
91 0.167202805993781
92 -1.66572896019846
93 -1.94429289420927
94 -1.34884265863882
95 -0.860027953549923
96 -0.512983818485411
97 -0.289802108192316
98 -0.15698038748503
99 -0.0877697413600843
};
\addplot [semithick, color1]
table {%
0 0.0260264535552638
1 0.0117514952100582
2 -0.00200872461261381
3 -0.00877924484240012
4 -0.00943088535452616
5 -0.00621731478441346
6 -0.00237555698694891
7 -0.00115569272003813
8 -0.00154458377192411
9 -0.00166721829941276
10 -0.00149059930773559
11 -0.00122636614939984
12 -0.000972076316817429
13 -0.00104984436710708
14 -0.0015753593756223
15 -0.00180884139444721
16 -0.00157019621804857
17 -0.00124325352278995
18 -0.000974631506432761
19 -0.00078596481883587
20 -0.000660766476061137
21 -0.000585760149405856
22 -0.000549944773674805
23 -0.000544159119877324
24 -0.000564697487156533
25 -0.000603566837681464
26 -0.000650300849586681
27 -0.000689610552373773
28 -0.00071539318185245
29 -0.000726485794680013
30 -0.000715714163945015
31 -0.000691934412070114
32 -0.000666606125166917
33 -0.000638583635418834
34 -0.000609861571837012
35 -0.000586772630543744
36 -0.000569932212264451
37 -0.000556093421214211
38 -0.000545795835324023
39 -0.000541724159006425
40 -0.000543220803021132
41 -0.000546738591431012
42 -0.000548567084931531
43 -0.000545710044003299
44 -0.000536117492900259
45 -0.000518450172291931
46 -0.000497118424479745
47 -0.000480280509227903
48 -0.000471543028296953
49 -0.00047177147485179
50 -0.000478672420276373
51 -0.000480337506131052
52 -0.000462671535252573
53 -0.00041911968079016
54 -0.000347084093152504
55 -0.000247892659622829
56 -4.71681478332304e-05
57 0.374514132363127
58 2.44729416944401
59 7.52056681315211
60 15.805050720896
61 26.6098449391957
62 38.2712480369933
63 49.5721357114505
64 59.8520986975037
65 67.8309491434172
66 72.8906057743895
67 75.5408475414556
68 75.9089755399109
69 73.4393345705315
70 66.9872499780401
71 58.6324639548447
72 49.004354620993
73 40.1468341063923
74 35.2828360756487
75 34.6749198008661
76 35.1909051945785
77 35.404090210582
78 34.4155027227034
79 31.9206000773965
80 28.6336839275686
81 25.8242353445049
82 23.5548200432618
83 21.0125459456661
84 17.9115495617251
85 14.0084309268165
86 9.05236032617103
87 5.2321813492495
88 4.11950911440502
89 3.49673899041315
90 1.99410759274616
91 0.526653817922595
92 -0.430495498190349
93 -0.563117700015384
94 -0.371818756069327
95 -0.178643090229608
96 -0.0413423729931213
97 0.0359420542243945
98 0.0684558374531924
99 0.0696655129604907
};
\addplot [semithick, color2]
table {%
0 0.0550573974363504
1 0.033352688855138
2 0.0167736806297796
3 0.00774893933865471
4 0.00380919430608378
5 0.00300558829712207
6 0.00329457164175437
7 0.00266786578419683
8 0.00150754777837293
9 0.000775531930726131
10 0.000400571883075151
11 0.00020819478636526
12 0.000106341532975349
13 -0.000102881387864368
14 -0.000498223623808841
15 -0.000704932095477912
16 -0.000638300878230098
17 -0.000506707736905957
18 -0.000391877734288268
19 -0.000308810556591078
20 -0.000251761205148106
21 -0.000216039171408979
22 -0.000197509172839881
23 -0.00019233921763808
24 -0.000199253494910447
25 -0.000214646345803897
26 -0.000233636895836255
27 -0.000248784148142683
28 -0.000257229075003584
29 -0.000258501320324391
30 -0.000248414719721834
31 -0.000231062365339566
32 -0.000212217110052599
33 -0.000191272209702256
34 -0.000169587336659942
35 -0.000151041644707154
36 -0.000136308277209747
37 -0.000123441166563297
38 -0.00011194119812019
39 -0.000102276060180304
40 -9.3182876427099e-05
41 -8.21983859186955e-05
42 -6.73965527821484e-05
43 -4.82329972857908e-05
44 -2.56659446053295e-05
45 -1.9706193845542e-06
46 1.7377628530117e-05
47 2.58606519851244e-05
48 2.10125109273247e-05
49 3.5707217803599e-06
50 -2.29083600743494e-05
51 -4.94921873895937e-05
52 -6.64527108299492e-05
53 -6.87530844795664e-05
54 -5.42181883120192e-05
55 -2.32991610506813e-05
56 0.00010390673827794
57 0.694814496109504
58 4.16207899299943
59 12.0229497793111
60 24.0603244245954
61 38.9356948490264
62 54.2806612656962
63 68.531496786711
64 81.0511399090251
65 90.4582779361151
66 96.1139891412475
67 98.7404853448933
68 98.5777719063399
69 95.0688723289219
70 86.7539557494397
71 76.1031327043773
72 63.8922716648676
73 52.5957214906519
74 46.2697677720025
75 45.4574239340064
76 46.2687356303356
77 46.8377642145166
78 45.9733758672948
79 43.2302141807156
80 39.394845556705
81 36.0335693053127
82 33.3388760866563
83 30.3360850545568
84 26.6189993213856
85 21.8785180296568
86 15.8589885682164
87 11.8936141127786
88 9.69115153539813
89 8.6666619625007
90 4.5481572847211
91 1.28776507956986
92 0.463022604570009
93 0.19569396863253
94 0.158252874759263
95 0.161493883799686
96 0.164950939375349
97 0.159646697272192
98 0.148449774930781
99 0.129372508394705
};
\addplot [semithick, color3]
table {%
0 0.368235049902719
1 0.299395462155612
2 0.239934042201548
3 0.193573983596287
4 0.158624376592949
5 0.132408018120086
6 0.111562014274057
7 0.0928229096624118
8 0.0762873119083645
9 0.0628162744475993
10 0.0519780299233421
11 0.0432150348341589
12 0.0361219072476995
13 0.030180696009715
14 0.0250802237632778
15 0.0212398475905469
16 0.0187583996544249
17 0.0172480707754292
18 0.0164913844890127
19 0.0162964922653108
20 0.0164743694381005
21 0.0168631716411967
22 0.0174182302181572
23 0.0182928996249352
24 0.0192134810460086
25 0.0200552753429062
26 0.0207591789633258
27 0.0212889941985313
28 0.0216847992438916
29 0.0219923960500297
30 0.0224007947346443
31 0.0229928044359044
32 0.0237014327304523
33 0.0244622364910422
34 0.0251692595901293
35 0.0257168557128355
36 0.026125106953981
37 0.026554262858033
38 0.0271925620670087
39 0.0281440440800995
40 0.0294569809088154
41 0.0310846865528427
42 0.032873076944328
43 0.0345413768664215
44 0.035769031126152
45 0.0362045556630643
46 0.0356143244902077
47 0.0342318499770342
48 0.0324512099325198
49 0.0303144800555661
50 0.0278567137559945
51 0.0252930873953662
52 0.0227875834583729
53 0.0204231798640628
54 0.0182033625143476
55 0.0160848867595026
56 0.0142901219881412
57 1.51042627066769
58 5.66984523673439
59 11.3381988612375
60 18.4427816900043
61 26.7076797138641
62 34.9764890470994
63 42.6359679689314
64 49.45987490243
65 54.4980674376779
66 57.3853779409139
67 58.6973382457268
68 58.543605792926
69 56.5245630475247
70 51.5800953075022
71 45.4064499588938
72 38.3319589335978
73 31.9376351112017
74 28.8913460932282
75 29.268205443278
76 30.2555962691571
77 30.6945146240106
78 29.950037910867
79 27.9265815407902
80 25.3776043900545
81 23.3030562303475
82 21.6921147408547
83 19.7700948506835
84 17.3082824415873
85 14.1086057644129
86 9.69831559496168
87 5.91713039680911
88 5.56889877771867
89 5.73089316876002
90 4.35500846848782
91 3.01333737728291
92 1.54486257031257
93 0.781697133890979
94 0.793355899572508
95 0.805807040395145
96 0.78182394856269
97 0.722594051625439
98 0.64177136075735
99 0.550180817857344
};
\addplot [semithick, color4]
table {%
0 0.0398927022890826
1 0.0342080786018579
2 0.0331293322511748
3 0.0298151595884531
4 0.0239607220067762
5 0.0167097615970169
6 0.0102377349894953
7 0.00688207191974317
8 0.00553498316573743
9 0.0044429938438563
10 0.00344228872123157
11 0.00261205124399641
12 0.00196423762749865
13 0.00171777622328294
14 0.00193402053440155
15 0.0019715959940917
16 0.00166280038357492
17 0.00131518132799334
18 0.0010421333561611
19 0.000854923484848475
20 0.000734407921919308
21 0.000665265592233497
22 0.00063525468001642
23 0.000634903797451876
24 0.000659859524158872
25 0.000702327341962143
26 0.000752388905414615
27 0.000796150446332334
28 0.000827838900092795
29 0.00084620121475752
30 0.000846063902660699
31 0.000835892321590217
32 0.000825720444783813
33 0.000814604025919336
34 0.000803596679312177
35 0.000796899062117156
36 0.00079434143791435
37 0.000793686641785577
38 0.000796914607722218
39 0.000808105276043592
40 0.000828495112975
41 0.000856280181741934
42 0.000888294520066347
43 0.000919999512217051
44 0.000945693466394314
45 0.000958458761467787
46 0.000955913993245902
47 0.000940686076933628
48 0.000914780237009557
49 0.00088122178392471
50 0.000842554510120426
51 0.000793920666330223
52 0.000728056052707273
53 0.000642645670125083
54 0.00053713586228016
55 0.000413068093838196
56 0.000209653235580289
57 0.721728091877018
58 5.18312872485428
59 16.7225046218544
60 36.0294004034964
61 61.4171570129089
62 88.8577752281845
63 115.472780943873
64 139.638953910264
65 158.336120182052
66 170.245632195765
67 176.592395498149
68 177.666963443472
69 172.176765139507
70 157.563291542931
71 138.481436387454
72 116.292844616818
73 95.7106113995529
74 84.3448662488998
75 82.916733943403
76 84.0545344234176
77 84.313570600891
78 81.5094324346457
79 74.9340051833608
80 66.4448285738399
81 59.1970583850719
82 53.1983197246912
83 46.3873487606142
84 38.1300693532018
85 27.7648526653278
86 15.0003521389472
87 6.4061487774684
88 4.66166579146354
89 3.00734669782754
90 0.343325463491828
91 1.27781194096225
92 1.6746964948892
93 1.40147093665183
94 0.971789127042943
95 0.61969296126126
96 0.369696215117167
97 0.208914431800852
98 0.113218746247565
99 0.0633439951978196
};
\addplot [semithick, color5]
table {%
0 0.188659425218449
1 0.131555525633872
2 0.0893810168571253
3 0.0608494900556445
4 0.042264527621112
5 0.0304145707870816
6 0.0225706333299873
7 0.0163798303293586
8 0.0114526247895047
9 0.00800536118095712
10 0.00565043498397498
11 0.00402266130510989
12 0.00288570530053289
13 0.00198978013543404
14 0.00124398329789852
15 0.000797130484290632
16 0.000574306734939536
17 0.000449730056923915
18 0.000376388837265012
19 0.000335943309447927
20 0.000318479801881923
21 0.000315769326779573
22 0.000321805451629017
23 0.000333381511011677
24 0.000347839417574072
25 0.000363983244599034
26 0.000381080300504056
27 0.000399440278764114
28 0.000418624876221185
29 0.000438231821558324
30 0.000461934497641191
31 0.000490884859471297
32 0.000524017239478246
33 0.00056178750561384
34 0.000602209285371065
35 0.00064077442025113
36 0.000675323321747999
37 0.000707795278138231
38 0.000741955416122233
39 0.000781829826244771
40 0.000832314442616869
41 0.000897572115539928
42 0.000978652769912467
43 0.0010711891098076
44 0.00116525855386092
45 0.00124574009274284
46 0.00129472568309658
47 0.0012979679439077
48 0.00125134791258644
49 0.00116081745140366
50 0.00103942787429344
51 0.00090501473086305
52 0.00077409721703606
53 0.000656752943176335
54 0.000557756254262079
55 0.000478232554915683
56 0.000457441614108593
57 0.542638367476558
58 3.23177313746824
59 9.37471001487284
60 19.0224730566929
61 31.3554813460819
62 44.5712324061419
63 57.4372079382034
64 69.3108163632388
65 78.7322106118208
66 84.9755549683432
67 88.6059656326258
68 89.6645958211296
69 87.23657465279
70 79.964779587783
71 70.3257186975482
72 58.978076651211
73 48.4745698296685
74 42.7922142435237
75 42.1152257107627
76 42.5958334019738
77 42.6225427483026
78 41.2496809212468
79 38.2315317884615
80 34.4665645755604
81 31.370707513231
82 28.9749941936593
83 26.3738913178284
84 23.2593673370172
85 19.4324800814622
86 14.4946985299558
87 10.0232471119191
88 8.23265473129386
89 7.74891562179456
90 6.51484153451503
91 5.01019040386115
92 3.51311457511584
93 2.41025097657453
94 1.73236221136538
95 1.2702962744033
96 0.941736215726429
97 0.700352944189406
98 0.51941399407445
99 0.380664922822378
};
\addplot [semithick, black]
table {%
0 -0.0478712427468991
1 -0.0410496943222295
2 -0.0397551987014097
3 -0.0357781915061437
4 -0.0287528664081314
5 -0.0200517139164203
6 -0.0122852819873944
7 -0.00825848630369181
8 -0.00664197979888492
9 -0.00533159261262756
10 -0.00413074646547789
11 -0.00313446149279569
12 -0.00235708515299838
13 -0.00206133146793952
14 -0.00232082464128186
15 -0.00236591519291003
16 -0.00199536046028991
17 -0.00157821759359201
18 -0.00125056002739332
19 -0.00102590818181817
20 -0.00088128950630317
21 -0.000798318710680197
22 -0.000762305616019703
23 -0.000761884556942251
24 -0.000791831428990646
25 -0.000842792810354571
26 -0.000902866686497538
27 -0.000955380535598801
28 -0.000993406680111354
29 -0.00101544145770902
30 -0.00101527668319284
31 -0.00100307078590826
32 -0.000990864533740576
33 -0.000977524831103203
34 -0.000964316015174612
35 -0.000956278874540587
36 -0.00095320972549722
37 -0.000952423970142692
38 -0.000956297529266662
39 -0.000969726331252311
40 -0.00099419413557
41 -0.00102753621809032
42 -0.00106595342407962
43 -0.00110399941466046
44 -0.00113483215967318
45 -0.00115015051376134
46 -0.00114709679189508
47 -0.00112882329232035
48 -0.00109773628441147
49 -0.00105746614070965
50 -0.00101106541214451
51 -0.000952704799596267
52 -0.000873667263248728
53 -0.000771174804150099
54 -0.000644563034736192
55 -0.000495681712605835
56 -0.000251583882696347
57 0.180395088494928
58 1.29578218121357
59 4.1806261554636
60 9.00735010087411
61 15.3542892532272
62 22.2144438070461
63 28.8681952359683
64 34.909738477566
65 39.5840300455129
66 42.5614080489414
67 44.1480988745372
68 44.4167408608681
69 43.0441912848766
70 39.3908228857327
71 34.6203590968634
72 29.0732111542045
73 23.9276528498882
74 21.086216562225
75 20.7291834858508
76 21.0136336058544
77 21.0783926502228
78 20.3773581086614
79 18.7335012958402
80 16.61120714346
81 14.799264596268
82 13.2995799311728
83 11.5968371901535
84 9.53251733830045
85 6.94121316633195
86 3.7500880347368
87 1.6015371943671
88 1.16541644786588
89 0.712904839500983
90 -0.411990556190194
91 -1.5333743291547
92 -2.00963579386704
93 -1.6817651239822
94 -1.16614695245153
95 -0.743631553513512
96 -0.4436354581406
97 -0.250697318161022
98 -0.135862495497078
99 -0.0760127942373835
};


==> plots/all/IliopsoasTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 -0.0755836130437033
1 -0.0648084630909881
2 -0.0627683058513654
3 -0.0564789199322331
4 -0.0453623170804797
5 -0.0315899255561579
6 -0.0192931686812118
7 -0.0129141590606211
8 -0.0103533727068299
9 -0.0082802151115085
10 -0.00637959650831878
11 -0.00480157297240593
12 -0.00356874209982049
13 -0.00309668316735257
14 -0.0035013647142015
15 -0.00356144730397752
16 -0.00295147317998197
17 -0.00225584032737223
18 -0.0016908996603568
19 -0.00128272584744681
20 -0.00100033138746999
21 -0.000818375568521847
22 -0.000713909556239174
23 -0.000665373892518895
24 -0.000663907682928706
25 -0.000696868536425991
26 -0.000749215824639969
27 -0.000797607089335781
28 -0.000829891654625985
29 -0.000841731980926158
30 -0.000813211312765016
31 -0.000755126301381552
32 -0.000689391057013939
33 -0.000617624479345127
34 -0.000548216016841145
35 -0.000498881623903886
36 -0.000468366897289222
37 -0.000440457800331179
38 -0.00040581468820765
39 -0.000364389724415017
40 -0.000313718960938979
41 -0.000251649161267994
42 -0.000181467129726113
43 -0.00011509092941796
44 -6.79088261735602e-05
45 -5.7188725832382e-05
46 -9.82267389158222e-05
47 -0.000194418983771255
48 -0.000329160836048233
49 -0.000477023929142232
50 -0.000613805237584182
51 -0.000710805830073965
52 -0.000745328071133693
53 -0.000713528331184626
54 -0.000620930739239838
55 -0.0004778741345112
56 -0.000160008701002472
57 1.62163559282698
58 8.55478383330771
59 22.0212148815176
60 40.5138397962281
61 62.0547283406391
62 82.8225067798742
63 101.234179548179
64 117.224138099586
65 128.2517610627
66 133.49612814753
67 134.74144505291
68 131.984453599815
69 124.517430310459
70 109.049860690167
71 92.1499394066698
72 74.1637489015608
73 59.3914521860084
74 54.5588819314825
75 58.1629367857414
76 61.3337400617525
77 62.6915574513503
78 61.0070868557909
79 56.0725948394682
80 49.6722697439343
81 44.9442992115618
82 41.6833474056339
83 37.3931633204185
84 31.5911911939374
85 24.0702001239359
86 13.4430525944496
87 4.82142690893628
88 5.49987896536318
89 7.09930880376212
90 3.77102104901797
91 0.421333221983507
92 -2.20964768323503
93 -2.65958271269376
94 -1.84514219062429
95 -1.17645894145224
96 -0.701716278537866
97 -0.396414152387323
98 -0.214721793971565
99 -0.120047171580165
};
\addplot [semithick, color1]
table {%
0 0.191509787943184
1 0.129982361322548
2 0.0825323419590503
3 0.0517225643696084
4 0.0339000805274856
5 0.0248331784133752
6 0.0198832475484003
7 0.014808246184497
8 0.00992008922986263
9 0.00658097782428453
10 0.00445726316382033
11 0.00307614570014071
12 0.00215379934756036
13 0.00123512264569322
14 0.000110669871857112
15 -0.000546616552073618
16 -0.000604930604256363
17 -0.000481311562427043
18 -0.000345884936218176
19 -0.000238376358533867
20 -0.000156826804617511
21 -9.94618600573536e-05
22 -6.36104352044955e-05
23 -4.50955039662941e-05
24 -4.36519156686164e-05
25 -5.4383815296841e-05
26 -7.01136358613684e-05
27 -7.87343258933684e-05
28 -7.60536110850757e-05
29 -6.17031111757284e-05
30 -2.62964979221243e-05
31 2.43013725869139e-05
32 7.99701974118531e-05
33 0.000141886842085645
34 0.000206376462597821
35 0.000264132642052903
36 0.000312654362141677
37 0.000356483357975799
38 0.00039930796356628
39 0.000443531880931587
40 0.000494736382334556
41 0.000559641657941244
42 0.000641743527312504
43 0.000738391775640972
44 0.000840609454275975
45 0.000933731553472984
46 0.000996656866435842
47 0.00100974938616951
48 0.00096667890778574
49 0.000872967822827092
50 0.000743218335761138
51 0.000603320565462786
52 0.000479735914215361
53 0.000387703533006941
54 0.000334269621711818
55 0.000319315380027841
56 0.000420496299304386
57 0.719658000083082
58 4.35694076412563
59 12.8129960924365
60 26.2991950419455
61 43.7271468041833
62 62.3929801117076
63 80.1674268456404
64 96.0044241566671
65 107.981924491897
66 115.062338435838
67 118.073573802759
68 117.400784799075
69 112.604538427649
70 101.792706114871
71 88.2505425801782
72 73.1486757866892
73 59.4640265820305
74 51.9027244973692
75 51.0755013616807
76 52.4046931708893
77 53.6355129770167
78 53.2552919040523
79 50.6044963194924
80 46.4850787330898
81 42.7840525253848
82 39.8751841966379
83 36.6262245321264
84 32.4949976379961
85 27.125385185724
86 19.7922999388548
87 13.0289474744786
88 10.4694225642017
89 9.66392704849858
90 7.63978301501349
91 5.3276750539997
92 3.21433790007316
93 1.99424094447911
94 1.4319494372097
95 1.09837611623832
96 0.865020466104604
97 0.680300092778572
98 0.527044053821373
99 0.396280306165624
};
\addplot [semithick, color2]
table {%
0 0.058019415494158
1 0.0229001388397124
2 -0.0047499277282405
3 -0.0145226379401203
4 -0.0144550666980758
5 -0.00970520602826128
6 -0.00417063987268231
7 -0.00219373911340864
8 -0.00260527644900042
9 -0.0026001656060577
10 -0.00222436422175472
11 -0.001780230521081
12 -0.00138439062374318
13 -0.00136440977033163
14 -0.00175497311301954
15 -0.00187811853288624
16 -0.00160173074593539
17 -0.00126755786303058
18 -0.00100054392041943
19 -0.000815703225055495
20 -0.00069518589984767
21 -0.000624714902218833
22 -0.000592783881724814
23 -0.000590255543080068
24 -0.000613158718088511
25 -0.000653717895824332
26 -0.000701890193106309
27 -0.0007433692096351
28 -0.000772316693177316
29 -0.000787519224388354
30 -0.00078297544716976
31 -0.00076710617892671
32 -0.000750341538808954
33 -0.000731519941540479
34 -0.000712011839883315
35 -0.000697053365854
36 -0.000686990316322389
37 -0.000679148123357821
38 -0.000674828339369591
39 -0.000677462139309059
40 -0.000687216759702911
41 -0.000701078407030882
42 -0.000715169292997294
43 -0.000725366500242527
44 -0.000727740403040719
45 -0.000718642407865623
46 -0.000700865441749943
47 -0.000682349516044329
48 -0.000667110396570518
49 -0.000656486345077944
50 -0.000648487912099463
51 -0.000631768429223449
52 -0.000594019284248314
53 -0.000531055681861741
54 -0.000441736445839083
55 -0.000326637593993373
56 4.01725822630686e-05
57 0.975784801458332
58 5.64975227218601
59 15.9061596731299
60 31.2614632728369
61 49.9553684512374
62 68.968755527635
63 86.3523799791005
64 101.420424809953
65 112.633405578811
66 119.246333557012
67 122.137161842308
68 121.660380601007
69 117.316275549214
70 107.256572820228
71 94.3572714498243
72 79.5864336904847
73 65.851186452859
74 58.1038100070723
75 57.308418928952
76 58.8168150677798
77 60.2504969782429
78 60.0283827251852
79 57.4663137734718
80 53.358592565095
81 49.6331795017244
82 46.7103335529304
83 43.4240523775074
84 39.178736384056
85 33.5607421006993
86 25.638572850376
87 17.8600920857473
88 14.6653555077271
89 13.4351561669093
90 7.87452396271216
91 0.954925383031147
92 -0.786043465369568
93 -0.876723085915246
94 -0.583857936501949
95 -0.30261260992228
96 -0.0874348822172738
97 0.0592875028929141
98 0.149136478934151
99 0.176412978469202
};
\addplot [semithick, color3]
table {%
0 -0.0306975118531288
1 -0.0303036581555265
2 -0.0330163334467872
3 -0.031546863751612
4 -0.0260949693584421
5 -0.0183834261525
6 -0.0112388239827274
7 -0.00759920316133789
8 -0.00622350972527906
9 -0.0050645808650275
10 -0.00395933373222055
11 -0.0030234719927387
12 -0.00228434822819658
13 -0.00201236862731676
14 -0.00228611483455451
15 -0.00234029791061554
16 -0.00197581107950008
17 -0.00156240220061783
18 -0.00123674018774663
19 -0.00101289927198413
20 -0.000868344844612522
21 -0.000784975116449687
22 -0.000748162488661294
23 -0.000746243307937755
24 -0.000774429555612067
25 -0.000823616331685548
26 -0.000882085374179974
27 -0.000933340016075768
28 -0.000970422538236044
29 -0.000991751521703434
30 -0.000990726733709317
31 -0.000977262272549922
32 -0.000963479150508347
33 -0.000948383639936042
34 -0.00093349556067388
35 -0.000924121105608635
36 -0.000920025756584482
37 -0.000918113521835676
38 -0.000920212907256662
39 -0.00093084010394609
40 -0.000951203121062088
41 -0.000979119249722107
42 -0.00101115787724355
43 -0.00104286594887973
44 -0.00106879610192955
45 -0.00108234351397463
46 -0.00108172147854019
47 -0.00106894139294858
48 -0.00104454281584147
49 -0.00101167964603902
50 -0.000973020392516436
51 -0.000921906109384742
52 -0.000849192354983524
53 -0.000752011502353882
54 -0.000629830307505352
55 -0.000484682173373778
56 -0.000243705280179798
57 1.02921656527309
58 6.61041226802187
59 18.6253208158022
60 35.1068906284843
61 53.6044663616187
62 70.3197900990795
63 84.1524394227104
64 95.6666104722504
65 102.538111821714
66 104.180313721502
67 103.116222373722
68 99.7776607418402
69 93.5467940786747
70 80.9177268501837
71 67.1787189041603
72 52.8658793766622
73 41.3139665408898
74 37.5367120870384
75 40.7346370926976
76 44.7613590010672
77 47.0417845175292
78 46.2633373123805
79 42.619917818952
80 38.2530206484494
81 35.1067542039968
82 33.0852482344015
83 30.3126095857705
84 26.3196046285079
85 20.9780290615992
86 13.0291555891394
87 5.92384755033307
88 5.7167791989806
89 6.81855556692058
90 4.54876694213219
91 1.92622054064507
92 -0.270686711943335
93 -0.920820016887231
94 -0.692503318092144
95 -0.448614527416522
96 -0.259928038250121
97 -0.136322477069115
98 -0.0646592139657425
99 -0.0316767643075026
};
\addplot [semithick, color4]
table {%
0 -0.0209236519949132
1 -0.0179420768965002
2 -0.0173762763380694
3 -0.015637998621425
4 -0.0125673564348597
5 -0.00876424048790569
6 -0.0053696739464794
7 -0.00360963458452094
8 -0.00290308890880242
9 -0.0023303424353339
10 -0.00180547436338438
11 -0.00137001627080094
12 -0.00103023917144724
13 -0.000900970599601238
14 -0.00101439035940939
15 -0.0010340986217479
16 -0.000872135868631071
17 -0.000689810287047697
18 -0.00054659710737553
19 -0.000448405860039803
20 -0.000385195659827545
21 -0.00034893062984838
22 -0.000333189959318475
23 -0.000333005922032197
24 -0.000346095156677508
25 -0.000368369452218079
26 -0.000394626653959146
27 -0.000417579504991604
28 -0.000434200043102462
29 -0.000443831044759899
30 -0.000443759024807283
31 -0.000438424048474655
32 -0.000433088917029058
33 -0.000427258374939819
34 -0.00042148504105718
35 -0.000417972152650467
36 -0.000416630683266781
37 -0.000416287243852054
38 -0.000417980306292905
39 -0.00042384979209134
40 -0.000434544225601865
41 -0.00044911744516772
42 -0.000465908909157632
43 -0.000482538121625005
44 -0.000496014555276516
45 -0.000502709930029376
46 -0.000501375203585011
47 -0.000493388188335536
48 -0.000479800620983511
49 -0.000462199271524988
50 -0.000441918354609157
51 -0.000416409989312989
52 -0.000381864115628138
53 -0.000337066520595545
54 -0.000281726812460468
55 -0.000216653486721501
56 -0.000109962752312471
57 0.702976405085106
58 5.04873661925892
59 16.2889107973016
60 35.0952026938495
61 59.8246862314935
62 86.5538032171922
63 112.47871481243
64 136.018288857293
65 154.230660774681
66 165.831373898554
67 172.013573492567
68 173.06027922253
69 167.712434957866
70 153.477870624587
71 134.890784329608
72 113.277515250448
73 93.2289538377554
74 82.1579083759469
75 80.7668057715811
76 81.8751044949591
77 82.1274241853136
78 79.395993847206
79 72.9910592771566
80 64.7219964984679
81 57.6621520102269
82 51.818953210475
83 45.1845822842519
84 37.1414039005571
85 27.044944438209
86 14.6114115944151
87 6.24004527731168
88 4.54079457360386
89 2.88913402115971
90 -0.180073600104579
91 -0.670210109455421
92 -0.878375358035148
93 -0.735069034606686
94 -0.509701683263799
95 -0.325027865276408
96 -0.193905012823989
97 -0.109575251033128
98 -0.0593830327315966
99 -0.0332238137662924
};
\addplot [semithick, color5]
table {%
0 0.153430607387691
1 0.101649055860028
2 0.0606863850768137
3 0.0350623408062296
4 0.0215263565095674
5 0.0159742123335255
6 0.0137439263219475
7 0.0104508935939209
8 0.00668675676648218
9 0.0041775739334038
10 0.00268271366767656
11 0.00176965745667815
12 0.00119105922807634
13 0.000496180167807915
14 -0.000500530932879905
15 -0.0010513663819206
16 -0.00100487641777445
17 -0.000797757821890762
18 -0.000604019114797106
19 -0.000459583433073393
20 -0.00035696645029303
21 -0.000289905067856585
22 -0.00025237003045677
23 -0.000238019295307992
24 -0.000245241263720712
25 -0.000267664376506565
26 -0.000296441533173373
27 -0.000317590363234071
28 -0.000325966388534777
29 -0.000320884140230447
30 -0.000293319420416215
31 -0.000250581094214907
32 -0.000203811007719354
33 -0.00015174971628582
34 -9.75919788603122e-05
35 -5.00010179968602e-05
36 -1.09061044459205e-05
37 2.39780651143937e-05
38 5.69109548652661e-05
39 8.84674866223343e-05
40 0.000122671733724229
41 0.000165461879086059
42 0.000220690997011521
43 0.000287791805441612
44 0.000361525215578004
45 0.000432462740989332
46 0.000484456197119517
47 0.000500801531158918
48 0.00047564003989279
49 0.000412337917343636
50 0.000321778045784746
51 0.000226315395090056
52 0.000149452306988821
53 0.000104028519761504
54 9.58124451136883e-05
55 0.000124351082007134
56 0.000276966128397118
57 0.649684726127944
58 3.989649448322
59 11.7742163077027
60 24.0710556710946
61 39.7471802138827
62 56.4068038347781
63 72.4155170948425
64 86.9609444791269
65 98.3038864001605
66 105.617733567231
67 109.641622507594
68 110.50865633544
69 107.279738885307
70 98.2919209313881
71 86.4792378705838
72 72.6647103044739
73 59.8577171878505
74 52.8655880240372
75 52.0918132742116
76 52.9125100386479
77 53.2657133027063
78 51.8766927572674
79 48.3358080287522
80 43.6932728066915
81 39.7699093905056
82 36.6605278806131
83 33.2004584747485
84 28.9705572742722
85 23.6540901701162
86 16.7799397299354
87 10.9623985278406
88 8.90500870516381
89 8.12536940055926
90 6.1462447682916
91 3.88254512448461
92 2.05237034060491
93 1.18635363381791
94 0.885204529262242
95 0.731531630398767
96 0.620600915338958
97 0.518147602275688
98 0.419490037783992
99 0.323800345564878
};
\addplot [semithick, black]
table {%
0 -0.0478712427468991
1 -0.0410496943222295
2 -0.0397551987014097
3 -0.0357781915061437
4 -0.0287528664081314
5 -0.0200517139164203
6 -0.0122852819873944
7 -0.00825848630369181
8 -0.00664197979888492
9 -0.00533159261262756
10 -0.00413074646547789
11 -0.00313446149279569
12 -0.00235708515299838
13 -0.00206133146793952
14 -0.00232082464128186
15 -0.00236591519291003
16 -0.00199536046028991
17 -0.00157821759359201
18 -0.00125056002739332
19 -0.00102590818181817
20 -0.00088128950630317
21 -0.000798318710680197
22 -0.000762305616019703
23 -0.000761884556942251
24 -0.000791831428990646
25 -0.000842792810354571
26 -0.000902866686497538
27 -0.000955380535598801
28 -0.000993406680111354
29 -0.00101544145770902
30 -0.00101527668319284
31 -0.00100307078590826
32 -0.000990864533740576
33 -0.000977524831103203
34 -0.000964316015174612
35 -0.000956278874540587
36 -0.00095320972549722
37 -0.000952423970142692
38 -0.000956297529266662
39 -0.000969726331252311
40 -0.00099419413557
41 -0.00102753621809032
42 -0.00106595342407962
43 -0.00110399941466046
44 -0.00113483215967318
45 -0.00115015051376134
46 -0.00114709679189508
47 -0.00112882329232035
48 -0.00109773628441147
49 -0.00105746614070965
50 -0.00101106541214451
51 -0.000952704799596267
52 -0.000873667263248728
53 -0.000771174804150099
54 -0.000644563034736192
55 -0.000495681712605835
56 -0.000251583882696347
57 0.180395088494928
58 1.29578218121357
59 4.1806261554636
60 9.00735010087411
61 15.3542892532272
62 22.2144438070461
63 28.8681952359683
64 34.909738477566
65 39.5840300455129
66 42.5614080489414
67 44.1480988745372
68 44.4167408608681
69 43.0441912848766
70 39.3908228857327
71 34.6203590968634
72 29.0732111542045
73 23.9276528498882
74 21.086216562225
75 20.7291834858508
76 21.0136336058544
77 21.0783926502228
78 20.3773581086614
79 18.7335012958402
80 16.61120714346
81 14.799264596268
82 13.2995799311728
83 11.5968371901535
84 9.53251733830045
85 6.94121316633195
86 3.7500880347368
87 1.6015371943671
88 1.16541644786588
89 0.712904839500983
90 -0.411990556190194
91 -1.5333743291547
92 -2.00963579386704
93 -1.6817651239822
94 -1.16614695245153
95 -0.743631553513512
96 -0.4436354581406
97 -0.250697318161022
98 -0.135862495497078
99 -0.0760127942373835
};


==> plots/all/RectusFemorisFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 -0.000703139033886595
1 -0.000544621124542507
2 -0.000533202565058065
3 -0.000412598906852997
4 -0.000252960811823242
5 -8.74443310694724e-05
6 7.56962847129953e-05
7 0.000247693782725893
8 0.000471127613169243
9 -0.00288704371644042
10 -0.011049176565938
11 -0.0135927048455992
12 0.39218006903755
13 1.06283595812572
14 2.23491936528716
15 2.22060758611137
16 1.69961438902635
17 1.31056098919004
18 0.763705861561045
19 0.153175143410207
20 -0.286504584516928
21 -0.397937518253345
22 -0.186670755537771
23 0.190858010544568
24 0.536028834601102
25 0.741156851345563
26 0.791497051897008
27 0.708995366650278
28 0.551320310382291
29 0.381866872931153
30 0.266162306416922
31 0.22385670314756
32 0.214973839790337
33 0.194382941021932
34 0.135510633080256
35 0.0366569415132512
36 -0.0850442686170473
37 -0.185312584457908
38 -0.220111195515366
39 -0.191763665507244
40 -0.136838527661173
41 -0.0909633816412851
42 -0.0666856364395241
43 -0.0733296757146231
44 -0.120932717101457
45 -0.175185206353823
46 -0.206814459660279
47 -0.213763480450859
48 -0.195514125353758
49 -0.163534158934213
50 -0.132061011614789
51 -0.10565172504085
52 -0.0845225192484623
53 -0.0683897072167824
54 -0.0568363665039214
55 -0.050163284678456
56 0.0109621525709096
57 3.67244300223426
58 4.66111497914196
59 -6.47672207524223
60 -22.3335035301099
61 -37.6807028966697
62 -43.9503680565097
63 -38.6487217446456
64 -26.70922905013
65 -16.0300597104341
66 -9.79252329635311
67 -6.66584967063405
68 -5.92223233426012
69 -6.94103077002652
70 -7.80510783099327
71 -6.81700119227912
72 -3.63164842794076
73 0.256216984369797
74 3.31223258928032
75 5.48506093833762
76 7.40973536982573
77 8.67805488844332
78 9.32086645275556
79 9.39312292325062
80 9.11103938938782
81 8.74928818798899
82 8.33900872096061
83 7.82779916854719
84 6.85900056177893
85 4.86156080271367
86 3.52105854676299
87 2.54491014080883
88 1.77377839204084
89 1.17827374771451
90 0.758906932070082
91 0.476673437635648
92 0.29136308414228
93 0.172910827915429
94 0.0993286350511289
95 0.054975972621865
96 0.0290763396261795
97 0.0144454382722514
98 0.00648432301335005
99 0.00236324242124302
};
\addplot [semithick, color1]
table {%
0 0.00297341138955667
1 0.00208516981014302
2 0.00136233726705306
3 0.000935155190539045
4 0.000684471108057165
5 0.000537845713095765
6 0.00045476594755129
7 0.000418073926717011
8 0.000435164979199486
9 -0.00268975230466111
10 -0.0101310183041982
11 -0.0303713493246958
12 0.0670178133201708
13 0.492727131519843
14 1.23242584573342
15 1.36531898983763
16 1.16376053500511
17 0.921433121994353
18 0.581427651803232
19 0.220695528905298
20 0.000415248048259931
21 0.0222176442486247
22 0.264464097845369
23 0.600055193008624
24 0.888026163853815
25 1.05853242005546
26 1.10236668623815
27 1.03789305439434
28 0.905356640574624
29 0.754555216625107
30 0.631606605610173
31 0.55175582527679
32 0.49658042429665
33 0.438924468063533
34 0.361305944630194
35 0.260770024621184
36 0.148618283020076
37 0.054120475812617
38 0.0027702997344376
39 -0.00763177383040761
40 0.000119293175984441
41 0.00650979223023107
42 0.00435257623599686
43 -0.0157114710700043
44 -0.0549557919552666
45 -0.0949390752959974
46 -0.121663158360527
47 -0.129893900076891
48 -0.120626948290382
49 -0.103176632215796
50 -0.0855375425307766
51 -0.0703086043407445
52 -0.0577756111007161
53 -0.0480807717676734
54 -0.0412998607116818
55 -0.0386139010519704
56 -0.00705702014244965
57 2.12324455309805
58 2.2770464878412
59 -6.28378023917827
60 -19.35456189782
61 -31.7076880639568
62 -36.4118801289315
63 -31.6354949552786
64 -21.6015066773696
65 -12.8951869036952
66 -7.97461832726554
67 -5.55831468473821
68 -4.81483111453547
69 -5.14003543448033
70 -5.27273250085444
71 -4.04723307452913
72 -1.25639364357252
73 1.96275888212221
74 4.55291445891657
75 6.51047290883199
76 8.21848037336939
77 9.4095187069484
78 10.0553913386345
79 10.1650619948013
80 9.91025225114353
81 9.53478582618087
82 9.0866799410534
83 8.53282550641992
84 7.56351077831722
85 5.66726576678058
86 4.15092142634153
87 3.00335123417883
88 2.08719154191565
89 1.38188333007044
90 0.892615380541452
91 0.566971120607324
92 0.354094712758348
93 0.217558984533811
94 0.131665923906843
95 0.0786429659121032
96 0.0464735906401208
97 0.0272374772603319
98 0.0158679420374377
99 0.00921494602462
};
\addplot [semithick, color2]
table {%
0 0.00386257606068963
1 0.00257647774992838
2 0.00164668297440833
3 0.00117412159017561
4 0.000918738960992446
5 0.000782446918836498
6 0.000721362332539824
7 0.000718395741039339
8 0.000778539453168907
9 -0.000815757652062395
10 -0.004563718403234
11 -0.0122867328331454
12 0.0883273528341182
13 1.10933242690269
14 2.49528807553943
15 3.12332570403676
16 1.7666732126656
17 1.07979107929014
18 0.763511807725485
19 0.540593337359715
20 0.412306730876486
21 0.412589496734877
22 0.536021558173264
23 0.7479836801038
24 1.04351153203867
25 1.42187313545941
26 1.71307499216992
27 1.67439952860022
28 1.36832263536181
29 1.03919032809366
30 0.823286929346386
31 0.715270147863379
32 0.653906686782277
33 0.57372459730461
34 0.450665260228767
35 0.314726650388717
36 0.199535568676976
37 0.117835963600053
38 0.0706224566237342
39 0.0508225799027694
40 0.0453149096675007
41 0.0428047981446011
42 0.0382337032550826
43 0.0256486121669797
44 0.00251831538072863
45 -0.0221175150460185
46 -0.0403890578138615
47 -0.0493872260907436
48 -0.0490358006916349
49 -0.0435695678271195
50 -0.0371202470317558
51 -0.0312029746533777
52 -0.026134521064984
53 -0.0221236693034235
54 -0.0192913490581956
55 -0.0181474178597131
56 0.0088332763017739
57 3.24653756931548
58 4.28821989959511
59 -2.68987926743219
60 -9.43994205471857
61 -15.8268065368175
62 -18.2618221539677
63 -15.8436878012933
64 -10.777592334665
65 -6.34637547898466
66 -3.75639661155968
67 -2.36042770415738
68 -1.81868275455284
69 -1.90275324924193
70 -1.96019795975442
71 -1.36152398322924
72 0.0896353779449706
73 3.20437822297864
74 8.41127687616947
75 10.2952515487529
76 11.8244355710256
77 12.8581755253979
78 13.3154924929286
79 13.1796589750808
80 12.6403026622588
81 11.9945586103305
82 11.3115457204326
83 10.5459806472087
84 9.31093809255457
85 6.95794575735244
86 5.07983156725334
87 3.66943762967108
88 2.56105892200328
89 1.71670797536597
90 1.12912191809839
91 0.734294600099951
92 0.472695799792022
93 0.301805027582984
94 0.19165230472038
95 0.121471030094607
96 0.077149899938153
97 0.0492993190129787
98 0.0318219729898613
99 0.0208460701082075
};
\addplot [semithick, color3]
table {%
0 0.0563344048990573
1 0.0501324407426503
2 0.0458061378740682
3 0.043353262862278
4 0.0425248641713836
5 0.0431509265394757
6 0.0451431840353484
7 0.0501652838080112
8 0.0570206984638232
9 0.0653369696862972
10 0.078404303399649
11 0.324377824115711
12 1.476273195239
13 2.17072992383784
14 3.19401207552411
15 3.20708521162066
16 2.97319106057079
17 2.87987779888958
18 2.64575495299413
19 2.29609026648933
20 1.99249001790323
21 1.88127167927653
22 1.93335664693047
23 2.06713740797676
24 2.18310171679387
25 2.22596304001537
26 2.18802313040823
27 2.07603138204419
28 1.91477721394073
29 1.73331169631907
30 1.57421906780803
31 1.46335707885392
32 1.3830149319744
33 1.30521223443033
34 1.20661416108972
35 1.07617257678894
36 0.910313971072471
37 0.730546630718721
38 0.587480269104806
39 0.510851761181575
40 0.494249498217594
41 0.503333342405258
42 0.516332215848781
43 0.520603350728054
44 0.467175549019024
45 0.377450284184486
46 0.293162298344407
47 0.209695130750754
48 0.145238404241604
49 0.110666029620351
50 0.0906229612843475
51 0.0764764208642298
52 0.0657500970348914
53 0.0578821696368174
54 0.0548756194800092
55 0.0739150705359896
56 0.359705171364618
57 3.74422777588813
58 6.09186586028128
59 1.38196793036514
60 -6.26956824835717
61 -16.2079201785683
62 -22.6312219886747
63 -22.2497125819586
64 -16.065920167202
65 -7.85748985266639
66 -1.72394672836531
67 1.64117450541609
68 2.20298144482035
69 1.27299441775007
70 0.0791070940370456
71 -0.0964645802640028
72 1.26814242122375
73 3.26509064984181
74 5.13039788159781
75 6.52086018524328
76 7.77397305127113
77 8.51915450589669
78 8.78765817249148
79 8.62728807501348
80 8.19904207307766
81 7.7201994516383
82 7.24027624079533
83 6.73068998653579
84 5.90536759243839
85 4.23460103935226
86 3.13482705844825
87 2.3528759481051
88 1.75613950954018
89 1.29272625688274
90 0.941264630721221
91 0.682486443363229
92 0.495401433261473
93 0.362040374046063
94 0.267797224601385
95 0.201337376721616
96 0.154281416478185
97 0.120633889513094
98 0.0962896408277009
99 0.0785583254246043
};
\addplot [semithick, color4]
table {%
0 0.00102356167494049
1 0.000965234671827578
2 0.00102027549118909
3 0.00101506158936773
4 0.00100372354318755
5 0.00101686446171064
6 0.00107083562697817
7 0.00117334100588425
8 0.00132505896530138
9 0.00422382228048507
10 0.0109613431473234
11 0.0375538748146768
12 0.0890495522498642
13 0.258355028599093
14 1.23641350576343
15 0.547832038412156
16 0.302249138053925
17 0.586915157233092
18 0.984968090865254
19 1.33897185832649
20 1.51683303554263
21 1.44866413672841
22 1.1737953961475
23 0.816769120982387
24 0.50188832540666
25 0.285022203066119
26 0.170057424401987
27 0.137914858125494
28 0.155185384472883
29 0.182596220807023
30 0.189041444769827
31 0.170884281136255
32 0.146126777922447
33 0.134947379255691
34 0.146637030593889
35 0.178495745616036
36 0.216891053748169
37 0.237045452183002
38 0.223734054431349
39 0.186007819182895
40 0.146859944569018
41 0.121318909487802
42 0.11206873513561
43 0.12375007373438
44 0.149576108635261
45 0.171139464020701
46 0.179221854004422
47 0.170410549420964
48 0.147594102798548
49 0.1207263522982
50 0.0966754151250293
51 0.0770891499473486
52 0.0616395513999829
53 0.0499893023853255
54 0.0419211428476856
55 0.0387620519168375
56 0.0280802867898961
57 4.23225253580906
58 7.05598355911044
59 7.58731495688748
60 18.8927074142857
61 29.2138863429332
62 32.7731467753208
63 28.216519841151
64 19.3260767437774
65 11.8332541398867
66 7.87804371127005
67 6.33661364979353
68 6.30279024370552
69 6.99212853750124
70 7.21303117685943
71 6.02801892484366
72 3.43361211140591
73 2.15497094059529
74 6.49868510408031
75 13.0492604595066
76 18.2277654309375
77 21.5308294480434
78 23.1502189948494
79 23.2923038665499
80 22.4537571941169
81 21.2395037602186
82 19.8574706576167
83 18.3387880281867
84 16.0960142662059
85 11.9665225298035
86 8.66917181572144
87 6.24305698059854
88 4.42723130847089
89 3.04265211156226
90 2.02223328393935
91 1.30272641910998
92 0.81239656443364
93 0.489574582447549
94 0.284314737097913
95 0.158323991731467
96 0.0836904936737829
97 0.0410415646737403
98 0.0175918671839715
99 0.00528520628301292
};
\addplot [semithick, color5]
table {%
0 0.00877999888496355
1 0.00667354464919367
2 0.00517815670837909
3 0.00421871702702718
4 0.00364006092520064
5 0.00334451407105536
6 0.00327643856911446
7 0.00341398304200303
8 0.00377453089316389
9 0.0033661419693977
10 0.00307985674886001
11 0.0175753275922012
12 0.336508605508394
13 0.989211224471705
14 2.05849480359228
15 2.6987651764655
16 2.97199448490688
17 3.1654286994762
18 3.23326653531238
19 3.18605852319526
20 3.08817243835263
21 3.00021340493145
22 2.95599903719689
23 2.94914431315389
24 2.9365655871952
25 2.87645732001987
26 2.74860184907393
27 2.54961799238556
28 2.29949936346242
29 2.02909586114303
30 1.77663687417745
31 1.56762046501665
32 1.39816273715325
33 1.24990769508149
34 1.10386118917486
35 0.949158772410999
36 0.783960762099088
37 0.620924062593238
38 0.482031370327137
39 0.379986302441512
40 0.313841320843018
41 0.273515522501943
42 0.249256039451107
43 0.230964379237153
44 0.202549471073397
45 0.16514435192416
46 0.128512063042306
47 0.0950742445500938
48 0.0676023997148045
49 0.0475413540589497
50 0.0333078047469054
51 0.0233070881979649
52 0.0163745431879431
53 0.0116373375643161
54 0.00857193544248872
55 0.00746710009415172
56 0.0521670389586846
57 2.60097406325932
58 5.06673669473394
59 3.48963715294808
60 3.17916006844762
61 4.0466716462175
62 4.68220045071982
63 4.16042416963924
64 2.85478657344348
65 1.75232618612588
66 1.5898474444363
67 2.48709866065053
68 3.74029499797078
69 4.49652387844443
70 4.70222295460833
71 4.75025447910375
72 5.16928037420407
73 6.22454287114345
74 7.55908011073731
75 8.79118426938995
76 10.4247548338864
77 11.9124524761094
78 12.910583975687
79 13.243940455048
80 13.0696007137899
81 12.6774833735134
82 12.0977893915447
83 11.3085597625607
84 9.94506645349526
85 7.39469346412886
86 5.37790890202448
87 3.86312523947779
88 2.6606088293756
89 1.73000588021288
90 1.08497282082169
91 0.665971011965885
92 0.404016248561644
93 0.245062260033064
94 0.150184870395107
95 0.093690866988648
96 0.0597378123795789
97 0.0389778864606385
98 0.0260228543055721
99 0.0177822294693747
};
\addplot [semithick, black]
table {%
0 -0.00122827400992859
1 -0.00115828160619309
2 -0.00122433058942691
3 -0.00121807390724127
4 -0.00120446825182506
5 -0.00122023735405277
6 -0.0012850027523738
7 -0.0014080092070611
8 -0.00159007075836166
9 -0.00506858673658209
10 -0.013153611776788
11 -0.0450646497776121
12 -0.106859462699837
13 0.0465614495892926
14 0.309103376440858
15 0.136958009603039
16 -0.270149822356201
17 -0.704298188679711
18 -1.18196170903831
19 -1.60676622999179
20 -1.82019964265116
21 -1.73839696407409
22 -1.408554475377
23 -0.980122945178864
24 -0.602265990487992
25 -0.342026643679343
26 -0.204068909282384
27 -0.165497829750592
28 -0.186222461367459
29 -0.219115464968428
30 -0.226849733723792
31 -0.205061137363506
32 -0.175352133506937
33 -0.16193685510683
34 -0.175964436712667
35 -0.214194894739243
36 -0.260269264497803
37 -0.284454542619603
38 -0.268480865317619
39 -0.223209383019474
40 -0.176231933482821
41 -0.145582691385362
42 -0.134482482162731
43 -0.148500088481256
44 -0.179491330362314
45 -0.205367356824842
46 -0.215066224805306
47 -0.204492659305157
48 -0.177112923358258
49 -0.14487162275784
50 -0.116010498150035
51 -0.0925069799368183
52 -0.0739674616799795
53 -0.0599871628623906
54 -0.0503053714172228
55 -0.046514462300205
56 -0.0336963441478754
57 1.04634952386591
58 -0.205481459850282
59 -9.10477794826498
60 -22.6712488971428
61 -35.0566636115199
62 -39.327776130385
63 -33.8598238093812
64 -23.1912920925329
65 -14.1999049678641
66 -9.45365245352406
67 -7.60393637975223
68 -7.56334829244663
69 -8.39055424500149
70 -8.65563741223131
71 -7.2336227098124
72 -4.12033453368709
73 -0.746537158816041
74 1.62467127602008
75 3.26231511487665
76 4.55694135773437
77 5.38270736201085
78 5.78755474871236
79 5.82307596663747
80 5.61343929852923
81 5.30987594005464
82 4.96436766440418
83 4.58469700704668
84 4.02400356655148
85 2.99163063245087
86 2.16729295393036
87 1.56076424514964
88 1.10680782711772
89 0.760663027890564
90 0.505558320984838
91 0.325681604777496
92 0.20309914110841
93 0.122393645611887
94 0.0710786842744782
95 0.0395809979328667
96 0.0209226234184457
97 0.0102603911684351
98 0.00439796679599288
99 0.00132130157075323
};


==> plots/all/RectusFemorisTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 -0.000852940378369353
1 -0.000623109081376945
2 -0.000592086360376895
3 -0.000406766392052254
4 -0.000162048482527511
5 9.85997215421364e-05
6 0.000366819714232829
7 0.000662462256124178
8 0.00105241838180764
9 -0.00341153295124754
10 -0.0142902288332669
11 -0.00999554433802565
12 0.648110041632489
13 1.67255381908519
14 3.45806398673764
15 3.4463006607993
16 2.71035053259827
17 2.19822316873114
18 1.45740802134323
19 0.610615860849163
20 -0.0152121512341339
21 -0.196551079602632
22 0.067117739806374
23 0.565343731944097
24 1.02195454078321
25 1.28410256240477
26 1.33019073671606
27 1.18963634210218
28 0.944070676680234
29 0.682280742398896
30 0.49926378103534
31 0.425687800588566
32 0.403474684599789
33 0.366806913566815
34 0.275960155062535
35 0.127185541140854
36 -0.056752997708048
37 -0.212942479694145
38 -0.274902672600739
39 -0.24256825582338
40 -0.166800330347167
41 -0.100431387629167
42 -0.0631784501018491
43 -0.0686587141048888
44 -0.136910615851629
45 -0.218437737972115
46 -0.268079831367657
47 -0.284024504999247
48 -0.263819339304029
49 -0.222039223071176
50 -0.179716092088062
51 -0.143890752892833
52 -0.115101062412251
53 -0.0930149984501165
54 -0.0769621008383482
55 -0.0663103222663352
56 0.0490950302584016
57 6.29270769312787
58 8.89566928943579
59 -6.64133106454663
60 -28.1349166346813
61 -49.4480462091764
62 -58.7977021224315
63 -52.3628698774327
64 -36.3729942371244
65 -21.3432579967131
66 -11.7226972814129
67 -6.0674239978756
68 -3.97125557057869
69 -5.05937415500523
70 -6.74298109698786
71 -6.28339920112962
72 -2.56832237286766
73 2.75740761557511
74 7.18521650269969
75 9.72548619568426
76 12.4016143785099
77 13.9610852641183
78 14.5096882036188
79 14.1919952440348
80 13.3929716949405
81 12.5674945629751
82 11.7537583531395
83 10.8599405339203
84 9.34995565057361
85 6.36201343160188
86 4.54887081365026
87 3.27798468335774
88 2.31394713500679
89 1.57630479863298
90 1.03940965626348
91 0.665551723063657
92 0.413229059717438
93 0.248344067819004
94 0.144107515347537
95 0.0804033602167685
96 0.0427990085038755
97 0.0213757620100295
98 0.00964126205650117
99 0.0035351880485773
};
\addplot [semithick, color1]
table {%
0 0.00693966966321178
1 0.00514666175241206
2 0.00380374686789225
3 0.00296735891912101
4 0.00246714681004837
5 0.00219693424840742
6 0.00209646976877041
7 0.00214110676309475
8 0.00234596420263254
9 -0.000445513950293629
10 -0.00728092847195284
11 -0.0165212649682076
12 0.232845635797512
13 0.912380777473057
14 2.08223601778452
15 2.58147009963629
16 2.63416214485481
17 2.60997352597421
18 2.42575349295785
19 2.13786134741013
20 1.90920875084651
21 1.86188170178317
22 2.00413419984383
23 2.23471490161445
24 2.42198106875898
25 2.49291662168676
26 2.43331180612149
27 2.25673126254902
28 2.00385474653498
29 1.72762841080247
30 1.48358817500959
31 1.29813933486726
32 1.15569315511862
33 1.02563001814003
34 0.883745188784995
35 0.720716658566066
36 0.542808519705163
37 0.378929208187281
38 0.261712695886796
39 0.19727008249615
40 0.167179666289071
41 0.150259693589146
42 0.135372465271164
43 0.109469796720206
44 0.062287755528833
45 0.00881184855498494
46 -0.0341341787027065
47 -0.0602018775417523
48 -0.0680421684737244
49 -0.0645074004083438
50 -0.057388931501217
51 -0.0498925334732355
52 -0.0429559576393238
53 -0.0372436463754391
54 -0.0331563483365072
55 -0.0315272453267285
56 0.0166390646731379
57 2.92093792976461
58 4.44050917879698
59 -3.27972920501679
60 -15.758376806319
61 -28.0994514828636
62 -33.372403568268
63 -29.4461419379541
64 -20.1450081114652
65 -11.7638239363808
66 -6.69647155643964
67 -3.72145716697275
68 -2.23365901303564
69 -2.00175349604639
70 -1.99689811743752
71 -1.01961125772524
72 1.38778657603709
73 4.34716788301013
74 6.8289337724602
75 8.62340908090997
76 10.263833872142
77 11.4113096231138
78 11.9941753740384
79 11.9991565715952
80 11.6100940457042
81 11.1091346382092
82 10.5544955711872
83 9.89969989334904
84 8.77429438764177
85 6.56645710952714
86 4.80455016154379
87 3.47649016494604
88 2.42291624710675
89 1.61525257050853
90 1.0543027644097
91 0.67924681990011
92 0.432319949989198
93 0.272283194993448
94 0.170123813790205
95 0.105800618222446
96 0.0657513626960999
97 0.0410011701879887
98 0.0257632736103969
99 0.0163955625843898
};
\addplot [semithick, color2]
table {%
0 0.00645739889997518
1 0.00395769886763014
2 0.00199637853377075
3 0.0010596224116399
4 0.000583109114669616
5 0.000318677647571864
6 0.00015503471331291
7 4.74593311318289e-05
8 -9.23535405928168e-07
9 -0.00364693525831591
10 -0.0106902547761002
11 -0.0352946449733959
12 0.0686815368498918
13 1.73994336109481
14 3.79699618026493
15 4.95847469206955
16 3.01223672875065
17 1.40931604211143
18 0.333558476762597
19 -0.374155636075737
20 -0.704479947671323
21 -0.650421900355
22 -0.237971595624948
23 0.490129365184271
24 1.45868344631691
25 2.45356989189914
26 3.0685359576572
27 3.00733387466792
28 2.45211443416127
29 1.82508828985931
30 1.40674444557689
31 1.21559373099311
32 1.12185955005986
33 0.977115042650197
34 0.718551731225975
35 0.403272100941011
36 0.131773752787819
37 -0.032034074417987
38 -0.0911270190106307
39 -0.0863951213232937
40 -0.0614536343907824
41 -0.0436104071512575
42 -0.0420646774075604
43 -0.0665740144864754
44 -0.108783965879943
45 -0.143401230286733
46 -0.160015993403864
47 -0.157412841163095
48 -0.139056833368206
49 -0.115168985455879
50 -0.0931183370026365
51 -0.0748833185477084
52 -0.0603361258638083
53 -0.049289953264965
54 -0.0416176617088632
55 -0.0386009902279673
56 0.00831123935841577
57 4.35112430833289
58 4.75184997455644
59 -7.13000516710805
60 -19.0327486303044
61 -29.8996637788817
62 -33.7466840612773
63 -29.1143357760474
64 -19.9137042797618
65 -12.0973339548997
66 -7.87805830643264
67 -6.08477828666766
68 -5.83836960002696
69 -6.42076936587415
70 -6.61521713376542
71 -5.37851762806008
72 -2.15330469708429
73 4.28111145047177
74 12.3625573941528
75 13.6683669915352
76 14.9370307343403
77 15.7502277841813
78 15.9806427168363
79 15.5886913025554
80 14.7723024181748
81 13.8690794384252
82 12.9714129367641
83 12.026917362713
84 10.5909988383571
85 7.89932734755634
86 5.75186630174442
87 4.15147616584002
88 2.91538286862758
89 1.98211481372834
90 1.32713753589223
91 0.880902976828085
92 0.580575560231798
93 0.380805942355076
94 0.249302176341568
95 0.163445375206269
96 0.107684954193787
97 0.0715301373727974
98 0.0480542319215689
99 0.0327706044519556
};
\addplot [semithick, color3]
table {%
0 -0.000899259519999515
1 -0.000906755094843535
2 -0.00101889334270266
3 -0.00103681201973511
4 -0.00103114100842329
5 -0.00104108450492
6 -0.00108621642667862
7 -0.00115478206627232
8 -0.0012502208863055
9 -0.00456875662934998
10 -0.0123116331990846
11 -0.0260611122658209
12 0.547501842398648
13 1.54485853651186
14 3.45034982939136
15 3.71769311830673
16 3.25436605588434
17 3.07184030215001
18 2.6184349952499
19 1.95822736633099
20 1.39782443864887
21 1.17382578931246
22 1.22995310475994
23 1.43417628487892
24 1.61960887553063
25 1.68540046944928
26 1.61369300392356
27 1.42013909208589
28 1.15872278797388
29 0.890005643312577
30 0.680987714347126
31 0.556370724762229
32 0.480046910038583
33 0.408019993546729
34 0.312058258067761
35 0.187006452453229
36 0.0462549216962423
37 -0.0709956737513925
38 -0.126300604770907
39 -0.122949858434389
40 -0.0938095834463629
41 -0.0683211587648386
42 -0.0568836494875552
43 -0.0682450880392772
44 -0.108449263418385
45 -0.151875203133656
46 -0.177145553895438
47 -0.180709636913706
48 -0.163632039681115
49 -0.136855318699354
50 -0.111007925645655
51 -0.0893027458220825
52 -0.0718645401198729
53 -0.0585472008217614
54 -0.0491969038604442
55 -0.0450010053706199
56 0.0161629927818948
57 6.71604088257948
58 11.5613893646428
59 1.3829162595454
60 -12.1538229105004
61 -26.7281879201016
62 -33.9820771116862
63 -31.0720524728549
64 -21.7898847150894
65 -12.4728998073656
66 -5.44012149215624
67 0.423331303648139
68 3.49348584802996
69 2.99708943539477
70 0.964260066903312
71 0.15150511439492
72 1.8485013394379
73 4.758501883558
74 7.03350515378636
75 7.79598050711078
76 8.93577759485195
77 9.48798328673788
78 9.46983994100133
79 8.95358256616681
80 8.18821022485726
81 7.48015995258428
82 6.848295460315
83 6.21626106933745
84 5.24840747445293
85 3.44605470763965
86 2.41736174496083
87 1.71626824940089
88 1.20385655775951
89 0.821257926473502
90 0.543401576027257
91 0.349347073748436
92 0.217924510414513
93 0.131703296074285
94 0.0769436902386223
95 0.043291500615067
96 0.0232848836972173
97 0.0117781035389357
98 0.00538669315846845
99 0.0019799640840008
};
\addplot [semithick, color4]
table {%
0 -0.000536856293328775
1 -0.000506263883062931
2 -0.000535132695746758
3 -0.000532398013436813
4 -0.000526451228211355
5 -0.000533343616801084
6 -0.00056165139779908
7 -0.000615415288254419
8 -0.00069499109039533
9 -0.00221538733688183
10 -0.0057492051490878
11 -0.0196969411093986
12 -0.0467063331051631
13 0.233025049147525
14 1.20435483555729
15 0.533627432456344
16 -0.0628799528621237
17 -0.307835964871343
18 -0.51661402654587
19 -0.702288378249896
20 -0.795576252019594
21 -0.759821784815812
22 -0.61565361514612
23 -0.428393963481976
24 -0.263239541533705
25 -0.1494936428363
26 -0.0891948191815574
27 -0.0723360998569247
28 -0.0813944604674228
29 -0.0957713957822821
30 -0.0991519043838233
31 -0.0896285040804172
32 -0.0766432373076916
33 -0.0707796624232292
34 -0.076910863933969
35 -0.093620703776304
36 -0.113758975176737
37 -0.124329921611034
38 -0.117348116966587
39 -0.0975607731136515
40 -0.0770277819207877
41 -0.0636315540654617
42 -0.0587798539315627
43 -0.0649066954251335
44 -0.0784524051832416
45 -0.0897623470532626
46 -0.0940015463454303
47 -0.0893800326312315
48 -0.0774128466173976
49 -0.0633207588645637
50 -0.0507060847340356
51 -0.0404331231911413
52 -0.0323298360003244
53 -0.0262193009387905
54 -0.0219875654904949
55 -0.0203306278687123
56 -0.0147280608982445
57 4.11040950020208
58 4.83758331120021
59 -3.97953331371987
60 -9.90919171916843
61 -15.3226318645695
62 -17.1894576841612
63 -14.7995148933638
64 -10.1364931681865
65 -6.20652092696448
66 -4.13202003265744
67 -3.32354268391542
68 -3.30580236707402
69 -3.6673590864366
70 -3.78322213119086
71 -3.16168529492415
72 -1.80092349683309
73 0.770763340812006
74 6.33018225163319
75 12.7109093046904
76 17.7551420587231
77 20.9725617185808
78 22.5499625009691
79 22.6883632879989
80 21.8715590917672
81 20.6887897448694
82 19.3425910481874
83 17.86328597759
84 15.678664560312
85 11.6562454279204
86 8.4443909322184
87 6.08118224865312
88 4.31243868627534
89 2.96375991235713
90 1.96979928056791
91 1.26894833722686
92 0.791332128131078
93 0.476880520140049
94 0.276942808249772
95 0.154218846799792
96 0.0815205028708918
97 0.0399774077549698
98 0.0171357318653809
99 0.00514816743281537
};
\addplot [semithick, color5]
table {%
0 0.00785611450830014
1 0.00582213864922275
2 0.0042999090146206
3 0.00335458162492188
4 0.00279037899557883
5 0.00248639708572003
6 0.00237443468047205
7 0.00242665778672111
8 0.00265993647180602
9 -0.000313054945930733
10 -0.00747758855240103
11 -0.0164586603784938
12 0.260507046094996
13 1.00605028028561
14 2.23068014731745
15 2.7516016029795
16 2.75488266237463
17 2.65726719293747
18 2.4006351928993
19 2.06023824106117
20 1.81291935917757
21 1.78223117786752
22 1.96816637066617
23 2.25589108537517
24 2.49890764738494
25 2.61304954626012
26 2.57804526887823
27 2.40708819066338
28 2.14660646789952
29 1.85800128598741
30 1.60365936607005
31 1.4117387931275
32 1.26412478239321
33 1.12664121453072
34 0.973070705966857
35 0.794549693766841
36 0.599708331780899
37 0.421056534457638
38 0.293605091057861
39 0.223285430215577
40 0.190100938295648
41 0.171273096477164
42 0.154781823085904
43 0.126443581995562
44 0.0751556834240565
45 0.0172249393362541
46 -0.0293190265474616
47 -0.0580151353240282
48 -0.0674648430298077
49 -0.0647721363215725
50 -0.0581172472147151
51 -0.0508935300276078
52 -0.0441162064258323
53 -0.0385193464999772
54 -0.0345472449683309
55 -0.0329791735352033
56 0.0236772810539149
57 3.22038589064262
58 4.72746737017204
59 -4.04859114426087
60 -18.0900709320346
61 -32.3357866515452
62 -38.7765204176753
63 -34.4756161781312
64 -23.6228555562802
65 -13.6239163721491
66 -7.53454787040018
67 -4.08219423344829
68 -2.5145145348067
69 -2.41988545596498
70 -2.45244408204676
71 -1.18099456684258
72 1.8656635609026
73 5.5768970359124
74 8.61483044453362
75 10.8973091877979
76 13.1908952361934
77 14.9364479900735
78 15.9260073900868
79 16.0872107368233
80 15.6658452320316
81 15.0346711382671
82 14.2518468382425
83 13.2773235090283
84 11.6615008641218
85 8.66420847057912
86 6.29625452387787
87 4.5218355857698
88 3.11940831002098
89 2.04318842280486
90 1.30125720548386
91 0.815506255930962
92 0.504888246696037
93 0.310178265092718
94 0.190001084001522
95 0.116614505369636
96 0.072049899938552
97 0.0449963029172194
98 0.0285091906320138
99 0.018402126248789
};
\addplot [semithick, black]
table {%
0 -0.00122827400992859
1 -0.00115828160619309
2 -0.00122433058942691
3 -0.00121807390724127
4 -0.00120446825182506
5 -0.00122023735405277
6 -0.0012850027523738
7 -0.0014080092070611
8 -0.00159007075836166
9 -0.00506858673658209
10 -0.013153611776788
11 -0.0450646497776121
12 -0.106859462699837
13 0.0465614495892926
14 0.309103376440858
15 0.136958009603039
16 -0.270149822356201
17 -0.704298188679711
18 -1.18196170903831
19 -1.60676622999179
20 -1.82019964265116
21 -1.73839696407409
22 -1.408554475377
23 -0.980122945178864
24 -0.602265990487992
25 -0.342026643679343
26 -0.204068909282384
27 -0.165497829750592
28 -0.186222461367459
29 -0.219115464968428
30 -0.226849733723792
31 -0.205061137363506
32 -0.175352133506937
33 -0.16193685510683
34 -0.175964436712667
35 -0.214194894739243
36 -0.260269264497803
37 -0.284454542619603
38 -0.268480865317619
39 -0.223209383019474
40 -0.176231933482821
41 -0.145582691385362
42 -0.134482482162731
43 -0.148500088481256
44 -0.179491330362314
45 -0.205367356824842
46 -0.215066224805306
47 -0.204492659305157
48 -0.177112923358258
49 -0.14487162275784
50 -0.116010498150035
51 -0.0925069799368183
52 -0.0739674616799795
53 -0.0599871628623906
54 -0.0503053714172228
55 -0.046514462300205
56 -0.0336963441478754
57 1.04634952386591
58 -0.205481459850282
59 -9.10477794826498
60 -22.6712488971428
61 -35.0566636115199
62 -39.327776130385
63 -33.8598238093812
64 -23.1912920925329
65 -14.1999049678641
66 -9.45365245352406
67 -7.60393637975223
68 -7.56334829244663
69 -8.39055424500149
70 -8.65563741223131
71 -7.2336227098124
72 -4.12033453368709
73 -0.746537158816041
74 1.62467127602008
75 3.26231511487665
76 4.55694135773437
77 5.38270736201085
78 5.78755474871236
79 5.82307596663747
80 5.61343929852923
81 5.30987594005464
82 4.96436766440418
83 4.58469700704668
84 4.02400356655148
85 2.99163063245087
86 2.16729295393036
87 1.56076424514964
88 1.10680782711772
89 0.760663027890564
90 0.505558320984838
91 0.325681604777496
92 0.20309914110841
93 0.122393645611887
94 0.0710786842744782
95 0.0395809979328667
96 0.0209226234184457
97 0.0102603911684351
98 0.00439796679599288
99 0.00132130157075323
};


==> plots/all/SoleusFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 0.110956780403308
1 0.0674842119863441
2 0.0354793748490442
3 0.020661466558972
4 0.0209488470975886
5 0.0559019043303899
6 0.304759781875483
7 0.737759172743813
8 0.819922335487857
9 0.795112680861952
10 1.12782719376516
11 -0.0714011886823307
12 0.178834894360616
13 -1.55376982699406
14 -5.22527767682475
15 -9.80923000184781
16 -13.9031229181919
17 -15.4120403168524
18 -13.674686521727
19 -9.28232386695612
20 -4.00993470718438
21 0.594718013402374
22 3.30780770399415
23 3.61989068682522
24 2.68090687887742
25 1.93013239968809
26 1.86799384572226
27 3.03394556928349
28 4.91129623842242
29 6.69063739171561
30 7.2288694632805
31 6.45664097247844
32 5.1997276780071
33 4.01812281510584
34 3.27386259029631
35 2.97923617361353
36 2.69636149266947
37 1.87547639881536
38 0.17118751191093
39 -2.32989789123221
40 -5.3590622845305
41 -8.71071060740843
42 -12.4040285842633
43 -16.7394508857207
44 -21.9186498933676
45 -27.5736218695858
46 -32.6457807617975
47 -35.5121462574406
48 -34.4791157129355
49 -28.1756144793213
50 -15.964705781206
51 2.15202432393665
52 25.2970682522354
53 54.6055817809659
54 91.7075741856586
55 131.637083412661
56 167.37909084388
57 194.770934435376
58 210.757939620808
59 208.518824355868
60 185.128374743117
61 151.252746657401
62 110.570603371833
63 72.536045257569
64 49.8542439590192
65 33.2922331605988
66 21.1234549271671
67 12.0783707055405
68 5.29751420474043
69 0.302477449857096
70 -2.81281283267363
71 -3.80719399189721
72 -3.4659045108651
73 -2.72890119796686
74 -2.02717452166314
75 -1.47678737692098
76 -1.05451606643657
77 -0.740124456972026
78 -0.514558771208535
79 -0.353688978577253
80 -0.239648847377606
81 -0.159910719161588
82 -0.103916019922914
83 -0.0648591672203302
84 -0.0387950656659869
85 -0.0220504044058504
86 -0.0116583688767618
87 -0.00565022949820947
88 -0.00227808939182389
89 0.00276526912591953
90 0.0271055768949933
91 0.0393039493810185
92 0.0710842434645972
93 0.144373630297885
94 0.266354346349725
95 0.307328611344092
96 0.645849159983786
97 0.741331275341931
98 0.497665299465117
99 -0.039410437316887
};
\addplot [semithick, color1]
table {%
0 0.127377064397142
1 0.0802534596956334
2 0.043737778049678
3 0.024423741229245
4 0.0167910182543234
5 0.0269592740306842
6 0.113262210799026
7 0.323057173906463
8 0.455272853478321
9 0.470595178315075
10 0.066256550753073
11 -1.96855611625203
12 -4.81512062908778
13 -8.36071473743211
14 -12.2198033607164
15 -16.0782431344775
16 -18.8424694419243
17 -19.5752123069326
18 -18.0743350115404
19 -15.2529050121422
20 -12.226304534302
21 -9.70200851217156
22 -8.19676641036009
23 -7.81523168074721
24 -7.93806018746442
25 -8.0183948529082
26 -7.66959492016732
27 -6.75393733054751
28 -5.52595755240499
29 -4.57954481687714
30 -4.45583706064295
31 -5.12338977284616
32 -6.19973026947099
33 -7.31462385724884
34 -8.21058039560761
35 -8.89639728000635
36 -9.65095865010167
37 -10.8303778321234
38 -12.6574642430615
39 -15.0934126503627
40 -17.9639916885164
41 -21.1429987911093
42 -24.6725567893696
43 -28.786405549156
44 -33.6271628446678
45 -38.8745564873424
46 -43.6038406579671
47 -46.441985166434
48 -45.9484130358624
49 -40.8900542762668
50 -30.5608721637754
51 -15.1754136675911
52 4.07773334904166
53 28.5310618558198
54 59.7087961631151
55 94.1795289998768
56 127.216494993021
57 154.778237183568
58 173.35848954188
59 177.086962229993
60 162.9652401592
61 137.694521871506
62 105.69206987559
63 73.875518056718
64 50.5123762986183
65 33.4429014886889
66 21.0173240030508
67 11.9874022704027
68 5.42706450063104
69 0.750871503863389
70 -2.09885427146879
71 -3.04995977442283
72 -2.82001303257533
73 -2.23010897576939
74 -1.65806653257537
75 -1.20763995056755
76 -0.86122009778057
77 -0.603111712179832
78 -0.41814513241693
79 -0.28642279424065
80 -0.193210934532269
81 -0.128198210308494
82 -0.0826373636525573
83 -0.0509336492068216
84 -0.0298961719239901
85 -0.0165137157630506
86 -0.00833570892828448
87 -0.00373660262008362
88 -0.00142523262203174
89 -0.000274197123981012
90 0.000926088968241898
91 0.00446228980505723
92 0.0150132474532132
93 0.0432686556535669
94 0.09593892011802
95 0.140604300001324
96 0.231570358882961
97 0.225411242115959
98 0.0965244417284369
99 0.0170967493911549
};
\addplot [semithick, color2]
table {%
0 0.278136008734766
1 0.187225446922156
2 0.12013912410662
3 0.0802825228622717
4 0.0603272142528199
5 0.0700166364095522
6 0.213612975511248
7 0.547702080080902
8 0.751303378408097
9 0.798892320025004
10 0.299293025955475
11 -0.697091696082104
12 -1.72581463331866
13 -3.00635616780171
14 -4.53041465914261
15 -6.20121648225143
16 -7.4776567699321
17 -7.79930097970614
18 -6.97309457469461
19 -5.36896911965004
20 -3.53342030053667
21 -1.87821782951009
22 -0.775559695214933
23 -0.363148163571962
24 -0.34483770711673
25 -0.384461103932733
26 -0.239166307639948
27 0.229931052791111
28 0.922263309000323
29 1.53738768270291
30 1.72437952287622
31 1.44916746730183
32 0.935536305835761
33 0.405408531993735
34 0.0142108428395391
35 -0.226537280155338
36 -0.46321450637434
37 -0.897828270213445
38 -1.66867995832832
39 -2.76672420641021
40 -4.1023919691284
41 -5.60491428720659
42 -7.29023885924722
43 -9.28092955807904
44 -11.6570293174025
45 -14.2551308209601
46 -16.5950089697309
47 -17.9557506232534
48 -17.5768442983541
49 -14.8055958016947
50 -9.25605971493158
51 -0.888747779095786
52 25.0615792628556
53 62.9852306302398
54 98.5985017175489
55 138.448865113354
56 176.745441699522
57 208.707301951237
58 230.217617736947
59 233.863516432749
60 215.366166529608
61 182.69184395403
62 140.95793064767
63 99.0201789101198
64 69.3126256428708
65 48.544956986318
66 31.025693463489
67 18.5205173339453
68 9.68094886038752
69 3.33056907405787
70 -0.570872745398135
71 -1.21916418225513
72 -1.20418136932852
73 -0.971629909008445
74 -0.727430215094684
75 -0.531434930891052
76 -0.378722815956253
77 -0.264165591035226
78 -0.182056228348239
79 -0.123627843391962
80 -0.0823537746622947
81 -0.0536872153583025
82 -0.0336642359553092
83 -0.019794760309644
84 -0.0107223610176791
85 -0.00509737548637808
86 -0.00179878964311994
87 -8.80428565424093e-05
88 0.000664230401856331
89 0.00144312835315106
90 0.00628569778546938
91 0.0216174162513833
92 0.0500523221392155
93 0.103962319318782
94 0.19947283513279
95 0.274648324460635
96 0.472087658284316
97 0.576695153360402
98 0.489093696324955
99 0.120872713782842
};
\addplot [semithick, color3]
table {%
0 0.471568034759128
1 0.369075705643232
2 0.293634332756389
3 0.244391589403821
4 0.228114882312837
5 0.290645333840369
6 0.834216081072701
7 1.42702816899155
8 1.43912387390216
9 1.3897134942299
10 2.3117930931151
11 3.58366303441142
12 6.4995557760209
13 6.4823283229076
14 4.27859605237756
15 1.12495182278461
16 -2.24624802535499
17 -3.95593520322919
18 -3.34027371196044
19 -0.74180752961194
20 2.15447263945554
21 4.2760699655926
22 5.34075955458913
23 5.22618066414385
24 4.53758412940177
25 4.0522716504489
26 4.00013480106195
27 4.63789110776887
28 5.6526824240057
29 6.61831054417649
30 6.94581540412329
31 6.61358352569136
32 6.06861767190731
33 5.58487776918756
34 5.34752753403932
35 5.36726632403209
36 5.40452404306785
37 5.16605770682307
38 4.46419842919763
39 3.34659130390463
40 1.95158490780249
41 0.393370082897497
42 -1.33059075052
43 -3.39116699926798
44 -5.92074864137655
45 -8.75346185817931
46 -11.377950380931
47 -12.9456400274412
48 -12.5719378203453
49 -9.56128432479743
50 -3.53802171867033
51 5.15671701319525
52 15.8096046163025
53 33.6173237994492
54 60.4751774045724
55 89.0739095190841
56 114.753248622337
57 133.925714128551
58 144.170727111227
59 141.39920636228
60 123.946147995131
61 99.7865935263604
62 73.1126514929605
63 49.5837029140239
64 35.3068990936127
65 25.2041555827119
66 17.6753876874687
67 11.6611683751418
68 6.66565436105592
69 2.70232099509236
70 0.183373939472553
71 -0.854574836003224
72 -0.952971514739561
73 -0.724888719454065
74 -0.46701549766399
75 -0.267979765786456
76 -0.121071022874961
77 -0.0197824479584024
78 0.0430670132614906
79 0.0794046641780053
80 0.0978851630569111
81 0.104254267867772
82 0.10348784086771
83 0.0984741894014479
84 0.0905473163409767
85 0.0811840462018724
86 0.0715803350616178
87 0.0624032222004974
88 0.0558402170631608
89 0.0750048880681256
90 0.236886956566058
91 0.282878636080424
92 0.378430499732308
93 0.548064014158956
94 0.773334050777019
95 0.794399543663318
96 1.36537573393745
97 1.54775017282422
98 1.3005720774191
99 0.565794899850534
};
\addplot [semithick, color4]
table {%
0 0.322791864733442
1 0.196320729373842
2 0.0955588105046611
3 0.0446684861514533
4 0.0272810008723249
5 0.0615622203028946
6 0.305371982282534
7 0.892123544917826
8 1.25984687023099
9 1.30132237713143
10 0.208253097686255
11 1.8481615079454
12 4.53067509210192
13 7.88309679697022
14 11.4587243237969
15 14.9395865417046
16 17.3814782826609
17 18.0503442535508
18 16.8415036053185
19 14.5960769626694
20 12.2737009102568
21 10.4373393507456
22 9.4639361063311
23 9.35867482118897
24 9.57004766557348
25 9.67850098724806
26 9.39279656464646
27 8.6544846835157
28 7.70163024773279
29 7.04234748227241
30 7.08981165750533
31 7.77657398249064
32 8.78867564036083
33 9.83422936527185
34 10.7199576301613
35 11.4747933354873
36 12.3371985437933
37 13.5927520810305
38 15.4053146203413
39 17.728931079385
40 20.4153596992317
41 23.3652684389799
42 26.6226891217368
43 30.3839342076752
44 34.7614858267001
45 39.4812203769869
46 43.7631366571646
47 46.4619775119449
48 46.3828599602637
49 42.5046939328738
50 34.2630887530665
51 21.8869217978357
52 11.9631493769467
53 51.8747909468724
54 147.42054633789
55 247.060227476739
56 335.956893238074
57 402.415337764826
58 438.125599417424
59 432.49012772463
60 383.60817575167
61 312.806570587017
62 234.420829890602
63 162.893517736578
64 113.299950582825
65 78.5667504526065
66 52.8205194876287
67 32.1770506770354
68 14.9028222951976
69 3.57531244498677
70 2.02600268525962
71 2.74221424381791
72 2.49640962478829
73 1.96558735722443
74 1.46016568894889
75 1.06374076053165
76 0.759592286085206
77 0.533150319750898
78 0.370693519928212
79 0.254842889709287
80 0.172728364330695
81 0.115319982044219
82 0.0750050257799097
83 0.046882201745774
84 0.0281181460751789
85 0.0160767033644435
86 0.00862267664967051
87 0.00433307198450929
88 0.00209274130147357
89 0.001104670555141
90 0.00139819804524141
91 0.00224769587229545
92 0.0265531838950624
93 0.103430339288898
94 0.248328328649409
95 0.373706954254015
96 0.605143629182247
97 0.518247590466356
98 0.0588532571269383
99 0.0337576097419223
};
\addplot [semithick, color5]
table {%
0 0.222094666423344
1 0.150451462964357
2 0.0987375096843169
3 0.0679113929278975
4 0.0517540736184267
5 0.0571691454806312
6 0.173677902270205
7 0.469678104997654
8 0.663258947140197
9 0.693040394998869
10 0.658151881890552
11 0.686319471814839
12 1.63344255641314
13 2.82672117589573
14 3.75880830126681
15 4.2945235130818
16 4.48348472803069
17 4.57873229289601
18 4.83722351572402
19 5.59550307518631
20 6.98632874692758
21 8.78211065913416
22 10.4852535605856
23 11.557868473676
24 11.9915636544666
25 12.1304267591479
26 12.2479144545235
27 12.6570893385811
28 13.4062131307278
29 14.3399310296197
30 15.0558240755141
31 15.3685901316912
32 15.4576449912556
33 15.5447365452005
34 15.8133603986368
35 16.345336734799
36 17.0611174821908
37 17.7862777171773
38 18.3597794334461
39 18.754498288432
40 19.0316936229763
41 19.264787478974
42 19.4849029035882
43 19.6491937206042
44 19.721035932283
45 19.7660834488192
46 19.9365860815027
47 20.4535627512174
48 21.5864189950756
49 23.7205456845124
50 27.5155080384367
51 33.9482526171256
52 44.2056640551019
53 60.5538558566599
54 87.1705278753689
55 125.135387252804
56 169.738945501681
57 213.52572344426
58 247.45525665483
59 259.19978232198
60 243.010590292134
61 208.797063839955
62 163.450669804703
63 117.345375994166
64 82.9495336197372
65 56.9287542473021
66 36.629056969445
67 20.7148411813282
68 9.57877555673151
69 3.62643763405297
70 1.34550562304503
71 0.700070732486365
72 0.480546920586531
73 0.346804440261708
74 0.24909543716923
75 0.178060132169134
76 0.126559474284358
77 0.0896351618317468
78 0.0635211633229613
79 0.0451266810200101
80 0.032232398867255
81 0.0232462933671241
82 0.0170525331644859
83 0.0128674553784838
84 0.0100382926883482
85 0.00808109412561317
86 0.00666756800258369
87 0.00553291417970085
88 0.00459472183699072
89 0.00492428713148725
90 0.01297989772995
91 0.0232965193260032
92 0.0421244709746246
93 0.0832183444791638
94 0.158258433827636
95 0.219204354435965
96 0.376700668489067
97 0.468248938738131
98 0.442320556812438
99 0.289603590950121
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};


==> plots/all/SoleusTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 0.162875911549735
1 0.0993313707303738
2 0.0524703795957336
3 0.0306364519613287
4 0.0310621266925596
5 0.0826804752318362
6 0.448127327988214
7 1.07610926960447
8 1.18706956051391
9 1.15270273035786
10 1.66774831406462
11 0.16135995996558
12 0.917051370604229
13 -1.14360819378424
14 -6.01650396115252
15 -12.2400452893168
16 -17.8910373502011
17 -19.9948887584923
18 -17.5908209914798
19 -11.4217358690489
20 -3.9647442546324
21 2.5766847739944
22 6.71679803636783
23 7.50464543306328
24 6.42020041017395
25 5.56300018643338
26 5.64400772912744
27 7.57173694158928
28 10.6343520600595
29 13.746232975388
30 15.1102367383043
31 14.5137465259371
32 13.2542143778972
33 12.1834965348117
34 11.8803209415749
35 12.4356104221131
36 13.2095991183325
37 13.3413480751382
38 12.2380256161256
39 10.011807108327
40 7.06934355748319
41 3.75116973902645
42 0.0704563156336255
43 -4.42337057253934
44 -10.0726334965798
45 -16.4039919685411
46 -22.0103637295345
47 -24.6352440645582
48 -21.9152736706715
49 -11.9312591115177
50 6.47897102121832
51 33.472318106968
52 68.176738829008
53 113.397230604181
54 170.888454681393
55 230.231778457601
56 279.601748419577
57 312.991452005915
58 326.583466600921
59 311.08241319926
60 263.615836086041
61 204.572267664173
62 141.085294916529
63 87.6849331557163
64 60.769738902595
65 41.6915947653381
66 27.5876333664223
67 16.5287697017793
68 7.55130041799529
69 0.525161436713883
70 -3.84785553073858
71 -5.20814458773117
72 -4.74126725757771
73 -3.73306299201173
74 -2.77311707423868
75 -2.02020076651618
76 -1.44254390058503
77 -1.01246325359933
78 -0.703893317865547
79 -0.48382456263647
80 -0.327816566280572
81 -0.21873274161
82 -0.142130430286434
83 -0.0886998034318081
84 -0.0530428758022828
85 -0.0301331207272159
86 -0.0159117012012499
87 -0.00768621876708151
88 -0.00304192291460934
89 0.00429500414865356
90 0.0405427111672761
91 0.0585175958724339
92 0.105671025440893
93 0.214165169244478
94 0.393936756222457
95 0.452898296622182
96 0.953652746713654
97 1.09792135597462
98 0.737987109223678
99 -0.053055744485078
};
\addplot [semithick, color1]
table {%
0 0.369304749393011
1 0.252804086814503
2 0.168524463177678
3 0.116476778305967
4 0.0887456815838113
5 0.0967682920792047
6 0.267965083226358
7 0.654039616940589
8 0.88113804270223
9 0.945408409810278
10 1.04675112300595
11 0.0990068684921315
12 0.366446454733725
13 0.842702732806684
14 0.649477068152957
15 -0.483251687898722
16 -1.81257942182571
17 -1.92922342444257
18 0.0191566209985015
19 3.94358744551105
20 9.0423767028515
21 14.3387725680531
22 18.7638429901221
23 21.3610401874076
24 22.3785310542896
25 22.7367383009954
26 23.1435671930828
27 24.3226782290668
28 26.2898955451268
29 28.5898210829725
30 30.2886337264502
31 30.987817792737
32 31.1195111964425
33 31.2277126875153
34 31.7928058303865
35 33.0326610534663
36 34.7329142786901
37 36.4213458590278
38 37.6468619985299
39 38.3052999828225
40 38.5385385302703
41 38.5338769414343
42 38.3429588974743
43 37.7478919735787
44 36.5385591603744
45 34.9583817233843
46 33.8323219810027
47 34.5212748309569
48 38.5241025732797
49 47.141629248265
50 61.3326471960645
51 81.4106414088283
52 107.114856586699
53 140.284103240299
54 183.355268166476
55 231.425301838339
56 275.328467481108
57 307.882081961124
58 324.138856052281
59 315.576872547069
60 278.054918517369
61 225.837018986493
62 167.54429736124
63 113.693829562932
64 76.2685247895206
65 50.2390837299971
66 32.1356322828499
67 19.5088404667325
68 10.6430965216893
69 4.44415959650196
70 0.545561401468557
71 -1.12985077422258
72 -1.41254566120708
73 -1.19480999984996
74 -0.896564377912207
75 -0.648113214675124
76 -0.450772331347163
77 -0.302688064171115
78 -0.198748275100696
79 -0.12654118300694
80 -0.0769352678784328
81 -0.0437861767493002
82 -0.0214504496844309
83 -0.00664392308352434
84 0.00213135139451405
85 0.0066491486254668
86 0.00844713367381748
87 0.00847718722067244
88 0.00764445232989447
89 0.0085083840272914
90 0.0226797615311433
91 0.0408751892148501
92 0.0739795227713099
93 0.143053087689911
94 0.262557340835257
95 0.353008136290872
96 0.614713941165204
97 0.800388858736508
98 0.763985041360152
99 0.497338155949409
};
\addplot [semithick, color2]
table {%
0 0.380799734834097
1 0.260846784052816
2 0.173791574402285
3 0.120068924664491
4 0.0914913548115691
5 0.100017026176588
6 0.278706112407525
7 0.684599502265987
8 0.926647771437285
9 0.996809583083568
10 0.432671542098504
11 -1.7394882592552
12 -4.36355573111268
13 -7.59287046397836
14 -11.0979797336112
15 -14.581152908856
16 -17.0633156073198
17 -17.7313511378319
18 -16.4260543081305
19 -13.970321603196
20 -11.3321778580175
21 -9.07598844787109
22 -7.64592346888056
23 -7.25053080626261
24 -7.36328804392993
25 -7.44193433327829
26 -7.08029232011825
27 -6.08631799548776
28 -4.62783299464785
29 -3.34122912905212
30 -3.08073368660625
31 -3.900820983735
32 -5.21261361410781
33 -6.49684533304003
34 -7.47474726287459
35 -8.19001162906191
36 -8.96519507845128
37 -10.1825622073516
38 -12.0507684468156
39 -14.4888742087749
40 -17.2967522261563
41 -20.3497755695289
42 -23.6940318001655
43 -27.5470185268078
44 -32.0350205165484
45 -36.8689560414509
46 -41.2270751545304
47 -43.8983371610978
48 -43.6089569013456
49 -39.2314183878008
50 -29.8841752538982
51 -13.1672018793222
52 43.7773799968906
53 110.164048892339
54 149.311550599686
55 192.894037106324
56 233.730039192464
57 266.202818735002
58 285.948533710941
59 285.009952480614
60 258.766548544681
61 217.214573821129
62 166.597209398559
63 116.845663926971
64 80.4521150782188
65 54.0540134021669
66 35.0898799707143
67 21.5834473596462
68 12.007983407515
69 4.27910527924214
70 -1.86990756445678
71 -2.71330353686812
72 -2.50411538731707
73 -1.97991935558317
74 -1.47264367953558
75 -1.07321488833506
76 -0.765959753138188
77 -0.53692736281214
78 -0.372667576921297
79 -0.255595441286861
80 -0.172678888677024
81 -0.114787758863154
82 -0.074178223619817
83 -0.0458870567484658
84 -0.0270733790149376
85 -0.0150559475480923
86 -0.00763413640679277
87 -0.00330706946899355
88 -0.000842158840882942
89 0.00146885812865911
90 0.0102581516730879
91 0.0361370971082749
92 0.0753150679354294
93 0.146307924497212
94 0.269620886114663
95 0.363677045604623
96 0.633498866768189
97 0.822219554442481
98 0.775183719912442
99 0.197278765046223
};
\addplot [semithick, color3]
table {%
0 0.0904620902970917
1 0.055203317271822
2 0.0279988949591468
3 0.0140924940997747
4 0.00940540952190951
5 0.0197074629348759
6 0.123932893374117
7 0.360467215583509
8 0.430679053729047
9 0.427012832612993
10 0.551562510409437
11 -0.525885487224819
12 0.80749017716736
13 0.701637764295826
14 -1.79711370497333
15 -5.73561095522771
16 -9.84961952000948
17 -11.6271357056909
18 -10.2299394927637
19 -5.85151761238651
20 -0.16269003756819
21 5.08989364823385
22 8.60461853603525
23 9.26193947595607
24 8.16455794243188
25 7.23660322450548
26 7.0433123621137
27 8.36159580385262
28 10.7347456161341
29 13.4591453488619
30 14.9219058739137
31 14.8037934795902
32 14.2419799414032
33 13.9156085859193
34 14.3027126192895
35 15.5552734973359
36 17.1982477126343
37 18.529990509793
38 19.0102452056811
39 18.7076242212975
40 17.939959572711
41 17.0107719052553
42 15.9905248709064
43 14.5465944173449
44 12.3733914174752
45 9.7279742244737
46 7.43960574845302
47 6.99246072582365
48 9.96348685566198
49 17.6359999404096
50 31.1198798370997
51 50.9063425724799
52 76.8666956966286
53 109.643639245625
54 151.675261822555
55 196.142459238788
56 231.642192470439
57 253.005709026601
58 258.660375062743
59 241.47512164667
60 194.485935304634
61 140.266026516645
62 91.2094695969032
63 53.4172860708642
64 36.1098226420567
65 24.445777675202
66 16.1810649206591
67 9.85489587921664
68 4.8341191995743
69 0.813294410937602
70 -2.00184882183088
71 -3.02019304134723
72 -2.82569423967877
73 -2.25204184440217
74 -1.68532310598864
75 -1.23455084847148
76 -0.885211114721233
77 -0.623287241156514
78 -0.434483963710409
79 -0.299314982461287
80 -0.203192902693287
81 -0.135818043009398
82 -0.0883928361287331
83 -0.055245439116269
84 -0.0331052476494625
85 -0.0188907766080656
86 -0.0100921293422654
87 -0.00503500968292392
88 -0.00239459664742046
89 -0.000909138749630374
90 0.00136451506832897
91 0.00463770474665733
92 0.015484998307806
93 0.0453783600162392
94 0.101636943004441
95 0.133399753243269
96 0.289532192790189
97 0.327793111327844
98 0.172754884841177
99 -0.0143668978934503
};
\addplot [semithick, color4]
table {%
0 0.314422271641424
1 0.191230376115578
2 0.0930810889519768
3 0.0435102876527619
4 0.0265736383226743
5 0.0599659882101129
6 0.29745406515808
7 0.868991886798324
8 1.22718060191969
9 1.26758070031711
10 0.0859800297159217
11 -0.969357451456137
12 -2.376331095402
13 -4.13467036719544
14 -6.01008069895497
15 -7.83578679331689
16 -9.1165547048706
17 -9.46737372697453
18 -8.83333893891657
19 -7.65561662493453
20 -6.43753448124128
21 -5.47436608192819
22 -4.96381779694973
23 -4.90860843853397
24 -5.01947312263151
25 -5.07635669857899
26 -4.92650523279951
27 -4.53926195325068
28 -4.03949148215909
29 -3.69369883440176
30 -3.71859371060249
31 -4.07879933886705
32 -4.60964487345361
33 -5.15803595820623
34 -5.62259887104946
35 -6.01850886724692
36 -6.47083887804527
37 -7.12937449400233
38 -8.08006034919282
39 -9.29879308397642
40 -10.7078201572371
41 -12.2550420887065
42 -13.9635534919485
43 -15.9363199061027
44 -18.2323380099279
45 -20.7078304577182
46 -22.9536879949828
47 -24.3692252635757
48 -24.3277282472525
49 -22.2936370055116
50 -17.9709296237919
51 -11.4796518826733
52 0.341607456643976
53 50.5297418939252
54 143.598114235179
55 240.654261902269
56 327.245947269274
57 391.981206675866
58 426.765545491195
59 421.276194596671
60 373.661691070391
61 304.695883799774
62 228.342588234489
63 158.669890657537
64 110.362223250363
65 76.529611962783
66 51.45094886544
67 31.3427396224789
68 14.516410578668
69 2.69183152774105
70 -1.06263483531255
71 -1.43828653464878
72 -1.30936244547456
73 -1.03094710230799
74 -0.765854328671045
75 -0.557930152860557
76 -0.398404814416819
77 -0.279636402432867
78 -0.194428097438512
79 -0.13366464620559
80 -0.0905957224636321
81 -0.0604851272011529
82 -0.0393400037409301
83 -0.0245896321331017
84 -0.0147479180266057
85 -0.00843220256139737
86 -0.00452257869559627
87 -0.00227268861396717
88 -0.00109763912181497
89 -0.000579397757948406
90 -0.00073335240883407
91 0.00162227754229525
92 0.0258646927378186
93 0.100748518748184
94 0.241889482782793
95 0.364017195977901
96 0.589453004690627
97 0.504810072588687
98 0.0563111905757758
99 -0.0177058067739215
};
\addplot [semithick, color5]
table {%
0 0.271478581587819
1 0.180680202997133
2 0.113381245383372
3 0.0745415918138948
4 0.0556829962121872
5 0.0666583637631102
6 0.219035975540044
7 0.593650615118213
8 0.833825017932516
9 0.87602440873431
10 0.602433166072229
11 -1.17925844864215
12 -2.87451375891345
13 -4.97840593773362
14 -7.64531533291528
15 -10.7428354029544
16 -13.1709997517774
17 -13.689931137271
18 -11.8374185331415
19 -8.32310686796021
20 -4.2519727921418
21 -0.479621549458135
22 2.23269184806527
23 3.45010445694897
24 3.71670982066922
25 3.77262144276502
26 4.15813346973959
27 5.23702301206097
28 6.83394909269448
29 8.34680968627609
30 9.02889862237807
31 8.75937183685218
32 7.98317518141032
33 7.17102047824255
34 6.6780488829034
35 6.56554468401046
36 6.54548829966675
37 6.18848246601976
38 5.17943842143821
39 3.51901229581824
40 1.38928845806609
41 -1.05378484960174
42 -3.82692972657176
43 -7.17366361722527
44 -11.263965413099
45 -15.7822368519741
46 -19.7842475665033
47 -21.8320969911177
48 -20.3988048160862
49 -14.169334347594
50 -2.29603646367587
51 15.343359461186
52 38.2561307000575
53 67.9034382771386
54 108.08757101667
55 157.625541898895
56 209.740787800643
57 257.283387022849
58 292.768185985965
59 304.034544577373
60 284.279129763689
61 244.081252059435
62 190.95981060009
63 137.046059960477
64 96.9136039913778
65 66.5786177105194
66 43.0435581845904
67 24.8938469523291
68 11.8861180985545
69 3.61497094689907
70 -0.915184227759001
71 -2.61438341508558
72 -2.65115202547885
73 -2.13195701286522
74 -1.57651462256445
75 -1.13505050693714
76 -0.795487464631372
77 -0.54484311959108
78 -0.368563902687603
79 -0.245434620651865
80 -0.160041772857905
81 -0.101856261445608
82 -0.0619413734215183
83 -0.0348037059078938
84 -0.0174729959333956
85 -0.00703956417838328
86 -0.00114327954017052
87 0.00171913494719837
88 0.00277585292549532
89 0.00394902259797774
90 0.011666945360618
91 0.0229910829462793
92 0.0459686546920702
93 0.0989523903827016
94 0.195712180504915
95 0.274886096456894
96 0.467958906075022
97 0.547698117688585
98 0.445727205902093
99 0.25796535851057
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};


==> plots/all/TibialisAnteriorFalse.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 35.6958267650983
1 45.4845955534775
2 23.2006640860671
3 -5.94819880084243
4 -23.6599873129014
5 -26.6838234198345
6 -15.7103191233897
7 -0.690713771225674
8 10.9005525733527
9 12.7066824197832
10 4.98662462552275
11 3.63183902135816
12 2.8131180165809
13 1.96596525014865
14 1.30519684525405
15 0.863623932478203
16 0.581102069491015
17 0.396426285960007
18 0.269622143955205
19 0.179759149040043
20 0.115257237963378
21 0.0695775828229044
22 0.035376265156455
23 0.0102598684712009
24 -0.00344953604346627
25 -0.00869535154627643
26 -0.00955901723664298
27 -0.00851036282660449
28 -0.00682160188094614
29 -0.00509515061413702
30 -0.00357355617389302
31 -0.00232389458697295
32 -0.00133701154535864
33 -0.000575913112832997
34 1.40134000613934e-06
35 0.000432795535468258
36 0.000750897971891984
37 0.000983831747110002
38 0.00115523483814161
39 0.00128357217418615
40 0.00138254808970697
41 0.00146220796069656
42 0.00152977183723104
43 0.00159031666299655
44 0.00164689593062338
45 0.00170047886230744
46 0.00175050058436275
47 0.00179550183737002
48 0.00183361679427924
49 0.00186302675374871
50 0.00188240473819946
51 0.00189302115797145
52 0.00190423683064843
53 0.00195255342860901
54 0.00208226083451551
55 0.00231686316104407
56 0.00271213585830712
57 0.00342776515060956
58 0.00488538239807405
59 0.00879458905527159
60 0.0282543675866143
61 0.229795108262365
62 0.629304389917176
63 0.770512911243934
64 0.0937593502678179
65 -0.0827350980516081
66 3.0331103834505
67 8.20056112042849
68 14.7786208786587
69 19.1919158632337
70 15.7953959323677
71 6.74770663207382
72 3.50112440050009
73 4.08869204844288
74 6.95476586538825
75 11.5034017946616
76 15.2116939030799
77 15.7499498140726
78 12.9174371066676
79 8.48850346652062
80 4.85495118762398
81 3.42065287242947
82 3.84530480074699
83 4.93943422781313
84 5.68440919478448
85 5.38712653103521
86 5.17093847052324
87 8.39634940051137
88 6.87187882459476
89 5.45568582282139
90 3.99844038521096
91 3.34052956834248
92 2.73266640533888
93 -0.674714299164882
94 -1.96402386287222
95 -1.26838275924565
96 -0.679723963061455
97 0.266794251850234
98 4.76054140704052
99 9.63726064716347
};
\addplot [semithick, color1]
table {%
0 12.8989910366705
1 14.4124196051158
2 0.135025894574493
3 -18.1816610967842
4 -30.4164966056303
5 -28.8947469057366
6 -17.4431529399936
7 -4.94129090455942
8 3.19222356663345
9 5.85902522886709
10 5.00194726967566
11 4.10244781831156
12 3.09518830641738
13 2.15026706310996
14 1.43302672708062
15 0.953112492256932
16 0.642935784725245
17 0.438574581060163
18 0.298340727545839
19 0.199596291049587
20 0.129338835675096
21 0.0798818184974931
22 0.0433754506572974
23 0.0169153353577732
24 0.00221251112179632
25 -0.0041507205339652
26 -0.00619269602053407
27 -0.00623480126623408
28 -0.00548580321975098
29 -0.00453926549554339
30 -0.0036540829636536
31 -0.00292040030145945
32 -0.00235025688045461
33 -0.00192410238021172
34 -0.00161279892776652
35 -0.00138743350111246
36 -0.00122334953392978
37 -0.00110133667569159
38 -0.00100732413468163
39 -0.000931476279820754
40 -0.000867136177754004
41 -0.000809888858085487
42 -0.000756880767730904
43 -0.000706297119058863
44 -0.000657025337457797
45 -0.000608555473223422
46 -0.000560901518326404
47 -0.00051453352134303
48 -0.000470345066941641
49 -0.000429536406946363
50 -0.00039343888575366
51 -0.000363434354185792
52 -0.000341019937421892
53 -0.000328425078094596
54 -0.0003287957588154
55 -0.000345749247640941
56 -0.00038420110349024
57 -0.000451625751123595
58 -0.000549888846617452
59 -0.000544019475262092
60 0.00342673525658735
61 0.0632870449080133
62 0.19383226217728
63 -0.0416521326133224
64 -1.15885320398908
65 -2.51437031863324
66 -2.67500450179725
67 -0.838068333261062
68 2.55127273468476
69 5.61266049740765
70 5.5595119332584
71 3.48918615452015
72 2.85450352709202
73 3.32629949165911
74 4.46157765431022
75 6.14095302989286
76 7.70692822589031
77 8.07941905287263
78 6.94062688239189
79 5.01061677238316
80 3.33797795602934
81 2.47143129291336
82 2.26139905968306
83 2.33969136061425
84 2.36300391755155
85 2.10763167103782
86 2.08714725559764
87 2.51004333878372
88 1.93049481467383
89 1.14591051314372
90 0.454454592554255
91 0.0933961300725506
92 -0.601391971608384
93 -1.46084228818577
94 -1.36194898925307
95 -0.852903325756125
96 -0.416655935912786
97 0.175380720028718
98 1.2391763785961
99 3.37728277814974
};
\addplot [semithick, color2]
table {%
0 26.5124687323549
1 34.4269138224884
2 7.3709028168395
3 -4.16262667582897
4 -11.1095846581403
5 -11.0231551663644
6 -5.71608175484592
7 0.383926459673313
8 13.400660911375
9 15.7890591232533
10 12.8942766727576
11 9.83401356997205
12 7.19055577055001
13 5.0611258726545
14 3.49721755342586
15 2.41701353193616
16 1.68198965278738
17 1.17655569097669
18 0.822603875930271
19 0.57203164969357
20 0.393917120988216
21 0.267914098319135
22 0.177030168002355
23 0.112030851176555
24 0.0421686436887898
25 0.0143172787961799
26 0.00730116794275066
27 0.00423337192014298
28 0.00260828015160738
29 0.00169795777388933
30 0.00117131581691172
31 0.000858459562368963
32 0.000668787424106412
33 0.00055276790896074
34 0.000482630079344138
35 0.000442227157354749
36 0.000421716202026987
37 0.000414812776159734
38 0.000417388702664834
39 0.000426657794764149
40 0.000440717910077045
41 0.000458300207590959
42 0.00047858129729309
43 0.000501062421189725
44 0.000525425457625547
45 0.00055131534813774
46 0.000578207458174176
47 0.000605344450957859
48 0.000631696819808114
49 0.000656004803261173
50 0.000676895401589256
51 0.000693165199445086
52 0.000704510833026097
53 0.000713693062942687
54 0.000726480809392408
55 0.000749198207905365
56 0.000791347692898118
57 0.000874202954971071
58 0.00105838924877877
59 0.00166458407800667
60 0.0130815575736787
61 0.127699331970977
62 0.382043025104435
63 0.295456373836528
64 -0.40347940850942
65 -0.917093769062228
66 -0.560623929511935
67 2.24453228440667
68 9.23182497089837
69 16.1676726640915
70 16.5930392442327
71 12.7048418962407
72 9.96677683986055
73 8.90987153962366
74 9.41769583462504
75 11.5142798081874
76 14.0210858889747
77 15.0305423697756
78 13.7378638038074
79 10.920400063495
80 8.05624719358964
81 6.19148591188992
82 5.45757422427245
83 5.46148841626054
84 5.64119844773992
85 5.47380715594469
86 5.47188586797207
87 6.7788501412256
88 6.50601348828689
89 5.64523902671378
90 3.69005909044599
91 1.89057553680992
92 0.916104054759498
93 0.186190517078751
94 -0.031491598606814
95 0.0430683875626376
96 0.16578450687651
97 1.1659458710245
98 3.09649631069174
99 6.76208379147349
};
\addplot [semithick, color3]
table {%
0 22.810002851429
1 26.610094518772
2 15.2562398348063
3 6.16558448381377
4 -1.48959724367545
5 -5.25963655570904
6 -1.49639899283946
7 4.95560926947803
8 9.7407152674218
9 11.3523896558281
10 7.9340256198584
11 6.42695571549212
12 5.13105308763837
13 3.94844267941269
14 3.00693462740717
15 2.30918839730723
16 1.79598549990052
17 1.41044332217371
18 1.11327096652843
19 0.880783080442304
20 0.69761871049041
21 0.55340045701613
22 0.438263186933966
23 0.346640596067312
24 0.278556998712165
25 0.22741105400379
26 0.18782577594868
27 0.156886001574217
28 0.132670244391435
29 0.113812839548495
30 0.0993115802254592
31 0.088379942923458
32 0.0803510714519354
33 0.0746336550144925
34 0.0706907872813219
35 0.0680412494191836
36 0.0662846720678116
37 0.0651197896993019
38 0.0643389891616792
39 0.0638041910160109
40 0.0634256778147564
41 0.063147979958135
42 0.0629385388387657
43 0.0627791935211728
44 0.0626568572786295
45 0.0625561761714472
46 0.0624588146754466
47 0.0623455062250041
48 0.0621987186273493
49 0.0620052345978821
50 0.0617586819036779
51 0.0614778360034386
52 0.0612593751554682
53 0.0615474380600894
54 0.0631518308638222
55 0.0665211492668994
56 0.072134950779382
57 0.0815830496964458
58 0.098285609532915
59 0.132508156669783
60 0.226008651844707
61 0.669588833201225
62 1.3782828821953
63 2.0923803782981
64 2.87763554225723
65 4.196039231458
66 7.00956667407191
67 8.25350356522456
68 10.2227679545096
69 12.8492489840982
70 11.6505602790021
71 7.67794134591085
72 6.03501581051457
73 6.05985139321471
74 7.36693815046821
75 9.8409700430712
76 12.1893746338964
77 12.5690512759347
78 10.9533931584411
79 8.50759488532078
80 6.26017798795972
81 5.05640156712839
82 4.98208954831952
83 5.47180779516346
84 5.96855470597203
85 5.77792835351326
86 5.65673444546033
87 7.76504838686202
88 6.76734224666548
89 5.79778709158281
90 4.94925576869388
91 4.71655083366356
92 4.56448457606525
93 2.68849334287823
94 1.25332489173264
95 1.20895505519651
96 1.19226680650645
97 1.53588252933089
98 5.28644396725918
99 8.5934710224398
};
\addplot [semithick, color4]
table {%
0 35.189873683595
1 36.6224396949992
2 3.87350638895071
3 18.0640987117295
4 28.0674006772893
5 26.4630060442253
6 16.5641594682862
7 5.88856432780704
8 5.98628061829584
9 13.365458872215
10 12.2892667629174
11 10.6152869980834
12 8.20152800027021
13 5.73158708750564
14 3.80966954161268
15 2.52322848231857
16 1.69807762529284
17 1.15764218641208
18 0.786239693832044
19 0.522981675361033
20 0.333950527409297
21 0.19981360249136
22 0.0988920238690586
23 0.0242480203589842
24 0.00641710113809294
25 0.00768992209580004
26 0.00829101150272394
27 0.00753874176311474
28 0.0063461728544889
29 0.00514530741448678
30 0.00410904250373587
31 0.00328237202843788
32 0.00265360837885034
33 0.00219048106132456
34 0.00185674009590593
35 0.00161918606273523
36 0.00145032282928414
37 0.00132891031970354
38 0.0012393795158306
39 0.00117077091991378
40 0.00111558783965642
41 0.00106880628912099
42 0.00102714373507161
43 0.000988495963032393
44 0.000951543286905161
45 0.000915569857493498
46 0.000880339447414216
47 0.000846014804494013
48 0.000813131114272882
49 0.000782513001489213
50 0.000755150305332382
51 0.000732238271296203
52 0.000715568113033924
53 0.000709212489447805
54 0.0007197319737873
55 0.000754563024728935
56 0.000824239528286591
57 0.000948091428362834
58 0.00115829403700565
59 0.00144119681092509
60 0.00852155519212798
61 0.168326649154994
62 0.524378267010502
63 0.664549063638655
64 1.0768779528193
65 2.3324143206474
66 2.75292684781049
67 1.63248338291382
68 3.53336107705985
69 11.3109855162691
70 10.7772665924651
71 5.33733054326598
72 4.77777792667024
73 7.41923903948657
74 11.5073864344864
75 16.5789895222344
76 21.0141220037791
77 22.0032206816667
78 18.7109179902384
79 13.1953232273899
80 8.51852744434733
81 6.26076043491352
82 5.86523345709071
83 6.18379254171552
84 6.23082002147202
85 5.41385307828685
86 5.36987905449372
87 6.39689474785237
88 4.4028310365123
89 1.84304510372627
90 0.111021023524853
91 0.39378519945327
92 0.968752339049222
93 1.6035907508248
94 1.41705303785487
95 0.917352196348118
96 0.499332554222005
97 0.113383076918664
98 3.22002498110445
99 9.36550328209253
};
\addplot [semithick, color5]
table {%
0 30.5402148146912
1 39.5499204535805
2 28.4281759188363
3 16.8197199111481
4 11.8302084070307
5 9.64253458688465
6 9.21195858091608
7 11.5933443303344
8 16.0119585432408
9 17.2312584445803
10 13.423220635682
11 10.2571899470437
12 7.59901306521001
13 5.4124305494531
14 3.77792430478853
15 2.63667267819633
16 1.85285201880348
17 1.30873300471167
18 0.923793508695091
19 0.64846954975234
20 0.450875415217653
21 0.31003179586675
22 0.208479667471274
23 0.136701259264185
24 0.0895135856273883
25 0.0598210915312937
26 0.040970482411967
27 0.0287026860839022
28 0.0205429021434164
29 0.0150229761921
30 0.0112460371504744
31 0.00864643968888768
32 0.00685590069306335
33 0.00562766121633758
34 0.00479220043361961
35 0.00423048128169767
36 0.00385792709248044
37 0.00361461863454501
38 0.00345870883858325
39 0.00336135705600401
40 0.00330293520744701
41 0.00327032556198686
42 0.00325493446711255
43 0.00325126093613121
44 0.00325570675395735
45 0.00326554240551093
46 0.0032783042987988
47 0.00329155060872489
48 0.00330283080952516
49 0.00330983257704408
50 0.00331063514524921
51 0.00330460896805808
52 0.00329504122742323
53 0.00329794665047999
54 0.00334181349627442
55 0.00345743068671958
56 0.00368905598917527
57 0.0041285791073622
58 0.00499975333223686
59 0.00710862625401167
60 0.0167467753356714
61 0.124008251140604
62 0.372884506746395
63 0.506269919372542
64 0.478124831261601
65 0.87988310174217
66 2.44592617270116
67 5.7024042037039
68 10.6101923881441
69 15.1521138870382
70 15.7397755605545
71 12.3330067964673
72 9.62835056933071
73 8.35374294345289
74 8.80867943681951
75 11.1663778123735
76 14.0585771290389
77 15.2528738341846
78 13.911538487651
79 11.0291862222328
80 8.17939472503136
81 6.34216177950787
82 5.64335921344248
83 5.71848204186306
84 5.97384410727348
85 5.84699560275242
86 5.89394962994502
87 7.38429685939714
88 7.22154613076608
89 6.63296949517363
90 5.89761336322511
91 5.38175132115194
92 4.79149473365275
93 3.32874683416671
94 2.22494944488144
95 1.65078848997434
96 1.28530229585695
97 1.32289114035293
98 3.26524351488531
99 7.46171795817308
};
\addplot [semithick, black]
table {%
0 8.79746842089874
1 9.1556099237498
2 -3.58573727503706
3 -21.6769184540753
4 -33.6808808127472
5 -31.7556072530703
6 -19.8769913619435
7 -7.06627719336845
8 0.901249267843663
9 3.34136471805376
10 3.07231669072934
11 2.65382174952085
12 2.05038200006755
13 1.43289677187641
14 0.952417385403171
15 0.630807120579643
16 0.424519406323209
17 0.289410546603021
18 0.196559923458011
19 0.130745418840258
20 0.0834876318523243
21 0.0499534006228399
22 0.0247230059672647
23 0.00606200508974605
24 -0.00483116106334403
25 -0.00922790651496005
26 -0.00994921380326873
27 -0.00904649011573769
28 -0.00761540742538667
29 -0.00617436889738414
30 -0.00493085100448304
31 -0.00393884643412546
32 -0.00318433005462041
33 -0.00262857727358947
34 -0.00222808811508711
35 -0.00194302327528228
36 -0.00174038739514097
37 -0.00159469238364425
38 -0.00148725541899672
39 -0.00140492510389654
40 -0.00133870540758771
41 -0.00128256754694518
42 -0.00123257248208593
43 -0.00118619515563887
44 -0.00114185194428619
45 -0.0010986838289922
46 -0.00105640733689706
47 -0.00101521776539282
48 -0.000975757337127458
49 -0.000939015601787056
50 -0.000906180366398858
51 -0.000878685925555444
52 -0.000858681735640709
53 -0.000851054987337366
54 -0.00086367836854476
55 -0.000905475629674723
56 -0.000989087433943909
57 -0.0011377097140354
58 -0.00138995284440678
59 -0.00172943617311011
60 0.000723244755708979
61 0.0420816622887486
62 0.131094566752626
63 -0.136160217727959
64 -1.29225354338316
65 -2.79889718477688
66 -3.30351221737259
67 -1.95898005949659
68 0.676896226184906
69 2.82774637906727
70 2.69431664811627
71 1.33433263581649
72 1.19444448166756
73 1.85480975987164
74 2.87684660862161
75 4.14474738055861
76 5.25353050094476
77 5.50080517041668
78 4.6777294975596
79 3.29883080684746
80 2.12963186108683
81 1.56519010872838
82 1.46630836427268
83 1.54594813542888
84 1.55770500536801
85 1.35346326957171
86 1.34246976362343
87 1.59922368696309
88 1.10070775912807
89 0.447155407053803
90 -0.133225228229824
91 -0.472542239343924
92 -1.16250280685907
93 -1.92430890098975
94 -1.70046364542584
95 -1.10082263561774
96 -0.597977848487545
97 0.0283457692296661
98 0.805006245276113
99 2.34137582052313
};


==> plots/all/TibialisAnteriorTrue.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\addplot [semithick, color0]
table {%
0 52.7778749078445
1 69.8260098893896
2 37.9243439524132
3 -3.90502048117182
4 -28.9336442854454
5 -34.494275045123
6 -20.13694003677
7 0.564728746798824
8 17.5109272901202
9 19.8343915454401
10 7.45048114621719
11 5.32984878439858
12 4.12074446639881
13 2.88019013873028
14 1.91435354631748
15 1.26816408268707
16 0.853995301562367
17 0.582914839433011
18 0.396690599324201
19 0.264702242579459
20 0.169939398010734
21 0.102765232122754
22 0.0523693436672181
23 0.0151893765056573
24 -0.00444404113375078
25 -0.0117070159893896
26 -0.0128903793123458
27 -0.0114543237398622
28 -0.00913966607298512
29 -0.00677075048876825
30 -0.00467960357876348
31 -0.00295841568280113
32 -0.00159534860759601
33 -0.000540571580067604
34 0.000262521650188327
35 0.000864866100140468
36 0.00131048967897309
37 0.00163767622601531
38 0.00187892556733836
39 0.0020597974092112
40 0.00219935515967179
41 0.00231164323016031
42 0.00240680652285639
43 0.00249201111269322
44 0.00257155994057118
45 0.00264677333017055
46 0.00271677972704824
47 0.00277944647426341
48 0.00283209622632611
49 0.00287216542255833
50 0.00289784363417502
51 0.00291119464793078
52 0.00292634577876196
53 0.00299794779008801
54 0.00319261656727696
55 0.00354642340507708
56 0.00414376076667146
57 0.0052243852571892
58 0.00741837313671336
59 0.0132575522434815
60 0.0420225085096093
61 0.338622819903553
62 0.926389947376866
63 1.16716977424174
64 0.304032230477849
65 0.240046084609652
66 4.91078017461624
67 12.3644707206547
68 21.8340752444812
69 28.4187161025932
70 23.5464543242841
71 9.99683078113816
72 5.19217228254065
73 6.04219885583977
74 10.2200009975395
75 16.8275147263364
76 22.1956137713051
77 22.9838397323442
78 18.8919778945231
79 12.4521450650334
80 7.13948877685514
81 5.03289133517152
82 5.65101039705409
83 7.25056661296234
84 8.34205330124228
85 7.91140021741329
86 7.59122054646765
87 12.3093914281296
88 10.0827456572615
89 8.00196207330243
90 5.87026879138703
91 4.9459277354448
92 4.13275817699299
93 -0.769165348139736
94 -2.686391618789
95 -1.7345774171067
96 -0.928559328628132
97 0.392391718492102
98 6.99117480933549
99 14.0717667295019
};
\addplot [semithick, color1]
table {%
0 23.5595005139448
1 32.7212641110482
2 21.5508700212319
3 2.22154084625787
4 -11.1394659822119
5 -11.8128847585025
6 -2.80261230707604
7 7.87592961931046
8 15.3119726195089
9 16.61923053625
10 12.3195703510229
11 8.90599447934765
12 6.2465490475738
13 4.22277248419741
14 2.80380020331181
15 1.86433805670314
16 1.25075187955025
17 0.844536569264357
18 0.569705476678504
19 0.381251042957177
20 0.251405282320552
21 0.162525439067144
22 0.100048496612818
23 0.056731299665682
24 0.030936911358367
25 0.0170704932194052
26 0.00979647413125117
27 0.00600281291303585
28 0.00400884056592617
29 0.00292955957696241
30 0.00231643697434379
31 0.00194898747968678
32 0.00172087930745886
33 0.00158066173928248
34 0.00150228589132835
35 0.00147074928332922
36 0.00147561136517193
37 0.00150852929778247
38 0.00156259480530521
39 0.00163209105043932
40 0.00171241153394198
41 0.00180002705675205
42 0.00189235205966111
43 0.00198759507914868
44 0.00208444670751015
45 0.00218158631490677
46 0.00227740139925594
47 0.002369912247157
48 0.00245682424334343
49 0.00253575759912533
50 0.00260458850347872
51 0.00266229683842062
52 0.00271130657399623
53 0.0027652604568499
54 0.00284939589868193
55 0.00299233308331344
56 0.00323633356414467
57 0.00366978718237356
58 0.00451474491338382
59 0.00662805755654722
60 0.0174665977549536
61 0.127846947635657
62 0.374427375283388
63 0.352867302961893
64 -0.359737244010774
65 -0.758497332137365
66 1.27389188725468
67 6.29983178586841
68 13.4734225779999
69 19.8217852304604
70 20.4714847861515
71 15.6007300026354
72 11.8709502109222
73 10.0873201239735
74 10.141167511678
75 11.9774557895183
76 14.2829230641973
77 15.0779024872868
78 13.55584719933
79 10.5445924094121
80 7.56870771060411
81 5.65283805616739
82 4.86189185856021
83 4.76152344752426
84 4.80752543996704
85 4.5419361350649
86 4.45472733083834
87 5.44379494118156
88 5.05272352953025
89 4.29491794372198
90 3.49483030335837
91 3.02380971211797
92 2.31522118311321
93 0.958923296591647
94 0.421861145204365
95 0.468035262609221
96 0.558554921710847
97 0.938159951905547
98 2.60534381834705
99 5.75527610821843
};
\addplot [semithick, color2]
table {%
0 32.8660866782758
1 44.2757441651124
2 8.2782781574934
3 -16.2898194043101
4 -27.3492839260517
5 -25.9456190361739
6 -15.772681129993
7 -4.07880788171509
8 19.8577053439813
9 22.5453352561917
10 17.234140808682
11 12.7959642301637
12 9.25012180448685
13 6.49706492915935
14 4.50144229348716
15 3.12020951669649
16 2.17454445823929
17 1.52157449463965
18 1.06445434866595
19 0.741848026238921
20 0.513514782742554
21 0.352517840878834
22 0.237310287986464
23 0.155442984425525
24 0.0591079110850328
25 0.0135812301608861
26 0.00118367016773512
27 -0.00224719057292261
28 -0.0029855787774062
29 -0.00283471297671176
30 -0.00242800940886728
31 -0.00200042181782219
32 -0.00163176922139935
33 -0.00133936759325447
34 -0.00111631181335407
35 -0.000948015363130859
36 -0.00081939340916092
37 -0.000717698677465004
38 -0.000633178104928399
39 -0.000558840991106966
40 -0.000489859422674541
41 -0.000422923183881963
42 -0.000355772995545768
43 -0.000286816488585842
44 -0.000214942293467739
45 -0.00013966816659101
46 -6.12827395703967e-05
47 1.90276139098902e-05
48 9.90237536170563e-05
49 0.000175470957358194
50 0.000244441411534517
51 0.000301807066513207
52 0.000344164827184455
53 0.000370720346432591
54 0.000383146415501189
55 0.000383440802808806
56 0.000375833551678531
57 0.000374650056628763
58 0.000446081947306361
59 0.00118622443560595
60 0.0178666060331516
61 0.164008545800637
62 0.485600881522305
63 0.249772923786099
64 -1.03812292739812
65 -2.26505723719338
66 -2.40537772782487
67 2.39840855432495
68 14.1943866087768
69 22.9952442225495
70 23.7859247465028
71 18.654563566678
72 14.5186579626456
73 12.3816311120828
74 12.3482565410616
75 14.5215730800572
76 17.4277489011496
77 18.7275966737111
78 17.3545499450197
79 14.0841087040536
80 10.5888006816014
81 8.17015919533535
82 7.12194082821899
83 7.04994254587769
84 7.28646797780941
85 7.15915666330185
86 7.14647392003433
87 8.86864419722355
88 8.77091825561807
89 7.94611902423277
90 5.68718761521491
91 2.79478569585016
92 0.311778123599727
93 -1.16068168226201
94 -1.15367954828942
95 -0.704414423293647
96 -0.237298553859894
97 1.70362571175106
98 4.03883736683246
99 8.36439748921283
};
\addplot [semithick, color3]
table {%
0 51.0349793831692
1 78.8453869890566
2 51.1241426340042
3 15.6080998654646
4 -3.74965486018077
5 -11.3808889888652
6 -5.39636692266081
7 5.74909480081534
8 15.3504042583303
9 15.6895264618156
10 7.21917114614572
11 4.81273291112199
12 3.39659246647315
13 2.27193988080563
14 1.47541214994194
15 0.956957208356995
16 0.628044627572409
17 0.416514260652481
18 0.276015113602396
19 0.180476930637725
20 0.114668717777434
21 0.0695565321493516
22 0.0371034048878584
23 0.0139281397175816
24 0.00020551963608611
25 -0.00597312874173653
26 -0.00782168961085815
27 -0.00763401572767549
28 -0.006657443878565
29 -0.00550585911563803
30 -0.00444691787565792
31 -0.00357266476945174
32 -0.00289322256975461
33 -0.00238521084609975
34 -0.00201496878628627
35 -0.00174906233806683
36 -0.00155865547942486
37 -0.00142089949481762
38 -0.00131874157794847
39 -0.00124003779056164
40 -0.00117641637881465
41 -0.00112222508961426
42 -0.00107374412738861
43 -0.00102857153496191
44 -0.00098520973189748
45 -0.000942892517842613
46 -0.000901441221907325
47 -0.000861157068891154
48 -0.000822774510050545
49 -0.000787347682626851
50 -0.000756088305455314
51 -0.000730314400571604
52 -0.000711633610673362
53 -0.000702476007156867
54 -0.00070599218438992
55 -0.000727577493702698
56 -0.000774165498764493
57 -0.000850833175149958
58 -0.000944383655087182
59 -0.000813238750523932
60 0.00417531223213698
61 0.0945078705597564
62 0.297369717969567
63 0.33072953751517
64 -0.322447543787761
65 -0.163404312524773
66 3.77360134864181
67 10.3808489064834
68 18.5122008845636
69 23.555944403879
70 19.2342564901127
71 8.69694686091017
72 5.05938979192167
73 4.61137729930938
74 6.1506623229219
75 9.84269007229215
76 14.0464382922604
77 14.7013757340818
78 11.7161583496041
79 7.89662651848676
80 4.79880412826221
81 3.35228155329028
82 3.28827902755301
83 3.90754015910694
84 4.64200077232556
85 4.46619232304252
86 4.42055025156595
87 8.32711683616326
88 6.6274128458992
89 5.26443457309076
90 3.94828584489675
91 3.32293114093653
92 2.72405930856367
93 0.00369070038227577
94 -0.989865718705709
95 -0.656797352346384
96 -0.318288216248901
97 0.333011739217178
98 4.01924156798094
99 9.35612010261112
};
\addplot [semithick, color4]
table {%
0 34.2774438615658
1 35.6728652113386
2 -0.933588167825725
3 -9.47458791603155
4 -14.7213021549084
5 -13.8797999994146
6 -8.68787242817381
7 -3.08854160472386
8 5.21580191102233
9 13.0189090843481
10 11.9706213029712
11 10.3400457592674
12 7.98887254146014
13 5.582974136143
14 3.7108895308318
15 2.45780429421942
16 1.65404857649975
17 1.12762595891384
18 0.765853472774085
19 0.509421408527889
20 0.325291604020418
21 0.194632683361059
22 0.0963278762239078
23 0.0236192992359805
24 -0.000400285289458138
25 -0.00403335057711914
26 -0.00434862091095527
27 -0.0039540567592509
28 -0.0033285564699193
29 -0.00269870466451281
30 -0.00215518554640519
31 -0.00172159834004694
32 -0.00139181291474068
33 -0.00114890345348067
34 -0.000973856905712032
35 -0.000849260234269898
36 -0.000760691766135983
37 -0.000697011118986924
38 -0.000650052370254206
39 -0.00061406728269557
40 -0.000585123854422768
41 -0.000560587013671977
42 -0.000538735077550143
43 -0.000518464389275695
44 -0.000499082775817573
45 -0.000480214775534744
46 -0.000461736487581343
47 -0.000443733272905447
48 -0.000426485835378915
49 -0.000410426689222707
50 -0.000396075003345945
51 -0.000384057681902173
52 -0.000375314213293492
53 -0.0003719806999315
54 -0.000377498150915155
55 -0.000395766975705179
56 -0.000432312178938045
57 -0.000497272282099902
58 -0.000607523179614782
59 -0.000755905185601522
60 0.00684632381830149
61 0.163962147710283
62 0.510781788286358
63 0.334894832264725
64 -0.564820587046368
65 -1.22334719767865
66 -1.44390527654988
67 -0.856234655252102
68 3.22838627043703
69 11.0177056768932
70 10.4978254234703
71 5.19894017558548
72 4.65389606501528
73 7.22686736412173
74 11.2090141626549
75 16.14911686639
76 20.4692518581114
77 21.4327044328403
78 18.2257670708194
79 12.8531848459839
80 8.29765258273566
81 6.09842667433346
82 5.71315522096145
83 6.02345446323777
84 6.06926257871435
85 5.27347857608976
86 5.23064474424685
87 6.23103119321725
88 4.28867108313508
89 1.78119561419545
90 -0.0582303310394899
91 -0.206539642624375
92 -0.508108893316843
93 -0.841080520677135
94 -0.74324181920672
95 -0.481149609120618
96 -0.260636921373402
97 0.110443194223313
98 3.13653372316884
99 9.12266738646734
};
\addplot [semithick, color5]
table {%
0 38.5640973820272
1 48.423813015079
2 24.0905197692455
3 -9.59774406108871
4 -31.085521126467
5 -29.6494152609416
6 -13.2496461278981
7 4.34469514264916
8 16.6029392016232
9 20.0552041462542
10 16.0511657155401
11 12.5433291690882
12 9.38369508162217
13 6.68032343952386
14 4.63650083216888
15 3.21532496506673
16 2.24840000397243
17 1.58235010831956
18 1.11226236105119
19 0.775539400293933
20 0.532976681865252
21 0.35949742337711
22 0.232655832509629
23 0.141553561434575
24 0.0828920691482908
25 0.048619717944491
26 0.0291836284798101
27 0.0181147581093454
28 0.0117199507296308
29 0.00794340335448898
30 0.00565418916442765
31 0.00423089883283243
32 0.0033283989647877
33 0.0027505880910746
34 0.00238245048775042
35 0.00215355532697827
36 0.00201870211235891
37 0.00194780374356054
38 0.00192050566096498
39 0.00192286569964073
40 0.00194530920150624
41 0.00198137662897102
42 0.00202678588046252
43 0.00207878478489697
44 0.00213549969982265
45 0.00219516349517363
46 0.00225569605590425
47 0.00231458202869854
48 0.00236889150466789
49 0.00241553358832723
50 0.00245165203665672
51 0.00247547233397403
52 0.00248847810023331
53 0.00250233435915477
54 0.00253846042655814
55 0.0026197385938995
56 0.00277925488129143
57 0.0030882272342658
58 0.00373555306823719
59 0.00553540029315185
60 0.017082047144749
61 0.154538935678406
62 0.47033552804613
63 0.345798961367192
64 -0.875740066564906
65 -1.97899611888137
66 -0.616101879238315
67 3.97167503689183
68 10.9997532517473
69 17.1825911334598
70 17.6689324245731
71 13.2405309042248
72 10.4585658476478
73 9.71070434305415
74 10.9086815082679
75 14.1340549280636
76 17.829066909288
77 19.3312737242376
78 17.5465537981819
79 13.7049883777152
80 9.9541907637015
81 7.66440443376281
82 6.89356156188025
83 7.05016807588957
84 7.33832542795949
85 7.05765315728168
86 7.10872622159234
87 8.85041200693976
88 8.23124945868394
89 7.00186439453894
90 5.68102924723028
91 4.81896853602042
92 3.50410007518747
93 1.21565083248677
94 0.36843577783574
95 0.47524125860133
96 0.660235042158292
97 1.33174221749044
98 3.96887198789288
99 9.44503379702146
};
\addplot [semithick, black]
table {%
0 8.79746842089874
1 9.1556099237498
2 -3.58573727503706
3 -21.6769184540753
4 -33.6808808127472
5 -31.7556072530703
6 -19.8769913619435
7 -7.06627719336845
8 0.901249267843663
9 3.34136471805376
10 3.07231669072934
11 2.65382174952085
12 2.05038200006755
13 1.43289677187641
14 0.952417385403171
15 0.630807120579643
16 0.424519406323209
17 0.289410546603021
18 0.196559923458011
19 0.130745418840258
20 0.0834876318523243
21 0.0499534006228399
22 0.0247230059672647
23 0.00606200508974605
24 -0.00483116106334403
25 -0.00922790651496005
26 -0.00994921380326873
27 -0.00904649011573769
28 -0.00761540742538667
29 -0.00617436889738414
30 -0.00493085100448304
31 -0.00393884643412546
32 -0.00318433005462041
33 -0.00262857727358947
34 -0.00222808811508711
35 -0.00194302327528228
36 -0.00174038739514097
37 -0.00159469238364425
38 -0.00148725541899672
39 -0.00140492510389654
40 -0.00133870540758771
41 -0.00128256754694518
42 -0.00123257248208593
43 -0.00118619515563887
44 -0.00114185194428619
45 -0.0010986838289922
46 -0.00105640733689706
47 -0.00101521776539282
48 -0.000975757337127458
49 -0.000939015601787056
50 -0.000906180366398858
51 -0.000878685925555444
52 -0.000858681735640709
53 -0.000851054987337366
54 -0.00086367836854476
55 -0.000905475629674723
56 -0.000989087433943909
57 -0.0011377097140354
58 -0.00138995284440678
59 -0.00172943617311011
60 0.000723244755708979
61 0.0420816622887486
62 0.131094566752626
63 -0.136160217727959
64 -1.29225354338316
65 -2.79889718477688
66 -3.30351221737259
67 -1.95898005949659
68 0.676896226184906
69 2.82774637906727
70 2.69431664811627
71 1.33433263581649
72 1.19444448166756
73 1.85480975987164
74 2.87684660862161
75 4.14474738055861
76 5.25353050094476
77 5.50080517041668
78 4.6777294975596
79 3.29883080684746
80 2.12963186108683
81 1.56519010872838
82 1.46630836427268
83 1.54594813542888
84 1.55770500536801
85 1.35346326957171
86 1.34246976362343
87 1.59922368696309
88 1.10070775912807
89 0.447155407053803
90 -0.133225228229824
91 -0.472542239343924
92 -1.16250280685907
93 -1.92430890098975
94 -1.70046364542584
95 -1.10082263561774
96 -0.597977848487545
97 0.0283457692296661
98 0.805006245276113
99 2.34137582052313
};


==> plots/all/VastiFalse.tex <==

\definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

%\addplot [semithick, color0]
%table {%
%0 1.85081008758896
%1 1.56442211676079
%2 7.85113026685683
%3 7.66859853777268
%4 2.67032355104249
%5 -4.59067920271834
%6 -13.2783112675103
%7 -24.971979242797
%8 -39.3573885210847
%9 -49.6584876421047
%10 -45.5506764567444
%11 -22.4047631340833
%12 14.290204783053
%13 54.5939696168273
%14 89.0566639268874
%15 115.902450328018
%16 128.88693540241
%17 127.938295819944
%18 118.39582319722
%19 105.732502880201
%20 94.8700795459742
%21 88.602140636828
%22 87.227226715004
%23 88.9982478413729
%24 91.156924889376
%25 91.4476261098003
%26 89.1033691521897
%27 83.6628317247274
%28 76.1568251325388
%29 68.2309216893107
%30 60.7729683727594
%31 54.5283290825125
%32 49.2904842788711
%33 44.344875828461
%34 39.2722122538663
%35 34.2156341131802
%36 29.3878621593102
%37 27.6350622856941
%38 25.2441520301198
%39 21.9194424794676
%40 19.1123361445872
%41 16.342766768558
%42 13.4966882539276
%43 10.7890496408515
%44 8.58176272966102
%45 6.98161980391376
%46 5.96720153568296
%47 5.23590766924128
%48 4.43915329283232
%49 3.28123719662843
%50 1.30848020335613
%51 -1.59655654553022
%52 -4.91083837803685
%53 -8.26343382883494
%54 -12.2602498188259
%55 -16.898702076601
%56 -22.1006435298165
%57 -28.292752799025
%58 -31.6961914403604
%59 -29.4500444879844
%60 -24.913405360231
%61 -20.1974513413109
%62 -15.9401384636987
%63 -12.2013908296357
%64 -9.0678880121246
%65 -6.507138868621
%66 -4.50618035328744
%67 -3.03001991017721
%68 -1.98684946796826
%69 -1.26065089345802
%70 -0.77058162129756
%71 -0.455601801094962
%72 -0.251106251960713
%73 -0.0213139847088711
%74 0.86718970241125
%75 3.30632858922436
%76 6.73338662755004
%77 10.5076763085005
%78 13.6310338465809
%79 15.340332223296
%80 15.3848350176041
%81 15.4670432904143
%82 16.329284695504
%83 17.45017601286
%84 18.750470614528
%85 19.1879850257069
%86 15.2062637571233
%87 9.38231288926775
%88 6.21827125996354
%89 3.79677854541717
%90 2.22565190496472
%91 1.27243560674077
%92 0.807673455787818
%93 1.30801764719885
%94 4.83403379707655
%95 4.29282815709496
%96 4.5359080442086
%97 4.48057665594185
%98 4.30627107286132
%99 5.13484256285415
%};
%\addplot [semithick, color1]
%table {%
%0 0.444288272574138
%1 -0.103848466828666
%2 -2.91367849470787
%3 -7.65545795842927
%4 -14.1659861181226
%5 -22.3809341992475
%6 -33.7089644869539
%7 -49.6017887970871
%8 -67.8514637859866
%9 -80.4669943572251
%10 -77.4765570805985
%11 -55.5946173681939
%12 -20.2772169046166
%13 18.2533689432365
%14 51.6538170160248
%15 79.2465192087199
%16 94.9221906472092
%17 98.1859342517866
%18 93.1207586525788
%19 84.6945410122749
%20 77.1614572473234
%21 72.993131528392
%22 72.5425645826322
%23 74.3928334365674
%24 76.4276470669714
%25 76.9541780649531
%26 75.2332151641358
%27 70.9222491123911
%28 64.8053364982846
%29 58.1195440430498
%30 51.5812914716576
%31 45.7860589989744
%32 40.7821563776856
%33 36.1352043434874
%34 31.5754875518795
%35 27.1904231576135
%36 23.1303552633649
%37 19.5464228128385
%38 16.5199320467606
%39 14.0058488598859
%40 11.801589837275
%41 9.65868108136572
%42 7.50036346276066
%43 5.45489845758643
%44 3.71199696442936
%45 2.28425188513159
%46 1.08622725837016
%47 -0.00839799240973027
%48 -1.14221963077911
%49 -2.47358488564672
%50 -4.19861306893397
%51 -6.29767708965346
%52 -8.50927561064212
%53 -10.9190999162058
%54 -13.88180574431
%55 -17.0559435999998
%56 -21.1001343125676
%57 -25.188494333677
%58 -25.957401853016
%59 -23.5277470699159
%60 -19.7868548131109
%61 -16.1476964068947
%62 -12.7973165535468
%63 -9.81550371798798
%64 -7.29656216918734
%65 -5.22644973869191
%66 -3.60457848119197
%67 -2.40877530982681
%68 -1.56611905988138
%69 -0.981454846874262
%70 -0.588964386335368
%71 -0.339027062759995
%72 -0.178217519663955
%73 -0.0885837770232065
%74 0.102414053896333
%75 1.14425018761877
%76 3.46780813514823
%77 6.64946129990584
%78 9.87434003264262
%79 12.2587084985472
%80 13.3440363266576
%81 13.8727635819025
%82 14.5245531181862
%83 15.3985754420518
%84 16.4893808910392
%85 17.0837617255064
%86 14.7887841867267
%87 10.4269429758914
%88 6.90794896509524
%89 4.24205893008348
%90 2.52897623013878
%91 1.48419974192149
%92 0.936098961113317
%93 1.15368049475902
%94 3.13415137676017
%95 3.48155687199902
%96 3.70472846175187
%97 3.7060591397654
%98 3.61609866545025
%99 4.06193710390472
%};

%\addplot [semithick, color3]
%table {%
%0 6.71377367162963
%1 7.62405814413369
%2 23.1966985430338
%3 28.6496464058224
%4 28.9891953606614
%5 27.659482780154
%6 27.6873091606339
%7 27.8018278741673
%8 25.7108072479676
%9 21.9347932384549
%10 20.5221077788289
%11 25.4180250835169
%12 35.783167693647
%13 48.2376992514261
%14 60.126977611789
%15 79.9834457251918
%16 91.9176993476597
%17 93.9320990526512
%18 89.8884341855356
%19 83.4876335915705
%20 78.0516769994901
%21 75.4874752626864
%22 75.9727387586439
%23 78.2693126153589
%24 80.5636716738514
%25 81.4186245490912
%26 80.2906044543172
%27 76.880379543043
%28 71.853823495976
%29 66.3008928409445
%30 60.8600981019686
%31 56.1093275917064
%32 52.0248404985893
%33 48.1666074472971
%34 44.2379862694975
%35 40.3055490691086
%36 36.4922775018314
%37 33.0043859562622
%38 30.000737115197
%39 27.4660406362573
%40 25.2342131023757
%41 23.0258153408808
%42 20.7586572280724
%43 18.6993937093639
%44 17.3051799824172
%45 16.4704608200461
%46 16.0273127001351
%47 15.8660502743866
%48 15.8958213667235
%49 15.8917755890973
%50 15.3200335174859
%51 13.9720061182285
%52 12.2321688684781
%53 10.4751871169354
%54 8.257155946157
%55 5.23295212313619
%56 2.043082401555
%57 -3.44463340099366
%58 -9.83610668535635
%59 -11.7517873057761
%60 -10.994753515469
%61 -9.03862322741058
%62 -7.12109907704741
%63 -5.33561906157709
%64 -3.78952777688963
%65 -2.50155755698356
%66 -1.49640620499279
%67 -0.776363811210583
%68 -0.296946911739641
%69 0.00886076947433877
%70 0.187147376282048
%71 0.272959250177867
%72 0.306532572183573
%73 0.97489041743493
%74 3.75665325954108
%75 7.50433381647523
%76 11.0248959853177
%77 14.1904792062966
%78 16.4131875973495
%79 17.266460461101
%80 16.7193257894658
%81 16.4967611830728
%82 16.8522357919686
%83 17.5306026938737
%84 18.4837297371656
%85 18.772132974793
%86 15.4388342145905
%87 10.2930127845692
%88 7.52052836050247
%89 5.37147301796104
%90 3.83731393627746
%91 2.79402669205706
%92 2.20459565342823
%93 2.81825481200773
%94 8.18567596674868
%95 6.67452405521978
%96 6.92567333817502
%97 6.82270854532038
%98 6.55061640316479
%99 7.81707347366101
%};
\addplot [semithick, color4]
table {%
0 0.128811599776039
1 0.686834828141457
2 4.21742601399584
3 9.81854457287477
4 16.9901537463137
5 25.6522028193041
6 37.3838448042939
7 53.8342537039005
8 73.3602229369809
9 89.1042067062009
10 92.1799893691356
11 79.2551905363515
12 54.2964629954948
13 25.7862746388159
14 12.2141949611299
15 78.6075460235023
16 125.197325603213
17 137.208392758935
18 127.30228277952
19 110.358456358721
20 98.3901858235452
21 97.7088252746803
22 108.145101234262
23 124.316626353534
24 139.471937328276
25 148.918923274672
26 150.885963530008
27 144.847265170544
28 133.333239099966
29 119.849496579931
30 106.236127521624
31 93.9615172424635
32 83.1573310006996
33 72.6971942349668
34 62.0236628629798
35 51.5942692633633
36 41.9967057714082
37 33.6900613883739
38 26.8395197601258
39 21.2569110398489
40 16.2965667189931
41 11.2444819532247
42 5.92076089450398
43 1.76148803609172
44 0.934788532695229
45 1.8812021250621
46 2.73865464366048
47 3.61223369661886
48 4.60120133204812
49 5.80927013444455
50 7.35080885962562
51 9.15257274592829
52 10.9747062861407
53 12.926161212741
54 15.3088264280609
55 17.7935990555686
56 20.9994204716323
57 24.100303591952
58 24.1566006490978
59 21.5487634786637
60 17.9440862581534
61 14.547348602439
62 11.4809845083701
63 8.78812945478964
64 6.53120891390052
65 4.68681930488095
66 3.24562342917985
67 2.18241811600948
68 1.4310790320017
69 0.908043653234679
70 0.555085113686546
71 0.328242410518445
72 0.181007666032826
73 0.119493547365954
74 0.200345878938158
75 1.47726631031125
76 6.90188118510709
77 14.8284527953066
78 23.1139083501298
79 29.3498351223422
80 32.2927904135011
81 33.6813925733046
82 35.1527365291173
83 37.0146467353709
84 39.299925579695
85 40.4249979314543
86 34.8670613437239
87 24.5732361788471
88 16.5203919516812
89 10.3589281085073
90 6.20227458405126
91 3.57820677072523
92 2.19598609399509
93 2.82941009419342
94 7.7277710065528
95 8.58963835330037
96 9.15872146428898
97 9.1998872339679
98 9.00311497478733
99 10.105773839265
};
\addplot [semithick, color5]
table {%
0 3.12644626243478
1 3.29811332196517
2 7.98224388892865
3 13.5532617450287
4 18.2088442245945
5 22.0074528426451
6 26.0835720502024
7 31.2902305827945
8 38.2300624434559
9 47.5593820183184
10 60.3691006143717
11 78.1763674377162
12 101.174676637323
13 127.687475716872
14 153.776386333659
15 175.603424606111
16 188.76422205162
17 191.086999634007
18 185.127350508619
19 174.786440021282
20 163.784742087971
21 154.653665685597
22 148.482665254935
23 144.975875918888
24 142.69866664911
25 139.854159061779
26 135.289040609443
27 128.121652720996
28 118.84010213213
29 108.762731706413
30 98.8314240568904
31 89.9534755813134
32 82.2862271322322
33 75.317192583776
34 68.603718929365
35 62.1041969908264
36 55.8752343212856
37 50.0916612934368
38 44.9446963710539
39 40.477529182803
40 36.5576536249383
41 32.9190036698135
42 29.4451269024277
43 26.1969161998323
44 23.3474132303374
45 21.0649801155213
46 19.4526673773264
47 18.4170246324621
48 17.7647971720145
49 17.2679537983095
50 16.6054658801358
51 15.5655381624358
52 14.222153708303
53 12.7589322226152
54 11.1507706714828
55 9.41730675868496
56 7.85252357512605
57 6.33294221886319
58 4.82341804018093
59 3.70330268265281
60 2.84006764958264
61 2.1910391974531
62 1.67242533590469
63 1.24747465634105
64 0.906590333243062
65 0.637655220162388
66 0.434625918333535
67 0.290258134026254
68 0.192309546809788
69 0.127506321527396
70 0.0865352171949983
71 0.0620002230470392
72 0.0483419392195717
73 0.0990172464541329
74 0.583739840036337
75 2.16767490839787
76 4.91578397542774
77 8.4550340133122
78 12.0150408222023
79 14.7160646328386
80 16.0486247348289
81 16.8892362261276
82 17.9957158847313
83 19.4374905840315
84 21.2175198150204
85 22.3825447252186
86 19.7217659621951
87 14.1786662721871
88 9.4756087317529
89 5.7513365080271
90 3.39909057611568
91 2.02364190704547
92 1.32325923632265
93 1.61025926928709
94 4.55671000432389
95 5.22809007659543
96 5.7448721851779
97 5.92520940541887
98 5.98677593372704
99 7.03964419964845
};
\addplot [semithick, color2]
table {%
0 1.53790752570507
1 0.664960473346622
2 0.356507483909818
3 -0.631386135558612
4 -2.66056466216296
5 -5.71803567245707
6 -10.3615919225862
7 -17.1481428122156
8 -25.007670418608
9 -30.0042507957643
10 -27.1429621497215
11 -14.7620023485932
12 4.38330288539286
13 29.1122993862514
14 128.599508810766
15 169.025714291966
16 185.367764300223
17 187.414806643468
18 179.552718532003
19 167.102449061692
20 154.822043136537
21 145.700719096405
22 140.516216594683
23 138.127193796296
24 136.414446668871
25 133.447314251915
26 128.299293009652
27 120.409165670369
28 110.513891417693
29 100.010825217469
30 89.8191843805573
31 80.7737608631267
32 72.9783626578425
33 65.8976186797165
34 59.1041570407542
35 52.5829878517318
36 46.4246245156858
37 45.4486158988148
38 42.9850763738833
39 38.3623857257927
40 34.2977827443108
41 30.4751385139348
42 26.7568635592664
43 20.7515774975129
44 12.6650260892686
45 7.23320426665732
46 5.05493462401883
47 3.91566956840659
48 3.11809587032028
49 2.37279989765785
50 1.46592646661894
51 0.332696886387816
52 -0.920658787490984
53 -2.31302524458976
54 -4.02665837489397
55 -5.91699868560855
56 -8.26786363378791
57 -10.7400391192657
58 -11.664664139619
59 -10.886643251198
60 -9.32588602656562
61 -7.70787477142767
62 -6.16216963386908
63 -4.75290476159622
64 -3.54463897538379
65 -2.54123820190141
66 -1.75006927228363
67 -1.16514640551429
68 -0.752831554270485
69 -0.466902033577278
70 -0.275425354779133
71 -0.154250441479646
72 -0.0767697790056722
73 -0.0227418512457294
74 0.46585083908402
75 2.61468201528377
76 6.28002535078247
77 10.8288119023616
78 15.1001768548962
79 17.9993988655042
80 19.0084603854156
81 19.2595461735017
82 19.7772623071477
83 20.6864144167216
84 21.9423207579199
85 22.6181618472236
86 19.5604259044181
87 13.8192028025579
88 9.28463896561325
89 5.89131578763852
90 3.67974165371619
91 2.29581046993199
92 1.5272207847157
93 1.71625213013776
94 4.44677173129427
95 4.93470974780242
96 5.27157414205787
97 5.3227983581911
98 5.22512374873426
99 5.85976152196663
};
\addplot [semithick, black]
table {%
0 -0.154573919731247
1 -0.824201793769748
2 -5.060911216795
3 -11.7822534874497
4 -20.3881844955764
5 -30.782643383165
6 -44.8606137651527
7 -64.6011044446806
8 -88.032267524377
9 -106.925048047441
10 -110.615987242963
11 -95.1062286436217
12 -65.1557555945938
13 -30.943529566579
14 -1.41279148788022
15 19.6518865058756
16 31.2993314008031
17 34.3020981897338
18 31.8255706948799
19 27.5896140896801
20 24.5975464558863
21 24.4272063186701
22 27.0362753085655
23 31.0791565883836
24 34.8679843320691
25 37.2297308186681
26 37.7214908825019
27 36.211816292636
28 33.3333097749914
29 29.9623741449827
30 26.5590318804061
31 23.4903793106159
32 20.7893327501749
33 18.1742985587417
34 15.5059157157449
35 12.8985673158408
36 10.4991764428521
37 8.42251534709348
38 6.70987994003144
39 5.31422775996224
40 4.07414167974829
41 2.81112048830617
42 1.480190223626
43 0.144934264946542
44 -1.12174623923427
45 -2.25744255007451
46 -3.28638557239257
47 -4.33468043594263
48 -5.52144159845774
49 -6.97112416133346
50 -8.82097063155075
51 -10.9830872951139
52 -13.1696475433689
53 -15.5113934552892
54 -18.370591713673
55 -21.3523188666824
56 -25.1993045659588
57 -28.9203643103424
58 -28.9879207789174
59 -25.8585161743964
60 -21.5329035097841
61 -17.4568183229268
62 -13.7771814100441
63 -10.5457553457476
64 -7.83745069668063
65 -5.62418316585714
66 -3.89474811501582
67 -2.61890173921138
68 -1.71729483840205
69 -1.08965238388161
70 -0.666102136423855
71 -0.393890892622134
72 -0.217209199239392
73 -0.143392256839144
74 -0.130350676305429
75 0.369316577577813
76 1.72547029627677
77 3.70711319882664
78 5.77847708753244
79 7.33745878058556
80 8.07319760337529
81 8.42034814332615
82 8.78818413227931
83 9.25366168384273
84 9.82498139492376
85 10.1062494828636
86 8.71676533593098
87 6.14330904471178
88 4.1300979879203
89 2.58973202712682
90 1.55056864601281
91 0.894551692681308
92 0.548996523498773
93 0.707352523548354
94 1.9319427516382
95 2.14740958832509
96 2.28968036607224
97 2.29997180849198
98 2.25077874369683
99 2.52644345981625
};


==> plots/all/VastiTrue.tex <==

\definecolor{color4}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color5}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

%\addplot [semithick, color0]
%table {%
%0 2.69300553645042
%1 2.3392493800586
%2 11.7247938072808
%3 11.9536167366054
%4 5.42395575570474
%5 -4.21382942881617
%6 -14.5685328669269
%7 -27.4494422055018
%8 -41.6574318336661
%9 -47.8934583457213
%10 -33.1264152053021
%11 7.85833870661644
%12 66.1597606442159
%13 128.774567000028
%14 183.096294981507
%15 228.382552642489
%16 250.544505974703
%17 248.240163693166
%18 230.717595341261
%19 206.675427076881
%20 184.755973234873
%21 170.179843396871
%22 163.950287493442
%23 163.602994542819
%24 164.495447567381
%25 162.526903875579
%26 156.469442544344
%27 145.373601935188
%28 131.009866605411
%29 116.355429446469
%30 103.001452265362
%31 92.2622296519506
%32 83.5167609215435
%33 75.3514867845257
%34 66.9066807007606
%35 58.3827910719229
%36 50.124595650663
%37 42.7607617437175
%38 36.7188046736899
%39 31.8707557110217
%40 27.7696104770978
%41 23.7170939056091
%42 19.5452019569822
%43 15.6020420726178
%44 12.4746015316775
%45 10.2678863551382
%46 8.89495513179257
%47 7.93127429113844
%48 6.88568416902402
%49 5.34355383316541
%50 2.66445230747665
%51 -1.32767527023748
%52 -5.90557716255388
%53 -10.525756429322
%54 -16.0312416881948
%55 -22.4539719228426
%56 -29.6137551182036
%57 -38.2357313158881
%58 -43.1807748250731
%59 -40.2394049595067
%60 -34.0809294181029
%61 -27.6296241034495
%62 -21.8057239030893
%63 -16.6912071106465
%64 -12.4046501357853
%65 -8.90160608888271
%66 -6.16434187519174
%67 -4.14498840168654
%68 -2.71795422119396
%69 -1.72452882135022
%70 -1.05412023452438
%71 -0.62322611017174
%72 -0.343460625493191
%73 0.00736605133389853
%74 1.445356459388
%75 5.27820531178729
%76 10.5102825940957
%77 16.0807917354007
%78 20.487627054302
%79 22.679437416908
%80 22.3784402841162
%81 22.1761819772579
%82 23.163579007716
%83 24.5606564762818
%84 26.1915881500659
%85 26.6166167084149
%86 20.8592475169853
%87 12.6788997438755
%88 8.49419421323478
%89 5.29795283519607
%90 3.16248091465156
%91 1.83377869503207
%92 1.17331006894504
%93 1.8799007516697
%94 6.92071773786843
%95 6.07962934351735
%96 6.41064762617349
%97 6.32995119373067
%98 6.07205382399689
%99 7.22024110076048
%};
%\addplot [semithick, color1]
%table {%
%0 1.07107345822998
%1 0.659893533081301
%2 -0.362840323028882
%3 -2.1404823373661
%4 -4.98976275325022
%5 -8.91857985587776
%6 -14.3655768758964
%7 -21.4285843282989
%8 -26.9691785769617
%9 -23.2729663390578
%10 -2.13660500189527
%11 37.5716473088353
%12 88.1741609449376
%13 139.08504448086
%14 182.129495532908
%15 216.951150222551
%16 235.986247255252
%17 237.655567471074
%18 226.73418726052
%19 209.159344035205
%20 190.685314411603
%21 175.260154822981
%22 164.312288429066
%23 157.017217150202
%24 151.186265438238
%25 144.601026257501
%26 136.167163200501
%27 125.19809600957
%28 112.463078027916
%29 99.4906743761763
%30 87.3031052949053
%31 76.7674071021706
%32 67.9020402186883
%33 60.0620599002035
%34 52.7421664850727
%35 45.8821686834911
%36 39.5486584777876
%37 33.9029185355956
%38 29.078718495896
%39 25.0456798772979
%40 21.5823747712836
%41 18.3787663470385
%42 15.31003262477
%43 12.4910792327869
%44 10.1370634123473
%45 8.28451619814947
%46 6.87348388878797
%47 5.77168484337135
%48 4.80122766051646
%49 3.75527166959446
%50 2.34993567416836
%51 0.497954873377527
%52 -1.58567524778084
%53 -3.91862016207698
%54 -6.84553889859071
%55 -10.1180730218552
%56 -14.2545979238623
%57 -18.7400392968762
%58 -20.533022977312
%59 -19.1918685748294
%60 -16.4062285259047
%61 -13.5134522666227
%62 -10.7555807561276
%63 -8.24792382179206
%64 -6.10715392816799
%65 -4.33551794784253
%66 -2.94600000615838
%67 -1.92779531447032
%68 -1.21846005219134
%69 -0.732216800009405
%70 -0.41137323996223
%71 -0.212968760628043
%72 -0.0888732308637186
%73 0.0366015472579295
%74 0.624832156873348
%75 2.71676302533193
%76 6.47208343089653
%77 11.119595859228
%78 15.4685475705233
%79 18.3979246634653
%80 19.3738905949599
%81 19.5606113209965
%82 20.0154443023209
%83 20.8575728556036
%84 22.025010828556
%85 22.5803062822727
%86 19.3819388199163
%87 13.5553269541016
%88 9.00872343440203
%89 5.65282560627615
%90 3.48569136591098
%91 2.14321148253872
%92 1.40614597597833
%93 1.58212827664313
%94 4.07321404864164
%95 4.44890848426531
%96 4.66344894410109
%97 4.60382659499297
%98 4.41497716847926
%99 4.83894655015731
%};
%\addplot [semithick, color3]
%table {%
%0 1.59808868563961
%1 1.53499111824596
%2 17.3073288841629
%3 26.7062119483618
%4 28.9470303651969
%5 29.0437641167794
%6 33.7423422599781
%7 43.3261606187279
%8 56.5099875685078
%9 75.2040995139197
%10 103.783531588528
%11 144.693044115909
%12 191.223905821128
%13 238.467300519098
%14 278.682891376515
%15 308.941828208541
%16 319.981250160451
%17 311.54133422345
%18 293.434093557034
%19 268.467411130557
%20 242.589849700253
%21 220.576490816255
%22 204.390070451837
%23 193.493532216465
%24 185.073789583053
%25 175.924070335465
%26 164.901557839167
%27 150.855427587157
%28 134.761901707508
%29 118.854425032525
%30 104.52842301706
%31 92.9988141716977
%32 83.7386758414045
%33 75.54014062612
%34 67.506807508681
%35 59.5604216349438
%36 51.8055381088
%37 44.7249302843003
%38 38.7379722433464
%39 33.8156240837113
%40 29.6908608050269
%41 25.8442374451622
%42 22.1040951214369
%43 18.6081794611395
%44 15.6726923671034
%45 13.4920377335834
%46 12.1574037806737
%47 11.3794893300731
%48 10.9261365344067
%49 10.3688878602878
%50 8.7918875884245
%51 5.94960059060117
%52 2.58515856227499
%53 -0.787344147164092
%54 -4.79714126931098
%55 -9.56200938117653
%56 -14.7851461421944
%57 -20.9694858573766
%58 -24.9707033409791
%59 -23.7858135724422
%60 -20.4140769130759
%61 -16.7541682134625
%62 -13.3355507067058
%63 -10.2680790472336
%64 -7.662850043
%65 -5.51447348456226
%66 -3.82590018349289
%67 -2.57575184778688
%68 -1.69028497578659
%69 -1.07278195215727
%70 -0.655594931667027
%71 -0.387364334737853
%72 -0.21316931291017
%73 -0.0846065933764375
%74 0.456930180513024
%75 2.48214100952083
%76 5.54557628874476
%77 8.72472112008979
%78 10.9637273249915
%79 11.7710713226253
%80 11.2677060390308
%81 11.139698471977
%82 11.5000047654111
%83 12.1396076907631
%84 13.0337792241829
%85 13.3496840280336
%86 10.5519605761537
%87 6.72139344345068
%88 4.48987928460676
%89 2.8158458791844
%90 1.69334848370387
%91 0.986902161859257
%92 0.615845502000617
%93 0.891089111906821
%94 3.43888107215454
%95 2.85019418345847
%96 3.03269877631928
%97 3.00123603970378
%98 2.87486611156167
%99 3.53925963164076
%};
\addplot [semithick, color4]
table {%
0 -0.0675614569073572
1 -0.360243656042092
2 -2.21203250638883
3 -5.14980931225603
4 -8.91130567570565
5 -13.4545351378951
6 -19.6077606688217
7 -28.2359711243363
8 -38.477307550627
9 -46.7349992711218
10 -48.3482418533082
11 -41.569207659993
12 -28.4783990826143
13 -13.5248555707768
14 7.2815504111117
15 76.5693497550738
16 121.951114078108
17 133.650749144991
18 124.001492323015
19 107.496998326783
20 95.8390502171039
21 95.1753565030202
22 105.341032758208
23 121.093250268729
24 135.855602808331
25 145.057640114579
26 146.973677453387
27 141.091555060036
28 129.876073418826
29 116.741947635085
30 103.481556368594
31 91.5252115249157
32 81.0011644452977
33 70.8122460650974
34 60.415466136373
35 50.2564937900845
36 40.9077832274583
37 32.816519840793
38 26.1436042686901
39 20.7057456753077
40 15.8740169364962
41 10.9529264688362
42 5.76724290072477
43 1.41048105104285
44 -0.490294936783544
45 -0.986687196862632
46 -1.436419530644
47 -1.89461020325605
48 -2.41332198387205
49 -3.04695194015034
50 -3.85548628281376
51 -4.80050826354622
52 -5.75621409182995
53 -6.77974875919986
54 -8.02945246251056
55 -9.33271132343479
56 -11.0141590022979
57 -12.640566730115
58 -12.6700944373012
59 -11.3022884406516
60 -9.41164159578772
61 -7.63005868593216
62 -6.02175612650506
63 -4.60935840008479
64 -3.42560755674674
65 -2.45822845962499
66 -1.7023237645468
67 -1.14467445288291
68 -0.75059842840016
69 -0.476267294674385
70 -0.291141163167395
71 -0.172162565420867
72 -0.0949382016048284
73 -0.0626741548518043
74 0.00867005557946524
75 1.43896262531578
76 6.72292395786563
77 14.4439693877604
78 22.5145933462757
79 28.5888302640114
80 31.4554783709873
81 32.8080757973572
82 34.2412696274883
83 36.054902809124
84 38.2809272046268
85 39.3768278243442
86 33.9630016456817
87 23.9360826125984
88 16.092038658235
89 10.0903339380524
90 6.04145728911621
91 3.48542830279574
92 2.13904689555016
93 2.75604699627767
94 7.52739947957349
95 8.36691967393068
96 8.92124716498305
97 8.96134555726132
98 8.76967535894743
99 9.84374364533663
};
\addplot [semithick, color5]
table {%
0 2.93683488672997
1 2.45140594893445
2 2.80660714788146
3 1.46658833018987
4 -2.76121649640325
5 -9.71329976479023
6 -20.2086914934474
7 -35.3451161093948
8 -51.87125967871
9 -59.5799710111399
10 -46.5597214260309
11 -9.83892136388979
12 43.0286599563731
13 99.9665746813034
14 150.51235569344
15 189.221165365761
16 211.598895599747
17 216.367443005056
18 208.593752193257
19 195.05243041968
20 181.825574168543
21 172.712656428619
22 168.763038989072
23 168.582165462765
24 169.393905055189
25 168.513043493796
26 164.482955546927
27 156.338319939092
28 145.026208287853
29 132.509011864406
30 120.071255877883
31 108.907324754379
32 99.2063369121241
33 90.231850332901
34 81.4212484523104
35 72.8230896297827
36 64.6226128623549
37 57.1050523295149
38 50.5105446743417
39 44.8518341634973
40 39.8589914405053
41 35.1079823874993
42 30.4421902815261
43 25.9824779278113
44 21.9709870848013
45 18.635245473406
46 16.0561601239521
47 14.0226236206707
48 12.2294454592289
49 10.3267218739235
50 7.85039730219049
51 4.66262888515685
52 1.11785780350866
53 -2.7521133759224
54 -7.40232489823414
55 -12.4378345980187
56 -18.5020141132069
57 -24.8176427574224
58 -27.1991000238493
59 -25.1893824882414
60 -21.230548595255
61 -17.1988649583149
62 -13.4486785531453
63 -10.1366089355739
64 -7.39183373835486
65 -5.18515942112855
66 -3.49724005111032
67 -2.28333745589556
68 -1.44828345239029
69 -0.880363606519045
70 -0.50660190269234
71 -0.274417877889158
72 -0.128221406896242
73 -0.00793123097838232
74 0.484801136645481
75 2.37554364065533
76 5.93399231283298
77 10.5906402454869
78 15.2183137773829
79 18.6102473254288
80 20.1323806923331
81 20.9233743320576
82 22.0002429592983
83 23.4974258945724
84 25.421839628939
85 26.6685617827293
86 23.4351143011229
87 16.8330112035055
88 11.3411647453882
89 7.03797026983221
90 4.25723979871765
91 2.5648467402975
92 1.67102843182582
93 2.02261511686977
94 5.60062595880539
95 6.39825889106108
96 7.01925196522152
97 7.25009725254398
98 7.31838634535873
99 8.55023510730944
};
\addplot [semithick, color2]
table {%
0 2.51020742187407
1 0.261111339347359
2 -3.0971276070069
3 -8.16581798060773
4 -14.9315572229121
5 -23.2945783231318
6 -34.7260925782469
7 -50.8072984023092
8 -69.7729048452914
9 -84.4877809071702
10 -85.6872516099865
11 -69.4814892520514
12 -36.6883807944833
13 27.584119435582
14 206.988079610647
15 262.410633859318
16 280.823375007168
17 283.030768389968
18 273.54193291437
19 257.833131610373
20 241.106466260674
21 226.925898752077
22 216.619769498003
23 209.490741138414
24 203.541779993401
25 196.643917147475
26 187.698322703102
27 175.907827861145
28 161.925411917749
29 147.29392409309
30 133.163083250627
31 120.64557656583
32 109.910283970436
33 100.31767348701
34 91.2545375510622
35 82.5653338173214
36 74.2491470722309
37 66.5091021032724
38 59.6013885099615
39 53.5956022717125
40 48.3282303998578
41 43.4446563278823
42 38.767575799612
43 31.439127956425
44 20.0340579943383
45 10.5149551277856
46 5.36318429654645
47 2.16240882549987
48 -0.229964551982915
49 -2.37334747374299
50 -4.6252305897132
51 -6.97734990494825
52 -9.20171462327275
53 -11.4616521299704
54 -14.1310195579575
55 -16.9059243733006
56 -20.4197322822993
57 -23.8795644584111
58 -24.2511313778439
59 -21.8007119232768
60 -18.244069247154
61 -14.8413939144287
62 -11.7400433711316
63 -8.99835334755993
64 -6.69107529168668
65 -4.79997484029711
66 -3.31988360191701
67 -2.22769677312724
68 -1.45639104508021
69 -0.919945945364443
70 -0.558542167680415
71 -0.327006744374606
72 -0.177137795978029
73 -0.101741970550328
74 0.639949937047889
75 3.93020555666966
76 8.72734502200539
77 14.376544177908
78 19.4319335976119
79 22.6509083870102
80 23.4875109311663
81 23.3955146034826
82 23.6866007182674
83 24.503107933153
84 25.7576419297472
85 26.3853116767982
86 22.7345883579601
87 16.028701935541
88 10.8489170340102
89 7.02364410629574
90 4.50030995528252
91 2.89212003705219
92 1.96753262657169
93 2.10822154855156
94 5.29486084169205
95 5.84078906310179
96 6.21687239201086
97 6.27083013067729
98 6.13522054924889
99 6.82294212166867
};
\addplot [semithick, black]
table {%
0 -0.154573919731247
1 -0.824201793769748
2 -5.060911216795
3 -11.7822534874497
4 -20.3881844955764
5 -30.782643383165
6 -44.8606137651527
7 -64.6011044446806
8 -88.032267524377
9 -106.925048047441
10 -110.615987242963
11 -95.1062286436217
12 -65.1557555945938
13 -30.943529566579
14 -1.41279148788022
15 19.6518865058756
16 31.2993314008031
17 34.3020981897338
18 31.8255706948799
19 27.5896140896801
20 24.5975464558863
21 24.4272063186701
22 27.0362753085655
23 31.0791565883836
24 34.8679843320691
25 37.2297308186681
26 37.7214908825019
27 36.211816292636
28 33.3333097749914
29 29.9623741449827
30 26.5590318804061
31 23.4903793106159
32 20.7893327501749
33 18.1742985587417
34 15.5059157157449
35 12.8985673158408
36 10.4991764428521
37 8.42251534709348
38 6.70987994003144
39 5.31422775996224
40 4.07414167974829
41 2.81112048830617
42 1.480190223626
43 0.144934264946542
44 -1.12174623923427
45 -2.25744255007451
46 -3.28638557239257
47 -4.33468043594263
48 -5.52144159845774
49 -6.97112416133346
50 -8.82097063155075
51 -10.9830872951139
52 -13.1696475433689
53 -15.5113934552892
54 -18.370591713673
55 -21.3523188666824
56 -25.1993045659588
57 -28.9203643103424
58 -28.9879207789174
59 -25.8585161743964
60 -21.5329035097841
61 -17.4568183229268
62 -13.7771814100441
63 -10.5457553457476
64 -7.83745069668063
65 -5.62418316585714
66 -3.89474811501582
67 -2.61890173921138
68 -1.71729483840205
69 -1.08965238388161
70 -0.666102136423855
71 -0.393890892622134
72 -0.217209199239392
73 -0.143392256839144
74 -0.130350676305429
75 0.369316577577813
76 1.72547029627677
77 3.70711319882664
78 5.77847708753244
79 7.33745878058556
80 8.07319760337529
81 8.42034814332615
82 8.78818413227931
83 9.25366168384273
84 9.82498139492376
85 10.1062494828636
86 8.71676533593098
87 6.14330904471178
88 4.1300979879203
89 2.58973202712682
90 1.55056864601281
91 0.894551692681308
92 0.548996523498773
93 0.707352523548354
94 1.9319427516382
95 2.14740958832509
96 2.28968036607224
97 2.29997180849198
98 2.25077874369683
99 2.52644345981625
};



==> plots/all/mc.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

%\addplot [semithick, color0]
%table {%
%0 0.162875911549735
%1 0.0993313707303738
%2 0.0524703795957336
%3 0.0306364519613287
%4 0.0310621266925596
%5 0.0826804752318362
%6 0.448127327988214
%7 1.07610926960447
%8 1.18706956051391
%9 1.15270273035786
%10 1.66774831406462
%11 0.16135995996558
%12 0.917051370604231
%13 -1.14360819378424
%14 -6.01650396115252
%15 -12.2400452893168
%16 -17.8910373502011
%17 -19.9948887584923
%18 -17.5908209914798
%19 -11.4217358690489
%20 -3.96474425463239
%21 2.5766847739944
%22 6.71679803636783
%23 7.50464543306329
%24 6.42020041017395
%25 5.56300018643338
%26 5.64400772912744
%27 7.57173694158928
%28 10.6343520600595
%29 13.746232975388
%30 15.1102367383043
%31 14.5137465259371
%32 13.2542143778972
%33 12.1834965348117
%34 11.8803209415749
%35 12.4356104221131
%36 13.2095991183325
%37 13.3413480751382
%38 12.2380256161256
%39 10.011807108327
%40 7.06934355748319
%41 3.75116973902645
%42 0.0704563156336295
%43 -4.42337057253934
%44 -10.0726334965798
%45 -16.4039919685411
%46 -22.0103637295345
%47 -24.6352440645582
%48 -21.9152736706715
%49 -11.9312591115177
%50 6.47897102121832
%51 33.472318106968
%52 68.176738829008
%53 113.397230604181
%54 170.888454681393
%55 230.231778457601
%56 279.601748419577
%57 312.991452005915
%58 326.583466600921
%59 311.08241319926
%60 263.615836086041
%61 204.572267664173
%62 141.085294916529
%63 87.6849331557163
%64 60.769738902595
%65 41.6915947653381
%66 27.5876333664223
%67 16.5287697017793
%68 7.55130041799529
%69 0.525161436713883
%70 -3.84785553073858
%71 -5.20814458773117
%72 -4.74126725757771
%73 -3.73306299201173
%74 -2.77311707423868
%75 -2.02020076651618
%76 -1.44254390058503
%77 -1.01246325359933
%78 -0.703893317865547
%79 -0.48382456263647
%80 -0.327816566280572
%81 -0.21873274161
%82 -0.142130430286434
%83 -0.0886998034318081
%84 -0.0530428758022828
%85 -0.0301331207272159
%86 -0.0159117012012499
%87 -0.00768621876708151
%88 -0.00304192291460934
%89 0.00429500414865356
%90 0.0405427111672761
%91 0.0585175958724339
%92 0.105671025440893
%93 0.214165169244478
%94 0.393936756222457
%95 0.452898296622182
%96 0.953652746713654
%97 1.09792135597462
%98 0.737987109223678
%99 -0.053055744485078
%};
%\addplot [semithick, color1]
%table {%
%0 0.369304749393011
%1 0.252804086814503
%2 0.168524463177678
%3 0.116476778305967
%4 0.0887456815838113
%5 0.0967682920792047
%6 0.267965083226358
%7 0.654039616940589
%8 0.88113804270223
%9 0.945408409810278
%10 1.04675112300595
%11 0.0990068684921315
%12 0.366446454733725
%13 0.842702732806684
%14 0.649477068152957
%15 -0.483251687898722
%16 -1.81257942182571
%17 -1.92922342444257
%18 0.0191566209985015
%19 3.94358744551105
%20 9.0423767028515
%21 14.3387725680531
%22 18.7638429901221
%23 21.3610401874076
%24 22.3785310542896
%25 22.7367383009954
%26 23.1435671930828
%27 24.3226782290668
%28 26.2898955451268
%29 28.5898210829725
%30 30.2886337264502
%31 30.987817792737
%32 31.1195111964425
%33 31.2277126875153
%34 31.7928058303865
%35 33.0326610534663
%36 34.7329142786901
%37 36.4213458590278
%38 37.6468619985299
%39 38.3052999828225
%40 38.5385385302703
%41 38.5338769414343
%42 38.3429588974743
%43 37.7478919735787
%44 36.5385591603744
%45 34.9583817233843
%46 33.8323219810027
%47 34.5212748309569
%48 38.5241025732797
%49 47.141629248265
%50 61.3326471960645
%51 81.4106414088283
%52 107.114856586699
%53 140.284103240299
%54 183.355268166476
%55 231.425301838339
%56 275.328467481108
%57 307.882081961124
%58 324.138856052281
%59 315.576872547069
%60 278.054918517369
%61 225.837018986493
%62 167.54429736124
%63 113.693829562932
%64 76.2685247895206
%65 50.2390837299971
%66 32.1356322828499
%67 19.5088404667325
%68 10.6430965216893
%69 4.44415959650196
%70 0.545561401468557
%71 -1.12985077422258
%72 -1.41254566120708
%73 -1.19480999984996
%74 -0.896564377912207
%75 -0.648113214675124
%76 -0.450772331347163
%77 -0.302688064171115
%78 -0.198748275100696
%79 -0.12654118300694
%80 -0.0769352678784328
%81 -0.0437861767493002
%82 -0.0214504496844309
%83 -0.00664392308352434
%84 0.00213135139451405
%85 0.0066491486254668
%86 0.00844713367381748
%87 0.00847718722067244
%88 0.00764445232989447
%89 0.0085083840272914
%90 0.0226797615311433
%91 0.0408751892148501
%92 0.0739795227713099
%93 0.143053087689911
%94 0.262557340835257
%95 0.353008136290872
%96 0.614713941165204
%97 0.800388858736508
%98 0.763985041360152
%99 0.497338155949409
%};

\addplot [semithick, color3]
table {%
0 0.0904620902970917
1 0.055203317271822
2 0.0279988949591468
3 0.0140924940997747
4 0.00940540952190951
5 0.0197074629348759
6 0.123932893374117
7 0.360467215583509
8 0.430679053729047
9 0.427012832612993
10 0.551562510409437
11 -0.525885487224819
12 0.80749017716736
13 0.701637764295826
14 -1.79711370497333
15 -5.73561095522771
16 -9.84961952000948
17 -11.6271357056909
18 -10.2299394927637
19 -5.85151761238651
20 -0.16269003756819
21 5.08989364823385
22 8.60461853603525
23 9.26193947595607
24 8.16455794243188
25 7.23660322450548
26 7.0433123621137
27 8.36159580385262
28 10.7347456161341
29 13.4591453488619
30 14.9219058739137
31 14.8037934795902
32 14.2419799414032
33 13.9156085859193
34 14.3027126192895
35 15.5552734973359
36 17.1982477126343
37 18.529990509793
38 19.0102452056811
39 18.7076242212975
40 17.939959572711
41 17.0107719052553
42 15.9905248709064
43 14.5465944173449
44 12.3733914174752
45 9.7279742244737
46 7.43960574845302
47 6.99246072582365
48 9.96348685566198
49 17.6359999404096
50 31.1198798370997
51 50.9063425724799
52 76.8666956966286
53 109.643639245625
54 151.675261822555
55 196.142459238788
56 231.642192470439
57 253.005709026601
58 258.660375062743
59 241.47512164667
60 194.485935304634
61 140.266026516645
62 91.2094695969032
63 53.4172860708642
64 36.1098226420567
65 24.445777675202
66 16.1810649206591
67 9.85489587921664
68 4.8341191995743
69 0.813294410937602
70 -2.00184882183088
71 -3.02019304134723
72 -2.82569423967877
73 -2.25204184440217
74 -1.68532310598864
75 -1.23455084847148
76 -0.885211114721233
77 -0.623287241156514
78 -0.434483963710409
79 -0.299314982461287
80 -0.203192902693287
81 -0.135818043009398
82 -0.0883928361287331
83 -0.055245439116269
84 -0.0331052476494625
85 -0.0188907766080656
86 -0.0100921293422654
87 -0.00503500968292392
88 -0.00239459664742046
89 -0.000909138749630374
90 0.00136451506832897
91 0.00463770474665733
92 0.015484998307806
93 0.0453783600162392
94 0.101636943004441
95 0.133399753243269
96 0.289532192790189
97 0.327793111327844
98 0.172754884841177
99 -0.0143668978934503
};
\addplot [semithick, color4]
table {%
0 0.314422271641424
1 0.191230376115578
2 0.0930810889519768
3 0.0435102876527619
4 0.0265736383226743
5 0.0599659882101129
6 0.29745406515808
7 0.868991886798324
8 1.22718060191969
9 1.26758070031711
10 0.0859800297159217
11 -0.969357451456137
12 -2.376331095402
13 -4.13467036719544
14 -6.01008069895498
15 -7.83578679331689
16 -9.1165547048706
17 -9.46737372697453
18 -8.83333893891657
19 -7.65561662493453
20 -6.43753448124128
21 -5.47436608192819
22 -4.96381779694973
23 -4.90860843853397
24 -5.01947312263151
25 -5.07635669857899
26 -4.92650523279951
27 -4.53926195325068
28 -4.0394914821591
29 -3.69369883440176
30 -3.71859371060249
31 -4.07879933886705
32 -4.60964487345361
33 -5.15803595820623
34 -5.62259887104946
35 -6.01850886724692
36 -6.47083887804527
37 -7.12937449400233
38 -8.08006034919282
39 -9.29879308397643
40 -10.7078201572371
41 -12.2550420887065
42 -13.9635534919485
43 -15.9363199061027
44 -18.2323380099279
45 -20.7078304577182
46 -22.9536879949828
47 -24.3692252635757
48 -24.3277282472525
49 -22.2936370055116
50 -17.9709296237919
51 -11.4796518826733
52 0.341607456643975
53 50.5297418939252
54 143.598114235179
55 240.654261902269
56 327.245947269274
57 391.981206675866
58 426.765545491195
59 421.276194596671
60 373.661691070391
61 304.695883799774
62 228.342588234489
63 158.669890657537
64 110.362223250363
65 76.529611962783
66 51.45094886544
67 31.3427396224789
68 14.516410578668
69 2.69183152774105
70 -1.06263483531255
71 -1.43828653464878
72 -1.30936244547456
73 -1.03094710230799
74 -0.765854328671045
75 -0.557930152860557
76 -0.398404814416819
77 -0.279636402432867
78 -0.194428097438512
79 -0.13366464620559
80 -0.0905957224636321
81 -0.0604851272011529
82 -0.0393400037409301
83 -0.0245896321331017
84 -0.0147479180266057
85 -0.00843220256139737
86 -0.00452257869559627
87 -0.00227268861396717
88 -0.00109763912181497
89 -0.000579397757948407
90 -0.00073335240883407
91 0.00162227754229525
92 0.0258646927378186
93 0.100748518748184
94 0.241889482782793
95 0.364017195977901
96 0.589453004690627
97 0.504810072588687
98 0.0563111905757758
99 -0.0177058067739215
};
\addplot [semithick, color5]
table {%
0 0.271478581587819
1 0.180680202997133
2 0.113381245383372
3 0.0745415918138948
4 0.0556829962121872
5 0.0666583637631102
6 0.219035975540044
7 0.593650615118213
8 0.833825017932516
9 0.87602440873431
10 0.602433166072229
11 -1.17925844864215
12 -2.87451375891345
13 -4.97840593773362
14 -7.64531533291528
15 -10.7428354029544
16 -13.1709997517774
17 -13.689931137271
18 -11.8374185331415
19 -8.32310686796021
20 -4.2519727921418
21 -0.479621549458135
22 2.23269184806527
23 3.45010445694897
24 3.71670982066922
25 3.77262144276502
26 4.15813346973959
27 5.23702301206097
28 6.83394909269448
29 8.34680968627609
30 9.02889862237807
31 8.75937183685218
32 7.98317518141032
33 7.17102047824254
34 6.6780488829034
35 6.56554468401046
36 6.54548829966675
37 6.18848246601976
38 5.17943842143821
39 3.51901229581824
40 1.38928845806609
41 -1.05378484960174
42 -3.82692972657177
43 -7.17366361722527
44 -11.263965413099
45 -15.7822368519741
46 -19.7842475665033
47 -21.8320969911177
48 -20.3988048160862
49 -14.169334347594
50 -2.29603646367587
51 15.343359461186
52 38.2561307000575
53 67.9034382771386
54 108.08757101667
55 157.625541898895
56 209.740787800643
57 257.283387022849
58 292.768185985965
59 304.034544577373
60 284.279129763689
61 244.081252059435
62 190.95981060009
63 137.046059960477
64 96.9136039913778
65 66.5786177105193
66 43.0435581845904
67 24.8938469523292
68 11.8861180985545
69 3.61497094689907
70 -0.915184227759001
71 -2.61438341508558
72 -2.65115202547885
73 -2.13195701286522
74 -1.57651462256445
75 -1.13505050693714
76 -0.795487464631372
77 -0.54484311959108
78 -0.368563902687603
79 -0.245434620651865
80 -0.160041772857905
81 -0.101856261445608
82 -0.0619413734215183
83 -0.0348037059078938
84 -0.0174729959333956
85 -0.00703956417838328
86 -0.00114327954017052
87 0.00171913494719837
88 0.00277585292549532
89 0.00394902259797774
90 0.011666945360618
91 0.0229910829462793
92 0.0459686546920702
93 0.0989523903827016
94 0.195712180504915
95 0.274886096456894
96 0.467958906075022
97 0.547698117688585
98 0.445727205902093
99 0.25796535851057
};

\addplot [semithick, color2]
table {%
0 0.38009761312757
1 0.260273505024521
2 0.17329402790057
3 0.119659602011654
4 0.0911589096475677
5 0.0997474768958957
6 0.278420618535114
7 0.684537020901506
8 0.926809797291856
9 0.996553594959473
10 0.207575784388574
11 -2.09156591307881
12 -5.18102257781063
13 -9.01476703620281
14 -13.1177176154125
15 -17.1284731562563
16 -19.9512343540363
17 -20.7216240892538
18 -19.3063016171404
19 -16.6713900622758
20 -13.9290684672406
21 -11.7345974164895
22 -10.5311966731483
23 -10.356311359379
24 -10.5806670318565
25 -10.6996569415055
26 -10.3567889330793
27 -9.45641875500788
28 -8.24580738950556
29 -7.32696692959485
30 -7.30617104677253
31 -8.14521207432267
32 -9.3956106297009
33 -10.6593137347266
34 -11.7009939850154
35 -12.5629101045319
36 -13.5385641087457
37 -14.975367305332
38 -17.0688338229362
39 -19.7586382873484
40 -22.8658606458388
41 -26.2734177797647
42 -30.0334022499368
43 -34.376335357851
44 -39.4350900156725
45 -44.8914064693324
46 -49.8376341715915
47 -52.9392006430422
48 -52.8023394673491
49 -48.2333219779054
50 -38.5418833689349
51 -23.2029768403535
52 37.5853734619525
53 109.92995537917
54 149.222822543953
55 193.007694850316
56 234.09715291581
57 266.857182096603
58 286.88796289847
59 286.152363019243
60 259.965433455833
61 218.327011543691
62 167.489033408749
63 117.461509949733
64 80.8393618656976
65 54.2627319370552
66 35.1733989275137
67 21.5919109504388
68 11.9799413794682
69 4.12155645001111
70 -2.30040081136281
71 -3.15282163285623
72 -2.87824579052294
73 -2.26818795929554
74 -1.68538655332693
75 -1.22790271918159
76 -0.876718713262897
77 -0.615193265875282
78 -0.427580405207789
79 -0.293806420757421
80 -0.199003510050563
81 -0.132743315829982
82 -0.0862232727004304
83 -0.0537816563477521
84 -0.0321526960696192
85 -0.0182898287880868
86 -0.00972016824281896
87 -0.00478288543921203
88 -0.00212598725915108
89 -0.000276298985637004
90 0.00556927648586009
91 0.0326177591812375
92 0.0750771638193872
93 0.145995507043672
94 0.269227195763189
95 0.363273627849288
96 0.632598789970312
97 0.820131342144354
98 0.769683034219944
99 0.0828541652373048
};

\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};
\addlegendentry{Power}


==> plots/all/nomc.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.2941176}
\addplot [semithick, color0]
table {%
0 0.110956780403308
1 0.0674842119863441
2 0.0354793748490442
3 0.020661466558972
4 0.0209488470975886
5 0.0559019043303899
6 0.304759781875483
7 0.737759172743813
8 0.819922335487857
9 0.795112680861952
10 1.12782719376516
11 -0.0714011886823307
12 0.178834894360616
13 -1.55376982699406
14 -5.22527767682475
15 -9.80923000184781
16 -13.9031229181919
17 -15.4120403168524
18 -13.674686521727
19 -9.28232386695612
20 -4.00993470718438
21 0.594718013402374
22 3.30780770399415
23 3.61989068682522
24 2.68090687887742
25 1.93013239968809
26 1.86799384572226
27 3.03394556928349
28 4.91129623842242
29 6.69063739171561
30 7.2288694632805
31 6.45664097247844
32 5.1997276780071
33 4.01812281510584
34 3.27386259029631
35 2.97923617361353
36 2.69636149266947
37 1.87547639881536
38 0.171187511910933
39 -2.3298978912322
40 -5.3590622845305
41 -8.71071060740843
42 -12.4040285842633
43 -16.7394508857207
44 -21.9186498933676
45 -27.5736218695858
46 -32.6457807617975
47 -35.5121462574406
48 -34.4791157129355
49 -28.1756144793213
50 -15.964705781206
51 2.15202432393665
52 25.2970682522354
53 54.6055817809659
54 91.7075741856586
55 131.637083412661
56 167.37909084388
57 194.770934435376
58 210.757939620808
59 208.518824355868
60 185.128374743117
61 151.252746657401
62 110.570603371833
63 72.536045257569
64 49.8542439590192
65 33.2922331605988
66 21.1234549271671
67 12.0783707055405
68 5.29751420474043
69 0.302477449857096
70 -2.81281283267363
71 -3.80719399189721
72 -3.4659045108651
73 -2.72890119796686
74 -2.02717452166314
75 -1.47678737692098
76 -1.05451606643657
77 -0.740124456972026
78 -0.514558771208535
79 -0.353688978577253
80 -0.239648847377606
81 -0.159910719161588
82 -0.103916019922914
83 -0.0648591672203302
84 -0.0387950656659869
85 -0.0220504044058504
86 -0.0116583688767618
87 -0.00565022949820947
88 -0.00227808939182389
89 0.00276526912591953
90 0.0271055768949933
91 0.0393039493810185
92 0.0710842434645972
93 0.144373630297885
94 0.266354346349725
95 0.307328611344092
96 0.645849159983786
97 0.741331275341931
98 0.497665299465117
99 -0.039410437316887
};
\addplot [semithick, color1]
table {%
0 0.127377064397142
1 0.0802534596956334
2 0.043737778049678
3 0.024423741229245
4 0.0167910182543234
5 0.0269592740306842
6 0.113262210799026
7 0.323057173906463
8 0.455272853478321
9 0.470595178315075
10 0.066256550753073
11 -1.96855611625203
12 -4.81512062908778
13 -8.36071473743211
14 -12.2198033607164
15 -16.0782431344775
16 -18.8424694419243
17 -19.5752123069326
18 -18.0743350115404
19 -15.2529050121422
20 -12.226304534302
21 -9.70200851217156
22 -8.19676641036009
23 -7.81523168074721
24 -7.93806018746442
25 -8.0183948529082
26 -7.66959492016732
27 -6.75393733054751
28 -5.52595755240499
29 -4.57954481687714
30 -4.45583706064295
31 -5.12338977284616
32 -6.19973026947099
33 -7.31462385724884
34 -8.21058039560761
35 -8.89639728000635
36 -9.65095865010167
37 -10.8303778321234
38 -12.6574642430615
39 -15.0934126503627
40 -17.9639916885164
41 -21.1429987911093
42 -24.6725567893696
43 -28.786405549156
44 -33.6271628446678
45 -38.8745564873424
46 -43.6038406579671
47 -46.441985166434
48 -45.9484130358624
49 -40.8900542762668
50 -30.5608721637754
51 -15.1754136675911
52 4.07773334904166
53 28.5310618558198
54 59.7087961631151
55 94.1795289998768
56 127.216494993021
57 154.778237183568
58 173.35848954188
59 177.086962229993
60 162.9652401592
61 137.694521871506
62 105.69206987559
63 73.875518056718
64 50.5123762986183
65 33.4429014886889
66 21.0173240030508
67 11.9874022704027
68 5.42706450063104
69 0.750871503863389
70 -2.09885427146879
71 -3.04995977442283
72 -2.82001303257533
73 -2.23010897576939
74 -1.65806653257537
75 -1.20763995056755
76 -0.86122009778057
77 -0.603111712179832
78 -0.41814513241693
79 -0.28642279424065
80 -0.193210934532269
81 -0.128198210308494
82 -0.0826373636525573
83 -0.0509336492068216
84 -0.0298961719239901
85 -0.0165137157630506
86 -0.00833570892828448
87 -0.00373660262008362
88 -0.00142523262203174
89 -0.000274197123981012
90 0.000926088968241898
91 0.00446228980505723
92 0.0150132474532132
93 0.0432686556535669
94 0.09593892011802
95 0.140604300001324
96 0.231570358882961
97 0.225411242115959
98 0.0965244417284369
99 0.0170967493911549
};
\addplot [semithick, color2]
table {%
0 0.278136008734766
1 0.187225446922156
2 0.12013912410662
3 0.0802825228622717
4 0.0603272142528199
5 0.0700166364095522
6 0.213612975511248
7 0.547702080080902
8 0.751303378408097
9 0.798892320025004
10 0.299293025955475
11 -0.697091696082104
12 -1.72581463331866
13 -3.00635616780171
14 -4.53041465914261
15 -6.20121648225143
16 -7.4776567699321
17 -7.79930097970614
18 -6.97309457469461
19 -5.36896911965004
20 -3.53342030053667
21 -1.87821782951009
22 -0.775559695214933
23 -0.363148163571962
24 -0.34483770711673
25 -0.384461103932733
26 -0.239166307639948
27 0.229931052791111
28 0.922263309000323
29 1.53738768270291
30 1.72437952287622
31 1.44916746730183
32 0.935536305835761
33 0.405408531993735
34 0.0142108428395391
35 -0.226537280155338
36 -0.46321450637434
37 -0.897828270213445
38 -1.66867995832832
39 -2.76672420641021
40 -4.1023919691284
41 -5.60491428720659
42 -7.29023885924722
43 -9.28092955807904
44 -11.6570293174025
45 -14.2551308209601
46 -16.5950089697309
47 -17.9557506232534
48 -17.5768442983541
49 -14.8055958016947
50 -9.25605971493158
51 -0.888747779095786
52 25.0615792628556
53 62.9852306302398
54 98.5985017175489
55 138.448865113354
56 176.745441699522
57 208.707301951237
58 230.217617736947
59 233.863516432749
60 215.366166529608
61 182.69184395403
62 140.95793064767
63 99.0201789101198
64 69.3126256428708
65 48.544956986318
66 31.025693463489
67 18.5205173339453
68 9.68094886038752
69 3.33056907405787
70 -0.570872745398135
71 -1.21916418225513
72 -1.20418136932852
73 -0.971629909008445
74 -0.727430215094684
75 -0.531434930891052
76 -0.378722815956253
77 -0.264165591035226
78 -0.182056228348239
79 -0.123627843391962
80 -0.0823537746622947
81 -0.0536872153583025
82 -0.0336642359553092
83 -0.019794760309644
84 -0.0107223610176791
85 -0.00509737548637808
86 -0.00179878964311994
87 -8.80428565424093e-05
88 0.000664230401856331
89 0.00144312835315106
90 0.00628569778546938
91 0.0216174162513833
92 0.0500523221392155
93 0.103962319318782
94 0.19947283513279
95 0.274648324460635
96 0.472087658284316
97 0.576695153360402
98 0.489093696324955
99 0.120872713782842
};
\addplot [semithick, color3]
table {%
0 0.471568034759128
1 0.369075705643232
2 0.293634332756389
3 0.244391589403821
4 0.228114882312837
5 0.290645333840369
6 0.834216081072701
7 1.42702816899155
8 1.43912387390216
9 1.3897134942299
10 2.3117930931151
11 3.58366303441142
12 6.4995557760209
13 6.4823283229076
14 4.27859605237756
15 1.12495182278461
16 -2.24624802535499
17 -3.95593520322919
18 -3.34027371196044
19 -0.74180752961194
20 2.15447263945554
21 4.2760699655926
22 5.34075955458913
23 5.22618066414385
24 4.53758412940177
25 4.0522716504489
26 4.00013480106195
27 4.63789110776887
28 5.6526824240057
29 6.61831054417649
30 6.94581540412329
31 6.61358352569136
32 6.06861767190731
33 5.58487776918756
34 5.34752753403932
35 5.36726632403209
36 5.40452404306785
37 5.16605770682307
38 4.46419842919763
39 3.34659130390463
40 1.95158490780249
41 0.393370082897497
42 -1.33059075052
43 -3.39116699926798
44 -5.92074864137655
45 -8.75346185817931
46 -11.377950380931
47 -12.9456400274412
48 -12.5719378203453
49 -9.56128432479743
50 -3.53802171867033
51 5.15671701319525
52 15.8096046163025
53 33.6173237994492
54 60.4751774045724
55 89.0739095190841
56 114.753248622337
57 133.925714128551
58 144.170727111227
59 141.39920636228
60 123.946147995131
61 99.7865935263604
62 73.1126514929605
63 49.5837029140239
64 35.3068990936127
65 25.2041555827119
66 17.6753876874687
67 11.6611683751418
68 6.66565436105592
69 2.70232099509236
70 0.183373939472553
71 -0.854574836003224
72 -0.952971514739561
73 -0.724888719454065
74 -0.46701549766399
75 -0.267979765786456
76 -0.121071022874961
77 -0.0197824479584024
78 0.0430670132614906
79 0.0794046641780053
80 0.0978851630569111
81 0.104254267867772
82 0.10348784086771
83 0.0984741894014479
84 0.0905473163409767
85 0.0811840462018724
86 0.0715803350616178
87 0.0624032222004974
88 0.0558402170631608
89 0.0750048880681256
90 0.236886956566058
91 0.282878636080424
92 0.378430499732308
93 0.548064014158956
94 0.773334050777019
95 0.794399543663318
96 1.36537573393745
97 1.54775017282422
98 1.3005720774191
99 0.565794899850534
};
\addplot [semithick, color4]
table {%
0 0.322791864733442
1 0.196320729373842
2 0.0955588105046611
3 0.0446684861514533
4 0.0272810008723249
5 0.0615622203028946
6 0.305371982282534
7 0.892123544917826
8 1.25984687023099
9 1.30132237713143
10 0.208253097686255
11 1.8481615079454
12 4.53067509210192
13 7.88309679697022
14 11.4587243237969
15 14.9395865417046
16 17.3814782826609
17 18.0503442535508
18 16.8415036053185
19 14.5960769626694
20 12.2737009102568
21 10.4373393507456
22 9.4639361063311
23 9.35867482118897
24 9.57004766557348
25 9.67850098724806
26 9.39279656464646
27 8.6544846835157
28 7.70163024773279
29 7.04234748227241
30 7.08981165750533
31 7.77657398249064
32 8.78867564036083
33 9.83422936527185
34 10.7199576301613
35 11.4747933354873
36 12.3371985437933
37 13.5927520810305
38 15.4053146203413
39 17.728931079385
40 20.4153596992317
41 23.3652684389799
42 26.6226891217368
43 30.3839342076752
44 34.7614858267001
45 39.4812203769869
46 43.7631366571646
47 46.4619775119449
48 46.3828599602637
49 42.5046939328738
50 34.2630887530665
51 21.8869217978357
52 11.9631493769467
53 51.8747909468724
54 147.42054633789
55 247.060227476739
56 335.956893238074
57 402.415337764826
58 438.125599417424
59 432.49012772463
60 383.60817575167
61 312.806570587017
62 234.420829890602
63 162.893517736578
64 113.299950582825
65 78.5667504526065
66 52.8205194876287
67 32.1770506770354
68 14.9028222951976
69 3.57531244498677
70 2.02600268525962
71 2.74221424381791
72 2.49640962478829
73 1.96558735722443
74 1.46016568894889
75 1.06374076053165
76 0.759592286085206
77 0.533150319750898
78 0.370693519928212
79 0.254842889709287
80 0.172728364330695
81 0.115319982044219
82 0.0750050257799097
83 0.046882201745774
84 0.0281181460751789
85 0.0160767033644435
86 0.00862267664967051
87 0.00433307198450929
88 0.00209274130147357
89 0.001104670555141
90 0.00139819804524141
91 0.00224769587229545
92 0.0265531838950624
93 0.103430339288898
94 0.248328328649409
95 0.373706954254015
96 0.605143629182247
97 0.518247590466356
98 0.0588532571269383
99 0.0337576097419223
};
\addplot [semithick, color5]
table {%
0 0.222094666423344
1 0.150451462964357
2 0.0987375096843169
3 0.0679113929278975
4 0.0517540736184267
5 0.0571691454806312
6 0.173677902270205
7 0.469678104997654
8 0.663258947140197
9 0.693040394998869
10 0.658151881890552
11 0.686319471814839
12 1.63344255641314
13 2.82672117589573
14 3.75880830126681
15 4.2945235130818
16 4.48348472803069
17 4.57873229289601
18 4.83722351572402
19 5.59550307518631
20 6.98632874692758
21 8.78211065913416
22 10.4852535605856
23 11.557868473676
24 11.9915636544666
25 12.1304267591479
26 12.2479144545235
27 12.6570893385811
28 13.4062131307278
29 14.3399310296197
30 15.0558240755141
31 15.3685901316912
32 15.4576449912556
33 15.5447365452005
34 15.8133603986368
35 16.345336734799
36 17.0611174821908
37 17.7862777171773
38 18.3597794334461
39 18.754498288432
40 19.0316936229763
41 19.264787478974
42 19.4849029035882
43 19.6491937206042
44 19.721035932283
45 19.7660834488192
46 19.9365860815027
47 20.4535627512174
48 21.5864189950756
49 23.7205456845124
50 27.5155080384367
51 33.9482526171256
52 44.2056640551019
53 60.5538558566599
54 87.1705278753689
55 125.135387252804
56 169.738945501681
57 213.52572344426
58 247.45525665483
59 259.19978232198
60 243.010590292134
61 208.797063839955
62 163.450669804703
63 117.345375994166
64 82.9495336197372
65 56.9287542473021
66 36.629056969445
67 20.7148411813282
68 9.57877555673151
69 3.62643763405297
70 1.34550562304503
71 0.700070732486365
72 0.480546920586531
73 0.346804440261708
74 0.24909543716923
75 0.178060132169134
76 0.126559474284358
77 0.0896351618317468
78 0.0635211633229613
79 0.0451266810200101
80 0.032232398867255
81 0.0232462933671241
82 0.0170525331644859
83 0.0128674553784838
84 0.0100382926883482
85 0.00808109412561317
86 0.00666756800258369
87 0.00553291417970085
88 0.00459472183699072
89 0.00492428713148725
90 0.01297989772995
91 0.0232965193260032
92 0.0421244709746246
93 0.0832183444791638
94 0.158258433827636
95 0.219204354435965
96 0.376700668489067
97 0.468248938738131
98 0.442320556812438
99 0.289603590950121
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};


==> plots/dl/j/0.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}


\addplot [semithick, color0]
table {%
0 156.804138183594
1 152.784530639648
2 140.793350219727
3 128.980682373047
4 122.82201385498
5 120.579681396484
6 122.344299316406
7 128.6552734375
8 131.312286376953
9 125.354278564453
10 110.94930267334
11 87.7131729125977
12 65.2893218994141
13 54.8084907531738
14 46.1688919067383
15 36.2449188232422
16 26.9297828674316
17 20.6285648345947
18 20.6152439117432
19 20.5226192474365
20 20.3649959564209
21 20.0916728973389
22 19.9048233032227
23 20.1627159118652
24 20.6484832763672
25 21.3031578063965
26 21.8477840423584
27 22.5877742767334
28 23.4450626373291
29 23.9945850372314
30 24.9348030090332
31 25.846263885498
32 26.5626907348633
33 27.1724128723145
34 27.533239364624
35 27.8385162353516
36 27.799467086792
37 27.7969055175781
38 27.6591567993164
39 27.3596038818359
40 26.9958667755127
41 26.5615367889404
42 26.0795078277588
43 25.8663444519043
44 25.9240665435791
45 26.0947456359863
46 26.1939525604248
47 26.2003955841064
48 26.1334629058838
49 25.9791603088379
50 25.7630920410156
51 25.6009063720703
52 25.5761375427246
53 25.7447681427002
54 26.2186012268066
55 30.2195606231689
56 37.8542556762695
57 41.8133811950684
58 49.1618118286133
59 57.7856674194336
60 63.257453918457
61 63.4202308654785
62 60.8575477600098
63 54.9881820678711
64 18.8747043609619
65 -18.8948307037354
66 4.67145538330078
67 67.1896896362305
68 131.18864440918
69 183.69938659668
70 210.369903564453
71 225.877258300781
72 235.690277099609
73 243.81901550293
74 243.765075683594
75 239.54638671875
76 234.587509155273
77 230.159622192383
78 224.658065795898
79 219.230895996094
80 215.280334472656
81 211.282760620117
82 209.3818359375
83 207.949920654297
84 205.74543762207
85 201.90869140625
86 196.605682373047
87 189.945098876953
88 182.032897949219
89 174.397369384766
90 166.274307250977
91 156.803527832031
92 149.143005371094
93 143.221145629883
94 139.282684326172
95 137.1875
96 141.136245727539
97 149.783782958984
98 156.251312255859
99 160.185607910156
};
\addplot [semithick, color1]
table {%
0 243.099716186523
1 239.595611572266
2 241.325500488281
3 168.980865478516
4 253.458984375
5 223.573608398438
6 248.030426025391
7 288.261199951172
8 268.355651855469
9 254.340270996094
10 173.551635742188
11 272.588165283203
12 317.734497070312
13 277.189758300781
14 120.48747253418
15 325.072631835938
16 347.537139892578
17 300.762420654297
18 230.050033569336
19 125.263854980469
20 131.893249511719
21 102.467796325684
22 100.83251953125
23 133.77067565918
24 77.4575119018555
25 70.4216156005859
26 47.8641319274902
27 57.3065147399902
28 43.9138641357422
29 30.8781261444092
30 27.887996673584
31 26.4803237915039
32 26.1163673400879
33 -5.48065900802612
34 26.051212310791
35 25.427225112915
36 -4.46154308319092
37 25.6797580718994
38 25.7186317443848
39 25.6173229217529
40 25.2800350189209
41 25.1360244750977
42 24.998514175415
43 24.2599849700928
44 25.2384605407715
45 24.1126842498779
46 -7.11865329742432
47 25.4064998626709
48 23.5706481933594
49 -7.92748928070068
50 24.9999904632568
51 -8.80693054199219
52 23.3377418518066
53 23.1832332611084
54 23.5421409606934
55 23.971887588501
56 -8.46223449707031
57 23.3201332092285
58 23.0615653991699
59 21.715705871582
60 23.5664005279541
61 25.4868412017822
62 26.1180782318115
63 26.5411586761475
64 27.2293186187744
65 27.7238903045654
66 28.2044448852539
67 28.6751441955566
68 29.0839614868164
69 -1.82023620605469
70 30.2180461883545
71 -1.76075637340546
72 0.898277461528778
73 29.1512546539307
74 0.350160002708435
75 -1.37270879745483
76 35.7848243713379
77 29.5814819335938
78 8.53195858001709
79 39.8180770874023
80 6.08356189727783
81 41.2156295776367
82 5.95000648498535
83 71.3553314208984
84 88.9065475463867
85 121.333633422852
86 85.5966110229492
87 74.2718200683594
88 107.707336425781
89 150.598388671875
90 156.54118347168
91 210.098129272461
92 170.96125793457
93 188.200454711914
94 151.712203979492
95 225.768493652344
96 275.115844726562
97 230.469299316406
98 265.591461181641
99 212.794921875
};

==> plots/dl/j/1.tex <==

\addplot [semithick, color0]
table {%
0 52.4639053344727
1 44.245849609375
2 33.3884544372559
3 24.9012241363525
4 26.4217205047607
5 32.2542266845703
6 39.7336845397949
7 73.8511199951172
8 126.390670776367
9 184.231796264648
10 237.885971069336
11 260.988189697266
12 222.885803222656
13 197.900390625
14 180.245254516602
15 170.231414794922
16 165.853134155273
17 164.765121459961
18 164.413314819336
19 162.85856628418
20 159.672897338867
21 155.612976074219
22 139.15625
23 112.439170837402
24 101.065841674805
25 97.0898056030273
26 93.3897171020508
27 89.5145034790039
28 85.0056991577148
29 79.7132949829102
30 74.4086303710938
31 69.5657348632812
32 65.1640930175781
33 61.2852401733398
34 58.8768844604492
35 56.8098182678223
36 54.6297721862793
37 52.3500213623047
38 50.3179626464844
39 48.5474548339844
40 46.775333404541
41 44.9005737304688
42 42.8903121948242
43 41.1792831420898
44 40.3921928405762
45 39.577564239502
46 38.7749137878418
47 37.9716949462891
48 37.2375564575195
49 36.5491523742676
50 35.6776161193848
51 34.1968421936035
52 32.2012672424316
53 30.851713180542
54 30.0125961303711
55 31.4953384399414
56 33.3756370544434
57 32.9022331237793
58 42.615104675293
59 63.2871513366699
60 92.3904418945312
61 105.441390991211
62 84.0405731201172
63 42.967357635498
64 -10.316029548645
65 -95.0390472412109
66 -178.766479492188
67 -259.240356445312
68 -332.039703369141
69 -388.298065185547
70 -421.057495117188
71 -448.434967041016
72 -460.153289794922
73 -463.787902832031
74 -467.03466796875
75 -472.301910400391
76 -473.194061279297
77 -470.922485351562
78 -462.994384765625
79 -450.637329101562
80 -433.276214599609
81 -410.642486572266
82 -375.359588623047
83 -316.758636474609
84 -260.794647216797
85 -218.790008544922
86 -242.052200317383
87 -274.45703125
88 -301.345520019531
89 -325.122894287109
90 -332.156646728516
91 -318.911529541016
92 -283.859954833984
93 -221.761611938477
94 -132.847503662109
95 -18.7842769622803
96 49.0828475952148
97 41.4159240722656
98 42.0720443725586
99 41.6150169372559
};
\addplot [semithick, color1]
table {%
0 52.8701133728027
1 44.4794006347656
2 28.1364326477051
3 -5.49691724777222
4 23.3334255218506
5 20.3049983978271
6 26.8757381439209
7 45.0032997131348
8 14.0875473022461
9 -23.085865020752
10 37.685977935791
11 154.151611328125
12 118.6728515625
13 53.0122985839844
14 14.1375169754028
15 65.958740234375
16 150.744705200195
17 107.852317810059
18 109.232307434082
19 44.9705848693848
20 92.7600402832031
21 62.0229377746582
22 34.6909332275391
23 67.2911834716797
24 93.4412384033203
25 30.5813407897949
26 32.6380767822266
27 41.7227363586426
28 -9.4569730758667
29 26.0380744934082
30 21.490047454834
31 -8.52042293548584
32 23.4893131256104
33 23.5953559875488
34 23.6172714233398
35 -8.22374057769775
36 22.8852272033691
37 -8.09407806396484
38 22.9406394958496
39 23.4187927246094
40 -7.72276020050049
41 22.2834053039551
42 22.3029861450195
43 -8.4148006439209
44 22.251256942749
45 23.8434791564941
46 22.1348285675049
47 -9.78557968139648
48 23.2227973937988
49 22.8834705352783
50 23.4064884185791
51 23.2665576934814
52 22.7822608947754
53 20.9604034423828
54 21.4233016967773
55 22.9087257385254
56 21.9685974121094
57 23.1279106140137
58 19.9084377288818
59 10.1247367858887
60 19.3268604278564
61 14.7474422454834
62 8.83895778656006
63 29.8444023132324
64 47.3590507507324
65 45.0563049316406
66 34.9716300964355
67 29.951488494873
68 9.14027214050293
69 -40.9584808349609
70 -31.8447742462158
71 -91.8312377929688
72 -85.8161773681641
73 -149.651977539062
74 -138.069061279297
75 -160.969985961914
76 -53.7557258605957
77 -114.751564025879
78 -33.113037109375
79 -72.2034072875977
80 -90.0143890380859
81 -48.942741394043
82 3.44061255455017
83 7.11695575714111
84 -53.0967254638672
85 -15.4179725646973
86 -8.2564172744751
87 -55.0831680297852
88 -55.4653511047363
89 -20.6841983795166
90 -23.8420333862305
91 -10.2262134552002
92 -28.7219219207764
93 -32.4624862670898
94 5.41793727874756
95 12.9358081817627
96 -8.16576480865479
97 24.445728302002
98 27.5085926055908
99 12.6705169677734
};

==> plots/dl/j/2.tex <==

\addplot [semithick, color0]
table {%
0 26.9997425079346
1 26.6522464752197
2 24.5316410064697
3 21.9716167449951
4 21.346305847168
5 23.9128093719482
6 28.7973937988281
7 49.63525390625
8 52.7316284179688
9 27.9594306945801
10 -30.8553161621094
11 -13.5931444168091
12 17.514533996582
13 35.2545585632324
14 42.1146049499512
15 48.0582580566406
16 49.701961517334
17 52.0574684143066
18 54.9251670837402
19 56.270450592041
20 55.3108291625977
21 55.3890228271484
22 57.4305953979492
23 59.0051422119141
24 60.0460662841797
25 59.2062835693359
26 59.1797332763672
27 60.005126953125
28 61.5635147094727
29 63.7652397155762
30 66.1598815917969
31 69.3042221069336
32 73.2704696655273
33 76.3967132568359
34 79.3541107177734
35 83.9579696655273
36 87.7831573486328
37 91.2147598266602
38 94.4065856933594
39 98.7025909423828
40 103.876258850098
41 112.44172668457
42 125.170066833496
43 139.115737915039
44 153.133056640625
45 163.99626159668
46 168.7578125
47 172.694580078125
48 168.13996887207
49 150.726669311523
50 136.761138916016
51 140.447067260742
52 176.655685424805
53 279.162292480469
54 445.851043701172
55 623.115295410156
56 757.477966308594
57 800.522216796875
58 813.3916015625
59 776.580383300781
60 721.50634765625
61 703.529235839844
62 643.04638671875
63 507.123748779297
64 265.229888916016
65 41.1088066101074
66 14.3478422164917
67 23.1520404815674
68 41.5673027038574
69 51.9717102050781
70 57.0447311401367
71 58.5784034729004
72 58.4485130310059
73 57.388557434082
74 56.2156219482422
75 54.5147171020508
76 52.8425025939941
77 51.3481559753418
78 50.0183410644531
79 48.807804107666
80 47.8170585632324
81 47.0257682800293
82 46.638069152832
83 46.5780639648438
84 46.7517585754395
85 46.1618118286133
86 45.6399002075195
87 43.432201385498
88 38.8872451782227
89 35.9778022766113
90 35.2101860046387
91 34.3188629150391
92 33.6499252319336
93 33.5490417480469
94 34.0071296691895
95 35.1233444213867
96 38.4284591674805
97 40.1230926513672
98 38.7078971862793
99 37.4832649230957
};
\addplot [semithick, color1]
table {%
0 -4.44107818603516
1 26.8444919586182
2 25.9056262969971
3 25.2074298858643
4 -5.68480920791626
5 25.76686668396
6 -5.59083414077759
7 25.7262325286865
8 26.337984085083
9 27.2122020721436
10 27.7836017608643
11 -3.31552314758301
12 28.0453243255615
13 28.0585250854492
14 28.0031414031982
15 28.154935836792
16 28.9351902008057
17 30.8037490844727
18 30.7969398498535
19 31.1071834564209
20 31.9512214660645
21 0.982203602790833
22 32.2544174194336
23 31.4403305053711
24 33.0496063232422
25 33.213508605957
26 33.3133888244629
27 2.22531199455261
28 33.827220916748
29 2.12188482284546
30 33.1012878417969
31 3.19451427459717
32 3.70879316329956
33 3.99575090408325
34 35.8426742553711
35 36.1936798095703
36 5.49537754058838
37 36.685417175293
38 37.3823471069336
39 6.74898386001587
40 38.393627166748
41 41.785472869873
42 11.4366855621338
43 13.8978261947632
44 43.9141464233398
45 44.8098831176758
46 53.9860420227051
47 53.8288536071777
48 64.5591888427734
49 69.4685974121094
50 80.8115158081055
51 94.2196731567383
52 100.853469848633
53 123.756874084473
54 130.040451049805
55 138.552505493164
56 285.665618896484
57 311.875335693359
58 404.036010742188
59 310.271331787109
60 397.086944580078
61 412.882080078125
62 292.522216796875
63 264.867156982422
64 269.771453857422
65 219.151260375977
66 137.704208374023
67 83.6328048706055
68 42.1549072265625
69 35.6997528076172
70 32.4821014404297
71 25.9013061523438
72 32.9512329101562
73 26.4476737976074
74 -4.4037766456604
75 26.39670753479
76 26.5193881988525
77 26.6363945007324
78 -4.51313400268555
79 -3.97227811813354
80 27.0219650268555
81 27.7488193511963
82 27.8866233825684
83 27.6994876861572
84 -3.66026949882507
85 27.6503944396973
86 27.3172798156738
87 27.283805847168
88 27.2131977081299
89 27.1837348937988
90 27.1463165283203
91 26.9585990905762
92 26.9401779174805
93 26.7743282318115
94 -4.75583410263062
95 26.6351661682129
96 -4.76037359237671
97 26.8526763916016
98 26.8048858642578
99 26.9386196136475
};

==> plots/dl/j/fc.tex <==
\addplot [semithick, color0]
table {%
0 26.6744117736816
1 26.688835144043
2 26.6551666259766
3 26.3724746704102
4 26.4281826019287
5 26.4183883666992
6 25.5133152008057
7 25.5133152008057
8 26.7286415100098
9 26.2372226715088
10 26.1126308441162
11 26.8012714385986
12 26.9593353271484
13 26.1626319885254
14 26.0356330871582
15 26.0328559875488
16 26.031587600708
17 26.0311717987061
18 26.0307159423828
19 26.0325012207031
20 26.0780506134033
21 26.145715713501
22 26.2200260162354
23 26.2658596038818
24 26.2929916381836
25 26.2799415588379
26 26.2521724700928
27 26.2180671691895
28 26.1611499786377
29 26.0942497253418
30 26.0306091308594
31 26.0324897766113
32 26.0346279144287
33 26.0369815826416
34 26.0584754943848
35 26.5192070007324
36 29.1719512939453
37 34.4570159912109
38 39.9966278076172
39 45.7346687316895
40 51.762149810791
41 60.9597473144531
42 70.3410110473633
43 79.8999099731445
44 89.6416015625
45 99.5549240112305
46 109.096084594727
47 118.060699462891
48 126.041084289551
49 132.753616333008
50 137.973602294922
51 140.632019042969
52 142.511856079102
53 149.822463989258
54 261.51513671875
55 403.787567138672
56 544.5859375
57 636.909729003906
58 640.824462890625
59 584.941223144531
60 415.587066650391
61 201.327682495117
62 173.866363525391
63 133.485168457031
64 85.1954650878906
65 35.2984657287598
66 25.5133152008057
67 25.5133152008057
68 25.5133152008057
69 25.5133152008057
70 25.5133152008057
71 25.5133152008057
72 25.5553359985352
73 26.4247798919678
74 26.6399364471436
75 26.5391330718994
76 26.4667453765869
77 26.4092311859131
78 26.3715000152588
79 26.3570404052734
80 26.3605651855469
81 26.391752243042
82 26.4603614807129
83 26.5533599853516
84 26.617712020874
85 26.6335563659668
86 26.6530990600586
87 26.6601715087891
88 26.6531505584717
89 26.6497039794922
90 26.6491298675537
91 26.6521377563477
92 26.6579933166504
93 26.6660404205322
94 26.6760101318359
95 26.6852264404297
96 26.6905136108398
97 26.6903018951416
98 26.6855525970459
99 26.6804485321045
};

==> plots/dl/j/lstm.tex <==

\addplot [semithick, color1]
table {%
0 4.46003437042236
1 4.39580774307251
2 4.15371990203857
3 3.87673282623291
4 3.46857690811157
5 2.9334409236908
6 2.23297214508057
7 1.44598567485809
8 0.656649708747864
9 0.380734175443649
10 1.21412646770477
11 2.1085376739502
12 2.7841784954071
13 3.24844908714294
14 3.49751758575439
15 3.49807667732239
16 3.50140333175659
17 4.1433629989624
18 5.13242864608765
19 6.13324022293091
20 7.11292552947998
21 8.06491851806641
22 8.8666410446167
23 9.6011381149292
24 10.3190755844116
25 10.9384880065918
26 11.5888004302979
27 12.2246751785278
28 12.8219175338745
29 13.3591337203979
30 13.854621887207
31 14.3194017410278
32 14.8163003921509
33 15.3162879943848
34 15.8610715866089
35 16.661979675293
36 17.5735836029053
37 18.7090950012207
38 20.0470123291016
39 21.5987205505371
40 23.3846778869629
41 25.4359531402588
42 27.8173923492432
43 30.6278781890869
44 33.8528709411621
45 37.4805221557617
46 41.5272331237793
47 46.0752944946289
48 51.1985092163086
49 56.7659873962402
50 62.7552299499512
51 69.2226104736328
52 76.1936340332031
53 83.4510726928711
54 90.9081344604492
55 98.4480209350586
56 105.905303955078
57 113.293975830078
58 120.552772521973
59 127.494705200195
60 134.023788452148
61 139.723251342773
62 144.394714355469
63 147.749771118164
64 149.421752929688
65 148.734527587891
66 145.799072265625
67 140.505554199219
68 132.707015991211
69 122.921653747559
70 111.478286743164
71 99.6704940795898
72 87.4070663452148
73 74.9675369262695
74 62.6378631591797
75 50.9577369689941
76 40.1704368591309
77 30.7022857666016
78 22.9109115600586
79 16.9544849395752
80 12.7671356201172
81 9.88352966308594
82 8.02287864685059
83 6.7566065788269
84 5.78765344619751
85 5.13165092468262
86 4.56285667419434
87 3.97252368927002
88 3.35352087020874
89 2.70130634307861
90 2.03252625465393
91 1.73129034042358
92 1.93004620075226
93 2.41646289825439
94 2.86847352981567
95 3.28408074378967
96 3.65632963180542
97 3.97165369987488
98 4.21126508712769
99 4.38706684112549
};

==> plots/dl/j/main.tex <==
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019807843137}
\definecolor{color2}{rgb}{0.172549019807843,0.627450980392157,0.172549019807843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\begin{groupplot}[group style={group size=4 by 2,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.45]
\nextgroupplot[
title = {\footnotesize Hip},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
xlabel={Gait Cycle in \si{\percent}},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize MEE in \si{W}},
ymin=-100,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/j/0}

\nextgroupplot[
title = {\footnotesize Knee},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
xlabel={Gait Cycle in \si{\percent}},
ymin=-100,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/j/1}

\nextgroupplot[
title = {\footnotesize Ankle},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
xlabel={Gait Cycle in \si{\percent}},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/j/2}


\end{groupplot}

\end{tikzpicture}

==> plots/dl/m/Gastrocnemius.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 60.6323661804199
1 56.6415367126465
2 51.2785186767578
3 46.0611000061035
4 40.6863632202148
5 37.7837181091309
6 36.743537902832
7 35.8961334228516
8 34.591495513916
9 27.2490921020508
10 21.8466987609863
11 20.4291534423828
12 19.1368618011475
13 20.5660133361816
14 28.63818359375
15 31.4416198730469
16 32.3803062438965
17 32.7056617736816
18 32.7986717224121
19 42.2186279296875
20 55.412654876709
21 69.1644134521484
22 76.2449951171875
23 77.4560852050781
24 76.1661911010742
25 72.5930633544922
26 73.6043014526367
27 81.7550430297852
28 87.5750427246094
29 93.1170349121094
30 96.8085250854492
31 100.279876708984
32 99.2000350952148
33 96.5188980102539
34 95.8490524291992
35 95.8139343261719
36 95.3891220092773
37 94.2678833007812
38 95.3525924682617
39 98.5308151245117
40 103.547882080078
41 109.474960327148
42 116.805305480957
43 123.945198059082
44 131.657730102539
45 139.196594238281
46 146.066482543945
47 153.325057983398
48 161.802597045898
49 170.626510620117
50 173.165756225586
51 173.087203979492
52 183.150817871094
53 242.924209594727
54 294.297058105469
55 340.299377441406
56 372.678527832031
57 383.287109375
58 354.935638427734
59 298.607604980469
60 183.34065246582
61 21.0428867340088
62 -101.390563964844
63 -193.313827514648
64 -213.378936767578
65 -168.090850830078
66 -55.0625915527344
67 54.5602722167969
68 22.303165435791
69 9.07088947296143
70 4.05713558197021
71 0.941595315933228
72 10.3562602996826
73 17.8382339477539
74 23.5036544799805
75 27.6916027069092
76 30.5023345947266
77 32.8504943847656
78 34.6896018981934
79 36.0324096679688
80 37.1310501098633
81 37.6512870788574
82 37.4841232299805
83 37.4024047851562
84 37.6929893493652
85 32.1798858642578
86 26.9700527191162
87 29.200065612793
88 31.6061973571777
89 32.9456520080566
90 31.5730895996094
91 29.3959083557129
92 27.7329616546631
93 23.7314128875732
94 24.04128074646
95 25.1133804321289
96 26.382532119751
97 27.5285987854004
98 38.0027236938477
99 51.7805709838867
};
\addplot [semithick, color1]
table {%
0 5.44756269454956
1 10.7198257446289
2 20.2868671417236
3 16.8201007843018
4 8.70940399169922
5 4.39435958862305
6 3.32017850875854
7 3.35982131958008
8 3.49956274032593
9 3.61064147949219
10 3.70813345909119
11 3.80866456031799
12 4.25853633880615
13 5.26407814025879
14 5.56746006011963
15 5.59759569168091
16 5.54985380172729
17 5.4778790473938
18 5.39906454086304
19 5.23303508758545
20 4.86174821853638
21 4.52651739120483
22 4.28549289703369
23 4.11703824996948
24 3.96939444541931
25 3.67365479469299
26 3.43981695175171
27 3.79582524299622
28 4.63841581344604
29 5.62048721313477
30 6.19532251358032
31 6.67184448242188
32 7.31681442260742
33 8.07809448242188
34 9.20865345001221
35 11.1476411819458
36 14.2123489379883
37 17.4959049224854
38 20.755708694458
39 23.5849208831787
40 26.2343883514404
41 28.9995880126953
42 31.6649227142334
43 34.1878128051758
44 35.8185577392578
45 36.3921356201172
46 36.1598892211914
47 35.8973579406738
48 35.6268882751465
49 36.8173828125
50 41.9576187133789
51 53.2135467529297
52 95.6760787963867
53 209.372207641602
54 254.638626098633
55 314.137298583984
56 334.876678466797
57 318.072845458984
58 259.341918945312
59 204.764984130859
60 102.483703613281
61 24.5230846405029
62 -25.570987701416
63 -121.989570617676
64 -137.120452880859
65 -112.058326721191
66 -34.982982635498
67 69.9934997558594
68 90.2384414672852
69 12.289927482605
70 5.90137243270874
71 6.18760776519775
72 5.22119522094727
73 4.65139627456665
74 4.31192207336426
75 4.28212547302246
76 4.265061378479
77 4.25541639328003
78 4.25460195541382
79 4.27542304992676
80 4.30191326141357
81 4.35135269165039
82 4.43812990188599
83 4.64703798294067
84 4.8633599281311
85 6.07077121734619
86 6.48827314376831
87 6.52242803573608
88 6.54711198806763
89 6.48999452590942
90 6.26857805252075
91 6.07148551940918
92 5.89577960968018
93 5.71536827087402
94 5.57872772216797
95 5.4531717300415
96 5.1438102722168
97 4.95763063430786
98 4.3883490562439
99 4.02868843078613
};
\addplot [semithick, color2]
table {%
0 14.2596940994263
1 19.9682235717773
2 17.4881706237793
3 16.4026374816895
4 13.4501876831055
5 10.6693592071533
6 15.7649936676025
7 17.6748104095459
8 14.9445133209229
9 17.4884967803955
10 17.8264331817627
11 18.5872592926025
12 11.2527523040771
13 16.7163276672363
14 15.6451759338379
15 19.7691402435303
16 13.2981796264648
17 19.9463806152344
18 11.5650262832642
19 18.1242942810059
20 22.2234573364258
21 19.6796760559082
22 17.7893180847168
23 15.2675342559814
24 19.1379089355469
25 14.8495721817017
26 14.6818132400513
27 15.7965211868286
28 15.1808576583862
29 15.5241088867188
30 16.3520755767822
31 14.4408750534058
32 13.9351758956909
33 15.4576864242554
34 12.7650022506714
35 10.2240781784058
36 10.1882305145264
37 12.2425384521484
38 13.0784873962402
39 13.5636940002441
40 13.5689926147461
41 12.8921957015991
42 10.3092041015625
43 13.3588600158691
44 12.9407405853271
45 18.49680519104
46 12.9633140563965
47 13.0837917327881
48 12.8525648117065
49 13.8663501739502
50 12.6060743331909
51 13.8578433990479
52 18.0443096160889
53 17.2637271881104
54 15.8712148666382
55 29.1175270080566
56 35.1860656738281
57 48.218189239502
58 102.473236083984
59 82.157470703125
60 96.8014907836914
61 107.142425537109
62 110.033782958984
63 36.7233467102051
64 -63.4208030700684
65 -94.2967376708984
66 -115.431716918945
67 -166.174819946289
68 -83.4344329833984
69 16.4915771484375
70 -127.067291259766
71 -111.854621887207
72 -21.9714412689209
73 -59.4545440673828
74 -29.263111114502
75 20.4834632873535
76 -2.16373610496521
77 21.3172817230225
78 26.0104866027832
79 13.561710357666
80 24.1903018951416
81 24.3890533447266
82 26.4609603881836
83 25.9287242889404
84 24.093391418457
85 15.5496387481689
86 13.6275272369385
87 18.237232208252
88 19.8470821380615
89 17.9572010040283
90 15.967827796936
91 12.6683320999146
92 15.2606058120728
93 19.3811264038086
94 14.0901355743408
95 16.6483707427979
96 16.3935527801514
97 15.7262058258057
98 17.7102680206299
99 18.6933002471924
};
\addplot [semithick, color3]
table {%
0 24.652156829834
1 26.8726863861084
2 21.1691188812256
3 24.1860485076904
4 22.9163131713867
5 -14.9506168365479
6 22.0308723449707
7 23.0614223480225
8 -12.8056612014771
9 25.3596134185791
10 23.4804973602295
11 26.6044044494629
12 -12.5083341598511
13 -11.2886524200439
14 24.6032066345215
15 22.8157939910889
16 23.1081638336182
17 29.5281887054443
18 21.9565696716309
19 26.8383407592773
20 -11.0748167037964
21 25.5430755615234
22 26.9271011352539
23 29.2724075317383
24 23.4643802642822
25 -11.5370388031006
26 23.458553314209
27 24.9876117706299
28 24.226713180542
29 -12.4754886627197
30 -14.6492643356323
31 22.0735015869141
32 24.4996128082275
33 22.2510375976562
34 22.4485969543457
35 22.6634559631348
36 22.4669971466064
37 -13.9286785125732
38 23.029167175293
39 -14.0842514038086
40 23.2068195343018
41 23.4419059753418
42 -11.2375221252441
43 -12.8965330123901
44 24.299108505249
45 24.1202011108398
46 -13.2705945968628
47 -11.0693826675415
48 25.7070236206055
49 23.1800003051758
50 23.4041938781738
51 25.6630306243896
52 25.9259452819824
53 30.9534816741943
54 34.7314682006836
55 41.8402366638184
56 63.3113441467285
57 131.912612915039
58 143.076202392578
59 62.0762825012207
60 183.847015380859
61 216.928359985352
62 114.150260925293
63 124.373435974121
64 37.4393005371094
65 -12.8221063613892
66 12.9793004989624
67 -64.1929244995117
68 -32.3727569580078
69 59.0683326721191
70 36.1582527160645
71 -93.4828948974609
72 29.1668529510498
73 -23.3870811462402
74 22.3230075836182
75 19.601770401001
76 38.0644035339355
77 40.9799156188965
78 37.9849853515625
79 24.7718601226807
80 29.0453433990479
81 37.4317398071289
82 76.4420166015625
83 -4.95967435836792
84 51.5258979797363
85 -0.375422984361649
86 -1.85570693016052
87 34.4843940734863
88 -4.14550590515137
89 31.6259613037109
90 29.2003517150879
91 28.3890724182129
92 30.3262939453125
93 30.6714115142822
94 22.2268810272217
95 22.514310836792
96 21.9052734375
97 25.5900535583496
98 24.3369827270508
99 25.4808540344238
};
\addplot [semithick, black]
table {%
0 1.60428182426596
1 1.31886564014862
2 1.07005919481706
3 0.746190576233121
4 0.484480716847473
5 0.313126773552802
6 0.20209497664241
7 0.130626145419529
8 0.084775728823891
9 0.0553797457639523
10 0.0364988869647465
11 0.024305453885247
12 0.0112540940898943
13 -0.00296737181586344
14 -0.00907604537839752
15 -0.00810476587202217
16 -0.00596609301237249
17 -0.00419594807813071
18 -0.00294753522040395
19 -0.0020181518335789
20 -0.00132655826070129
21 -0.000936059574635552
22 -0.000810061166204007
23 -0.000825303542959739
24 -0.000196972332970264
25 0.0187238187959437
26 0.274135924105149
27 0.962683376506946
28 1.86880054316162
29 2.75916307885887
30 3.28322531582964
31 3.3967615231752
32 3.27960105233965
33 3.1843301754431
34 3.31169501599964
35 3.65483487961174
36 4.01845821075806
37 4.18518744482879
38 4.03622084120403
39 3.639090392806
40 3.11057415399899
41 2.5373380435307
42 1.88372463639367
43 1.03254601130528
44 -0.0625240261804354
45 -1.27511127867516
46 -2.24111565339786
47 -2.46941976056092
48 -1.55967272479002
49 0.902236048081438
50 5.10386856379369
51 11.0885392884815
52 21.9539229415514
53 39.3616936675908
54 54.6269232699768
55 71.0921986348105
56 86.7087941164458
57 98.5487227523976
58 104.61921034631
59 106.187420255415
60 96.9558548042194
61 84.7783270941233
62 71.0112875434252
63 49.3102148591214
64 33.4198633830589
65 22.0099947584132
66 14.0385542539668
67 8.60468109308154
68 4.94993584879746
69 2.53163685812154
70 0.999234999509869
71 0.116487376371921
72 -0.297445653240986
73 -0.409692534639694
74 -0.405225224806352
75 -0.359267936460651
76 -0.300090109592255
77 -0.243702686273325
78 -0.192762256843325
79 -0.148738672809835
80 -0.113346551305285
81 -0.0845460054170611
82 -0.0613239650447634
83 -0.0438737081945733
84 -0.0311891858153112
85 -0.0168858429320758
86 -0.691141061883476
87 -1.39228033306388
88 -2.12261202484492
89 -2.59722082007809
90 -2.60194900898487
91 -2.65234345257158
92 -2.47479116381102
93 -1.67630876820262
94 -0.759029628869384
95 -0.460357319434518
96 -0.247279483330563
97 -0.105282703751684
98 0.336450852583659
99 0.582878305465145
};



==> plots/dl/m/Gluteals.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 -0.797882199287415
1 -5.39846706390381
2 -5.20062685012817
3 0.0874634683132172
4 17.4616298675537
5 15.0735807418823
6 -3.63036465644836
7 -14.9942111968994
8 -19.996919631958
9 -19.825325012207
10 -14.8695726394653
11 -4.34711837768555
12 57.8179702758789
13 135.884216308594
14 165.330749511719
15 176.219680786133
16 167.476043701172
17 148.212677001953
18 124.305381774902
19 105.781829833984
20 91.2327423095703
21 81.1185684204102
22 72.7591094970703
23 65.4459838867188
24 60.4884071350098
25 57.1400718688965
26 53.5585479736328
27 50.5939598083496
28 48.2663078308105
29 46.1724433898926
30 42.2310066223145
31 37.0386238098145
32 31.7959671020508
33 22.7704734802246
34 16.3556308746338
35 15.1114892959595
36 14.3419322967529
37 13.4319896697998
38 12.2631511688232
39 11.0973958969116
40 9.83522987365723
41 8.53515911102295
42 7.90297985076904
43 7.53568553924561
44 7.27371215820312
45 7.17305755615234
46 7.23491239547729
47 7.5003342628479
48 8.1475305557251
49 9.1643533706665
50 12.950611114502
51 17.8942337036133
52 19.6262893676758
53 16.767520904541
54 12.0054655075073
55 6.56582117080688
56 3.79632711410522
57 1.74989438056946
58 -1.79947221279144
59 -0.358522683382034
60 14.9018898010254
61 28.2743663787842
62 36.4271240234375
63 42.5821914672852
64 47.4619216918945
65 51.3142051696777
66 54.4279861450195
67 57.076114654541
68 58.7711791992188
69 59.3940925598145
70 59.5858039855957
71 58.7955703735352
72 56.8482704162598
73 55.309440612793
74 54.5651626586914
75 53.631420135498
76 52.5327758789062
77 51.3358001708984
78 50.054859161377
79 48.7331619262695
80 47.4097900390625
81 46.0934104919434
82 44.7507057189941
83 43.3510246276855
84 41.7741203308105
85 39.5928916931152
86 36.2417030334473
87 29.3392009735107
88 6.23204803466797
89 31.1720695495605
90 -133.540466308594
91 -206.237243652344
92 -89.381233215332
93 20.4809284210205
94 8.1483268737793
95 7.0235767364502
96 6.0942816734314
97 5.28913116455078
98 4.01564168930054
99 1.22312593460083
};
\addplot [semithick, color1]
table {%
0 37.2327537536621
1 56.9115028381348
2 40.0513687133789
3 53.781909942627
4 73.4221115112305
5 69.8169250488281
6 35.4156684875488
7 16.6123638153076
8 13.7612180709839
9 13.1300926208496
10 14.9502038955688
11 31.6289520263672
12 107.743156433105
13 185.298202514648
14 241.358306884766
15 261.728149414062
16 247.947769165039
17 223.652191162109
18 196.272583007812
19 173.862670898438
20 154.151657104492
21 137.793914794922
22 123.482116699219
23 108.720611572266
24 98.2917785644531
25 93.3101119995117
26 93.7228698730469
27 95.4672241210938
28 96.9375686645508
29 96.9515686035156
30 86.4399795532227
31 70.9669189453125
32 56.1895980834961
33 47.451530456543
34 43.2325897216797
35 40.9470367431641
36 39.8037986755371
37 38.2184791564941
38 35.7654724121094
39 32.6814460754395
40 28.8520965576172
41 24.773567199707
42 21.1298408508301
43 18.3347625732422
44 16.2352142333984
45 15.1863355636597
46 15.2119455337524
47 16.5602855682373
48 19.2166080474854
49 23.3417949676514
50 29.5757884979248
51 36.4394950866699
52 41.313232421875
53 40.3487014770508
54 32.2678833007812
55 18.9687385559082
56 7.69412088394165
57 5.72316789627075
58 4.60681343078613
59 3.96145439147949
60 3.67085719108582
61 3.29738068580627
62 2.59233069419861
63 1.55033445358276
64 0.646016359329224
65 -0.039358377456665
66 -0.612487316131592
67 -1.08421719074249
68 -1.33041214942932
69 -1.32210755348206
70 -1.20037353038788
71 -0.821096837520599
72 -0.157760247588158
73 0.377050250768661
74 0.71576327085495
75 1.09463560581207
76 1.50973439216614
77 1.94192755222321
78 2.31966805458069
79 2.69927501678467
80 3.07556319236755
81 3.26500654220581
82 3.33562707901001
83 3.40589237213135
84 3.47740840911865
85 3.55475497245789
86 3.61170482635498
87 3.78264832496643
88 5.91805791854858
89 107.609321594238
90 -21.9286193847656
91 -123.791160583496
92 16.6951866149902
93 47.9168128967285
94 9.44730758666992
95 11.8347454071045
96 12.9748659133911
97 11.0863103866577
98 11.9970302581787
99 14.8922290802002
};
\addplot [semithick, color2]
table {%
0 9.16342830657959
1 16.2110500335693
2 26.6161594390869
3 26.1264972686768
4 34.6976890563965
5 38.7656402587891
6 42.6523170471191
7 42.4137420654297
8 50.448070526123
9 65.767204284668
10 70.5801162719727
11 78.0951919555664
12 72.020378112793
13 110.309730529785
14 117.106178283691
15 101.426765441895
16 157.78694152832
17 131.966262817383
18 108.57795715332
19 150.572784423828
20 149.664077758789
21 142.152038574219
22 152.160797119141
23 136.506820678711
24 138.110412597656
25 165.364181518555
26 92.8785858154297
27 149.293884277344
28 100.933113098145
29 99.2315673828125
30 68.2598495483398
31 139.179733276367
32 75.4538803100586
33 107.624923706055
34 88.6072006225586
35 69.7564010620117
36 91.3356857299805
37 73.1495895385742
38 63.0420227050781
39 62.6674880981445
40 62.8433113098145
41 21.7303657531738
42 38.1326332092285
43 30.3184661865234
44 12.5261192321777
45 16.9688758850098
46 24.0024852752686
47 12.1369781494141
48 11.5205965042114
49 13.3324356079102
50 12.1679639816284
51 13.0721349716187
52 13.7866477966309
53 11.6771650314331
54 12.4763631820679
55 12.3336563110352
56 13.0237236022949
57 13.9270992279053
58 13.1404314041138
59 15.9408483505249
60 19.9051513671875
61 13.6707038879395
62 30.1555938720703
63 26.24241065979
64 33.7051620483398
65 18.7736892700195
66 49.2958564758301
67 46.7156753540039
68 46.8795967102051
69 51.8885383605957
70 55.0041847229004
71 40.6861991882324
72 42.6219177246094
73 39.1169013977051
74 37.0260429382324
75 46.342399597168
76 41.569896697998
77 35.5531425476074
78 35.8363914489746
79 39.1003189086914
80 19.8306770324707
81 35.2823219299316
82 30.497652053833
83 18.4643058776855
84 35.6245956420898
85 19.0233974456787
86 13.2527303695679
87 21.1758766174316
88 22.538143157959
89 24.5872192382812
90 16.0919170379639
91 12.1283617019653
92 -33.5355072021484
93 -69.0295791625977
94 -2.60923624038696
95 -21.0723667144775
96 -10.4214382171631
97 -9.8606424331665
98 -26.1246471405029
99 -31.0615901947021
};
\addplot [semithick, color3]
table {%
0 29.2625312805176
1 10.5157222747803
2 13.8495807647705
3 38.7149772644043
4 41.1069526672363
5 47.3896675109863
6 16.622371673584
7 42.1592597961426
8 29.9005031585693
9 37.2437934875488
10 22.2342071533203
11 26.2293586730957
12 -10.5541591644287
13 32.2558822631836
14 56.8986129760742
15 99.8493728637695
16 125.53311920166
17 85.3592834472656
18 134.010940551758
19 106.068061828613
20 120.190071105957
21 111.044021606445
22 112.270164489746
23 82.5242767333984
24 26.0998935699463
25 79.3344650268555
26 55.2672996520996
27 31.8465957641602
28 59.8284301757812
29 57.2081565856934
30 38.8665313720703
31 41.8629112243652
32 41.6118125915527
33 32.5040283203125
34 32.7287864685059
35 27.540340423584
36 28.8151435852051
37 23.9029712677002
38 30.2091541290283
39 23.5863857269287
40 24.665412902832
41 23.8630123138428
42 27.7608070373535
43 24.579906463623
44 -12.0595817565918
45 23.9924278259277
46 28.6124324798584
47 25.1652030944824
48 24.8455486297607
49 25.3997077941895
50 24.3522243499756
51 24.7788047790527
52 24.9471874237061
53 28.3705711364746
54 24.3429279327393
55 27.9619846343994
56 24.4276905059814
57 -12.3955459594727
58 -11.840991973877
59 25.9475078582764
60 24.8755970001221
61 25.815673828125
62 31.2176284790039
63 40.017147064209
64 4.73128700256348
65 46.6897506713867
66 49.2361221313477
67 9.53739070892334
68 47.4822273254395
69 41.431396484375
70 51.2056541442871
71 43.736011505127
72 47.9935569763184
73 50.5346527099609
74 27.3133907318115
75 44.7539253234863
76 45.7297325134277
77 46.3239898681641
78 42.972053527832
79 40.7798690795898
80 44.0731201171875
81 44.1432762145996
82 46.3497047424316
83 44.0695571899414
84 42.194938659668
85 41.7953147888184
86 29.0542831420898
87 1.10031747817993
88 30.7719287872314
89 31.7921600341797
90 29.3625526428223
91 24.177791595459
92 -36.4914016723633
93 -45.0703277587891
94 -17.2514324188232
95 2.32076048851013
96 9.85519599914551
97 21.8889408111572
98 -15.4778900146484
99 -43.5509452819824
};
\addplot [semithick, black]
table {%
0 76.211858607035
1 102.388494526893
2 111.656100608832
3 120.369526759119
4 129.233602514894
5 133.166804360078
6 126.922309888644
7 114.079273031574
8 102.110480332218
9 96.5742006217253
10 98.3428710602753
11 105.145700296969
12 114.349203779314
13 123.043730066444
14 130.020512173298
15 129.385818981766
16 119.386170515249
17 105.438477289834
18 90.9082368204417
19 78.8263061671865
20 69.3935973728013
21 62.1572905745999
22 56.2350124342235
23 50.5783606406912
24 45.2595317230816
25 40.4302249842852
26 36.4074974363596
27 33.1993934503656
28 30.7356017843156
29 29.0038038364909
30 27.0675883316929
31 24.8513511987484
32 22.5852110900021
33 20.3054425192321
34 18.3272893819696
35 16.8790961478522
36 15.8985619279154
37 15.0688417839676
38 14.1210433964654
39 12.9877046205597
40 11.6175585538998
41 10.1371337904132
42 8.68431554521839
43 7.42639594971327
44 6.37884003511182
45 5.61849717369024
46 5.12651531705603
47 4.89604370391192
48 4.91869824067009
49 5.2133498906217
50 5.82455160958728
51 6.75485413481894
52 7.76396570836084
53 8.24565346458385
54 7.36558048581441
55 5.88700158237592
56 2.79399173644851
57 1.15886193331105
58 0.185366034679489
59 -0.365465053208651
60 -0.641651327281765
61 -0.731414369970568
62 -0.706321430093662
63 -0.627185679948078
64 -0.523068949158417
65 -0.418714310244732
66 -0.327308066722162
67 -0.252662243455939
68 -0.190076236078738
69 -0.138796581661797
70 -0.100064291700627
71 -0.0696429846689901
72 -0.0461995941030362
73 -0.0310240086766971
74 -0.0215817408823646
75 -0.0149127156996076
76 -0.0102495334313434
77 -0.0070505798936426
78 -0.0048969367352429
79 -0.00348024649210347
80 -0.00257781598819961
81 -0.00202798823121672
82 -0.00171356229754124
83 -0.00154534978591423
84 -0.00143765358213916
85 -0.00123590406625106
86 -0.000316102966340527
87 0.00615480949556608
88 0.102832710293066
89 1.40805619953343
90 2.9757300970776
91 3.91667175860393
92 4.09086744637716
93 3.69426863741391
94 5.85878526754537
95 11.0949032515285
96 16.6930914671581
97 23.6592647726372
98 33.0147934299705
99 50.3661196622867
};



==> plots/dl/m/Hamstrings.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 12.09752368927
1 47.7390174865723
2 129.551025390625
3 155.366333007812
4 169.22346496582
5 170.488388061523
6 156.599670410156
7 134.478622436523
8 115.407958984375
9 107.662734985352
10 107.80339050293
11 112.358215332031
12 117.156448364258
13 112.333724975586
14 97.7373428344727
15 84.2517166137695
16 68.0883941650391
17 50.2630767822266
18 37.4417915344238
19 30.71337890625
20 27.089822769165
21 24.5225734710693
22 22.7641868591309
23 20.6386775970459
24 13.7511253356934
25 11.2695999145508
26 17.8994293212891
27 21.930004119873
28 24.3667755126953
29 25.6846599578857
30 25.2975254058838
31 24.1264972686768
32 22.9207592010498
33 22.1395530700684
34 22.0266704559326
35 22.6455917358398
36 23.3362693786621
37 23.5652523040771
38 23.2895889282227
39 22.6766605377197
40 21.8803405761719
41 20.5514907836914
42 20.7977733612061
43 22.1574993133545
44 23.6324272155762
45 25.575065612793
46 28.0870323181152
47 31.2774333953857
48 39.0961494445801
49 54.6530113220215
50 33.8857574462891
51 -42.8023643493652
52 -35.6304244995117
53 75.7901840209961
54 70.2588195800781
55 -14.2119197845459
56 -10.4528789520264
57 50.1880111694336
58 81.4743576049805
59 45.4343185424805
60 5.73637294769287
61 46.156005859375
62 35.4321060180664
63 9.77080535888672
64 -10.3720922470093
65 2.48076128959656
66 10.9869537353516
67 16.2650814056396
68 9.74924087524414
69 -68.8288116455078
70 -160.077972412109
71 -178.588226318359
72 -169.202514648438
73 -152.193695068359
74 -117.613494873047
75 -57.2875366210938
76 9.97839164733887
77 59.2615585327148
78 70.9556121826172
79 70.608283996582
80 70.89306640625
81 71.2565994262695
82 71.3443984985352
83 71.6027603149414
84 70.8960113525391
85 68.4773559570312
86 58.6427383422852
87 45.9096488952637
88 40.6811027526855
89 37.323802947998
90 30.7747611999512
91 19.353199005127
92 4.1371111869812
93 -12.5818862915039
94 -20.1643314361572
95 -21.0646877288818
96 -23.7927837371826
97 -18.2468166351318
98 -3.05364155769348
99 1.49791848659515
};
\addplot [semithick, color1]
table {%
0 123.069534301758
1 169.852310180664
2 237.841415405273
3 267.754577636719
4 288.52685546875
5 291.725402832031
6 273.188720703125
7 245.242385864258
8 223.191787719727
9 218.495513916016
10 229.244964599609
11 245.905899047852
12 259.353240966797
13 251.687713623047
14 219.583297729492
15 195.031326293945
16 169.155471801758
17 140.131942749023
18 118.328109741211
19 114.255714416504
20 114.424194335938
21 107.049835205078
22 84.1040191650391
23 50.0082969665527
24 32.8121376037598
25 27.3063430786133
26 31.8335266113281
27 55.2583465576172
28 93.303581237793
29 117.676498413086
30 112.955841064453
31 92.8380661010742
32 73.659065246582
33 60.418571472168
34 58.5641937255859
35 67.3831634521484
36 78.4712753295898
37 82.2202987670898
38 76.9484786987305
39 66.2391204833984
40 53.9937324523926
41 44.8756103515625
42 41.5124702453613
43 46.9574127197266
44 63.7690544128418
45 87.2032318115234
46 120.030769348145
47 164.580825805664
48 205.668716430664
49 211.23991394043
50 66.1884536743164
51 -104.269241333008
52 -240.883590698242
53 -324.309112548828
54 -328.917846679688
55 -262.883728027344
56 -248.536605834961
57 -274.300384521484
58 -285.571685791016
59 -261.183410644531
60 -197.457855224609
61 -9.81138515472412
62 146.538986206055
63 16.9213428497314
64 5.43769359588623
65 4.46358633041382
66 1.68182849884033
67 -0.953960597515106
68 -3.88704252243042
69 -10.6445121765137
70 -19.3947792053223
71 -23.4876289367676
72 -23.7532787322998
73 -22.5022964477539
74 -20.5175018310547
75 -17.9659061431885
76 -15.1740922927856
77 -12.7063388824463
78 -10.2022676467896
79 -7.72708225250244
80 -5.7602915763855
81 -3.76018667221069
82 -1.66463625431061
83 -0.515358448028564
84 0.289849102497101
85 1.18204414844513
86 3.54186511039734
87 4.56199216842651
88 4.52085256576538
89 4.41377115249634
90 4.37316131591797
91 4.39889287948608
92 4.55960512161255
93 5.65485525131226
94 7.58131074905396
95 11.3008871078491
96 21.2462043762207
97 75.1308364868164
98 136.465637207031
99 137.278274536133
};
\addplot [semithick, color2]
table {%
0 26.0053577423096
1 36.6281089782715
2 32.3986968994141
3 36.5005950927734
4 58.3690032958984
5 52.595890045166
6 66.4205093383789
7 90.0774383544922
8 135.314987182617
9 111.95100402832
10 133.293655395508
11 169.830612182617
12 152.618316650391
13 102.743103027344
14 134.113708496094
15 187.479904174805
16 146.476119995117
17 185.578109741211
18 179.830856323242
19 124.302589416504
20 178.794921875
21 162.893844604492
22 177.978408813477
23 72.8083724975586
24 113.345039367676
25 63.0239143371582
26 53.7246513366699
27 44.6703758239746
28 60.5307388305664
29 33.042839050293
30 25.8571357727051
31 18.2539691925049
32 17.0500717163086
33 16.5751647949219
34 12.9458274841309
35 14.9188327789307
36 26.8859767913818
37 12.8584728240967
38 21.0304546356201
39 29.7777004241943
40 17.2210731506348
41 12.3777055740356
42 35.4898796081543
43 13.9842767715454
44 27.2470035552979
45 36.6075706481934
46 18.0342140197754
47 18.7500305175781
48 83.3755035400391
49 37.3721771240234
50 50.7643814086914
51 107.910774230957
52 -7.17685890197754
53 -33.6405372619629
54 -49.2076797485352
55 -130.410583496094
56 -138.031692504883
57 -346.932037353516
58 -267.955780029297
59 -291.897308349609
60 -321.057220458984
61 -322.563262939453
62 -265.634979248047
63 -49.1920013427734
64 -130.699493408203
65 -52.5622863769531
66 46.0423851013184
67 50.4243011474609
68 57.5834999084473
69 88.5694122314453
70 86.9786529541016
71 86.3768615722656
72 82.8191528320312
73 92.5862045288086
74 136.29231262207
75 92.8439559936523
76 113.679550170898
77 104.402313232422
78 122.809425354004
79 98.8528289794922
80 62.6040878295898
81 67.184326171875
82 86.0078430175781
83 106.062164306641
84 97.4812927246094
85 74.4023742675781
86 85.5278930664062
87 76.4863433837891
88 67.2586975097656
89 45.2297401428223
90 40.4151802062988
91 36.2573165893555
92 31.2028026580811
93 29.3084468841553
94 26.3295803070068
95 24.911413192749
96 20.3191757202148
97 19.303129196167
98 15.3082313537598
99 22.3208827972412
};
\addplot [semithick, color3]
table {%
0 34.9592323303223
1 102.630065917969
2 127.014183044434
3 130.692321777344
4 149.870010375977
5 191.009567260742
6 178.79216003418
7 178.716567993164
8 181.262603759766
9 182.546417236328
10 212.476272583008
11 158.241622924805
12 158.445983886719
13 197.271606445312
14 178.346008300781
15 174.102905273438
16 199.342758178711
17 152.081329345703
18 84.8870697021484
19 110.476264953613
20 114.189254760742
21 89.645378112793
22 89.2388916015625
23 77.2032623291016
24 29.70583152771
25 35.3263969421387
26 2.60742163658142
27 9.84753036499023
28 47.6510810852051
29 40.4194450378418
30 44.8887634277344
31 43.4887542724609
32 32.250415802002
33 35.7340316772461
34 35.468936920166
35 34.8371315002441
36 44.1742706298828
37 12.590220451355
38 49.7024116516113
39 37.9183387756348
40 41.088737487793
41 46.8502235412598
42 41.256950378418
43 46.0075988769531
44 43.0438385009766
45 4.89745044708252
46 33.0526809692383
47 55.2759895324707
48 32.6524810791016
49 41.0717887878418
50 85.5846557617188
51 122.57275390625
52 46.9769630432129
53 -36.7706985473633
54 -55.4535102844238
55 -57.6477394104004
56 -23.3819389343262
57 -50.3732566833496
58 -93.7242126464844
59 -46.2297210693359
60 -77.0580825805664
61 -62.3531532287598
62 -40.3241691589355
63 -12.4574518203735
64 -12.1348934173584
65 11.9169130325317
66 30.7665996551514
67 -3.48096966743469
68 11.6915159225464
69 18.6393089294434
70 23.2148532867432
71 55.1067352294922
72 75.3697204589844
73 75.5854034423828
74 74.025764465332
75 61.9940986633301
76 16.9925270080566
77 15.6606721878052
78 87.1629943847656
79 69.1860885620117
80 16.3244285583496
81 38.586254119873
82 77.4287490844727
83 57.0342826843262
84 17.1643753051758
85 69.664176940918
86 47.2088050842285
87 10.6313381195068
88 44.8788909912109
89 32.9115028381348
90 35.3801689147949
91 24.9123039245605
92 27.8254127502441
93 25.3501720428467
94 25.2803268432617
95 26.2456665039062
96 28.4870567321777
97 30.4571685791016
98 4.44383001327515
99 80.8017883300781
};
\addplot [semithick, black]
table {%
0 104.770766106655
1 103.803585169611
2 112.677389028367
3 116.374748497656
4 117.976340246812
5 115.756878479748
6 107.595938143453
7 95.8709069385438
8 84.594094892638
9 76.6660667690499
10 72.7185675584693
11 71.5611150733077
12 71.3729184422678
13 68.4240407843941
14 59.9415522650763
15 50.9605160854361
16 41.8553391562318
17 32.9249181899618
18 25.4978787729966
19 20.7560189394104
20 18.0754877254521
21 16.4788960512797
22 14.9871795797929
23 12.8559069418336
24 10.4852649709027
25 8.49608249684329
26 7.34032989144525
27 7.27938314968931
28 8.12854473879145
29 9.541556752843
30 10.5431508588465
31 10.803979739981
32 10.6072551828745
33 10.2132877455355
34 10.0295419870608
35 10.2589991721158
36 10.807352462129
37 11.2702298122078
38 11.3291144390866
39 10.9294256892336
40 10.1109282645712
41 9.10384410689177
42 8.0631011296135
43 7.15826722178536
44 6.52060855817574
45 6.10124391596789
46 5.85477694847973
47 5.88246134122582
48 6.24508943286071
49 7.0517886651121
50 8.42281701184272
51 10.3423120570089
52 12.4738451949941
53 14.4983229262463
54 15.7680165829671
55 11.6270647553607
56 7.69604355198761
57 5.24545336887124
58 3.53783656288641
59 2.32874270380477
60 1.49464076296067
61 0.925478705855691
62 0.538959267054774
63 0.273969120056367
64 0.100857532363958
65 0.00725679873232066
66 -0.0349982681045421
67 -0.0474418148162101
68 -0.0459481352460599
69 -0.0499571455436858
70 -0.0553297991838648
71 -0.0512825865659347
72 -0.0420309745897262
73 -0.0329394638742147
74 -0.0252159381935043
75 -0.018839893024341
76 -0.0139964230134186
77 -0.0104661885956958
78 -0.00778811604327029
79 -0.00578807844734126
80 -0.00437674937265149
81 -0.00332303470188547
82 -0.0025171254026194
83 -0.00194370223840992
84 -0.00155430062610861
85 -0.00131574824325905
86 -0.00240922513205707
87 -1.61591514288325
88 -4.34544016586339
89 -7.70413962961976
90 -9.97412877091537
91 -9.61256632273531
92 -5.53570918951987
93 3.05835670004276
94 16.4614665815685
95 35.2619263097827
96 58.859944462798
97 85.6941131879598
98 109.462546393149
99 114.339961603512
};



==> plots/dl/m/Iliopsoas.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 5.86881017684937
1 5.69003200531006
2 5.34241008758545
3 5.06716012954712
4 4.96652698516846
5 5.07535123825073
6 5.38800621032715
7 5.5063214302063
8 5.35321092605591
9 5.22510576248169
10 5.17118644714355
11 5.14902496337891
12 5.53095149993896
13 8.11029815673828
14 16.2896842956543
15 23.5268650054932
16 25.2669429779053
17 25.0433330535889
18 23.9246273040771
19 22.3843212127686
20 20.7758083343506
21 19.5143489837646
22 18.772123336792
23 18.5281085968018
24 18.7886829376221
25 19.3072376251221
26 19.867696762085
27 20.1580753326416
28 20.238130569458
29 20.0904922485352
30 19.3944702148438
31 18.4638156890869
32 17.7696723937988
33 16.8519306182861
34 16.0181102752686
35 15.4540672302246
36 15.090428352356
37 14.8051414489746
38 15.1047077178955
39 15.7344207763672
40 16.392707824707
41 17.0697612762451
42 17.7271041870117
43 18.3614768981934
44 18.9759197235107
45 19.6100540161133
46 20.2088146209717
47 20.778829574585
48 21.3300094604492
49 22.0081310272217
50 22.9563293457031
51 24.4633293151855
52 27.3421764373779
53 31.1212482452393
54 36.2783889770508
55 43.1731338500977
56 61.7254333496094
57 66.5425567626953
58 82.0448379516602
59 109.69401550293
60 174.340484619141
61 245.827606201172
62 303.867950439453
63 358.917083740234
64 399.585418701172
65 420.122711181641
66 426.806823730469
67 419.801696777344
68 404.976898193359
69 366.512176513672
70 325.90380859375
71 277.998413085938
72 236.953521728516
73 211.251159667969
74 206.321212768555
75 203.324417114258
76 197.712448120117
77 186.558792114258
78 166.788757324219
79 141.78434753418
80 120.000099182129
81 91.4661407470703
82 57.2251129150391
83 19.3081684112549
84 2.13584804534912
85 -1.14042699337006
86 0.400925040245056
87 2.60816097259521
88 2.0970094203949
89 0.692710340023041
90 -0.47076553106308
91 -0.360746741294861
92 0.916926920413971
93 2.38956260681152
94 3.80484008789062
95 4.76135778427124
96 5.21934461593628
97 5.64826822280884
98 5.97809028625488
99 6.12033367156982
};
\addplot [semithick, color1]
table {%
0 6.60160493850708
1 6.6199836730957
2 6.64736032485962
3 6.7217493057251
4 6.76037359237671
5 6.73382711410522
6 6.65167427062988
7 6.62243223190308
8 6.66672229766846
9 6.70538091659546
10 6.72722148895264
11 6.73848247528076
12 6.74345254898071
13 6.84754610061646
14 7.18099308013916
15 6.91820669174194
16 6.87692832946777
17 6.93135499954224
18 7.02893161773682
19 7.13957834243774
20 7.13621759414673
21 7.04268598556519
22 6.97300148010254
23 6.92482137680054
24 6.89812994003296
25 6.88225936889648
26 6.86637306213379
27 6.83735466003418
28 6.79453754425049
29 6.74206638336182
30 6.6695556640625
31 6.59222364425659
32 6.51866102218628
33 6.44472217559814
34 6.37699365615845
35 6.32125759124756
36 6.27441120147705
37 6.23155784606934
38 6.19229221343994
39 6.15764093399048
40 6.12371778488159
41 6.08810138702393
42 6.05080795288086
43 6.01336860656738
44 5.97773456573486
45 5.94488191604614
46 5.91932678222656
47 5.90353631973267
48 5.89728927612305
49 5.90156841278076
50 5.91479969024658
51 5.92692470550537
52 5.93109941482544
53 5.91972970962524
54 5.88089275360107
55 5.79999589920044
56 5.23300743103027
57 5.57135248184204
58 21.7219257354736
59 102.52677154541
60 194.474899291992
61 271.392425537109
62 349.073669433594
63 421.553741455078
64 473.432556152344
65 492.602630615234
66 497.995422363281
67 483.728515625
68 466.055877685547
69 411.504364013672
70 363.235137939453
71 315.494598388672
72 266.227020263672
73 253.381759643555
74 277.931365966797
75 288.020843505859
76 286.146942138672
77 271.913970947266
78 243.060607910156
79 205.92512512207
80 178.516906738281
81 160.057144165039
82 135.746841430664
83 102.235557556152
84 61.2479438781738
85 27.9104347229004
86 10.6154022216797
87 10.426775932312
88 12.80872631073
89 9.65851211547852
90 8.25188159942627
91 7.37344789505005
92 7.13423252105713
93 7.01578855514526
94 6.90393352508545
95 6.81402397155762
96 6.73383712768555
97 6.66198444366455
98 6.59207201004028
99 6.55905389785767
};
\addplot [semithick, color2]
table {%
0 13.030782699585
1 10.3831300735474
2 14.5851593017578
3 11.3983469009399
4 13.9433755874634
5 19.5167942047119
6 21.6691951751709
7 17.1157875061035
8 13.6610670089722
9 14.6954898834229
10 14.2165241241455
11 14.1590747833252
12 12.3281860351562
13 17.9291400909424
14 12.8188314437866
15 12.8511848449707
16 20.0486888885498
17 20.7993144989014
18 17.8320045471191
19 16.6708984375
20 17.3886814117432
21 18.2933769226074
22 17.3730525970459
23 18.2167358398438
24 20.5425777435303
25 19.9997043609619
26 20.9407424926758
27 13.314811706543
28 21.6081466674805
29 10.2217397689819
30 13.5312061309814
31 18.2282199859619
32 18.8516006469727
33 14.0318422317505
34 12.3304290771484
35 17.490629196167
36 19.3101291656494
37 19.3746528625488
38 16.5044326782227
39 13.1863508224487
40 13.5498685836792
41 15.8592748641968
42 17.1339244842529
43 10.6271314620972
44 15.1046390533447
45 17.9184398651123
46 18.732967376709
47 16.5015411376953
48 15.3202428817749
49 16.8086948394775
50 15.346474647522
51 16.2371730804443
52 17.1865158081055
53 13.0942258834839
54 17.2428169250488
55 16.664134979248
56 16.9407520294189
57 14.8540706634521
58 15.165943145752
59 12.3364849090576
60 11.3233699798584
61 19.4555797576904
62 33.9925422668457
63 56.5330276489258
64 76.0809631347656
65 128.265426635742
66 141.989410400391
67 181.975372314453
68 225.706985473633
69 313.857543945312
70 309.224273681641
71 207.866409301758
72 239.168518066406
73 181.06298828125
74 273.967163085938
75 256.929168701172
76 237.161499023438
77 310.614959716797
78 241.205215454102
79 188.380645751953
80 68.4192199707031
81 65.4846572875977
82 170.606369018555
83 115.757438659668
84 111.523460388184
85 129.287200927734
86 111.224830627441
87 76.4761123657227
88 94.7494888305664
89 34.7127838134766
90 20.5793170928955
91 21.2019348144531
92 13.3719415664673
93 12.4065637588501
94 15.0395097732544
95 15.6647624969482
96 14.7950248718262
97 15.4610633850098
98 13.0178337097168
99 11.7445440292358
};
\addplot [semithick, color3]
table {%
0 26.6880550384521
1 22.2805671691895
2 22.1030521392822
3 -13.8033504486084
4 -14.1764087677002
5 21.6301975250244
6 -13.5338306427002
7 23.471378326416
8 26.6015701293945
9 23.2692394256592
10 23.0836296081543
11 -13.305233001709
12 23.81569480896
13 23.1673145294189
14 -9.71076393127441
15 22.9144096374512
16 24.8908405303955
17 27.387077331543
18 29.1945457458496
19 -13.8187389373779
20 -10.3139162063599
21 22.9644813537598
22 22.8609199523926
23 24.9780540466309
24 22.9352359771729
25 27.4213275909424
26 24.2967147827148
27 24.6020355224609
28 23.3179607391357
29 29.2100791931152
30 27.0538024902344
31 27.8900718688965
32 26.8468494415283
33 23.6983528137207
34 22.7252655029297
35 22.9125537872314
36 -12.8354520797729
37 24.1746158599854
38 27.236759185791
39 22.8886127471924
40 22.8518123626709
41 22.7337532043457
42 25.3505382537842
43 23.6634693145752
44 24.885368347168
45 23.0597476959229
46 22.9171905517578
47 22.3806304931641
48 23.8093891143799
49 25.1482181549072
50 23.9769668579102
51 -14.4213314056396
52 22.5169639587402
53 23.8441467285156
54 23.2452964782715
55 25.0792865753174
56 22.2997016906738
57 22.578182220459
58 -12.996919631958
59 28.0640716552734
60 0.822622776031494
61 45.9775466918945
62 94.85400390625
63 182.363418579102
64 172.831802368164
65 320.821960449219
66 138.000442504883
67 290.413909912109
68 386.165893554688
69 459.352478027344
70 344.549102783203
71 342.694885253906
72 303.544891357422
73 278.430450439453
74 315.874420166016
75 288.878997802734
76 278.066009521484
77 210.025817871094
78 218.542770385742
79 266.259979248047
80 178.759475708008
81 218.477249145508
82 186.219436645508
83 215.859573364258
84 113.735054016113
85 92.3031234741211
86 107.551803588867
87 104.16072845459
88 19.3176689147949
89 75.260871887207
90 69.3554077148438
91 41.9481735229492
92 41.4538536071777
93 39.2679290771484
94 22.8455123901367
95 24.2528457641602
96 27.5410499572754
97 22.8406734466553
98 28.0204124450684
99 22.9053440093994
};
\addplot [semithick, black]
table {%
0 0.191509787943184
1 0.129360872164764
2 0.0815766576691378
3 0.0507992418964271
4 0.0331959488037797
5 0.0243930326033539
6 0.0195953889278714
7 0.0144479236124151
8 0.00952636450094502
9 0.00628967584527414
10 0.00425366175476991
11 0.00293061000799553
12 0.00204787062113738
13 0.0011136775459142
14 -5.26104471754388e-05
15 -0.000633794099996827
16 -0.000599432795543893
17 -0.000457118056848892
18 -0.000321467909738262
19 -0.000218885747757528
20 -0.000141312068832507
21 -8.8337121015857e-05
22 -5.66362417705217e-05
23 -4.16482705962001e-05
24 -4.42846456914847e-05
25 -5.77502051652931e-05
26 -7.44575439437733e-05
27 -8.03161493541776e-05
28 -7.43959573137583e-05
29 -5.65187092320261e-05
30 -1.3344121646452e-05
31 4.12145656482814e-05
32 9.82081417711812e-05
33 0.00016340023179277
34 0.000228515733012544
35 0.000283310977690019
36 0.000329160015895734
37 0.000372530400149806
38 0.000415720018563474
39 0.000461313235560381
40 0.000517018480184007
41 0.000589261154348816
42 0.000679748004286211
43 0.00078263181368053
44 0.000886163314743826
45 0.000972651021524113
46 0.00101710628987917
47 0.00100322533948359
48 0.000932943740064647
49 0.000815343902343951
50 0.000671092769178324
51 0.000532782149350696
52 0.000422269159485414
53 0.000348725273361004
54 0.00031729994368886
55 0.000321778691108817
56 0.000546136891553294
57 1.67289930710442
58 8.063474204774
59 19.6476739307801
60 36.2764767086937
61 55.3807590048209
62 73.8339724439967
63 90.9514167727637
64 104.987548394718
65 113.542908672372
66 118.011819741389
67 118.198953260691
68 115.70467681814
69 105.704230397201
70 92.6658161227683
71 77.4407349414227
72 62.1119522459456
73 52.3048201573709
74 50.7582983881336
75 52.0271102823223
76 53.6003723180182
77 53.7531577919249
78 51.4901310288674
79 47.2728228889861
80 43.3341021095045
81 40.4391042983482
82 37.3062148444016
83 33.306271831018
84 28.2358081246306
85 20.8329885319193
86 13.399498581458
87 10.5491054508476
88 9.88508139546514
89 7.87458733213254
90 5.52654416094174
91 3.31688741714102
92 2.03501845379266
93 1.45248260645616
94 1.11026311901512
95 0.872523063479217
96 0.684958129113834
97 0.529690251271779
98 0.39738037875147
99 0.287373120166802
};



==> plots/dl/m/RectusFemoris.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 14.8607387542725
1 14.9421081542969
2 15.0471773147583
3 15.2122383117676
4 15.4236497879028
5 15.6702280044556
6 15.9440622329712
7 16.2408065795898
8 16.5589942932129
9 16.3202533721924
10 27.6801834106445
11 19.3040542602539
12 24.961353302002
13 29.1579456329346
14 22.1158866882324
15 19.692174911499
16 19.7872943878174
17 20.0152626037598
18 20.2766799926758
19 20.5649604797363
20 20.9394912719727
21 21.3429050445557
22 21.7506408691406
23 22.0971832275391
24 22.5888767242432
25 24.2626914978027
26 25.3862590789795
27 25.7608051300049
28 26.0330257415771
29 27.1806564331055
30 29.7391738891602
31 32.8400268554688
32 35.5953407287598
33 37.5898551940918
34 38.7786521911621
35 39.3489952087402
36 39.7925071716309
37 41.0400276184082
38 43.6694526672363
39 47.4861946105957
40 51.3408584594727
41 54.3627090454102
42 56.3023910522461
43 56.0697021484375
44 54.9286956787109
45 54.7146682739258
46 55.4153518676758
47 57.242977142334
48 60.5904808044434
49 64.8885040283203
50 69.5505828857422
51 72.1164245605469
52 70.4943389892578
53 65.7617721557617
54 54.9882278442383
55 43.030704498291
56 74.4364471435547
57 128.03938293457
58 125.509216308594
59 90.5189971923828
60 67.1303405761719
61 59.5440521240234
62 46.3517265319824
63 -51.6694297790527
64 -100.145324707031
65 -107.708129882812
66 -89.7490463256836
67 -26.694860458374
68 27.4925136566162
69 43.3091430664062
70 18.522424697876
71 -40.2460289001465
72 -94.9815826416016
73 -118.652931213379
74 -146.215515136719
75 -157.980743408203
76 -164.167724609375
77 -167.093688964844
78 -166.427261352539
79 -166.532653808594
80 -165.701309204102
81 -163.203491210938
82 -157.530349731445
83 -142.994049072266
84 -135.31657409668
85 -135.046234130859
86 -134.986572265625
87 -103.860343933105
88 -11.8074264526367
89 67.8310012817383
90 61.1586456298828
91 52.0630111694336
92 46.4919700622559
93 42.3708457946777
94 39.2026824951172
95 31.7878608703613
96 21.697883605957
97 16.4019355773926
98 15.2599630355835
99 15.1248168945312
};
\addplot [semithick, color1]
table {%
0 6.12017583847046
1 6.11897277832031
2 6.11650848388672
3 6.11304187774658
4 6.1091570854187
5 6.11038494110107
6 6.11057806015015
7 6.10826778411865
8 6.10250568389893
9 6.27580976486206
10 6.80020761489868
11 6.38536357879639
12 6.4034948348999
13 6.91584491729736
14 8.50823020935059
15 9.11342239379883
16 9.23579216003418
17 9.69835948944092
18 9.6746187210083
19 9.33686256408691
20 8.97874450683594
21 8.70238399505615
22 8.51275539398193
23 8.39988327026367
24 8.19133281707764
25 7.96749305725098
26 7.72646379470825
27 7.45478630065918
28 7.18920135498047
29 6.92562103271484
30 6.73625755310059
31 6.59121513366699
32 6.4743824005127
33 6.40046453475952
34 6.35577726364136
35 6.32342624664307
36 6.24994277954102
37 6.17294216156006
38 6.11190843582153
39 6.07219171524048
40 6.05498456954956
41 6.04656362533569
42 6.04261255264282
43 6.04194355010986
44 6.01255178451538
45 6.01789999008179
46 6.04601335525513
47 6.10011005401611
48 6.13713312149048
49 6.16584920883179
50 6.19950819015503
51 6.23518657684326
52 6.27691745758057
53 6.32745027542114
54 6.37258386611938
55 6.28781175613403
56 5.10826253890991
57 50.6759948730469
58 16.5977306365967
59 11.567590713501
60 8.11298561096191
61 6.6031322479248
62 6.0896167755127
63 6.5822811126709
64 7.23848342895508
65 6.79634809494019
66 10.0921745300293
67 20.1587657928467
68 30.9342651367188
69 29.9304656982422
70 21.4125156402588
71 15.9199686050415
72 15.6351146697998
73 22.5993537902832
74 24.1045989990234
75 52.9204978942871
76 80.2235717773438
77 97.3529891967773
78 78.9561538696289
79 57.4324913024902
80 38.8865623474121
81 25.184513092041
82 17.2963161468506
83 15.5098676681519
84 -0.27708026766777
85 -3.37131834030151
86 -0.752522349357605
87 16.8415946960449
88 48.0379104614258
89 84.8786468505859
90 58.6848182678223
91 14.1557664871216
92 5.46118402481079
93 5.17923164367676
94 5.30999422073364
95 5.48754835128784
96 5.63207101821899
97 5.82796382904053
98 5.99492216110229
99 6.06730699539185
};
\addplot [semithick, color2]
table {%
0 13.917552947998
1 12.2697744369507
2 14.1112689971924
3 13.8756589889526
4 14.3822889328003
5 16.2437553405762
6 15.1999187469482
7 16.8835296630859
8 17.2171001434326
9 13.7222337722778
10 12.7471466064453
11 16.930290222168
12 18.7835025787354
13 18.9977283477783
14 13.4275350570679
15 14.426420211792
16 13.1300020217896
17 13.9360637664795
18 12.8573808670044
19 13.2464771270752
20 9.98447418212891
21 12.7556800842285
22 12.7206039428711
23 11.3450164794922
24 11.7313222885132
25 9.68493270874023
26 12.1002149581909
27 12.7424259185791
28 13.3578748703003
29 11.9738912582397
30 12.1672306060791
31 12.103461265564
32 13.0604772567749
33 13.9898462295532
34 14.4052248001099
35 12.0648603439331
36 14.773042678833
37 14.5555229187012
38 12.5960464477539
39 10.7621212005615
40 10.6415014266968
41 11.2077007293701
42 12.1927814483643
43 11.9773683547974
44 12.3002138137817
45 15.0018100738525
46 15.0373620986938
47 11.5377635955811
48 9.44316101074219
49 11.7140703201294
50 9.5474853515625
51 16.2265548706055
52 12.1725997924805
53 15.6030015945435
54 11.4319581985474
55 16.0821552276611
56 15.8470287322998
57 16.7052307128906
58 14.2797603607178
59 13.2451248168945
60 14.7579746246338
61 14.0571203231812
62 14.8819465637207
63 14.753662109375
64 12.6680927276611
65 12.3497266769409
66 13.0524797439575
67 13.2538232803345
68 11.1647930145264
69 10.5014419555664
70 8.74827575683594
71 11.6285009384155
72 9.81115436553955
73 8.0255708694458
74 10.8495836257935
75 7.99887943267822
76 10.9010696411133
77 10.3855113983154
78 10.3077402114868
79 8.79857540130615
80 9.59650039672852
81 11.4552936553955
82 10.5619239807129
83 10.1873016357422
84 13.3448448181152
85 8.01119995117188
86 21.2449245452881
87 5.5327525138855
88 0.964344382286072
89 9.26508712768555
90 11.4145698547363
91 8.83403015136719
92 10.5654363632202
93 13.2163362503052
94 14.9580717086792
95 12.7613172531128
96 10.7966203689575
97 11.3528537750244
98 14.7150096893311
99 11.3992376327515
};
\addplot [semithick, color3]
table {%
0 24.4122447967529
1 -13.8331651687622
2 24.4569301605225
3 -13.8345746994019
4 21.0916652679443
5 24.1285972595215
6 22.4051933288574
7 22.9322128295898
8 -14.0825490951538
9 24.8197727203369
10 -13.2741498947144
11 -13.9547672271729
12 25.2432594299316
13 24.3120784759521
14 22.8341522216797
15 22.0364551544189
16 22.5160446166992
17 -12.1591396331787
18 21.9165496826172
19 21.9984798431396
20 21.7112503051758
21 -15.1321754455566
22 21.6688594818115
23 21.6076126098633
24 21.5124740600586
25 -16.0599479675293
26 20.8830757141113
27 21.1235637664795
28 19.8946895599365
29 19.6068534851074
30 21.3436222076416
31 22.7844543457031
32 20.2127285003662
33 23.9274635314941
34 23.9223594665527
35 20.7969093322754
36 22.2939567565918
37 -17.3480968475342
38 23.902982711792
39 22.3219432830811
40 22.2786655426025
41 22.0029983520508
42 23.7588119506836
43 22.5384006500244
44 22.6986656188965
45 23.815523147583
46 22.6843185424805
47 26.5617904663086
48 23.3812656402588
49 22.3771686553955
50 -13.1439447402954
51 19.9551067352295
52 21.7500476837158
53 -14.8310070037842
54 22.7543106079102
55 23.3114166259766
56 21.0048675537109
57 -11.9712772369385
58 22.6701583862305
59 22.8299922943115
60 -14.8090705871582
61 -15.3825969696045
62 20.056058883667
63 16.8439464569092
64 14.7664022445679
65 -20.8886108398438
66 15.8474044799805
67 16.57200050354
68 -19.5908908843994
69 -21.1351470947266
70 -22.3199405670166
71 -25.965669631958
72 10.8759317398071
73 11.2186908721924
74 11.1452016830444
75 10.136058807373
76 11.3802881240845
77 12.8398303985596
78 8.45616722106934
79 6.85271024703979
80 9.60409069061279
81 12.0270948410034
82 11.6461277008057
83 10.688572883606
84 14.3366899490356
85 -19.4878768920898
86 15.3693170547485
87 -22.5577697753906
88 19.6220474243164
89 -16.6176357269287
90 18.9421558380127
91 19.6712474822998
92 22.6884746551514
93 21.1331901550293
94 -14.7872848510742
95 -14.9299030303955
96 22.3889751434326
97 24.1118335723877
98 22.2983722686768
99 22.7794342041016
};
\addplot [semithick, black]
table {%
0 0.00693966966321178
1 0.00512855056139388
2 0.00377671005782079
3 0.00294232744060452
4 0.00244734761710853
5 0.00218375459742315
6 0.00209089839672875
7 0.00214488588744488
8 0.00236344927351842
9 -0.000723323499901417
10 -0.00800955124662523
11 -0.0175732745293021
12 0.266993669023896
13 1.00881793160914
14 2.25697849692935
15 2.6387333236434
16 2.63329144413318
17 2.60519756683321
18 2.38636333039984
19 2.07957075880761
20 1.86661824885624
21 1.86062261964982
22 2.04461182502676
23 2.29149893747831
24 2.4631859523213
25 2.50282684480858
26 2.40888760333954
27 2.20045425979088
28 1.92739938026879
29 1.64603181764017
30 1.41396947102505
31 1.24609970847753
32 1.11314889471443
33 0.98252370579742
34 0.832859286081625
35 0.660332166826918
36 0.476701468199174
37 0.321507404688231
38 0.225064325976238
39 0.179499992402323
40 0.158966115546903
41 0.144209468160874
42 0.128973256282064
43 0.0947566605595052
44 0.0367764730047329
45 -0.0140682987220821
46 -0.0512273357232388
47 -0.0681604334940192
48 -0.067933000762683
49 -0.0612161373228022
50 -0.0535617256796318
51 -0.0460735783196393
52 -0.0395785352356486
53 -0.034610686596905
54 -0.0314490816829967
55 -0.0316227786690674
56 0.0780632289268542
57 6.68939974250306
58 1.3348984003457
59 -9.92029088102631
60 -24.5155056942581
61 -33.7051102804263
62 -32.8295663010624
63 -23.6851761304992
64 -13.8513760776268
65 -7.8869413883525
66 -4.38555952978521
67 -2.37312812732318
68 -1.9372871451746
69 -2.14524311572876
70 -1.65075978809129
71 0.525614454550302
72 3.60480060271749
73 6.35430904824586
74 8.1797887567626
75 9.95427005335213
76 11.24411929831
77 11.9710337539787
78 12.0762229360683
79 11.7092402481009
80 11.2135092361173
81 10.6641692471273
82 10.0548710474601
83 9.14209955268916
84 6.84331727114286
85 4.99758286037127
86 3.61877786874634
87 2.52425707028242
88 1.67975021048512
89 1.09340802887977
90 0.702355384179024
91 0.44559355885772
92 0.279673448001167
93 0.174098405033738
94 0.107855217641519
95 0.0667632292600625
96 0.0414665651609898
97 0.0259533993942876
98 0.0164471101997537
99 0.0112923486633634
};



==> plots/dl/m/Soleus.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\addplot[semithick, color0]
table {%
0 6.32368946075439
1 5.8567533493042
2 5.13817501068115
3 4.73629140853882
4 4.60328483581543
5 5.30232429504395
6 7.33052062988281
7 15.4346199035645
8 17.8008232116699
9 13.3208808898926
10 2.93909072875977
11 10.7767534255981
12 6.14474391937256
13 0.0162312481552362
14 -3.94823598861694
15 -5.57912015914917
16 -5.34803247451782
17 -5.47894954681396
18 -7.60097742080688
19 -7.62405395507812
20 -7.93235445022583
21 -8.65588283538818
22 -9.69829750061035
23 -10.4625034332275
24 -10.7409467697144
25 -10.6979808807373
26 -10.3874464035034
27 -10.1357278823853
28 -10.1095275878906
29 -10.2726230621338
30 -10.6858549118042
31 -11.2868022918701
32 -11.9949188232422
33 -12.6798658370972
34 -13.3964824676514
35 -14.3312664031982
36 -15.2848796844482
37 -16.5202732086182
38 -16.4947967529297
39 -15.8551111221313
40 -14.2646207809448
41 -12.0508680343628
42 -9.26776885986328
43 -5.51892375946045
44 -1.48589217662811
45 3.39165544509888
46 8.9429349899292
47 16.0587291717529
48 24.6747913360596
49 51.0254096984863
50 98.4655380249023
51 158.315002441406
52 232.772186279297
53 314.485534667969
54 416.142425537109
55 472.178283691406
56 514.087219238281
57 533.146789550781
58 532.088012695312
59 485.922821044922
60 408.924346923828
61 321.025268554688
62 155.037506103516
63 16.7108497619629
64 -22.4022560119629
65 61.7357978820801
66 52.1970291137695
67 18.1941375732422
68 2.11218476295471
69 -4.38031101226807
70 14.8002548217773
71 23.6562976837158
72 26.85302734375
73 27.7261638641357
74 27.8675918579102
75 27.3171272277832
76 26.3256988525391
77 25.1352519989014
78 23.6847496032715
79 22.0518760681152
80 20.3071556091309
81 18.2610893249512
82 15.7556486129761
83 13.0101280212402
84 10.1536617279053
85 7.4464111328125
86 5.06872129440308
87 3.82843279838562
88 4.23949527740479
89 4.63318395614624
90 4.97784280776978
91 5.4751410484314
92 6.3630895614624
93 7.07081460952759
94 7.46693754196167
95 6.89487028121948
96 5.51404571533203
97 4.24032115936279
98 3.81555676460266
99 3.9221818447113
};
\addplot [semithick, color1]
table {%
0 4.16062831878662
1 4.22697734832764
2 4.43802547454834
3 4.5829439163208
4 4.63570261001587
5 4.38732433319092
6 8.89822483062744
7 19.7025299072266
8 26.2328186035156
9 19.1956424713135
10 5.56719732284546
11 6.14491891860962
12 5.92824411392212
13 5.76293134689331
14 5.7153148651123
15 5.54707384109497
16 5.40296411514282
17 5.58191442489624
18 6.26346778869629
19 7.39577102661133
20 8.98825454711914
21 11.0972471237183
22 14.3527145385742
23 15.7317523956299
24 16.0349197387695
25 16.4112091064453
26 17.9107551574707
27 21.6505966186523
28 26.8902835845947
29 31.4976425170898
30 33.168098449707
31 32.6733055114746
32 31.8602256774902
33 31.5705680847168
34 32.5322418212891
35 34.574161529541
36 36.7906608581543
37 38.3484649658203
38 38.8261985778809
39 38.7808647155762
40 38.5998916625977
41 38.4460639953613
42 38.7449607849121
43 38.7426948547363
44 38.4196243286133
45 38.4799766540527
46 40.0105667114258
47 45.5176696777344
48 61.5389938354492
49 88.3888854980469
50 124.695465087891
51 171.133987426758
52 231.726654052734
53 320.601989746094
54 432.649230957031
55 523.642211914062
56 594.487426757812
57 634.097534179688
58 651.946716308594
59 591.238037109375
60 460.627990722656
61 295.312805175781
62 93.2810287475586
63 18.4755420684814
64 -0.222568467259407
65 46.8698501586914
66 142.907730102539
67 56.0128707885742
68 6.27787399291992
69 5.82500600814819
70 4.5496563911438
71 4.20160722732544
72 4.15321493148804
73 4.21249628067017
74 4.31674146652222
75 4.45229339599609
76 4.65660429000854
77 4.86458778381348
78 5.07604885101318
79 5.29441738128662
80 5.5302562713623
81 5.90218925476074
82 6.21348428726196
83 5.93826103210449
84 5.66446685791016
85 5.4006142616272
86 5.24584674835205
87 5.07457494735718
88 4.84850645065308
89 4.69984769821167
90 4.58130264282227
91 4.40765619277954
92 4.14326190948486
93 4.70757675170898
94 6.94486331939697
95 5.9861626625061
96 4.43335866928101
97 4.83475160598755
98 4.89929294586182
99 4.85421895980835
};
\addplot [semithick, color2]
table {%
0 12.8906888961792
1 13.454155921936
2 17.9447479248047
3 17.1155376434326
4 17.4301528930664
5 21.6228904724121
6 21.9014854431152
7 16.8690814971924
8 19.4332904815674
9 17.5772285461426
10 19.58127784729
11 18.5124092102051
12 18.0864505767822
13 13.9133195877075
14 14.7403049468994
15 11.89870262146
16 15.544581413269
17 14.3290176391602
18 17.8903007507324
19 17.8980178833008
20 16.7395362854004
21 11.6898498535156
22 12.433331489563
23 14.5895404815674
24 12.9993867874146
25 13.282940864563
26 13.9165315628052
27 10.6670951843262
28 13.4154081344604
29 13.4494781494141
30 11.8683252334595
31 13.7494430541992
32 14.5275030136108
33 13.3267936706543
34 12.5464420318604
35 11.6320552825928
36 12.7073497772217
37 12.8481941223145
38 12.521523475647
39 12.5756902694702
40 13.9495058059692
41 14.5513648986816
42 12.0408926010132
43 14.2739219665527
44 13.0978240966797
45 15.6608047485352
46 13.3998985290527
47 24.37353515625
48 17.4679088592529
49 20.0570106506348
50 27.3241367340088
51 33.6575393676758
52 48.8756294250488
53 61.6944122314453
54 89.903923034668
55 157.221633911133
56 127.46639251709
57 249.074249267578
58 286.438446044922
59 267.146484375
60 357.139801025391
61 416.55859375
62 373.772399902344
63 444.254028320312
64 357.618682861328
65 320.173736572266
66 253.749206542969
67 219.035217285156
68 257.380523681641
69 -28.8058853149414
70 127.662750244141
71 81.5289688110352
72 41.259578704834
73 46.9345092773438
74 32.882396697998
75 26.2465324401855
76 19.5263671875
77 25.6624393463135
78 18.452465057373
79 16.4257049560547
80 21.8155632019043
81 12.569239616394
82 24.2968006134033
83 19.3267440795898
84 17.2964534759521
85 11.6883592605591
86 17.4283828735352
87 18.4725589752197
88 19.8368434906006
89 13.8700437545776
90 21.8737716674805
91 20.9925136566162
92 20.8696956634521
93 16.5168113708496
94 18.8141841888428
95 16.5410861968994
96 14.5139141082764
97 16.3099327087402
98 18.0060043334961
99 17.074104309082
};
\addplot [semithick, color3]
table {%
0 24.3460693359375
1 24.3135623931885
2 27.5234756469727
3 24.3290500640869
4 28.2120532989502
5 24.0775413513184
6 24.6986217498779
7 23.6006031036377
8 27.5437679290771
9 24.1418151855469
10 24.0261745452881
11 23.8712997436523
12 24.6631145477295
13 27.9328498840332
14 23.6546211242676
15 27.3162670135498
16 -8.05002784729004
17 24.6529674530029
18 25.4550514221191
19 -9.21949100494385
20 24.3519477844238
21 28.6228656768799
22 -10.6795606613159
23 25.3210983276367
24 25.5798778533936
25 29.4506492614746
26 -11.1036262512207
27 26.1587715148926
28 26.5545806884766
29 -10.2251672744751
30 30.4734191894531
31 30.3785152435303
32 27.1197204589844
33 -6.53625297546387
34 26.1212711334229
35 -8.73891258239746
36 27.4642372131348
37 27.189811706543
38 -5.07689762115479
39 -3.75507164001465
40 -8.50116062164307
41 29.492769241333
42 -8.16585254669189
43 30.5630836486816
44 41.1739768981934
45 34.8739738464355
46 32.2362442016602
47 36.58642578125
48 41.9578514099121
49 38.2809715270996
50 45.7529830932617
51 68.3292846679688
52 79.0842819213867
53 131.925994873047
54 186.306182861328
55 209.226303100586
56 285.866455078125
57 399.562561035156
58 466.364227294922
59 465.184204101562
60 416.832733154297
61 421.8017578125
62 278.504302978516
63 246.54817199707
64 456.489288330078
65 307.732452392578
66 340.699615478516
67 256.615600585938
68 48.9527244567871
69 141.872985839844
70 79.91650390625
71 13.8799209594727
72 24.0339660644531
73 48.0423164367676
74 42.4251251220703
75 37.0151481628418
76 37.3628807067871
77 -5.74064207077026
78 27.9885196685791
79 -1.48956716060638
80 -8.38218879699707
81 -3.25861644744873
82 30.5852470397949
83 29.5990772247314
84 -6.47218227386475
85 29.6241245269775
86 27.3342971801758
87 -11.1402006149292
88 25.1730499267578
89 -11.6314897537231
90 25.3506183624268
91 24.7056541442871
92 -12.4025506973267
93 27.1903991699219
94 24.3086433410645
95 24.3794116973877
96 24.8016872406006
97 -9.47407531738281
98 24.3966045379639
99 24.3603801727295
};
\addplot [semithick, black]
table {%
0 0.369304749393011
1 0.251627312445023
2 0.166828486662018
3 0.114919508975367
4 0.0876551054424964
5 0.0972479334811367
6 0.278861922571797
7 0.682278798237165
8 0.898430150916583
9 0.950054611239325
10 1.05749517986891
11 -0.0194579789814049
12 0.41906978660397
13 0.90600420752663
14 0.607716836161893
15 -0.675775545085891
16 -2.02911349358568
17 -1.90876401269036
18 0.442358711320452
19 4.76486332143231
20 10.1117550482063
21 15.46241013662
22 19.6950163590587
23 21.8586836686028
24 22.5426933866117
25 22.8014199391233
26 23.2637810931226
27 24.714325114964
28 26.9026173790791
29 29.2789606239994
30 30.7213507703577
31 31.1075348607625
32 31.1251471191154
33 31.2782300570256
34 32.0578903196936
35 33.5575376024208
36 35.3940636590916
37 37.0246703256569
38 38.0282052819037
39 38.4824588899673
40 38.5759249571389
41 38.5046571339107
42 38.2258670710893
43 37.3873142684391
44 35.871680146895
45 34.2111375586938
46 33.5096272296361
47 35.418396288732
48 41.3909083744007
49 52.6668316564875
50 69.9984627356415
51 93.2886232931656
52 122.093275988026
53 160.79716375882
54 209.836521166767
55 257.811589325816
56 297.622676042388
57 321.481759574333
58 327.808179759924
59 297.975723143205
60 248.173711578614
61 190.900140829586
62 129.437394860253
63 86.8872183810078
64 57.3908472935429
65 36.9572371119832
66 22.7760464380614
67 12.8754222825192
68 5.89940427992587
69 1.20506659146156
70 -0.9932840418485
71 -1.46420380865569
72 -1.27971042491066
73 -0.96526440616734
74 -0.701033528262978
75 -0.489352273911556
76 -0.328602513226582
77 -0.215930995594116
78 -0.137827720624021
79 -0.0840823033998235
80 -0.0483471257928688
81 -0.0243421308267174
82 -0.00827723559179142
83 0.00133048504507427
84 0.0063358997290732
85 0.00842422570503067
86 0.00858785405350789
87 0.00773657072400436
88 0.00696891743975518
89 0.0209640682355403
90 0.0381210011915714
91 0.0687230903391171
92 0.134428495741537
93 0.257636952146907
94 0.339643430286094
95 0.606937550381734
96 0.801347319968563
97 0.769398612233424
98 0.498720068569826
99 0.360528806528182
};



==> plots/dl/m/TibialisAnterior.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 6.30845928192139
1 -7.09251594543457
2 -26.7360744476318
3 -32.3331642150879
4 -31.7229843139648
5 -27.8934650421143
6 -20.5503082275391
7 -12.4468641281128
8 -6.31457185745239
9 -2.03963041305542
10 2.96678066253662
11 6.27243947982788
12 6.83601140975952
13 6.96128606796265
14 7.00279760360718
15 6.99036884307861
16 6.98199939727783
17 6.96644639968872
18 6.90119409561157
19 6.75715637207031
20 6.51232671737671
21 6.13808536529541
22 5.46551847457886
23 4.5669903755188
24 3.85185861587524
25 3.41702365875244
26 3.140958070755
27 2.99885821342468
28 2.92377686500549
29 2.89794588088989
30 2.90760064125061
31 2.94259238243103
32 2.9954297542572
33 3.06052470207214
34 3.13420510292053
35 3.21381545066833
36 3.29598832130432
37 3.37920784950256
38 3.46247243881226
39 3.54511094093323
40 3.62671828269958
41 3.70710301399231
42 3.78615522384644
43 3.86385321617126
44 3.93467664718628
45 4.00303936004639
46 4.06934213638306
47 4.13284969329834
48 4.19262886047363
49 4.25522613525391
50 4.31384611129761
51 4.36478614807129
52 4.40746164321899
53 4.4417986869812
54 4.46775579452515
55 4.48576641082764
56 4.49824523925781
57 4.51212024688721
58 4.55269956588745
59 4.75423240661621
60 6.83544063568115
61 16.304012298584
62 9.58553886413574
63 10.526704788208
64 27.6519393920898
65 11.4694242477417
66 -0.307712644338608
67 -0.00439424486830831
68 -1.1173849105835
69 -3.04448318481445
70 -2.32361030578613
71 1.07856285572052
72 5.36777019500732
73 7.24346208572388
74 10.8135032653809
75 13.6357936859131
76 13.2527914047241
77 10.6117906570435
78 8.0116138458252
79 6.28129529953003
80 6.13720273971558
81 6.58037948608398
82 6.92388772964478
83 6.79319715499878
84 6.06630086898804
85 6.06592273712158
86 5.61764097213745
87 4.49564123153687
88 2.25754022598267
89 0.640442609786987
90 0.0545830279588699
91 -1.4314022064209
92 -2.06547379493713
93 -1.17924833297729
94 0.511003494262695
95 2.47399425506592
96 4.69059228897095
97 6.88400363922119
98 10.7598752975464
99 45.9143905639648
};
\addplot [semithick, color1]
table {%
0 110.939918518066
1 103.320930480957
2 13.6256408691406
3 0.0544925034046173
4 -0.986287474632263
5 0.775772213935852
6 2.75143504142761
7 4.84780168533325
8 9.99531269073486
9 15.2359409332275
10 10.5400762557983
11 11.5948886871338
12 11.1759405136108
13 8.94483375549316
14 7.17855453491211
15 6.44140529632568
16 6.1123685836792
17 5.97418403625488
18 5.93861150741577
19 6.00853443145752
20 6.13368844985962
21 6.21642112731934
22 6.29061698913574
23 6.38794612884521
24 6.47162485122681
25 6.56556129455566
26 6.65076446533203
27 6.62722444534302
28 6.53533840179443
29 6.4928994178772
30 6.4862265586853
31 6.505202293396
32 6.5423846244812
33 6.592200756073
34 6.6505389213562
35 6.65735530853271
36 6.63187885284424
37 6.605872631073
38 6.57970094680786
39 6.55361843109131
40 6.52777099609375
41 6.50222873687744
42 6.47703313827515
43 6.45219326019287
44 6.42773151397705
45 6.40377426147461
46 6.38051176071167
47 6.35823917388916
48 6.33959531784058
49 6.32272338867188
50 6.30767726898193
51 6.29471254348755
52 6.28401041030884
53 6.27560091018677
54 6.26950836181641
55 6.26563453674316
56 6.26332664489746
57 6.26070594787598
58 6.25084924697876
59 6.19851779937744
60 5.92752313613892
61 17.9888496398926
62 12.8482732772827
63 5.51022100448608
64 4.10704660415649
65 4.3932466506958
66 5.48429584503174
67 8.65632152557373
68 12.9578857421875
69 13.2353868484497
70 9.74352073669434
71 8.15050888061523
72 7.4144287109375
73 14.4242076873779
74 35.8774642944336
75 60.7799415588379
76 62.8056945800781
77 44.3203620910645
78 27.1401500701904
79 13.1751489639282
80 8.51137828826904
81 9.60569763183594
82 14.1968193054199
83 16.1612281799316
84 11.5213012695312
85 9.94042205810547
86 17.7923011779785
87 10.7267837524414
88 8.12473297119141
89 7.05646705627441
90 6.55357694625854
91 5.80362272262573
92 5.47125387191772
93 5.68989229202271
94 5.97388744354248
95 6.50821542739868
96 6.35712289810181
97 9.9740047454834
98 39.3430137634277
99 150.397521972656
};
\addplot [semithick, color2]
table {%
0 24.4985885620117
1 20.179500579834
2 17.5909023284912
3 13.9868764877319
4 11.5332622528076
5 10.4324340820312
6 11.9578676223755
7 11.7728433609009
8 13.3400630950928
9 11.9480228424072
10 10.8519353866577
11 11.8300151824951
12 9.49459362030029
13 12.5054035186768
14 11.7376546859741
15 11.6936054229736
16 12.4046640396118
17 13.0076866149902
18 13.3611249923706
19 12.9143972396851
20 13.7905921936035
21 12.0789985656738
22 13.1564979553223
23 13.3932752609253
24 12.9380569458008
25 13.5294036865234
26 13.3105125427246
27 18.4703998565674
28 18.2615852355957
29 18.1247749328613
30 19.4451675415039
31 15.9441232681274
32 15.2845067977905
33 16.7521095275879
34 15.6132955551147
35 16.2237491607666
36 18.961030960083
37 15.8760833740234
38 19.7017803192139
39 15.4742822647095
40 14.9647493362427
41 14.1951847076416
42 11.3972644805908
43 13.8858823776245
44 14.8823051452637
45 16.8417701721191
46 15.4469709396362
47 10.1863508224487
48 16.7829627990723
49 13.7680988311768
50 15.1692523956299
51 12.8338603973389
52 16.882791519165
53 17.7988567352295
54 14.7241535186768
55 13.8956365585327
56 15.1914882659912
57 13.2784900665283
58 14.8951215744019
59 17.7578659057617
60 16.620454788208
61 16.3162136077881
62 12.528904914856
63 11.2673807144165
64 14.7277030944824
65 18.0621719360352
66 12.7495584487915
67 18.0632972717285
68 14.2308769226074
69 12.7270059585571
70 14.0359859466553
71 8.79102993011475
72 9.71462726593018
73 9.03211498260498
74 14.3338222503662
75 10.2495002746582
76 14.2615976333618
77 10.3469400405884
78 12.9953365325928
79 11.9252605438232
80 10.2827796936035
81 11.7682209014893
82 11.5467739105225
83 10.4715719223022
84 9.4329948425293
85 10.7231416702271
86 11.7748870849609
87 10.5340709686279
88 12.0967292785645
89 12.697340965271
90 11.7930927276611
91 11.1513137817383
92 15.0592651367188
93 13.9178647994995
94 16.2161102294922
95 16.767448425293
96 16.7631072998047
97 14.6947860717773
98 13.3416042327881
99 11.1146831512451
};
\addplot [semithick, color3]
table {%
0 31.6767272949219
1 41.2884140014648
2 67.17529296875
3 -5.99295854568481
4 24.9372234344482
5 21.3942031860352
6 23.3906669616699
7 24.6088924407959
8 27.1536865234375
9 -12.4039840698242
10 -13.7170877456665
11 26.2732601165771
12 23.3756160736084
13 -13.5868263244629
14 22.5883922576904
15 25.0055484771729
16 23.9581336975098
17 27.0368461608887
18 26.2540245056152
19 26.6027927398682
20 24.6368732452393
21 23.3640632629395
22 27.7045783996582
23 27.7240581512451
24 -13.1164770126343
25 28.1357135772705
26 -7.62544059753418
27 29.1399097442627
28 24.2564430236816
29 30.8389835357666
30 27.704174041748
31 28.8939418792725
32 31.8222141265869
33 31.6835460662842
34 27.2093563079834
35 30.0197010040283
36 31.4452972412109
37 30.846809387207
38 32.1920890808105
39 30.8724727630615
40 32.0506706237793
41 -13.0484294891357
42 30.5519466400146
43 24.0549640655518
44 28.6398525238037
45 34.5746841430664
46 31.9085636138916
47 -5.38276052474976
48 23.5280933380127
49 28.3788242340088
50 24.0197601318359
51 33.7093238830566
52 32.6550331115723
53 27.475700378418
54 25.7455711364746
55 28.95725440979
56 29.2954597473145
57 31.5661487579346
58 27.5576019287109
59 29.0757598876953
60 32.5235176086426
61 28.636157989502
62 25.6338806152344
63 -7.09927749633789
64 30.4532527923584
65 29.30517578125
66 -10.1815624237061
67 27.6921005249023
68 -12.1363439559937
69 24.8427276611328
70 24.0809154510498
71 26.5383567810059
72 -12.916332244873
73 -13.2678117752075
74 26.986852645874
75 23.6278305053711
76 24.0887012481689
77 -13.1528635025024
78 -13.7869520187378
79 23.6818656921387
80 23.308219909668
81 22.9239768981934
82 23.5904998779297
83 24.5627593994141
84 23.8563079833984
85 -13.271824836731
86 -12.4086942672729
87 23.9670467376709
88 26.3445415496826
89 23.6195869445801
90 24.1922740936279
91 23.6321506500244
92 26.9013843536377
93 27.0431995391846
94 27.6065502166748
95 -13.2192802429199
96 27.8614692687988
97 26.2461452484131
98 26.1826362609863
99 -6.01077604293823
};
\addplot [semithick, black]
table {%
0 23.5595005139448
1 32.8138071776856
2 21.3210141608961
3 1.63083548601132
4 -11.6715618767212
5 -11.8203228049121
6 -2.22701376466097
7 8.63636621810401
8 15.8924601326745
9 16.6911089278124
10 11.8338438424907
11 8.5441254569367
12 5.93324317356977
13 3.96718490992338
14 2.61441199525876
15 1.73197206754626
16 1.15909089136053
17 0.780109780401285
18 0.52351916610521
19 0.347879507897762
20 0.227286725926249
21 0.145310413446369
22 0.0872823149418162
23 0.0476056717260574
24 0.0256730922948858
25 0.014202960194245
26 0.00824824929830739
27 0.00517230904451075
28 0.00355638060203216
29 0.00267353408784941
30 0.00216339535426995
31 0.00185265930414941
32 0.00165886519136919
33 0.00154214362109051
34 0.00148175312145087
35 0.00146482413972526
36 0.00148167917948568
37 0.00152429841487741
38 0.00158606678653515
39 0.0016615163994928
40 0.00174634162357476
41 0.00183733388319728
42 0.00193219280813492
43 0.00202938977482573
44 0.00212770572604792
45 0.00222567043306402
46 0.00232146851860461
47 0.00241287178002422
48 0.00249739574794579
49 0.0025726150639841
50 0.00263656194297333
51 0.00268908213776372
52 0.00273538304658145
53 0.00279895200459941
54 0.00290861264390923
55 0.00309465806480748
56 0.00341664783602837
57 0.0040053439903195
58 0.00521820333094884
59 0.00865687217387175
60 0.0306811861265764
61 0.27982416435499
62 0.528779982587619
63 0.0533403079234887
64 -1.09409733633836
65 -0.135240181478355
66 4.00926590303062
67 10.9503746389028
68 18.8348994485813
69 22.0184019707722
70 16.8620113553698
71 12.5127653114581
72 10.22056852383
73 9.7270559317688
74 11.3197927775736
75 13.9504448253527
76 15.3357708205386
77 14.2146041542264
78 11.2202543592428
79 8.00281650290632
80 5.83227254139521
81 4.88788051388032
82 4.74349909543525
83 4.84952469595884
84 4.58702934601007
85 4.28640793970892
86 5.48868930491915
87 5.14334804539915
88 4.38814374649155
89 3.54063644858634
90 3.08257499630652
91 2.42962739421142
92 0.99954975548358
93 0.419171771313
94 0.463994669502424
95 0.544806531638373
96 0.888516283450327
97 2.54330523195761
98 5.64523455142928
99 16.6493902303441
};



==> plots/dl/m/Vasti.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot[semithick, color0]
table {%
0 2.63950085639954
1 1.13416028022766
2 1.68378376960754
3 -6.17559432983398
4 -10.6394920349121
5 -14.419322013855
6 -17.7769374847412
7 -21.0532531738281
8 -23.7874412536621
9 -24.5046653747559
10 -23.5300407409668
11 -17.2858505249023
12 -8.04077434539795
13 6.7978048324585
14 25.082799911499
15 70.2064361572266
16 95.8495635986328
17 94.8024063110352
18 74.3761901855469
19 45.1341819763184
20 19.2860507965088
21 12.4713268280029
22 9.28880310058594
23 7.85444068908691
24 7.48370599746704
25 8.48311519622803
26 8.65256023406982
27 8.73360824584961
28 7.98904800415039
29 6.82587623596191
30 5.19966650009155
31 3.61522626876831
32 2.47123289108276
33 1.36947774887085
34 0.522700011730194
35 -0.223345726728439
36 -0.82368391752243
37 -0.988669157028198
38 -0.396385937929153
39 0.11129642277956
40 0.328358083963394
41 0.185026377439499
42 -0.149414256215096
43 -0.675630390644073
44 -1.4347095489502
45 -2.29203915596008
46 -3.32087349891663
47 -4.44729852676392
48 -5.72677755355835
49 -6.93126678466797
50 -7.77368402481079
51 -7.90405941009521
52 -4.05087995529175
53 1.00693106651306
54 7.22675037384033
55 13.7352352142334
56 20.1160717010498
57 28.5862331390381
58 36.2647323608398
59 42.7187576293945
60 48.036376953125
61 52.1239204406738
62 54.5593910217285
63 55.8436622619629
64 55.763298034668
65 54.2535667419434
66 51.8863143920898
67 49.1683158874512
68 45.9810829162598
69 42.08349609375
70 38.3609733581543
71 34.6023597717285
72 29.874095916748
73 23.2197132110596
74 19.9541530609131
75 5.95113754272461
76 -8.78018569946289
77 -22.6595439910889
78 -38.0008239746094
79 -55.2126274108887
80 -80.9210052490234
81 -110.361061096191
82 -135.788024902344
83 -158.233245849609
84 -176.304458618164
85 -187.02018737793
86 -196.111907958984
87 -166.427093505859
88 -82.8268356323242
89 -13.142707824707
90 22.4363803863525
91 22.0028095245361
92 14.8521528244019
93 -51.5493507385254
94 -67.587776184082
95 -76.7129135131836
96 -72.0627136230469
97 -78.5123977661133
98 -114.555511474609
99 -140.666519165039
};
\addplot [semithick, color1]
table {%
0 15.1553630828857
1 9.50832939147949
2 5.44195699691772
3 4.26555156707764
4 2.93520975112915
5 2.16091156005859
6 1.19101214408875
7 0.167071521282196
8 0.416624873876572
9 2.98385405540466
10 8.944504737854
11 17.0400390625
12 32.9632759094238
13 76.3786010742188
14 136.310607910156
15 182.099563598633
16 200.372955322266
17 191.999603271484
18 170.331741333008
19 144.055435180664
20 119.220581054688
21 105.246711730957
22 105.327621459961
23 111.173377990723
24 118.276092529297
25 123.389923095703
26 125.175926208496
27 122.342720031738
28 116.592010498047
29 110.95100402832
30 104.726181030273
31 98.7029418945312
32 92.0984497070312
33 85.1257019042969
34 77.8305892944336
35 70.2954254150391
36 63.4948654174805
37 57.3226280212402
38 51.9209136962891
39 47.5615577697754
40 43.2863349914551
41 38.1392021179199
42 32.3415908813477
43 26.2754077911377
44 20.1253528594971
45 14.1836376190186
46 9.72940731048584
47 8.27234745025635
48 7.5373797416687
49 6.73221635818481
50 5.83719968795776
51 5.03488683700562
52 4.26562547683716
53 3.34155368804932
54 2.55122637748718
55 2.13195824623108
56 1.77877080440521
57 1.62724220752716
58 1.46533024311066
59 1.41346406936646
60 1.35263395309448
61 1.27381420135498
62 1.39622938632965
63 1.60107517242432
64 1.76015472412109
65 1.82338929176331
66 1.96045005321503
67 2.44935202598572
68 3.44762468338013
69 4.71862125396729
70 6.14338111877441
71 6.69479131698608
72 8.6583194732666
73 19.4663124084473
74 32.7858695983887
75 35.7400970458984
76 2.70425367355347
77 -30.7395782470703
78 -63.1468772888184
79 -92.6748733520508
80 -122.882247924805
81 -144.617721557617
82 -162.013198852539
83 -176.78076171875
84 -185.628692626953
85 -203.400726318359
86 -221.079116821289
87 -199.541061401367
88 -128.19319152832
89 -67.811164855957
90 3.23380899429321
91 56.5455436706543
92 -27.5475330352783
93 -98.2837829589844
94 -119.769371032715
95 -129.446655273438
96 -127.716125488281
97 -135.800628662109
98 -164.491638183594
99 -188.521926879883
};
\addplot [semithick, color2]
table {%
0 36.6324348449707
1 37.8410263061523
2 29.5543613433838
3 39.6204566955566
4 32.872184753418
5 24.1819553375244
6 24.4742736816406
7 24.3729972839355
8 18.8621196746826
9 20.9540538787842
10 14.4070358276367
11 16.5405578613281
12 18.0112800598145
13 19.0971622467041
14 23.3342819213867
15 26.9315605163574
16 34.8092002868652
17 45.6413345336914
18 39.6457481384277
19 36.4423522949219
20 25.2612628936768
21 25.0771999359131
22 21.1665840148926
23 20.2322101593018
24 19.5052928924561
25 22.5731105804443
26 33.0685539245605
27 19.6189422607422
28 21.1506881713867
29 16.2232666015625
30 15.5091466903687
31 15.5557556152344
32 14.8595943450928
33 13.2465496063232
34 13.8123435974121
35 15.6597719192505
36 15.5883159637451
37 15.9854459762573
38 16.3668727874756
39 13.4392766952515
40 19.1746082305908
41 25.8883438110352
42 24.3961849212646
43 22.4686450958252
44 29.8025989532471
45 27.0525760650635
46 28.4128303527832
47 32.0111351013184
48 19.114465713501
49 24.8868865966797
50 25.4693775177002
51 25.222074508667
52 23.6085643768311
53 26.0017776489258
54 25.931713104248
55 31.5881004333496
56 27.6070690155029
57 29.97145652771
58 27.0638046264648
59 34.8288726806641
60 42.1251640319824
61 34.0272483825684
62 38.1686820983887
63 41.4867362976074
64 39.036018371582
65 47.5739631652832
66 43.8867111206055
67 39.3101348876953
68 35.5914611816406
69 35.7718772888184
70 43.2754173278809
71 35.731502532959
72 27.568323135376
73 39.2540321350098
74 24.4087886810303
75 31.3740520477295
76 35.3926162719727
77 39.7596702575684
78 28.7399673461914
79 33.5511131286621
80 36.6936492919922
81 36.5497665405273
82 39.8185806274414
83 36.606086730957
84 38.5490379333496
85 41.9538345336914
86 38.4580879211426
87 13.086877822876
88 -14.401894569397
89 32.1616630554199
90 47.7009391784668
91 16.0210437774658
92 19.7995166778564
93 23.8053188323975
94 36.8998794555664
95 4.74583148956299
96 40.0486183166504
97 26.4811782836914
98 20.3904876708984
99 -9.09677791595459
};
\addplot [semithick, color3]
table {%
0 -22.4806861877441
1 -19.1462230682373
2 -15.2734842300415
3 38.2668266296387
4 5.22016525268555
5 1.41987538337708
6 -5.04877281188965
7 -1.74075031280518
8 0.796704947948456
9 -1.71076381206512
10 11.684229850769
11 -8.14396381378174
12 29.7884826660156
13 23.7698879241943
14 -3.4384183883667
15 -5.18140554428101
16 1.46538090705872
17 15.9780426025391
18 27.3466682434082
19 15.6523551940918
20 -3.00978899002075
21 37.1136093139648
22 72.8619079589844
23 56.0746192932129
24 88.1121978759766
25 68.3914337158203
26 -8.80608463287354
27 25.9234638214111
28 51.2570457458496
29 -10.1986999511719
30 25.8717441558838
31 27.1771869659424
32 34.9366836547852
33 27.1500587463379
34 -14.1092987060547
35 30.2246398925781
36 27.6195678710938
37 27.4336986541748
38 27.1908702850342
39 -9.54705047607422
40 27.9274845123291
41 34.170783996582
42 31.8033313751221
43 -5.42891693115234
44 33.0926704406738
45 32.0202789306641
46 35.1188621520996
47 39.9627532958984
48 35.260311126709
49 1.9386579990387
50 7.53109550476074
51 3.76478314399719
52 41.4347152709961
53 42.9221572875977
54 42.8921089172363
55 39.8275299072266
56 47.2885932922363
57 48.4940948486328
58 -7.06709003448486
59 33.0632972717285
60 49.865650177002
61 32.5483512878418
62 44.2157669067383
63 12.8813161849976
64 31.4770126342773
65 23.8184547424316
66 19.1044692993164
67 12.3203783035278
68 25.8832874298096
69 -6.99543523788452
70 12.0809373855591
71 36.9189109802246
72 44.4584350585938
73 30.7381000518799
74 44.6268196105957
75 6.48893260955811
76 41.2576026916504
77 29.4007740020752
78 -8.03177928924561
79 23.3445053100586
80 35.473690032959
81 32.5171661376953
82 11.3056688308716
83 14.9474115371704
84 15.2309160232544
85 -75.8846435546875
86 -112.019554138184
87 -115.565277099609
88 -246.817443847656
89 -231.793853759766
90 -172.294372558594
91 -202.916076660156
92 -212.023193359375
93 -190.665679931641
94 -128.8271484375
95 -149.695999145508
96 -94.7362518310547
97 -85.1014099121094
98 -74.7399826049805
99 -85.0432510375977
};
\addplot [semithick, black]
table {%
0 1.07107345822998
1 0.655740200504042
2 -0.383627680652003
3 -2.1948180483985
4 -5.10621878261905
5 -9.11923043868085
6 -14.7004500527399
7 -21.9350030372119
8 -27.4069329717225
9 -22.8641124962668
10 0.166451386368252
11 42.1947614116122
12 94.4440790631183
13 145.75553356627
14 188.05083817864
15 222.051205289123
16 238.640540963086
17 237.45382591247
18 224.381095849117
19 205.588809659102
20 186.959440599729
21 172.150218097517
22 162.101590317451
23 155.498508282063
24 149.824504540188
25 142.859866829939
26 133.815672736104
27 122.010773110715
28 108.750085495716
29 95.7086613836883
30 83.7007241139982
31 73.6524385896103
32 65.195970397078
33 57.5334174166683
34 50.2739463081901
35 43.5173653471146
36 37.3162608637911
37 31.8982571682427
38 27.3506141483287
39 23.572033376147
40 20.2559357013746
41 17.0742927279236
42 14.0324649638656
43 11.328279470745
44 9.20110793789204
45 7.53457750199643
46 6.3103300701289
47 5.29401832152974
48 4.34634397342728
49 3.18737867179429
50 1.51249267654242
51 -0.557992636038998
52 -2.69899807716784
53 -5.29393868335751
54 -8.66698262951666
55 -11.8916279458246
56 -17.2620142595466
57 -20.6992817882201
58 -20.3034274765342
59 -17.5923082040834
60 -14.6271090086366
61 -11.7715789009087
62 -9.09789957253753
63 -6.80066781376597
64 -4.87424035377157
65 -3.33503347968858
66 -2.19081738107032
67 -1.39378081561575
68 -0.845903429914448
69 -0.479172365704627
70 -0.253175279896633
71 -0.114532110004941
72 -0.0228932559291446
73 0.19745786698595
74 1.84120513578368
75 5.3434366939768
76 10.0461314311425
77 14.7133680749927
78 18.1460021455863
79 19.3456331831056
80 19.4869202423773
81 19.8747680245836
82 20.6563029009021
83 21.8402438109105
84 22.9950376711948
85 20.2301617450475
86 14.1714265655387
87 9.43219878525255
88 5.9032375281645
89 3.62676551099744
90 2.2160240601327
91 1.40699542019955
92 1.39637736743438
93 4.04996178470269
94 4.43749951701865
95 4.66567886195184
96 4.60993091568304
97 4.4064535593475
98 4.83263401593551
99 5.46388743811519
};



==> plots/dl/m/m4_fc.tex <==
\addplot [semithick, color0]
table {%
0 9.32949161529541
1 13.182201385498
2 20.8602142333984
3 25.8808917999268
4 27.1183910369873
5 17.0219326019287
6 -14.6922369003296
7 -37.1520690917969
8 -41.4078483581543
9 -40.1196708679199
10 30.0456733703613
11 75.4299392700195
12 73.5674591064453
13 73.8047180175781
14 76.2078018188477
15 78.7337112426758
16 79.6546783447266
17 79.793815612793
18 78.7015686035156
19 74.3752899169922
20 67.3976974487305
21 61.0654220581055
22 57.691535949707
23 56.8278617858887
24 56.6649475097656
25 56.8557205200195
26 56.5412712097168
27 54.8743362426758
28 52.3914070129395
29 50.1433372497559
30 49.3940696716309
31 49.9452743530273
32 50.89892578125
33 51.6494674682617
34 51.7062034606934
35 51.0753936767578
36 50.223560333252
37 49.6589088439941
38 49.6640281677246
39 47.2142028808594
40 44.3696479797363
41 41.3938865661621
42 38.223201751709
43 35.1587982177734
44 30.0380992889404
45 24.2029724121094
46 15.7934579849243
47 5.25384855270386
48 -6.89436674118042
49 -23.1380863189697
50 -43.4958534240723
51 -18.819019317627
52 29.4876518249512
53 105.458709716797
54 198.961090087891
55 273.155151367188
56 318.716064453125
57 335.313690185547
58 341.258117675781
59 289.135345458984
60 193.674743652344
61 98.1533584594727
62 9.46989345550537
63 -38.9930381774902
64 -51.0865440368652
65 -37.4884796142578
66 -4.84490585327148
67 -32.491943359375
68 -13.1817827224731
69 39.3356552124023
70 80.4028930664062
71 86.462287902832
72 87.9669723510742
73 88.3783493041992
74 88.5019073486328
75 88.3814926147461
76 87.9648056030273
77 87.4077529907227
78 86.7785415649414
79 86.0459899902344
80 85.0469284057617
81 83.7129821777344
82 81.7400665283203
83 77.1368865966797
84 71.1591110229492
85 63.5613212585449
86 56.1085548400879
87 50.044376373291
88 45.1807746887207
89 41.4747886657715
90 37.9075584411621
91 32.3040618896484
92 20.8067569732666
93 8.9938383102417
94 -1.53513753414154
95 1.90849280357361
96 18.5261535644531
97 32.2740707397461
98 37.7393798828125
99 37.088508605957
};


==> plots/dl/m/m4_lstm.tex <==

\addplot [semithick, color1]
table {%
0 15.1506805419922
1 15.1114673614502
2 15.1008787155151
3 15.1075420379639
4 15.1172904968262
5 15.1008882522583
6 15.0219078063965
7 14.8896512985229
8 14.745020866394
9 14.6407079696655
10 14.7363510131836
11 14.9725742340088
12 15.1558103561401
13 15.3037672042847
14 15.434419631958
15 15.5522613525391
16 15.6536884307861
17 15.7361450195312
18 15.7952165603638
19 15.8274803161621
20 15.8360166549683
21 15.8264656066895
22 15.8050546646118
23 15.7762813568115
24 15.7431154251099
25 15.7097587585449
26 15.679705619812
27 15.6524858474731
28 15.6285524368286
29 15.6089582443237
30 15.5934467315674
31 15.58092212677
32 15.5715560913086
33 15.5656538009644
34 15.5632514953613
35 15.5640983581543
36 15.5674619674683
37 15.5722618103027
38 15.5772848129272
39 15.5819158554077
40 15.5967102050781
41 15.6346387863159
42 15.6802806854248
43 15.7955141067505
44 15.9482679367065
45 16.1466388702393
46 16.4185314178467
47 16.7622833251953
48 17.1336631774902
49 17.5698986053467
50 18.1270179748535
51 18.925666809082
52 20.7277145385742
53 24.060884475708
54 30.5924949645996
55 41.9391098022461
56 59.1263046264648
57 83.408935546875
58 113.990951538086
59 145.350860595703
60 170.41584777832
61 186.196090698242
62 194.432510375977
63 198.702682495117
64 200.485717773438
65 200.842971801758
66 200.359191894531
67 199.359451293945
68 197.922821044922
69 195.864364624023
70 192.944305419922
71 188.971176147461
72 183.475021362305
73 176.195526123047
74 165.951538085938
75 151.022048950195
76 128.691253662109
77 97.3057861328125
78 62.702693939209
79 35.6067008972168
80 20.4887714385986
81 15.3167848587036
82 15.1587171554565
83 15.5229253768921
84 15.7639036178589
85 15.8599729537964
86 15.8737878799438
87 15.8370199203491
88 15.7757797241211
89 15.7044944763184
90 15.6301460266113
91 15.551157951355
92 15.4599838256836
93 15.3558044433594
94 15.246431350708
95 15.1658878326416
96 15.1356678009033
97 15.1496706008911
98 15.1782960891724
99 15.1999053955078
};

==> plots/dl/m/m8_fc.tex <==

\addplot [semithick, color2]
table {%
0 2.58892941474915
1 2.6107702255249
2 2.63383960723877
3 2.64688658714294
4 2.65161442756653
5 2.6283483505249
6 2.53247737884521
7 6.53533411026001
8 16.1728248596191
9 5.15446758270264
10 2.76206231117249
11 14.174186706543
12 3.39631700515747
13 3.08393931388855
14 3.15542221069336
15 3.17500638961792
16 3.16940593719482
17 3.17422962188721
18 3.20775961875916
19 3.31142163276672
20 3.40684366226196
21 3.48627209663391
22 3.53024458885193
23 3.54652619361877
24 3.54956030845642
25 3.55073118209839
26 3.55082964897156
27 3.55999970436096
28 5.94501447677612
29 12.423225402832
30 15.5637559890747
31 15.8031158447266
32 15.8596591949463
33 16.6452140808105
34 19.2145919799805
35 23.6402626037598
36 28.6164207458496
37 33.7153739929199
38 37.5973968505859
39 40.7834014892578
40 44.5566673278809
41 49.2580337524414
42 54.4425811767578
43 59.1592254638672
44 63.3702049255371
45 67.7969818115234
46 73.6633377075195
47 83.1967086791992
48 98.2073211669922
49 118.590728759766
50 146.96305847168
51 182.467681884766
52 223.721710205078
53 278.715545654297
54 353.053985595703
55 407.622802734375
56 450.414978027344
57 475.329376220703
58 469.635986328125
59 408.890899658203
60 353.936645507812
61 309.859680175781
62 221.727569580078
63 150.371337890625
64 106.67406463623
65 119.675407409668
66 84.245361328125
67 43.4375190734863
68 2.74984526634216
69 19.1788024902344
70 31.6176109313965
71 35.6233901977539
72 36.6343002319336
73 36.4302864074707
74 35.8629455566406
75 34.8680229187012
76 33.5738334655762
77 32.204029083252
78 30.53342628479
79 28.3832874298096
80 25.8606624603271
81 23.0198497772217
82 19.374267578125
83 14.9175596237183
84 9.81864070892334
85 4.99623203277588
86 2.70692276954651
87 2.71321368217468
88 2.68516826629639
89 2.66530013084412
90 2.6535370349884
91 2.63812136650085
92 2.60912036895752
93 2.57011365890503
94 2.53963208198547
95 2.58630275726318
96 2.67482948303223
97 2.70976758003235
98 2.69412446022034
99 2.68436026573181
};

==> plots/dl/m/m8_lstm.tex <==
\addplot [semithick, color3]
table {%
0 17.0779647827148
1 17.1578426361084
2 17.2075233459473
3 17.2745990753174
4 17.369722366333
5 17.4375782012939
6 17.3624954223633
7 17.0751819610596
8 16.6043663024902
9 16.0929279327393
10 15.983512878418
11 16.534631729126
12 17.5341682434082
13 18.6798572540283
14 19.7510566711426
15 20.6397857666016
16 21.3112258911133
17 21.7675590515137
18 22.0213050842285
19 22.0942420959473
20 22.0198135375977
21 21.8424873352051
22 21.6132202148438
23 21.3761692047119
24 21.1617984771729
25 20.9888000488281
26 20.8604011535645
27 20.7740325927734
28 20.7239151000977
29 20.7108764648438
30 20.7375087738037
31 20.8056240081787
32 20.917573928833
33 21.0724754333496
34 21.2676162719727
35 21.5017852783203
36 21.776798248291
37 22.0973377227783
38 22.4684143066406
39 22.8946914672852
40 23.3791790008545
41 23.9244651794434
42 24.5338382720947
43 25.2107772827148
44 25.9574127197266
45 26.7731399536133
46 27.6517677307129
47 28.5863456726074
48 29.5736141204834
49 30.6227569580078
50 31.7744674682617
51 33.1285209655762
52 34.8984642028809
53 37.4533462524414
54 41.5156898498535
55 48.1687469482422
56 59.0469398498535
57 76.1620941162109
58 100.956146240234
59 131.148864746094
60 160.778427124023
61 184.327392578125
62 200.016372680664
63 209.840316772461
64 215.851348876953
65 219.410095214844
66 221.247634887695
67 221.738967895508
68 221.107543945312
69 219.493194580078
70 217.002532958984
71 213.67448425293
72 209.354736328125
73 203.590667724609
74 195.562210083008
75 184.090957641602
76 167.969848632812
77 146.688812255859
78 121.147987365723
79 94.2569961547852
80 70.2526550292969
81 52.0900192260742
82 39.9855880737305
83 32.5191535949707
84 28.0515995025635
85 25.3292961120605
86 23.5558986663818
87 22.284387588501
88 21.286901473999
89 20.4579238891602
90 19.7489376068115
91 19.1251277923584
92 18.5453472137451
93 17.9822120666504
94 17.4322967529297
95 16.9483871459961
96 16.6278533935547
97 16.5383586883545
98 16.6596698760986
99 16.9077796936035
};

==> plots/dl/m/main.tex <==
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019807843137}
\definecolor{color2}{rgb}{0.172549019807843,0.627450980392157,0.172549019807843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\begin{groupplot}[group style={group size=4 by 2,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.45]
\nextgroupplot[
title = {\footnotesize Gastrocnemius},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize MEE in \si{W}},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Gastrocnemius}

\nextgroupplot[
title = {\footnotesize Gluteals},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Gluteals}

\nextgroupplot[
title = {\footnotesize Hamstrings},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Hamstrings}


\nextgroupplot[
title = {\footnotesize Iliopsoas},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Iliopsoas}

\nextgroupplot[
title = {\footnotesize Rectus Femoris},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize MEE in \si{W}},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
xlabel={Gait Cycle in \si{\percent}},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/RectusFemoris}


\nextgroupplot[
title = {\footnotesize Soleus},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
xlabel={Gait Cycle in \si{\percent}},
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Soleus}


\nextgroupplot[
title = {\footnotesize Tibialis Anterior},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
xlabel={Gait Cycle in \si{\percent}},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/TibialisAnterior}


\nextgroupplot[
title = {\footnotesize Vasti},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xlabel={Gait Cycle in \si{\percent}},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-100,ymax=550,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
\input{plots/dl/m/Vasti}



\end{groupplot}

\end{tikzpicture}

==> plots/kimr/ankle.tex <==
\addplot [semithick, color1]
table {%
0 17.3298336894542
1 40.1561861837261
2 79.2446115259609
3 112.700510134692
4 116.811834253699
5 84.9998633312377
6 37.9186910302684
7 5.17853882049794
8 0.296075179738014
9 -0.866472067526597
10 -0.0463156449562497
11 2.59960416560378
12 35.5011998116984
13 67.299009185997
14 87.3772409472826
15 97.3827361881741
16 99.4349856727941
17 97.1003133877033
18 92.7946007539598
19 89.0637088029995
20 85.7421069394843
21 81.7262418462974
22 76.1375526380437
23 68.8962986026793
24 61.8545733645003
25 56.6620814068911
26 54.0631666986468
27 53.9126745346008
28 55.9176540749288
29 60.1827375560102
30 65.7390129318684
31 72.6871262283895
32 81.5312178105441
33 91.9639947618573
34 103.943000019319
35 117.705518903702
36 133.367679508827
37 150.712226786896
38 169.778534772718
39 190.470661164778
40 212.839398004153
41 237.575913550768
42 265.213079934521
43 296.168759681125
44 329.785619518502
45 362.073772453695
46 386.554430516992
47 395.962365102995
48 382.772204595987
49 341.391588435201
50 269.89872030595
51 168.950303529014
52 62.4843372609719
53 3.30791212663379
54 -14.9910785342285
55 -34.07702566193
56 -51.8081267389745
57 -65.3497272145326
58 -72.0342244843476
59 -70.0414230475107
60 -60.2304426295911
61 -45.9276639135185
62 -30.7699525237912
63 -17.8583681284843
64 -8.46477306516873
65 -2.13423829120407
66 3.61133323216527
67 10.4563877619133
68 11.2555230446201
69 4.93624935718359
70 2.2667901555005
71 1.83916745723319
72 1.84686560290413
73 2.03821435457357
74 2.14344071332523
75 2.06269926720847
76 1.86826682032699
77 1.69833776335352
78 1.66286872605574
79 1.79261494635452
80 2.02486880347506
81 2.25546588971619
82 2.41258529255025
83 2.4866513348304
84 2.5202004072872
85 2.56060389810953
86 2.62179964760759
87 2.68015859445927
88 2.7094611316615
89 2.70813698012809
90 2.7010465925971
91 2.67930169612483
92 2.68969103239787
93 2.69792831102358
94 2.73175782969087
95 2.83524530940976
96 3.02369250168221
97 3.22202460039429
98 3.60584468278521
99 2.90733094025161
};

\addplot [semithick, color0]
table {%
0 10.481541733218
1 25.6691980615226
2 50.9794520487059
3 72.463231748284
4 75.1064741174929
5 54.8206430738436
6 24.7882673615217
7 2.69092562779302
8 -3.59227182071805
9 -5.72144879122582
10 -4.32995846830267
11 0.0381167421141111
12 21.9005650118183
13 42.9214106883913
14 56.4393057607967
15 63.3835382140847
16 65.0392377776744
17 63.7371560352957
18 61.1181244513159
19 58.9357901110901
20 57.148133161464
21 55.0224718585111
22 51.9291936100355
23 47.7121812887555
24 43.4849764134312
25 40.3222915108223
26 38.7706732504109
27 38.834303371335
28 40.3642921795213
29 43.4503323126829
30 47.4348309111993
31 52.3075810492283
32 58.3664659363658
33 65.4226100111344
34 73.4762503669822
35 82.7160425956171
36 93.2409085770479
37 104.90768659753
38 117.709887076515
39 131.559146859534
40 146.467683276545
41 162.869795149082
42 181.110112689221
43 201.455198936248
44 223.483336029168
45 244.659215144956
46 260.856785928899
47 267.459896339926
48 259.69481877204
49 234.009586464015
50 189.183226194586
51 125.63263943039
52 55.3129605806587
53 4.81157813520665
54 -28.0247168203329
55 -62.3285796036965
56 -94.2844528181538
57 -118.826548877245
58 -131.169496052621
59 -128.027009494581
60 -110.893905796367
61 -85.6770675020778
62 -58.85500995069
63 -35.9700421794481
64 -19.3119577263924
65 -8.0901884972049
66 -0.278004255393705
67 5.54130100493819
68 6.32570678634231
69 2.23472115174548
70 -0.206907955089222
71 -0.989317447237257
72 -1.00197496030644
73 -0.682463691851666
74 -0.504172739224054
75 -0.644367527918941
76 -0.979304800970154
77 -1.27070050933061
78 -1.32957778129774
79 -1.10360369803983
80 -0.701881875422385
81 -0.304401823840473
82 -0.0336001280593093
83 0.0958262740749395
84 0.158011430277411
85 0.233656829019336
86 0.344023925209782
87 0.445083474735411
88 0.490740782478927
89 0.477238690811539
90 0.435416674688042
91 0.424880966426219
92 0.455245609343655
93 0.488071724359972
94 0.573830515599874
95 0.788698900054936
96 1.15207198704044
97 1.50097952901677
98 1.6611846676536
99 0.879922798855502
};

==> plots/kimr/hip.tex <==
\addplot [semithick, color0]
table {%
0 42.841857870963
1 52.7733657116953
2 71.7666858768179
3 88.7455111926344
4 98.1925506650639
5 94.601418125052
6 77.6533680584874
7 55.3081743506924
8 40.0004235365779
9 40.8438805783793
10 58.4546276509931
11 87.3546184872436
12 120.010729524507
13 146.887325591114
14 162.048048924154
15 162.797392329946
16 150.258391327942
17 129.381864556856
18 106.643523250697
19 87.4022832611753
20 73.3476423970357
21 64.2270539177342
22 58.3229843589739
23 53.5131468430281
24 48.729058833339
25 43.6609463346131
26 38.9187751500342
27 35.2806896056732
28 33.3451296078804
29 33.024019119692
30 33.009780025573
31 32.4375257118635
32 31.1520002828101
33 29.1953829079685
34 27.1174745726982
35 25.5700969319589
36 24.786846960464
37 24.4828394777093
38 24.1673548107566
39 23.4584435153093
40 22.089057907778
41 20.0463746984079
42 17.5629496160969
43 14.9930707236891
44 12.6718408598563
45 10.807923646632
46 9.47610635014824
47 8.6885229123853
48 8.45355905193439
49 8.81908309667441
50 9.88065399117746
51 11.6836737584288
52 14.044125408123
53 16.3646808755435
54 17.4856717982192
55 15.9237230534955
56 11.0795280948072
57 4.6272571563513
58 1.26259386051242
59 6.10099822277796
60 20.4650788556936
61 41.7036467295712
62 64.5613773649332
63 84.734944052877
64 101.316945019627
65 115.71177828441
66 129.979045178018
67 144.42585114474
68 156.539752470995
69 161.647265273133
70 156.818421652614
71 142.947470226146
72 122.069820158403
73 100.157320482745
74 83.421343458813
75 72.5106432481337
76 65.5886023855226
77 60.8798305884262
78 56.4261585797772
79 51.0442466254732
80 45.2533428593064
81 40.0070431408328
82 35.3802790420317
83 30.9230469534748
84 26.3669131902646
85 21.3095222564546
86 15.4637367293366
87 9.3915174236632
88 4.02698115844311
89 0.638624298998886
90 1.10239398661677
91 4.45661916569335
92 10.5116138518319
93 17.875927366253
94 25.047350736022
95 30.0210328479787
96 31.5784487923299
97 29.885725325148
98 26.069914528052
99 23.5101203565156
};

\addplot [semithick, color1]
table {%
0 56.9304803390062
1 72.581518039863
2 102.8672906433
3 130.02928431006
4 145.130475393817
5 139.450143520952
6 112.703468995327
7 77.6271878826873
8 53.8914094155821
9 55.8442095131151
10 84.3768197381214
11 130.761207588871
12 183.068924097061
13 226.216632228549
14 250.831445809398
15 252.686534104038
16 233.560398596707
17 201.255015766487
18 165.949032260722
19 136.045751303836
20 114.178615048344
21 99.9770972905232
22 90.7977474855203
23 83.3658386927082
24 76.0336899105233
25 68.2939844652728
26 61.0531240857972
27 55.4822485732998
28 52.502258234207
29 51.981795992402
30 51.897988333053
31 50.9378099526005
32 48.8854760787794
33 45.8076758843774
34 42.553403436958
35 40.127811965613
36 38.8809760379811
37 38.3681254850245
38 37.8428529566221
39 36.7301943292311
40 34.6252107914126
41 31.5062466702131
42 27.7262965189506
43 23.8240277767946
44 20.3067691237291
45 17.4874416119268
46 15.4784950790706
47 14.29812360753
48 13.9561002331763
49 14.5242255689486
50 16.1495000471756
51 18.8995628424752
52 22.4903714872079
53 26.0065503488182
54 27.66810895403
55 25.2111255784418
56 17.784311774283
57 8.10624951420121
58 2.91311248305316
59 9.78171579759659
60 31.6236740638274
61 64.5921051694982
62 100.428294264093
63 132.26700719179
64 158.545713500454
65 181.367269542981
66 203.94253798487
67 226.776682350049
68 245.943365484727
69 254.09230463554
70 246.634096499103
71 224.978008283481
72 192.276114869524
73 157.90271073918
74 131.629284025337
75 114.455228859576
76 103.491077230739
77 95.9807517801744
78 88.8758048759642
79 80.333730652503
80 71.1820290114555
81 62.9115064288609
82 55.6117965625308
83 48.5741719817589
84 41.4026391030166
85 33.4906668454753
86 24.420143992955
87 15.1178726614099
88 7.08939993406046
89 2.20923901534308
90 2.42050053647074
91 6.75576235070594
92 15.3221943269356
93 25.8352049400858
94 35.9194339462683
95 42.4263280753094
96 43.4940200402759
97 39.4840354853365
98 32.2671354250425
99 27.2661506083072
};

==> plots/kimr/knee.tex <==

\addplot [semithick, color0]
table {%
0 140.324937688141
1 116.236290711196
2 81.8275942817695
3 41.724968941186
4 5.96368818060334
5 -6.21484544018933
6 -18.2424698970645
7 -37.1382861371672
8 -60.6990888207726
9 -79.1530665732969
10 -81.2194629860926
11 -63.2274577547305
12 -31.6287979595062
13 2.23954989121049
14 42.3685253279727
15 93.2393700754725
16 122.486522394869
17 133.427968153357
18 136.292074149574
19 138.181503996858
20 141.233354963302
21 145.690559739113
22 149.896769454249
23 151.73563308387
24 150.670915326685
25 146.553552443185
26 139.29211328082
27 128.074385199765
28 114.16666422029
29 98.715509057128
30 82.4615460170979
31 67.4911403502768
32 54.8528179490951
33 44.1898893422552
34 35.1502325551154
35 27.4389763187955
36 20.6228869137422
37 14.5020726630445
38 9.25606432542567
39 5.06618055459761
40 1.96567640352046
41 0.548595357243908
42 0.479216517108812
43 0.861550747634425
44 1.60395245105327
45 3.03752203369847
46 4.83576667158654
47 6.39722049614923
48 7.35132203032145
49 7.53104241525621
50 7.12204651088844
51 6.57267501231157
52 6.33841052368954
53 6.72735339269104
54 7.53321929095934
55 7.3993381698966
56 3.75922004919352
57 -1.683717877673
58 -6.84958579691732
59 -14.1885789282122
60 -21.6853295091186
61 -26.5350668190125
62 -26.7181760998887
63 -22.774972499371
64 -17.6764722342244
65 -14.5951288966997
66 -14.8662204480735
67 -17.3612222313426
68 -19.7195511031752
69 -19.9160342827089
70 -17.4499152911354
71 -13.3767891902003
72 -8.82117405550159
73 -4.77314649945535
74 -1.63373506278397
75 1.56308109712452
76 7.31497750677879
77 15.8524380244798
78 23.0744281344323
79 27.0600491507911
80 27.2649830483701
81 24.8837872987848
82 21.4358210091606
83 18.0893846130504
84 14.5563154822269
85 9.09442381055267
86 0.75960043102757
87 -4.30411018047739
88 -10.5454232091219
89 -18.4322756874001
90 -27.3266228774597
91 -36.3341505901127
92 -44.4979615031074
93 -50.6113599381654
94 -52.6546180604809
95 -48.8608953814687
96 -37.8927011699848
97 -20.1345991773057
98 1.9047681142466
99 50.0409136982836
};


\addplot [semithick, color1]
table {%
0 214.4574055449
1 178.078639254962
2 125.815523649653
3 64.6580613827223
4 10.2288422881454
5 -2.01037758791041
6 -9.09812094667772
7 -19.8688221923351
8 -33.2963541139513
9 -43.8895229021402
10 -45.2988064618092
11 -35.4368649795991
12 -17.8950802362012
13 0.981535732371189
14 42.5183828863468
15 120.491329099492
16 167.03188445726
17 184.57028826985
18 189.486584298066
19 193.278333764667
20 199.431391936782
21 208.249062477784
22 216.920351516953
23 221.835901854853
24 221.969175329572
25 217.054202988632
26 207.011955742335
27 190.663691261061
28 170.056229789
29 147.035070888244
30 122.694840484283
31 100.23451374147
32 81.291714069906
33 65.3192216734832
34 51.8106903726103
35 40.374733805907
36 30.3814863062904
37 21.5144748171651
38 14.0101631900477
39 8.11041530648918
40 3.83786173022959
41 1.87095263353905
42 1.60242407009758
43 1.79400221675294
44 2.49059936757646
45 4.44261671730711
46 7.16522564906005
47 9.63570380554367
48 11.2599081189378
49 11.7475866529326
50 11.3401152546203
51 10.6801392208848
52 10.4457297369353
53 11.1216133899269
54 12.4257960945957
55 12.319738564308
56 6.93310704091722
57 0.402864830968704
58 -2.53795873643515
59 -6.69726304011458
60 -10.9314169966261
61 -13.6586928358031
62 -13.7470521699869
63 -11.508784324655
64 -8.62371743602582
65 -6.8831919285504
66 -7.04083368218595
67 -8.46008496618615
68 -9.80811704059295
69 -9.93956133769731
70 -8.56631014741045
71 -6.27895901637361
72 -3.71297808683889
73 -1.43056505341587
74 0.337238289047194
75 2.94264119474664
76 10.7689736420351
77 24.3119124519971
78 35.8626434749425
79 42.4032112028415
80 43.0335254498875
81 39.5739848679532
82 34.3655068027439
83 29.2487504182031
84 23.804537810733
85 15.3243886295185
86 2.85307087050666
87 -1.06396672550315
88 -4.58620460861192
89 -9.03579802838235
90 -14.0545516674876
91 -19.142007542732
92 -23.7637494762207
93 -27.2460423228067
94 -28.4593330743228
95 -26.4127653520805
96 -20.3515160711012
97 -10.4808449062052
98 2.61691655744141
99 69.5929210034134
};

==> plots/kimr/main.tex <==
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019807843137}
\definecolor{color2}{rgb}{0.172549019807843,0.627450980392157,0.172549019807843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\begin{groupplot}[group style={group size=3 by 1,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.6]
\nextgroupplot[
title = {\footnotesize Hip},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize MEE in \si{W}},
ymin=-200,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize},
xlabel={\footnotesize Gait Cycle in \si{\percent}}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/kimr/hip}


\nextgroupplot[
title = {\footnotesize Knee},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-200,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize},
xlabel={\footnotesize Gait Cycle in \si{\percent}}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/kimr/knee}

\nextgroupplot[
title = {\footnotesize Ankle},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-200,ymax=500,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize},
xlabel={\footnotesize Gait Cycle in \si{\percent}}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/kimr/ankle}
\end{groupplot}

\end{tikzpicture}

==> plots/thermo/am/ammain.tex <==
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019807843137}
\definecolor{color2}{rgb}{0.172549019807843,0.627450980392157,0.172549019807843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\begin{groupplot}[group style={group size=2 by 2,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.4]
\nextgroupplot[
title = {\footnotesize Soleus, Original Parameters},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize Heat in \si{W}},
ymin=-75,ymax=200,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/thermo/am/nomc}

\nextgroupplot[
title = {\footnotesize Soleus, Optimised Parameters},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-75,ymax=200,xmin=-0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick label style = {font=\footnotesize}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/thermo/am/mc}

\end{groupplot}

\end{tikzpicture}

==> plots/thermo/am/mc.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot [semithick, color0]
table {%
0 0.000848374130001314
1 0.000870646473284734
2 0.00461394838313236
3 0.00828857312399108
4 0.0174184711912989
5 0.0518351816662885
6 0.294355476238547
7 0.624865486221724
8 0.548630225054058
9 0.494445849008331
10 1.74999499632905
11 3.67156985693972
12 9.52215459340126
13 13.8287436686307
14 15.7470309654056
15 16.1346851170598
16 15.1215737390024
17 14.288098291185
18 14.3962171440754
19 16.300567398871
20 19.3466742672151
21 22.4003050201461
22 24.6916352148055
23 25.2795600380215
24 24.5965750861921
25 23.9453600652951
26 23.4837297013376
27 24.0091844583165
28 25.262044825115
29 27.1217511451635
30 28.5759035325036
31 29.2837797944239
32 29.9465305426171
33 30.8616310477781
34 32.2407175880606
35 34.2296651942734
36 36.6416185837209
37 39.1580381624629
38 41.4973125419953
39 43.6843346823988
40 45.8442002777689
41 48.1287829332019
42 50.6348828754509
43 53.2847821545239
44 55.9497953105534
45 58.5826203573395
46 61.1088846457807
47 63.6099079929194
48 66.1796105602433
49 68.7978312139789
50 71.5547951441988
51 75.0421101293499
52 80.3066732286246
53 87.3854411140853
54 96.7025168201299
55 105.259912994466
56 108.588790648471
57 106.587546785431
58 99.8536926785918
59 85.1165762265719
60 61.1496078875854
61 37.8381724795426
62 15.2475054241107
63 0.0182958890444464
64 0.000409668215412766
65 0.000355519202630233
66 0.000289339817511967
67 0.000224535575995974
68 0.000171672649089481
69 0.000138448470741596
70 0.000127801086433699
71 0.000138095839062896
72 0.000159145991898185
73 0.000173613682295098
74 0.000173047071366465
75 0.00016018645272089
76 0.00014839054793482
77 0.00014820969482473
78 0.000164231651727042
79 0.000198088947428735
80 0.000246111875622599
81 0.000294297179759944
82 0.000326483075066973
83 0.000343479772862812
84 0.000361869515339892
85 0.000401333657846482
86 0.000465333372816932
87 0.000543577221492453
88 0.000932816953447726
89 0.00639310298843656
90 0.0431983062520328
91 0.0583015643347722
92 0.0923831795091358
93 0.162305061554139
94 0.269189325542291
95 0.26492488745374
96 0.649518654629783
97 0.838220244439923
98 0.710207762378064
99 0.0110600242423091
};
\addplot [semithick, color1]
table {%
0 0.272971149426427
1 0.194460636067085
2 0.140329206784791
3 0.103362800232248
4 0.0807516059267614
5 0.078561154088008
6 0.175394829591797
7 0.37769449050411
8 0.487365398139941
9 0.542201255721867
10 1.10001440869712
11 2.31680067802661
12 5.80325656525603
13 10.3024188891709
14 14.3999462567092
15 17.4442521621468
16 19.0451945173674
17 19.7311896798184
18 20.2289609473807
19 21.4588798007144
20 23.7708177951597
21 26.8635797889478
22 30.1205663177195
23 32.5914499728344
24 33.8625882529778
25 34.3509394856931
26 34.4149230706585
27 34.7080598492857
28 35.5318518424062
29 37.0406380616994
30 38.7964077154566
31 40.3197065717258
32 41.6659219648755
33 43.0287879258415
34 44.65675498658
35 46.802413056051
36 49.5375525312421
37 52.7326483562644
38 56.1332395429395
39 59.5800172780845
40 63.0369701693483
41 66.5721990682102
42 70.2901858435585
43 74.208613022789
44 78.2523421524145
45 82.3358461757687
46 86.3480859696001
47 90.2756478452908
48 94.1835345255961
49 98.1472619677135
50 102.448353699744
51 107.674947566231
52 114.884363099434
53 124.882339632877
54 138.808989488329
55 154.87605594453
56 168.07856739059
57 174.826500550433
58 173.368888100682
59 160.419431717906
60 134.437563071475
61 103.916299558189
62 73.5731371753145
63 47.7343589794255
64 30.9987081326553
65 20.1659588246568
66 13.2158357932532
67 8.79764003779518
68 5.98812181056967
69 4.17524897298222
70 2.9767646237801
71 2.16080631835891
72 1.58314588853886
73 1.16389482881935
74 0.855634448826461
75 0.628375697962858
76 0.460738411955084
77 0.337092319529962
78 0.246083948813158
79 0.179270284644205
80 0.130338769318401
81 0.0945978017037632
82 0.0685555812514608
83 0.0496147190114044
84 0.0358731266847288
85 0.025941192662799
86 0.0187943456534221
87 0.0136768736020836
88 0.0101557418916627
89 0.00983398869346059
90 0.024357599185433
91 0.0407816250868579
92 0.0661746640458099
93 0.112354315313649
94 0.188160356067535
95 0.240336957135447
96 0.433003969938198
97 0.647007431196654
98 0.747831745732676
99 0.537847287639716
};
\addplot [semithick, color2]
table {%
0 0.278269090193865
1 0.198674609246271
2 0.143585645362178
3 0.105861428667
4 0.0827523095957025
5 0.080550490564324
6 0.180147523924286
7 0.38945535669177
8 0.505340163988246
9 0.565977822303449
10 0.255326315914998
11 0.062253749522663
12 0.0989373293025013
13 0.172040116548144
14 0.236177519419512
15 0.282174783202547
16 0.305326063314585
17 0.314453361099259
18 0.320823771981015
19 0.338372667289902
20 0.373271252734471
21 0.426650939971415
22 0.494909613868683
23 0.546737544908323
24 0.568572615056339
25 0.575926446273403
26 0.585787209380155
27 0.625606559680256
28 0.725606193685663
29 0.875963159550323
30 0.95190124806889
31 0.913042306269173
32 0.842012738752818
33 0.79669830889125
34 0.787129374015818
35 0.804720229917752
36 0.833882253030091
37 0.860073229711276
38 0.87881752301158
39 0.896928154805422
40 0.920562922051151
41 0.951016948263823
42 0.987503107053411
43 1.02832257890927
44 1.07171735159568
45 1.11640605354628
46 1.1608337378059
47 1.20462781074573
48 1.24875196217348
49 1.29664186361152
50 1.38071077936825
51 2.29422021000051
52 45.0234418840162
53 93.6731250876072
54 101.973600453351
55 111.262754240964
56 118.672616040704
57 122.39689191503
58 121.625281820533
59 114.465166841282
60 99.5792047603091
61 81.0418391972052
62 61.0890079454344
63 42.6331710632496
64 29.6145240438277
65 20.5236255210433
66 14.2452634551587
67 9.94345286052562
68 6.99838813650953
69 3.78499503944788
70 0.0604642943289506
71 0.0429836720402892
72 0.0310644203177071
73 0.0224764984782161
74 0.0162600231818128
75 0.0117570655194569
76 0.0084952132674644
77 0.00613267642907741
78 0.00442310197573895
79 0.00318745171417529
80 0.00229535246367083
81 0.00165206415154027
82 0.00118868600950169
83 0.000855182175008684
84 0.000615599086135228
85 0.000444625339860072
86 0.000326977193521227
87 0.00026521514069507
88 0.000311597488598466
89 0.00101007026245
90 0.00719710915658556
91 0.0324822809844441
92 0.0668623330680669
93 0.113595367581966
94 0.190502312164995
95 0.243839261472671
96 0.440196710577571
97 0.658378876765162
98 0.752653910077582
99 0.122155648449886
};
\addplot [semithick, color3]
table {%
0 0.00975772735104496
1 0.0061204011059377
2 0.00410819356112132
3 0.00292499510972084
4 0.00258491694964432
5 0.00431564028359407
6 0.0474881532479361
7 0.136749786586261
8 0.115117670229709
9 0.101238159482937
10 0.611714434605459
11 1.6757553669544
12 6.20323237288175
13 10.1026688110873
14 11.8839402808041
15 12.1157531256071
16 10.9326026990864
17 9.96195543872503
18 9.91432962392746
19 11.6026045935955
20 14.5095273791636
21 17.564438169346
22 19.9156086354242
23 20.4491545314406
24 19.6071827352235
25 18.8106201741352
26 18.2764089178703
27 18.7111699996483
28 19.9437385815297
29 21.8786750272133
30 23.3978816390229
31 24.1014053390943
32 24.750284479885
33 25.6743894351055
34 27.1204465360802
35 29.2750109107659
36 31.9485460839441
37 34.7812782477565
38 37.4291418093017
39 39.9057039060198
40 42.351358787746
41 44.9506540204263
42 47.8266467288116
43 50.8817263549503
44 53.9451060204835
45 56.9459923000646
46 59.780569076744
47 62.5625161354051
48 65.4389214496872
49 68.4715740604695
50 72.0955265495842
51 77.0776305853191
52 84.6820955196241
53 95.1536873563864
54 109.513440744733
55 123.512095562314
56 130.426085690405
57 129.44829961892
58 122.078783257711
59 106.435399960395
60 79.786347655304
61 53.2308380926587
62 28.7892195615671
63 11.6817748202629
64 7.27061046428761
65 4.52907433010293
66 2.82124142680828
67 1.75736878210784
68 1.09465602938787
69 0.681846313840509
70 0.42471125825972
71 0.264549519088397
72 0.164791170751777
73 0.102653868192723
74 0.0639479265660401
75 0.0398366709805344
76 0.0248176376837072
77 0.0154632528241176
78 0.00963787475884254
79 0.00601087285216763
80 0.00375293573592629
81 0.00234677746999884
82 0.00147005094853208
83 0.000922858986447531
84 0.000581469983876031
85 0.000369016802711363
86 0.000237159464965683
87 0.00015523983121839
88 0.000111708281902157
89 0.000411806810247519
90 0.00302635514080976
91 0.00462092729553339
92 0.00884471074429866
93 0.019506917214585
94 0.0395010393958601
95 0.0399026683521138
96 0.137902008229028
97 0.197925233246506
98 0.159003307516094
99 0.0260635563397038
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};


==> plots/thermo/am/nomc.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\addplot [semithick, color0]
table {%
0 0.00057215737912349
1 0.000587509711190708
2 0.00311466464257113
3 0.00559650234185355
4 0.0117627572112281
5 0.035009962213285
6 0.198940358315371
7 0.422886810513787
8 0.371848843057515
9 0.335709918905003
10 1.19015745390915
11 2.49458624894906
12 6.46922419223492
13 9.39112176591939
14 10.6840151743348
15 10.9328919526549
16 10.2293215294546
17 9.64905764477747
18 9.70805708389717
19 10.9828693880141
20 13.0308716366162
21 15.0859199679775
22 16.4475365940242
23 16.613474808564
24 15.9679610577596
25 15.3677631703833
26 14.9089525960774
27 15.0498321038767
28 15.6042396743746
29 16.4682326361026
30 17.0723639685609
31 17.2536362897684
32 17.4019249370841
33 17.6719668658493
34 18.1574517640122
35 18.9108392406041
36 19.8253279508721
37 20.7476533881181
38 21.5599263307928
39 22.2849500193859
40 22.9856231218828
41 23.7296280932713
42 24.5589129923561
43 25.4456033682156
44 26.3441970284228
45 27.2421045018228
46 28.1149581730097
47 28.9956633201437
48 29.9188470558945
49 30.8379025770807
50 31.6061666435515
51 32.5398265480518
52 34.2955584977129
53 36.9433069248107
54 40.7608312078775
55 44.4188930118035
56 45.7171952978043
57 44.5917173233511
58 41.5240931989245
59 35.3270459423276
60 25.6970227895616
61 16.5827994999381
62 7.12401941259562
63 0.0123937064046917
64 0.000280264960654814
65 0.000244887511346028
66 0.000200546540577344
67 0.000156389454649542
68 0.000119931511232503
69 9.68193724510574e-05
70 8.92955408229604e-05
71 9.62642195774303e-05
72 0.000110612190953849
73 0.000120288803535733
74 0.000119520873501609
75 0.000110295001168239
76 0.000101863564127212
77 0.00010144697012117
78 0.000112111859794195
79 0.000134889495121706
80 0.000167213659130844
81 0.00019954390860596
82 0.000220957869912147
83 0.000232081683502331
84 0.000244168344791554
85 0.000270490545342974
86 0.000313355383640764
87 0.000365807645083218
88 0.000627472631142006
89 0.00429899372467728
90 0.0290468350610065
91 0.0392000103207145
92 0.0621199018189837
93 0.109167444174619
94 0.181156398723962
95 0.178424773400355
96 0.437831230765305
97 0.565351734643558
98 0.479095411957797
99 0.00745862804879792
};
\addplot [semithick, color1]
table {%
0 0.029243921846789
1 0.0208438771758224
2 0.015046985149775
3 0.0110856947685759
4 0.00866184421286382
5 0.00842796875804685
6 0.0188243231236133
7 0.040575983725849
8 0.052429670351543
9 0.0584250242235631
10 0.118626853720413
11 0.249237693282448
12 0.621689481434523
13 1.09900141893216
14 1.53066582783979
15 1.84926071556805
16 2.0153044972688
17 2.08520079732839
18 2.13546931484176
19 2.26238734306114
20 2.5021365580062
21 2.82279870872312
22 3.15995691723724
23 3.41517810467955
24 3.54599701122375
25 3.59580633178947
26 3.60176095740843
27 3.63144428967133
28 3.71599874487436
29 3.87127216184975
30 4.05193692836344
31 4.2084990061426
32 4.34668049896201
33 4.48645138107737
34 4.6533687605859
35 4.87335472257841
36 5.15367960245033
37 5.48092466511319
38 5.82891330134811
39 6.18130464489925
40 6.53443995056163
41 6.89532333566667
42 7.27467015671458
43 7.67431550005425
44 8.0866201473723
45 8.50290796504196
46 8.91192333063035
47 9.31238784789991
48 9.71101891645394
49 10.1155784431818
50 10.5548343399043
51 11.0888924898118
52 11.8260109349362
53 12.8492708632496
54 14.2773254993234
55 15.9287353411901
56 17.2894678365315
57 17.9877064002494
58 17.8422759047192
59 16.5161609538449
60 13.8562150984479
61 10.7420690653156
62 7.65055739020274
63 5.01156523086874
64 3.29233863996816
65 2.16919745253343
66 1.43981282960118
67 0.969257579829399
68 0.665137976263849
69 0.465821419688417
70 0.33234895084275
71 0.240697318158663
72 0.175678517170618
73 0.128595852899925
74 0.0941322941633004
75 0.0688489620704332
76 0.0502906455216769
77 0.0366686715212458
78 0.0266870914969242
79 0.0193886734104952
80 0.0140631026645642
81 0.010185768144569
82 0.00736866728333428
83 0.00532499288810718
84 0.00384560336622463
85 0.0027783282742816
86 0.00201150305132012
87 0.00146308376132752
88 0.00108605693973654
89 0.00105140754218818
90 0.00260392662253159
91 0.00435947256486532
92 0.00707412622339198
93 0.0120126993933448
94 0.0201245836803514
95 0.0257182320331964
96 0.0463588091862238
97 0.0692883677619519
98 0.0800922629128479
99 0.0576058810814617
};
\addplot [semithick, color2]
table {%
0 0.173748944226689
1 0.124110753469524
2 0.0897262009998328
3 0.0661657750705962
4 0.0517285349268877
5 0.0503587576967175
6 0.112684528711295
7 0.24389632435259
8 0.316937495675036
9 0.355573193393431
10 0.302348137931473
11 0.459561075087447
12 1.10931658514049
13 1.9266103974094
14 2.64206915044174
15 3.15318332594804
16 3.4077709726828
17 3.50523844999412
18 3.57179724936413
19 3.76108861202536
20 4.12726491907965
21 4.6162279187098
22 5.09720915136468
23 5.43731715231529
24 5.58559100902707
25 5.6130768213468
26 5.5787105281594
27 5.58353279820374
28 5.67671972839666
29 5.87649760446437
30 6.09034423844019
31 6.24227451073531
32 6.36008147766851
33 6.48291051004929
34 6.64432655592825
35 6.87321090165607
36 7.17264426668927
37 7.52033800108877
38 7.88183044229943
39 8.23811985615855
40 8.58594105658522
41 8.93343385283836
42 9.29206491028591
43 9.66284188807325
44 10.0366138345099
45 10.4038771868853
46 10.7533207633476
47 11.0844728597025
48 11.4049965609696
49 11.7230742620279
50 12.0694574018367
51 12.6514972783522
52 28.3137240453243
53 46.3302648828531
54 50.0907373079145
55 54.2847093453898
56 57.5146370761842
57 58.936760523466
58 58.2068513298674
59 54.4797489785067
60 47.1720286747953
61 38.2526875036938
62 28.7707870164106
63 20.0623247589852
64 15.315015696969
65 13.0988992332155
66 9.16243682318175
67 6.43565409224838
68 4.54733438636015
69 2.68474649762794
70 0.693630088009301
71 0.498183545526278
72 0.358700396219588
73 0.258487306004187
74 0.186256964793219
75 0.134168164043158
76 0.0966018616805633
77 0.0695104357501538
78 0.04998569753533
79 0.0359259162118067
80 0.0258098660528897
81 0.0185377640831171
82 0.0133138434186669
83 0.00956297870022448
84 0.00687227093054482
85 0.00494590848469663
86 0.00357120984420075
87 0.00259728542052669
88 0.00195297606691223
89 0.00211793399689615
90 0.00713410132103095
91 0.0212558698079919
92 0.0416466005458091
93 0.0707699906949302
94 0.118732798792019
95 0.152064888336502
96 0.274707128161071
97 0.41104497213319
98 0.471289990009558
99 0.141350545001485
};
\addplot [semithick, color3]
table {%
0 0.390867127827638
1 0.319994266494795
2 0.269744170970392
3 0.233224294341962
4 0.221294520678614
5 0.275254196029184
6 0.757826311043453
7 1.20368166227404
8 1.12388647525645
9 1.06417874604861
10 2.25552119263661
11 3.51144837678614
12 6.11415746893494
13 7.62224201204594
14 8.18805481176734
15 8.25810180101645
16 7.90053990998728
17 7.59314605202717
18 7.57858776285738
19 8.10137767408818
20 8.91206936967616
21 9.67512183381514
22 10.2138718324305
23 10.3328629254985
24 10.1477589188941
25 9.96954391235838
26 9.84745718219565
27 9.94684533048058
28 10.2214190249899
29 10.6335192271776
30 10.945547343647
31 11.0860249700168
32 11.2126988158007
33 11.3898670211617
34 11.6595307944776
35 12.0464376788701
36 12.5053839211956
37 12.9690529706625
38 13.383786344086
39 13.7563756392827
40 14.1114083112633
41 14.475827470106
42 14.865240424432
43 15.2647547031489
44 15.651963776077
45 16.0192504059077
46 16.3562808563764
47 16.6779806727434
48 17.0021432376821
49 17.3350987900176
50 17.7213736214421
51 18.2338178595099
52 18.9792029964595
53 19.9492683524766
54 21.1804282739897
55 22.3138055847093
56 22.844405991618
57 22.7695603368233
58 22.20369296577
59 20.902184499621
60 18.4385046178147
61 15.4582714539998
62 11.6594201021942
63 8.08078043011018
64 6.59667490257113
65 5.3870032268638
66 4.39914137715823
67 3.59241874672661
68 2.93362408398988
69 2.39563859422358
70 1.95631774322454
71 1.59757757459117
72 1.30464437942137
73 1.06544273392135
74 0.87010922504961
75 0.71059411626709
76 0.580337505170656
77 0.473990215904988
78 0.387187717375621
79 0.316370750868956
80 0.258630379970939
81 0.211568166307296
82 0.173200331639157
83 0.141924741424157
84 0.116483554027984
85 0.0959039109532308
86 0.0793865744705047
87 0.0662650415802455
88 0.0576448340529374
89 0.075669970085538
90 0.236296813099193
91 0.282369118972865
92 0.371791288176067
93 0.522200058484927
94 0.71122722558055
95 0.700940465173872
96 1.21393155396946
97 1.41804760851045
98 1.28660873276164
99 0.595149909023107
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};

\end{tikzpicture}


==> plots/thermo/length/barmc.tex <==

\draw[draw=black,fill=color0] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.0642646952343096);
\draw[draw=black,fill=color0] (axis cs:0.7,0) rectangle (axis cs:0.9,0.477812702942312);
\draw[draw=black,fill=color0] (axis cs:1.7,0) rectangle (axis cs:1.9,0.292539526482175);
\draw[draw=black,fill=color0] (axis cs:2.7,0) rectangle (axis cs:2.9,0.016613553094777);
\draw[draw=black,fill=color0] (axis cs:3.7,0) rectangle (axis cs:3.9,0.566570588354461);
\draw[draw=black,fill=color0] (axis cs:4.7,0) rectangle (axis cs:4.9,0.115539833957732);
\draw[draw=black,fill=color0] (axis cs:5.7,0) rectangle (axis cs:5.9,0.41128487993343);
\draw[draw=black,fill=color0] (axis cs:6.7,0) rectangle (axis cs:6.9,0.0922810863558905);
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.00395655116701915);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,0.47999960512076);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,0.153520769741269);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,0.00505274469354635);
\draw[draw=black,fill=color1] (axis cs:3.9,0) rectangle (axis cs:4.1,0.546878902496447);
\draw[draw=black,fill=color1] (axis cs:4.9,0) rectangle (axis cs:5.1,0.0429334884449069);
\draw[draw=black,fill=color1] (axis cs:5.9,0) rectangle (axis cs:6.1,0.0979318930495563);
\draw[draw=black,fill=color1] (axis cs:6.9,0) rectangle (axis cs:7.1,0.100965560587994);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,0.00233460331088653);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,0.282755473984617);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,0.0852778202992319);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,0.00226008456691849);
\draw[draw=black,fill=color2] (axis cs:4.1,0) rectangle (axis cs:4.3,0.244438674107618);
\draw[draw=black,fill=color2] (axis cs:5.1,0) rectangle (axis cs:5.3,0.0215409354660487);
\draw[draw=black,fill=color2] (axis cs:6.1,0) rectangle (axis cs:6.3,0.0471559170458733);
\draw[draw=black,fill=color2] (axis cs:7.1,0) rectangle (axis cs:7.3,0.0363211243150463);
\draw[draw=black,fill=color3] (axis cs:0.3,0) rectangle (axis cs:0.5,5.55835019545037e-05);
\draw[draw=black,fill=color3] (axis cs:1.3,0) rectangle (axis cs:1.5,0);
\draw[draw=black,fill=color3] (axis cs:2.3,0) rectangle (axis cs:2.5,0);
\draw[draw=black,fill=color3] (axis cs:3.3,0) rectangle (axis cs:3.5,0.000994994912851127);
\draw[draw=black,fill=color3] (axis cs:4.3,0) rectangle (axis cs:4.5,1.35617864321924e-05);
\draw[draw=black,fill=color3] (axis cs:5.3,0) rectangle (axis cs:5.5,0.00753674292180445);
\draw[draw=black,fill=color3] (axis cs:6.3,0) rectangle (axis cs:6.5,8.72108338245692e-06);
\draw[draw=black,fill=color3] (axis cs:7.3,0) rectangle (axis cs:7.5,3.72391716491061e-08);
\path [draw=black, semithick]
(axis cs:-0.2,0.040687687070039)
--(axis cs:-0.2,0.0878417033985801);

\path [draw=black, semithick]
(axis cs:0.8,0.266575556395012)
--(axis cs:0.8,0.689049849489613);

\path [draw=black, semithick]
(axis cs:1.8,0.110536462407466)
--(axis cs:1.8,0.474542590556884);

\path [draw=black, semithick]
(axis cs:2.8,0.00803571696690782)
--(axis cs:2.8,0.0251913892226461);

\path [draw=black, semithick]
(axis cs:3.8,0.399253114307244)
--(axis cs:3.8,0.733888062401678);

\path [draw=black, semithick]
(axis cs:4.8,0.0607091024962335)
--(axis cs:4.8,0.170370565419231);

\path [draw=black, semithick]
(axis cs:5.8,0.300154488571929)
--(axis cs:5.8,0.52241527129493);

\path [draw=black, semithick]
(axis cs:6.8,0.0459873170835293)
--(axis cs:6.8,0.138574855628252);

\path [draw=black, semithick]
(axis cs:0,0.000749942212234859)
--(axis cs:0,0.00716316012180344);

\path [draw=black, semithick]
(axis cs:1,0.302681613426207)
--(axis cs:1,0.657317596815313);

\path [draw=black, semithick]
(axis cs:2,0.0591939107314153)
--(axis cs:2,0.247847628751124);

\path [draw=black, semithick]
(axis cs:3,0.00311212218108637)
--(axis cs:3,0.00699336720600633);

\path [draw=black, semithick]
(axis cs:4,0.403810487765234)
--(axis cs:4,0.68994731722766);

\path [draw=black, semithick]
(axis cs:5,0.0191763430104192)
--(axis cs:5,0.0666906338793946);

\path [draw=black, semithick]
(axis cs:6,0.0115924063354322)
--(axis cs:6,0.18427137976368);

\path [draw=black, semithick]
(axis cs:7,0.0406903174583854)
--(axis cs:7,0.161240803717602);

\path [draw=black, semithick]
(axis cs:0.2,0.000275526130998737)
--(axis cs:0.2,0.00439368049077432);

\path [draw=black, semithick]
(axis cs:1.2,0.174980564230611)
--(axis cs:1.2,0.390530383738622);

\path [draw=black, semithick]
(axis cs:2.2,0.0290070903195224)
--(axis cs:2.2,0.141548550278941);

\path [draw=black, semithick]
(axis cs:3.2,0.00118159224461012)
--(axis cs:3.2,0.00333857688922686);

\path [draw=black, semithick]
(axis cs:4.2,0.191259927839286)
--(axis cs:4.2,0.297617420375949);

\path [draw=black, semithick]
(axis cs:5.2,0.00526172188571498)
--(axis cs:5.2,0.0378201490463825);

\path [draw=black, semithick]
(axis cs:6.2,-0.00262494821162141)
--(axis cs:6.2,0.096936782303368);

\path [draw=black, semithick]
(axis cs:7.2,0.0143925135544012)
--(axis cs:7.2,0.0582497350756914);

\path [draw=black, semithick]
(axis cs:0.4,-2.1907323888375e-05)
--(axis cs:0.4,0.000133074327797382);

\path [draw=black, semithick]
(axis cs:1.4,0)
--(axis cs:1.4,0);

\path [draw=black, semithick]
(axis cs:2.4,0)
--(axis cs:2.4,0);

\path [draw=black, semithick]
(axis cs:3.4,0.000543862145344542)
--(axis cs:3.4,0.00144612768035771);

\path [draw=black, semithick]
(axis cs:4.4,-1.42413194903759e-05)
--(axis cs:4.4,4.13648923547607e-05);

\path [draw=black, semithick]
(axis cs:5.4,0.00256273792669176)
--(axis cs:5.4,0.0125107479169171);

\path [draw=black, semithick]
(axis cs:6.4,-2.54738787211217e-05)
--(axis cs:6.4,4.29160454860355e-05);

\path [draw=black, semithick]
(axis cs:7.4,-2.74326091674513e-07)
--(axis cs:7.4,3.48804434972725e-07);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 0.040687687070039
0.8 0.266575556395012
1.8 0.110536462407466
2.8 0.00803571696690782
3.8 0.399253114307244
4.8 0.0607091024962335
5.8 0.300154488571929
6.8 0.0459873170835293
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 0.0878417033985801
0.8 0.689049849489613
1.8 0.474542590556884
2.8 0.0251913892226461
3.8 0.733888062401678
4.8 0.170370565419231
5.8 0.52241527129493
6.8 0.138574855628252
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 0.000749942212234859
1 0.302681613426207
2 0.0591939107314153
3 0.00311212218108637
4 0.403810487765234
5 0.0191763430104192
6 0.0115924063354322
7 0.0406903174583854
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 0.00716316012180344
1 0.657317596815313
2 0.247847628751124
3 0.00699336720600633
4 0.68994731722766
5 0.0666906338793946
6 0.18427137976368
7 0.161240803717602
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 0.000275526130998737
1.2 0.174980564230611
2.2 0.0290070903195224
3.2 0.00118159224461012
4.2 0.191259927839286
5.2 0.00526172188571498
6.2 -0.00262494821162141
7.2 0.0143925135544012
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 0.00439368049077432
1.2 0.390530383738622
2.2 0.141548550278941
3.2 0.00333857688922686
4.2 0.297617420375949
5.2 0.0378201490463825
6.2 0.096936782303368
7.2 0.0582497350756914
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 -2.1907323888375e-05
1.4 0
2.4 0
3.4 0.000543862145344542
4.4 -1.42413194903759e-05
5.4 0.00256273792669176
6.4 -2.54738787211217e-05
7.4 -2.74326091674513e-07
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 0.000133074327797382
1.4 0
2.4 0
3.4 0.00144612768035771
4.4 4.13648923547607e-05
5.4 0.0125107479169171
6.4 4.29160454860355e-05
7.4 3.48804434972725e-07
};


==> plots/thermo/length/barnomc.tex <==

\draw[draw=black,fill=color0] (axis cs:-0.3,0) rectangle (axis cs:-0.1,0.00610971452489228);
\draw[draw=black,fill=color0] (axis cs:0.7,0) rectangle (axis cs:0.9,0.0978154577243947);
\draw[draw=black,fill=color0] (axis cs:1.7,0) rectangle (axis cs:1.9,0.0669928258509485);
\draw[draw=black,fill=color0] (axis cs:2.7,0) rectangle (axis cs:2.9,0.00710634174411276);
\draw[draw=black,fill=color0] (axis cs:3.7,0) rectangle (axis cs:3.9,0.116995838945391);
\draw[draw=black,fill=color0] (axis cs:4.7,0) rectangle (axis cs:4.9,0.0369667054064522);
\draw[draw=black,fill=color0] (axis cs:5.7,0) rectangle (axis cs:5.9,0.0511429251678275);
\draw[draw=black,fill=color0] (axis cs:6.7,0) rectangle (axis cs:6.9,0.0149048790097013);
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,0.00107237674483629);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,0.104128043767525);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,0.03064471462096);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,0.00177507237388663);
\draw[draw=black,fill=color1] (axis cs:3.9,0) rectangle (axis cs:4.1,0.127845723460038);
\draw[draw=black,fill=color1] (axis cs:4.9,0) rectangle (axis cs:5.1,0.0142562460200323);
\draw[draw=black,fill=color1] (axis cs:5.9,0) rectangle (axis cs:6.1,0.022892765272181);
\draw[draw=black,fill=color1] (axis cs:6.9,0) rectangle (axis cs:7.1,0.0131078927068089);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,0.00129668072645017);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,0.139481593159904);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,0.0461506956723566);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,0.00253401074412998);
\draw[draw=black,fill=color2] (axis cs:4.1,0) rectangle (axis cs:4.3,0.156034209474898);
\draw[draw=black,fill=color2] (axis cs:5.1,0) rectangle (axis cs:5.3,0.0166967998319054);
\draw[draw=black,fill=color2] (axis cs:6.1,0) rectangle (axis cs:6.3,0.0381579972195033);
\draw[draw=black,fill=color2] (axis cs:7.1,0) rectangle (axis cs:7.3,0.0262362611582444);
\draw[draw=black,fill=color3] (axis cs:0.3,0) rectangle (axis cs:0.5,4.1655921497491e-05);
\draw[draw=black,fill=color3] (axis cs:1.3,0) rectangle (axis cs:1.5,0);
\draw[draw=black,fill=color3] (axis cs:2.3,0) rectangle (axis cs:2.5,0);
\draw[draw=black,fill=color3] (axis cs:3.3,0) rectangle (axis cs:3.5,0.000989086208785645);
\draw[draw=black,fill=color3] (axis cs:4.3,0) rectangle (axis cs:4.5,5.28000810597895e-05);
\draw[draw=black,fill=color3] (axis cs:5.3,0) rectangle (axis cs:5.5,0.0037881078710208);
\draw[draw=black,fill=color3] (axis cs:6.3,0) rectangle (axis cs:6.5,2.46258512281994e-06);
\draw[draw=black,fill=color3] (axis cs:7.3,0) rectangle (axis cs:7.5,5.53876213782445e-08);
\path [draw=black, semithick]
(axis cs:-0.2,0.00332852906293993)
--(axis cs:-0.2,0.00889089998684463);

\path [draw=black, semithick]
(axis cs:0.8,0.0575925695550115)
--(axis cs:0.8,0.138038345893778);

\path [draw=black, semithick]
(axis cs:1.8,0.0263073527723129)
--(axis cs:1.8,0.107678298929584);

\path [draw=black, semithick]
(axis cs:2.8,0.00452051546382544)
--(axis cs:2.8,0.00969216802440007);

\path [draw=black, semithick]
(axis cs:3.8,0.0833318074189219)
--(axis cs:3.8,0.15065987047186);

\path [draw=black, semithick]
(axis cs:4.8,0.0202050852999817)
--(axis cs:4.8,0.0537283255129227);

\path [draw=black, semithick]
(axis cs:5.8,0.0223802377454315)
--(axis cs:5.8,0.0799056125902235);

\path [draw=black, semithick]
(axis cs:6.8,0.00662833251471201)
--(axis cs:6.8,0.0231814255046905);

\path [draw=black, semithick]
(axis cs:0,0.000160882245296597)
--(axis cs:0,0.00198387124437598);

\path [draw=black, semithick]
(axis cs:1,0.0640155213336673)
--(axis cs:1,0.144240566201383);

\path [draw=black, semithick]
(axis cs:2,0.0109866118383888)
--(axis cs:2,0.0503028174035312);

\path [draw=black, semithick]
(axis cs:3,0.00106921792536661)
--(axis cs:3,0.00248092682240665);

\path [draw=black, semithick]
(axis cs:4,0.095553671424591)
--(axis cs:4,0.160137775495484);

\path [draw=black, semithick]
(axis cs:5,0.0037476131669055)
--(axis cs:5,0.0247648788731591);

\path [draw=black, semithick]
(axis cs:6,-0.000578308343174787)
--(axis cs:6,0.0463638388875367);

\path [draw=black, semithick]
(axis cs:7,0.00516358887631233)
--(axis cs:7,0.0210521965373055);

\path [draw=black, semithick]
(axis cs:0.2,0.000204285712005575)
--(axis cs:0.2,0.00238907574089477);

\path [draw=black, semithick]
(axis cs:1.2,0.0892498410433739)
--(axis cs:1.2,0.189713345276434);

\path [draw=black, semithick]
(axis cs:2.2,0.0191596935053186)
--(axis cs:2.2,0.0731416978393946);

\path [draw=black, semithick]
(axis cs:3.2,0.00124153389560817)
--(axis cs:3.2,0.00382648759265178);

\path [draw=black, semithick]
(axis cs:4.2,0.110501809290316)
--(axis cs:4.2,0.20156660965948);

\path [draw=black, semithick]
(axis cs:5.2,0.00332347140801389)
--(axis cs:5.2,0.0300701282557969);

\path [draw=black, semithick]
(axis cs:6.2,3.5862217901271e-05)
--(axis cs:6.2,0.0762801322211053);

\path [draw=black, semithick]
(axis cs:7.2,0.00889563348400854)
--(axis cs:7.2,0.0435768888324803);

\path [draw=black, semithick]
(axis cs:0.4,-1.27310342911526e-05)
--(axis cs:0.4,9.60428772861345e-05);

\path [draw=black, semithick]
(axis cs:1.4,0)
--(axis cs:1.4,0);

\path [draw=black, semithick]
(axis cs:2.4,0)
--(axis cs:2.4,0);

\path [draw=black, semithick]
(axis cs:3.4,0.00065177524818245)
--(axis cs:3.4,0.00132639716938884);

\path [draw=black, semithick]
(axis cs:4.4,-4.6982518613326e-05)
--(axis cs:4.4,0.000152582680732905);

\path [draw=black, semithick]
(axis cs:5.4,0.00183442485683591)
--(axis cs:5.4,0.00574179088520568);

\path [draw=black, semithick]
(axis cs:6.4,-6.49998852544124e-06)
--(axis cs:6.4,1.14251587710811e-05);

\path [draw=black, semithick]
(axis cs:7.4,-4.08018466403713e-07)
--(axis cs:7.4,5.18793709160202e-07);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 0.00332852906293993
0.8 0.0575925695550115
1.8 0.0263073527723129
2.8 0.00452051546382544
3.8 0.0833318074189219
4.8 0.0202050852999817
5.8 0.0223802377454315
6.8 0.00662833251471201
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 0.00889089998684463
0.8 0.138038345893778
1.8 0.107678298929584
2.8 0.00969216802440007
3.8 0.15065987047186
4.8 0.0537283255129227
5.8 0.0799056125902235
6.8 0.0231814255046905
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 0.000160882245296597
1 0.0640155213336673
2 0.0109866118383888
3 0.00106921792536661
4 0.095553671424591
5 0.0037476131669055
6 -0.000578308343174787
7 0.00516358887631233
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 0.00198387124437598
1 0.144240566201383
2 0.0503028174035312
3 0.00248092682240665
4 0.160137775495484
5 0.0247648788731591
6 0.0463638388875367
7 0.0210521965373055
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 0.000204285712005575
1.2 0.0892498410433739
2.2 0.0191596935053186
3.2 0.00124153389560817
4.2 0.110501809290316
5.2 0.00332347140801389
6.2 3.5862217901271e-05
7.2 0.00889563348400854
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 0.00238907574089477
1.2 0.189713345276434
2.2 0.0731416978393946
3.2 0.00382648759265178
4.2 0.20156660965948
5.2 0.0300701282557969
6.2 0.0762801322211053
7.2 0.0435768888324803
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 -1.27310342911526e-05
1.4 0
2.4 0
3.4 0.00065177524818245
4.4 -4.6982518613326e-05
5.4 0.00183442485683591
6.4 -6.49998852544124e-06
7.4 -4.08018466403713e-07
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 9.60428772861345e-05
1.4 0
2.4 0
3.4 0.00132639716938884
4.4 0.000152582680732905
5.4 0.00574179088520568
6.4 1.14251587710811e-05
7.4 5.18793709160202e-07
};


==> plots/thermo/length/main.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\begin{groupplot}[group style={group size=2 by 2,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.95]
\nextgroupplot[
ylabel={\footnotesize $\Delta$Metabolic rate in \si{\watt\per\kilo\gram}},
tick align=outside,
tick pos=left,
title = {(a) Original MEE Models},
ylabel style={align=center},
xlabel style={align=center, text width = 1cm},
x grid style={white!69.0196078431373!black},
xmin=-0.69, xmax=7.89,
xtick style={color=black},
tick align=outside, height = 5cm, width = 9.4cm,
xtick={0.1,1.1,2.1,3.1,4.1,5.1,6.1,7.1},
xticklabels={
  Iliop-\\ soas,
  Glute-\\als,
  Ham-\\strings,
  Rectus\\Femoris,
  Vasti,
  Gastro-\\cnemius,
  Soleus,
  Tibialis\\Anterior
},
y grid style={white!69.0196078431373!black},
tick label style = {font=\scriptsize, align = center},
ymin=-0.1, ymax=0.9,
ytick style={color=black},
ymajorgrids = true,
grid style = dotted,
legend image post style={scale=0.7},legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.986,0.97)}, anchor=north east, draw=white!80!black, font = \footnotesize}
]


% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};

\input{plots/thermo/length/barnomc}


\nextgroupplot[
tick align = outside,
tick pos=left,
title = {(b) MC-MEE Models},
x grid style={white!69.0196078431373!black},
xmin=-0.69, xmax=7.89,
tick align=outside, height = 5cm, width =9.4cm,
xtick style={color=black},
xtick={0.1,1.1,2.1,3.1,4.1,5.1,6.1,7.1},
xticklabels={
  Iliop-\\ soas,
  Glute-\\als,
  Ham-\\strings,
  Rectus\\Femoris,
  Vasti,
  Gastro-\\cnemius,
  Soleus,
  Tibialis\\Anterior
},
tick label style = {font=\scriptsize, align = center},
y grid style={white!69.0196078431373!black},
ymin=-0.1, ymax=0.9,
ytick style={color=black},
legend image post style={scale=0.6},
legend columns = 2,
ymajorgrids = true,
grid style = dotted,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.986,0.97)}, anchor=north east, draw=white!80!black, font = \footnotesize}
]
\addlegendimage{ybar, ybar legend, draw=black, fill=color0}
\addlegendentry{BHAR04}
\addlegendimage{ybar, ybar legend, draw=black, fill=color1}
\addlegendentry{HOUD06}
\addlegendimage{ybar, ybar legend, draw=black, fill=color2}
\addlegendentry{LICH05}
\addlegendimage{ybar, ybar legend, draw=black, fill=color3}
\addlegendentry{UMBE03}
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80)
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80)
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/thermo/length/barmc}

\end{groupplot}

\end{tikzpicture}

==> plots/thermo/length/mc.tex <==
\draw[draw=black,fill=color0] (axis cs:-0.3,0) rectangle (axis cs:-0.1,-0.0642646952343096);
\draw[draw=black,fill=color0] (axis cs:0.7,0) rectangle (axis cs:0.9,-0.477812702942312);
\draw[draw=black,fill=color0] (axis cs:1.7,0) rectangle (axis cs:1.9,-0.292539526482175);
\draw[draw=black,fill=color0] (axis cs:2.7,0) rectangle (axis cs:2.9,-0.016613553094777);
\draw[draw=black,fill=color0] (axis cs:3.7,0) rectangle (axis cs:3.9,-0.566570588354461);
\draw[draw=black,fill=color0] (axis cs:4.7,0) rectangle (axis cs:4.9,-0.115539833957732);
\draw[draw=black,fill=color0] (axis cs:5.7,0) rectangle (axis cs:5.9,-0.41128487993343);
\draw[draw=black,fill=color0] (axis cs:6.7,0) rectangle (axis cs:6.9,-0.0922810863558905);
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,-0.00395655116701915);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,-0.47999960512076);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,-0.153520769741269);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,-0.00505274469354635);
\draw[draw=black,fill=color1] (axis cs:3.9,0) rectangle (axis cs:4.1,-0.546878902496447);
\draw[draw=black,fill=color1] (axis cs:4.9,0) rectangle (axis cs:5.1,-0.0429334884449069);
\draw[draw=black,fill=color1] (axis cs:5.9,0) rectangle (axis cs:6.1,-0.0979318930495563);
\draw[draw=black,fill=color1] (axis cs:6.9,0) rectangle (axis cs:7.1,-0.100965560587994);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,-0.00233460331088653);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,-0.282755473984617);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,-0.0852778202992319);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,-0.00226008456691849);
\draw[draw=black,fill=color2] (axis cs:4.1,0) rectangle (axis cs:4.3,-0.244438674107618);
\draw[draw=black,fill=color2] (axis cs:5.1,0) rectangle (axis cs:5.3,-0.0215409354660487);
\draw[draw=black,fill=color2] (axis cs:6.1,0) rectangle (axis cs:6.3,-0.0471559170458733);
\draw[draw=black,fill=color2] (axis cs:7.1,0) rectangle (axis cs:7.3,-0.0363211243150463);
\draw[draw=black,fill=color3] (axis cs:0.3,0) rectangle (axis cs:0.5,-5.55835019545037e-05);
\draw[draw=black,fill=color3] (axis cs:1.3,0) rectangle (axis cs:1.5,0);
\draw[draw=black,fill=color3] (axis cs:2.3,0) rectangle (axis cs:2.5,0);
\draw[draw=black,fill=color3] (axis cs:3.3,0) rectangle (axis cs:3.5,-0.000994994912851127);
\draw[draw=black,fill=color3] (axis cs:4.3,0) rectangle (axis cs:4.5,-1.35617864321924e-05);
\draw[draw=black,fill=color3] (axis cs:5.3,0) rectangle (axis cs:5.5,-0.00753674292180445);
\draw[draw=black,fill=color3] (axis cs:6.3,0) rectangle (axis cs:6.5,-8.72108338245692e-06);
\draw[draw=black,fill=color3] (axis cs:7.3,0) rectangle (axis cs:7.5,-3.72391716491061e-08);
\path [draw=black, semithick]
(axis cs:-0.2,-0.0878417033985801)
--(axis cs:-0.2,-0.040687687070039);

\path [draw=black, semithick]
(axis cs:0.8,-0.689049849489613)
--(axis cs:0.8,-0.266575556395012);

\path [draw=black, semithick]
(axis cs:1.8,-0.474542590556884)
--(axis cs:1.8,-0.110536462407466);

\path [draw=black, semithick]
(axis cs:2.8,-0.0251913892226461)
--(axis cs:2.8,-0.00803571696690782);

\path [draw=black, semithick]
(axis cs:3.8,-0.733888062401678)
--(axis cs:3.8,-0.399253114307244);

\path [draw=black, semithick]
(axis cs:4.8,-0.170370565419231)
--(axis cs:4.8,-0.0607091024962335);

\path [draw=black, semithick]
(axis cs:5.8,-0.52241527129493)
--(axis cs:5.8,-0.300154488571929);

\path [draw=black, semithick]
(axis cs:6.8,-0.138574855628252)
--(axis cs:6.8,-0.0459873170835293);

\path [draw=black, semithick]
(axis cs:0,-0.00716316012180344)
--(axis cs:0,-0.000749942212234859);

\path [draw=black, semithick]
(axis cs:1,-0.657317596815313)
--(axis cs:1,-0.302681613426207);

\path [draw=black, semithick]
(axis cs:2,-0.247847628751124)
--(axis cs:2,-0.0591939107314153);

\path [draw=black, semithick]
(axis cs:3,-0.00699336720600633)
--(axis cs:3,-0.00311212218108637);

\path [draw=black, semithick]
(axis cs:4,-0.68994731722766)
--(axis cs:4,-0.403810487765234);

\path [draw=black, semithick]
(axis cs:5,-0.0666906338793946)
--(axis cs:5,-0.0191763430104192);

\path [draw=black, semithick]
(axis cs:6,-0.18427137976368)
--(axis cs:6,-0.0115924063354322);

\path [draw=black, semithick]
(axis cs:7,-0.161240803717602)
--(axis cs:7,-0.0406903174583854);

\path [draw=black, semithick]
(axis cs:0.2,-0.00439368049077432)
--(axis cs:0.2,-0.000275526130998737);

\path [draw=black, semithick]
(axis cs:1.2,-0.390530383738622)
--(axis cs:1.2,-0.174980564230611);

\path [draw=black, semithick]
(axis cs:2.2,-0.141548550278941)
--(axis cs:2.2,-0.0290070903195224);

\path [draw=black, semithick]
(axis cs:3.2,-0.00333857688922686)
--(axis cs:3.2,-0.00118159224461012);

\path [draw=black, semithick]
(axis cs:4.2,-0.297617420375949)
--(axis cs:4.2,-0.191259927839286);

\path [draw=black, semithick]
(axis cs:5.2,-0.0378201490463825)
--(axis cs:5.2,-0.00526172188571498);

\path [draw=black, semithick]
(axis cs:6.2,-0.096936782303368)
--(axis cs:6.2,0.00262494821162141);

\path [draw=black, semithick]
(axis cs:7.2,-0.0582497350756914)
--(axis cs:7.2,-0.0143925135544012);

\path [draw=black, semithick]
(axis cs:0.4,-0.000133074327797382)
--(axis cs:0.4,2.1907323888375e-05);

\path [draw=black, semithick]
(axis cs:1.4,0)
--(axis cs:1.4,0);

\path [draw=black, semithick]
(axis cs:2.4,0)
--(axis cs:2.4,0);

\path [draw=black, semithick]
(axis cs:3.4,-0.00144612768035771)
--(axis cs:3.4,-0.000543862145344542);

\path [draw=black, semithick]
(axis cs:4.4,-4.13648923547607e-05)
--(axis cs:4.4,1.42413194903759e-05);

\path [draw=black, semithick]
(axis cs:5.4,-0.0125107479169171)
--(axis cs:5.4,-0.00256273792669176);

\path [draw=black, semithick]
(axis cs:6.4,-4.29160454860355e-05)
--(axis cs:6.4,2.54738787211217e-05);

\path [draw=black, semithick]
(axis cs:7.4,-3.48804434972725e-07)
--(axis cs:7.4,2.74326091674513e-07);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 -0.0878417033985801
0.8 -0.689049849489613
1.8 -0.474542590556884
2.8 -0.0251913892226461
3.8 -0.733888062401678
4.8 -0.170370565419231
5.8 -0.52241527129493
6.8 -0.138574855628252
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 -0.040687687070039
0.8 -0.266575556395012
1.8 -0.110536462407466
2.8 -0.00803571696690782
3.8 -0.399253114307244
4.8 -0.0607091024962335
5.8 -0.300154488571929
6.8 -0.0459873170835293
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 -0.00716316012180344
1 -0.657317596815313
2 -0.247847628751124
3 -0.00699336720600633
4 -0.68994731722766
5 -0.0666906338793946
6 -0.18427137976368
7 -0.161240803717602
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 -0.000749942212234859
1 -0.302681613426207
2 -0.0591939107314153
3 -0.00311212218108637
4 -0.403810487765234
5 -0.0191763430104192
6 -0.0115924063354322
7 -0.0406903174583854
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 -0.00439368049077432
1.2 -0.390530383738622
2.2 -0.141548550278941
3.2 -0.00333857688922686
4.2 -0.297617420375949
5.2 -0.0378201490463825
6.2 -0.096936782303368
7.2 -0.0582497350756914
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 -0.000275526130998737
1.2 -0.174980564230611
2.2 -0.0290070903195224
3.2 -0.00118159224461012
4.2 -0.191259927839286
5.2 -0.00526172188571498
6.2 0.00262494821162141
7.2 -0.0143925135544012
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 -0.000133074327797382
1.4 0
2.4 0
3.4 -0.00144612768035771
4.4 -4.13648923547607e-05
5.4 -0.0125107479169171
6.4 -4.29160454860355e-05
7.4 -3.48804434972725e-07
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 2.1907323888375e-05
1.4 0
2.4 0
3.4 -0.000543862145344542
4.4 1.42413194903759e-05
5.4 -0.00256273792669176
6.4 2.54738787211217e-05
7.4 2.74326091674513e-07
};

==> plots/thermo/length/nomc.tex <==
py
\draw[draw=black,fill=color0] (axis cs:-0.3,0) rectangle (axis cs:-0.1,-0.00610971452489228);
\draw[draw=black,fill=color0] (axis cs:0.7,0) rectangle (axis cs:0.9,-0.0978154577243947);
\draw[draw=black,fill=color0] (axis cs:1.7,0) rectangle (axis cs:1.9,-0.0669928258509485);
\draw[draw=black,fill=color0] (axis cs:2.7,0) rectangle (axis cs:2.9,-0.00710634174411276);
\draw[draw=black,fill=color0] (axis cs:3.7,0) rectangle (axis cs:3.9,-0.116995838945391);
\draw[draw=black,fill=color0] (axis cs:4.7,0) rectangle (axis cs:4.9,-0.0369667054064522);
\draw[draw=black,fill=color0] (axis cs:5.7,0) rectangle (axis cs:5.9,-0.0511429251678275);
\draw[draw=black,fill=color0] (axis cs:6.7,0) rectangle (axis cs:6.9,-0.0149048790097013);
\draw[draw=black,fill=color1] (axis cs:-0.1,0) rectangle (axis cs:0.1,-0.00107237674483629);
\draw[draw=black,fill=color1] (axis cs:0.9,0) rectangle (axis cs:1.1,-0.104128043767525);
\draw[draw=black,fill=color1] (axis cs:1.9,0) rectangle (axis cs:2.1,-0.03064471462096);
\draw[draw=black,fill=color1] (axis cs:2.9,0) rectangle (axis cs:3.1,-0.00177507237388663);
\draw[draw=black,fill=color1] (axis cs:3.9,0) rectangle (axis cs:4.1,-0.127845723460038);
\draw[draw=black,fill=color1] (axis cs:4.9,0) rectangle (axis cs:5.1,-0.0142562460200323);
\draw[draw=black,fill=color1] (axis cs:5.9,0) rectangle (axis cs:6.1,-0.022892765272181);
\draw[draw=black,fill=color1] (axis cs:6.9,0) rectangle (axis cs:7.1,-0.0131078927068089);
\draw[draw=black,fill=color2] (axis cs:0.1,0) rectangle (axis cs:0.3,-0.00129668072645017);
\draw[draw=black,fill=color2] (axis cs:1.1,0) rectangle (axis cs:1.3,-0.139481593159904);
\draw[draw=black,fill=color2] (axis cs:2.1,0) rectangle (axis cs:2.3,-0.0461506956723566);
\draw[draw=black,fill=color2] (axis cs:3.1,0) rectangle (axis cs:3.3,-0.00253401074412998);
\draw[draw=black,fill=color2] (axis cs:4.1,0) rectangle (axis cs:4.3,-0.156034209474898);
\draw[draw=black,fill=color2] (axis cs:5.1,0) rectangle (axis cs:5.3,-0.0166967998319054);
\draw[draw=black,fill=color2] (axis cs:6.1,0) rectangle (axis cs:6.3,-0.0381579972195033);
\draw[draw=black,fill=color2] (axis cs:7.1,0) rectangle (axis cs:7.3,-0.0262362611582444);
\draw[draw=black,fill=color3] (axis cs:0.3,0) rectangle (axis cs:0.5,-4.1655921497491e-05);
\draw[draw=black,fill=color3] (axis cs:1.3,0) rectangle (axis cs:1.5,0);
\draw[draw=black,fill=color3] (axis cs:2.3,0) rectangle (axis cs:2.5,0);
\draw[draw=black,fill=color3] (axis cs:3.3,0) rectangle (axis cs:3.5,-0.000989086208785645);
\draw[draw=black,fill=color3] (axis cs:4.3,0) rectangle (axis cs:4.5,-5.28000810597895e-05);
\draw[draw=black,fill=color3] (axis cs:5.3,0) rectangle (axis cs:5.5,-0.0037881078710208);
\draw[draw=black,fill=color3] (axis cs:6.3,0) rectangle (axis cs:6.5,-2.46258512281994e-06);
\draw[draw=black,fill=color3] (axis cs:7.3,0) rectangle (axis cs:7.5,-5.53876213782445e-08);
\path [draw=black, semithick]
(axis cs:-0.2,-0.00889089998684463)
--(axis cs:-0.2,-0.00332852906293993);

\path [draw=black, semithick]
(axis cs:0.8,-0.138038345893778)
--(axis cs:0.8,-0.0575925695550115);

\path [draw=black, semithick]
(axis cs:1.8,-0.107678298929584)
--(axis cs:1.8,-0.0263073527723129);

\path [draw=black, semithick]
(axis cs:2.8,-0.00969216802440007)
--(axis cs:2.8,-0.00452051546382544);

\path [draw=black, semithick]
(axis cs:3.8,-0.15065987047186)
--(axis cs:3.8,-0.0833318074189219);

\path [draw=black, semithick]
(axis cs:4.8,-0.0537283255129227)
--(axis cs:4.8,-0.0202050852999817);

\path [draw=black, semithick]
(axis cs:5.8,-0.0799056125902235)
--(axis cs:5.8,-0.0223802377454315);

\path [draw=black, semithick]
(axis cs:6.8,-0.0231814255046905)
--(axis cs:6.8,-0.00662833251471201);

\path [draw=black, semithick]
(axis cs:0,-0.00198387124437598)
--(axis cs:0,-0.000160882245296597);

\path [draw=black, semithick]
(axis cs:1,-0.144240566201383)
--(axis cs:1,-0.0640155213336673);

\path [draw=black, semithick]
(axis cs:2,-0.0503028174035312)
--(axis cs:2,-0.0109866118383888);

\path [draw=black, semithick]
(axis cs:3,-0.00248092682240665)
--(axis cs:3,-0.00106921792536661);

\path [draw=black, semithick]
(axis cs:4,-0.160137775495484)
--(axis cs:4,-0.095553671424591);

\path [draw=black, semithick]
(axis cs:5,-0.0247648788731591)
--(axis cs:5,-0.0037476131669055);

\path [draw=black, semithick]
(axis cs:6,-0.0463638388875367)
--(axis cs:6,0.000578308343174787);

\path [draw=black, semithick]
(axis cs:7,-0.0210521965373055)
--(axis cs:7,-0.00516358887631233);

\path [draw=black, semithick]
(axis cs:0.2,-0.00238907574089477)
--(axis cs:0.2,-0.000204285712005575);

\path [draw=black, semithick]
(axis cs:1.2,-0.189713345276434)
--(axis cs:1.2,-0.0892498410433739);

\path [draw=black, semithick]
(axis cs:2.2,-0.0731416978393946)
--(axis cs:2.2,-0.0191596935053186);

\path [draw=black, semithick]
(axis cs:3.2,-0.00382648759265178)
--(axis cs:3.2,-0.00124153389560817);

\path [draw=black, semithick]
(axis cs:4.2,-0.20156660965948)
--(axis cs:4.2,-0.110501809290316);

\path [draw=black, semithick]
(axis cs:5.2,-0.0300701282557969)
--(axis cs:5.2,-0.00332347140801389);

\path [draw=black, semithick]
(axis cs:6.2,-0.0762801322211053)
--(axis cs:6.2,-3.5862217901271e-05);

\path [draw=black, semithick]
(axis cs:7.2,-0.0435768888324803)
--(axis cs:7.2,-0.00889563348400854);

\path [draw=black, semithick]
(axis cs:0.4,-9.60428772861345e-05)
--(axis cs:0.4,1.27310342911526e-05);

\path [draw=black, semithick]
(axis cs:1.4,0)
--(axis cs:1.4,0);

\path [draw=black, semithick]
(axis cs:2.4,0)
--(axis cs:2.4,0);

\path [draw=black, semithick]
(axis cs:3.4,-0.00132639716938884)
--(axis cs:3.4,-0.00065177524818245);

\path [draw=black, semithick]
(axis cs:4.4,-0.000152582680732905)
--(axis cs:4.4,4.6982518613326e-05);

\path [draw=black, semithick]
(axis cs:5.4,-0.00574179088520568)
--(axis cs:5.4,-0.00183442485683591);

\path [draw=black, semithick]
(axis cs:6.4,-1.14251587710811e-05)
--(axis cs:6.4,6.49998852544124e-06);

\path [draw=black, semithick]
(axis cs:7.4,-5.18793709160202e-07)
--(axis cs:7.4,4.08018466403713e-07);

\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 -0.00889089998684463
0.8 -0.138038345893778
1.8 -0.107678298929584
2.8 -0.00969216802440007
3.8 -0.15065987047186
4.8 -0.0537283255129227
5.8 -0.0799056125902235
6.8 -0.0231814255046905
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
-0.2 -0.00332852906293993
0.8 -0.0575925695550115
1.8 -0.0263073527723129
2.8 -0.00452051546382544
3.8 -0.0833318074189219
4.8 -0.0202050852999817
5.8 -0.0223802377454315
6.8 -0.00662833251471201
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 -0.00198387124437598
1 -0.144240566201383
2 -0.0503028174035312
3 -0.00248092682240665
4 -0.160137775495484
5 -0.0247648788731591
6 -0.0463638388875367
7 -0.0210521965373055
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0 -0.000160882245296597
1 -0.0640155213336673
2 -0.0109866118383888
3 -0.00106921792536661
4 -0.095553671424591
5 -0.0037476131669055
6 0.000578308343174787
7 -0.00516358887631233
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 -0.00238907574089477
1.2 -0.189713345276434
2.2 -0.0731416978393946
3.2 -0.00382648759265178
4.2 -0.20156660965948
5.2 -0.0300701282557969
6.2 -0.0762801322211053
7.2 -0.0435768888324803
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.2 -0.000204285712005575
1.2 -0.0892498410433739
2.2 -0.0191596935053186
3.2 -0.00124153389560817
4.2 -0.110501809290316
5.2 -0.00332347140801389
6.2 -3.5862217901271e-05
7.2 -0.00889563348400854
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 -9.60428772861345e-05
1.4 0
2.4 0
3.4 -0.00132639716938884
4.4 -0.000152582680732905
5.4 -0.00574179088520568
6.4 -1.14251587710811e-05
7.4 -5.18793709160202e-07
};
\addplot [semithick, black, mark=-, mark size=2, mark options={solid}, only marks]
table {%
0.4 1.27310342911526e-05
1.4 0
2.4 0
3.4 -0.00065177524818245
4.4 4.6982518613326e-05
5.4 -0.00183442485683591
6.4 6.49998852544124e-06
7.4 4.08018466403713e-07
};


==> plots/thermo/sl/mc.tex <==


\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}


\addplot [semithick, color0]
table {%
0 0.0813295712363733
1 0.0493805419136285
2 0.023966728586436
3 0.0111807572994743
4 0.00682340528317947
5 0.015454738489824
6 0.0774288561790339
7 0.228212897153293
8 0.323477617902107
9 0.332926287066668
10 -0.0212245633173077
11 -1.29241608743966
12 -3.16829311227472
13 -5.51263570605072
14 -8.01306573800189
15 -10.4472265563311
16 -12.1548371500104
17 -12.6225739454164
18 -11.7772338091729
19 -10.2070109127165
20 -8.58297742953929
21 -7.29881302525703
22 -6.61811385084031
23 -6.5445048195314
24 -6.69231747732997
25 -6.76815869416405
26 -6.56836609463445
27 -6.05206589650836
28 -5.38573646777617
29 -4.92470119104868
30 -4.95789280519298
31 -5.438144489498
32 -6.14590539628691
33 -6.87705927464015
34 -7.49644749029219
35 -8.02430276957554
36 -8.62738121283645
37 -9.5053875900881
38 -10.7729093814601
39 -12.3978102788098
40 -14.2764250812077
41 -16.3392910673995
42 -18.6171996137331
43 -21.247431677853
44 -24.308645815093
45 -27.6091478734963
46 -30.6034843867177
47 -32.4907790431437
48 -32.4354522785984
49 -29.723457606048
50 -23.9601176193007
51 -15.305485864979
52 -4.17597672207816
53 13.0430917533774
54 37.3308012767908
55 63.2068085939499
56 87.0237344615878
57 105.800070779278
58 117.198374067973
59 117.843305041531
60 106.564184260539
61 88.5324525378766
62 67.2325820197675
63 46.9432578325272
64 32.4443415886733
65 22.0495516329838
66 14.3822141546976
67 8.48428249694448
68 3.8254231715468
69 0.396342831365396
70 -1.41678010951348
71 -1.91762559098874
72 -1.74573485382366
73 -1.37453177702471
74 -1.02109129457138
75 -0.743872040330914
76 -0.531181547830716
77 -0.37283107959308
78 -0.25922532560342
79 -0.178211183932754
80 -0.120788640959361
81 -0.080643060336697
82 -0.0524508824256096
83 -0.0327846411097422
84 -0.019662970027408
85 -0.0112424103477302
86 -0.00602982259446218
87 -0.00303010960716282
88 -0.00146345030628879
89 -0.000772494173613802
90 -0.000977757430466986
91 0.000202864658955968
92 0.00664954995799163
93 0.0260025228681151
94 0.0626653485178146
95 0.0945466706049386
96 0.152848184788309
97 0.130139213918109
98 0.0140491755370406
99 -0.0236066370370803
};
\addplot [semithick, color1]
table {%
0 0.0156356337832237
1 0.0092632684039572
2 0.00430555376672167
3 0.00194685653585499
4 0.00117382543896863
5 0.00281658291547306
6 0.0162272580639273
7 0.0533142402070228
8 0.0788109270045424
9 0.0778765598055547
10 0.0077588332559608
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0.18445116480343
53 2.43306587070415
54 7.69114209367458
55 14.7841890246239
56 23.2606767809992
57 32.451746969485
58 41.2385680972437
59 47.0349088980058
60 47.7153115079759
61 43.7190767815501
62 35.3659527132745
63 25.236091149362
64 16.944829011159
65 10.4314372921887
66 5.71466661768946
67 2.66693775967846
68 0.929269137320271
69 0.140230466641991
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
80 0
81 0
82 0
83 0
84 0
85 0
86 0
87 0
88 0
89 0
90 0
91 8.03972492865269e-05
92 0.0011665627517344
93 0.00484118755403823
94 0.0123149026053696
95 0.0192444405919212
96 0.0304240639314442
97 0.0238195299232657
98 0.0024231243189026
99 0
};
\addplot [semithick, color2]
table {%
0 0.0211305567503443
1 0.0125187134347895
2 0.0058186799122265
3 0.00263105180679035
4 0.00158634983378401
5 0.003806431255848
6 0.0219300990401945
7 0.0720507779802792
8 0.106507915745863
9 0.105245178373167
10 0.0132715874207012
11 0.0639741469330086
12 0.156850203409167
13 0.272909003613312
14 0.39657405372424
15 0.516855910586708
16 0.601213521842252
17 0.624335653907847
18 0.582678937260811
19 0.505529625637608
20 0.426101372333057
21 0.363558864433793
22 0.330617040580336
23 0.327360881139472
24 0.334817551775291
25 0.338617796918787
26 0.328779735116327
27 0.303356305530711
28 0.270542714088131
29 0.247886889581716
30 0.249701694164974
31 0.273634398396919
32 0.308787399979286
33 0.345063194708402
34 0.37582579716226
35 0.402121668135068
36 0.43219189077617
37 0.475861962193307
38 0.538726198461798
39 0.619150853108125
40 0.712008071188047
41 0.813887398747375
42 0.926321589094007
43 1.05606311245004
44 1.20697562477199
45 1.36965192950558
46 1.51729607920007
47 1.61054456054597
48 1.60834052279383
49 1.47566887793162
50 1.19311235537659
51 0.767109107048925
52 0.515889255474852
53 3.28813255484431
54 10.3940855061297
55 19.9798837401671
56 31.4353135655874
57 43.8564557403665
58 55.731281223581
59 63.5646642468044
60 64.484184757606
61 59.0835296997315
62 47.7948179906641
63 34.1049594523391
64 22.8998501761635
65 14.0974188028603
66 7.72300560044782
67 3.60419542065433
68 1.2558476691593
69 0.207881253685484
70 0.0703381166197823
71 0.0948517876849701
72 0.0863813389053017
73 0.0680403708955569
74 0.0505522502299282
75 0.0368291279369332
76 0.0262968167718858
77 0.0184544413967188
78 0.0128287167303264
79 0.0088175951795487
80 0.00597517468259977
81 0.00398859847154089
82 0.00259407222595957
83 0.00162180357216797
84 0.000973480134460332
85 0.000557589909385275
86 0.000300066543264415
87 0.000151585801504041
88 7.37048140187316e-05
89 3.92354180821908e-05
90 5.00049835642253e-05
91 0.000122311318087662
92 0.00157653477755477
93 0.00654255463948173
94 0.0166428014358417
95 0.0260076278131137
96 0.0411161720971795
97 0.032190567762603
98 0.00329895283378862
99 0.00120764847772551
};
\addplot [semithick, color3]
table {%
0 6.39676268793862e-06
1 2.73382242417187e-06
2 9.98771859937231e-07
3 3.77452190686907e-07
4 2.42354184059806e-07
5 1.26757555798941e-06
6 0.000101744555546753
7 0.000686542767791661
8 0.000599665941592283
9 0.000444078847198517
10 0.000870194751103948
11 0.01615295535527
12 0.0410679148079071
13 0.0586851095727361
14 0.0694152027788033
15 0.0761397692108308
16 0.0755517200972221
17 0.071321959844917
18 0.0655352096910889
19 0.0611701492213638
20 0.056223675576315
21 0.0502626997825239
22 0.0457332282083375
23 0.0431947299421368
24 0.0414324058965265
25 0.0401842350679499
26 0.0382593218190946
27 0.0358074244231522
28 0.0329633318837675
29 0.0312873003754375
30 0.0317982238970872
31 0.034276919484694
32 0.0381062299511371
33 0.0422943891399796
34 0.0462152394028218
35 0.0500145891547935
36 0.0543398812421454
37 0.0600147592731135
38 0.0674809407890876
39 0.0766376105397883
40 0.0870324240430798
41 0.0984400116048523
42 0.111105088178931
43 0.1255891116049
44 0.14206838903183
45 0.159446376793257
46 0.174800660306388
47 0.184317604752606
48 0.183997358291255
49 0.170058599388371
50 0.140059791195118
51 0.0930181445638852
52 0.138557854543199
53 1.52125415252071
54 5.30668449334968
55 10.8653068072884
56 17.226883470516
57 22.9535749664741
58 27.050191950676
59 26.9171897551169
60 18.7975437114124
61 8.83354577723169
62 3.81504256268549
63 1.01213181645665
64 0.514224532062791
65 0.275015731947482
66 0.15469362194366
67 0.053264427849953
68 0.0137575963870257
69 0.00276794021934884
70 0.00464314222093945
71 0.00591453214586625
72 0.00520613931539863
73 0.00400911607441923
74 0.00292779418399325
75 0.00210139318596614
76 0.00148199089730565
77 0.00102988972044634
78 0.000710385444602303
79 0.000485612337689653
80 0.000328198767620147
81 0.000219157973667159
82 0.000143143858626517
83 9.03439922121523e-05
84 5.50576568762049e-05
85 3.22506265552038e-05
86 1.79231723735395e-05
87 9.43686726886008e-06
88 4.98463244563162e-06
89 4.65910629131749e-06
90 1.59975818089605e-05
91 3.6105724181967e-06
92 1.99158974165439e-06
93 1.38579794296194e-05
94 5.3821446228313e-05
95 7.03463276516992e-05
96 0.000344277265599781
97 0.000305980464747168
98 2.14060165108277e-05
99 7.86774571535262e-05
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};

==> plots/thermo/sl/nomc.tex <==

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}

\addplot [semithick, color0]
table {%
0 0.0296866568408243
1 0.0178165199316929
2 0.00847500758030781
3 0.00389784267925516
4 0.00236583966827924
5 0.00550138704138131
6 0.0294764279894785
7 0.0918414760005698
8 0.133111774872596
9 0.134072167674092
10 -0.00130814119686298
11 -0.348193628096914
12 -0.853579187352001
13 -1.48517543654919
14 -2.15882366260333
15 -2.81461810445715
16 -3.27467050845332
17 -3.40068485736897
18 -3.172939279242
19 -2.74990089976692
20 -2.31236525149238
21 -1.96639473368046
22 -1.78300556243278
23 -1.763174336312
24 -1.80299698019404
25 -1.82342958599753
26 -1.76960287277939
27 -1.63050491437436
28 -1.45098713867286
29 -1.32677826566012
30 -1.335720516274
31 -1.46510653830124
32 -1.65578649064398
33 -1.85276881241722
34 -2.01964001752238
35 -2.16185106440581
36 -2.32432820565066
37 -2.56087449206615
38 -2.90236127447231
39 -3.34013061535613
40 -3.84625376733525
41 -4.40201657390382
42 -5.01571463053522
43 -5.72433320472601
44 -6.5490639297503
45 -7.43826191902434
46 -8.2449749462098
47 -8.75343656325042
48 -8.73853081651367
49 -8.00788433695342
50 -6.45516592107772
51 -4.12349606671225
52 -1.044532567939
53 4.69357711943713
54 14.0916063933087
55 25.4531335316724
56 37.6726722365575
57 49.5753826708188
58 59.7024465675272
59 65.0692464823828
60 63.5293080156381
61 56.4683045107083
62 44.841376486587
63 31.8002721170197
64 21.5289760483523
65 13.6503006599359
66 7.91812450871932
67 4.03395164682697
68 1.57168869942979
69 0.1737004736069
70 -0.381698905902912
71 -0.516633163535294
72 -0.470323573310113
73 -0.370316658101082
74 -0.275095215797971
75 -0.200408759284163
76 -0.143107186698453
77 -0.100445520241069
78 -0.0698386591544751
79 -0.0480124004212297
80 -0.0325420238399029
81 -0.021726284617131
82 -0.014130946856935
83 -0.00883260680890381
84 -0.00529745872056371
85 -0.00302885091386115
86 -0.00162451228079792
87 -0.000816350761881549
88 -0.00039427246119762
89 -0.000208119932588564
90 -0.000263420511723482
91 9.07721815982254e-05
92 0.00232604567184788
93 0.0093486013010418
94 0.0231158654634115
95 0.0354770993802335
96 0.0567320219229188
97 0.0464176430817843
98 0.00483971619874597
99 -0.00635993367537816
};
\addplot [semithick, color1]
table {%
0 0.0174351763669924
1 0.0103294001763505
2 0.00480109027373776
3 0.00217092492280573
4 0.00130892382337831
5 0.00314075019691371
6 0.0180948921047791
7 0.0594503039511578
8 0.0878814655690317
9 0.0868395598086549
10 0.00865181597978508
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0.205680091643969
53 2.71309325585205
54 8.57633407931918
55 16.485736789502
56 25.9378038469708
57 36.1866963421119
58 45.9848137828046
59 52.4482693449906
60 53.2069811228349
61 48.7508101594364
62 39.4363050127364
63 28.1405733917047
64 18.8950500129439
65 11.6320164230038
66 6.37238130154243
67 2.97388202131444
68 1.03622095056778
69 0.156369927297227
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
80 0
81 0
82 0
83 0
84 0
85 0
86 0
87 0
88 0
89 0
90 0
91 8.96503614861876e-05
92 0.00130082525605559
93 0.0053983714379976
94 0.0137322542753163
95 0.0214593294046233
96 0.0339256424011753
97 0.026560976737418
98 0.00270200750701548
99 0
};
\addplot [semithick, color2]
table {%
0 0.0236890983247174
1 0.0140345111091717
2 0.00652322048062203
3 0.0029496262538121
4 0.00177842910785094
5 0.00426732363711107
6 0.0245854512293196
7 0.0807748694988555
8 0.119404165175314
9 0.117988532348716
10 0.0579670069711275
11 1.06114103836493
12 2.60167889206314
13 4.52674959115315
14 6.57798537897188
15 8.57310404184607
16 9.97234619657821
17 10.3558736745607
18 9.66491250232344
19 8.38523462352792
20 7.06775587269184
21 6.03036147267478
22 5.48395448101772
23 5.42994446953951
24 5.55362848254438
25 5.61666325941813
26 5.4534790417764
27 5.03177987480621
28 4.48749987788301
29 4.11170705696543
30 4.14180927344241
31 4.53878173555528
32 5.12186559660025
33 5.72357326027066
34 6.23383344310479
35 6.67000382077336
36 7.16877947948839
37 7.89313622593438
38 8.93586714378185
39 10.2698732326932
40 11.8100986133644
41 13.499973986731
42 15.3649231765511
43 17.516949603058
44 20.0201398401277
45 22.7184564445389
46 25.167434255519
47 26.7141495313781
48 26.6775910929928
49 24.4769626557259
50 19.7901893869115
51 12.7240610999549
52 4.70181289506983
53 3.68626801066858
54 11.652627825162
55 22.3990988987798
56 35.241581313819
57 49.166706986565
58 62.4793665527236
59 71.2612355230852
60 72.2920939168953
61 66.237513803582
62 53.5819361586092
63 38.2344747169901
64 25.6726223001955
65 15.8043701399509
66 8.65812676840003
67 4.04060057243809
68 1.40790890022797
69 0.51714241955218
70 1.1667003889041
71 1.57330936480009
72 1.43280978419784
73 1.12858761365668
74 0.838511646850765
75 0.610885817703771
76 0.436186065665431
77 0.306104356915698
78 0.212790298030285
79 0.146257708047376
80 0.0991103964816492
81 0.0661589990116438
82 0.0430279515619155
83 0.0269009030850603
84 0.0161471433419908
85 0.00924876006625748
86 0.00497721249228392
87 0.00251435810434204
88 0.00122254389671238
89 0.000650799022424106
90 0.000829434118728121
91 0.000348379564685645
92 0.00176742561964076
93 0.00733474380162717
94 0.0186579541784189
95 0.0291566975606294
96 0.0460946228276838
97 0.0360882836106227
98 0.00407353500682364
99 0.0200313004716639
};
\addplot [semithick, color3]
table {%
0 2.94074813144451e-06
1 1.25680497742136e-06
2 4.59159831954978e-07
3 1.73523996218446e-07
4 1.11416141052953e-07
5 5.82735460962259e-07
6 4.6774458613719e-05
7 0.000315620488055136
8 0.000275681087959307
9 0.000204153898436071
10 0.117294019425621
11 2.29000846715977
12 5.82220841760826
13 8.31980246722588
14 9.84101042916645
15 10.7943538718138
16 10.7109860038508
17 10.1113318490045
18 9.29094285156441
19 8.67210715150326
20 7.97084436208753
21 7.12575535267215
22 6.48361104975595
23 6.123727524072
24 5.87388240919585
25 5.69692892278819
26 5.42403349644205
27 5.07642739750714
28 4.67321969629523
29 4.43560829572573
30 4.50804204948258
31 4.85944733466337
32 5.40232962453964
33 5.99608598635199
34 6.55194589575518
35 7.09058064774674
36 7.70377837442426
37 8.50830723339719
38 9.56678962952132
39 10.864932959884
40 12.3386082356173
41 13.9558647395674
42 15.7513957711321
43 17.8047993467935
44 20.1410705745866
45 22.6047521882972
46 24.78153275129
47 26.1307523141496
48 26.0853508942892
49 24.1092496046333
50 19.8563111635672
51 13.1872053110883
52 4.78435929738165
53 0.699357710254393
54 2.43961254611004
55 4.99504706519001
56 7.91961932120037
57 10.5523193505218
58 12.4356342911011
59 12.374489931501
60 9.60559943939896
61 6.12667942560651
62 2.84802391811574
63 0.779543049769101
64 0.385236545335237
65 0.175464742696512
66 0.0711164384032821
67 0.0244869591563177
68 0.00632470326663801
69 0.178002243991043
70 0.658259418559549
71 0.838504681987093
72 0.738075655585007
73 0.568373375293894
74 0.415074104025072
75 0.297915030584438
76 0.210102215256628
77 0.146007719837687
78 0.100711519799724
79 0.0688453809601932
80 0.0465288202828056
81 0.0310700800135397
82 0.0202935401644442
83 0.0128080900722199
84 0.00780553760320719
85 0.00457217928597376
86 0.00254097257071776
87 0.00133786700166307
88 0.000706672571991699
89 0.000660522648756871
90 0.00226798112115431
91 0.000496350228853208
92 9.15582474619135e-07
93 6.37085180447462e-06
94 2.47430341172399e-05
95 3.23399259418802e-05
96 0.000158272672428566
97 0.000140666697181121
98 0.000233173348885706
99 0.0111541225177344
};
\addplot [semithick, black]
table {%
0 0.0806979661833604
1 0.0490801823434606
2 0.0238897026261653
3 0.0111671215378633
4 0.00682025021808123
5 0.0153905550757236
6 0.0763429955706336
7 0.223030886229456
8 0.314961717557747
9 0.325330594282857
10 -0.0610221189471252
11 -2.21779380953448
12 -5.4368101105223
13 -9.45971615636426
14 -13.7504691885562
15 -17.9275038500455
16 -20.8577739391931
17 -21.6604131042609
18 -20.2098043263822
19 -17.5152923552033
20 -14.7284410923082
21 -12.5248072208947
22 -11.3567233275973
23 -11.2304097854268
24 -11.4840571986882
25 -11.6142011846977
26 -11.2713558775758
27 -10.3853816202188
28 -9.24195629727935
29 -8.45081697872689
30 -8.50777398900639
31 -9.33188877898876
32 -10.546410768433
33 -11.8010752383262
34 -12.8639491561935
35 -13.7697520025848
36 -14.804638252552
37 -16.3113024972366
38 -18.4863775444096
39 -21.274717295262
40 -24.498431639078
41 -28.0383221267759
42 -31.9472269460842
43 -36.4607210492103
44 -41.7137829920401
45 -47.3774644523843
46 -52.5157639885975
47 -55.7543730143339
48 -55.6594319523164
49 -51.0056327194485
50 -41.1157065036798
51 -26.2643061574029
52 -7.95395767753851
53 12.9686977367181
54 36.8551365844724
55 61.7650568691848
56 83.9892233095185
57 100.603834441206
58 109.531399854356
59 108.122531931157
60 95.9020439379176
61 78.2016426467542
62 58.6052074726506
63 40.7233794341446
64 28.3249876457063
65 19.6416876131516
66 13.2051298719072
67 8.04426266925885
68 3.7257055737994
69 0.128680156877746
70 -2.43120322231154
71 -3.29065709258149
72 -2.99569154974595
73 -2.35870482866932
74 -1.75219882673867
75 -1.27648891263798
76 -0.911510743302247
77 -0.639780383701078
78 -0.444832223913854
79 -0.305811467651145
80 -0.207274037196834
81 -0.138383978453063
82 -0.0900060309358916
83 -0.0562586420949287
84 -0.0337417752902147
85 -0.0192920440373322
86 -0.0103472119796046
87 -0.00519968638141114
88 -0.00251128956176828
89 -0.00132560466616919
90 -0.00167783765428969
91 1.31668787057282e-05
92 0.00663829597376559
93 0.0258575848222245
94 0.0620820821623523
95 0.0934267385635038
96 0.151285907295562
97 0.129561897616589
98 0.0137301713085735
99 -0.0405091316903067
};

==> plots/thermo/sl/slmain.tex <==
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019807843137}
\definecolor{color2}{rgb}{0.172549019807843,0.627450980392157,0.172549019807843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\begin{groupplot}[group style={group size=2 by 2,  horizontal sep=1.5cm, vertical sep=2 cm}, scale = 0.4]
\nextgroupplot[
title = {\footnotesize Soleus, Original Parameters},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ylabel={\footnotesize Heat in \si{W}},
ymin=-75,ymax=150,xmin=0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
tick label style = {font=\footnotesize}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/thermo/sl/nomc}

\nextgroupplot[
title = {\footnotesize Soleus, Optimised Parameters},
tick align=outside, height = 6.5cm, width = 8cm,
tick pos=left,
x grid style={white!69.0198078431373!black},
xtick style={color=black},
y grid style={white!69.0198078431373!black},
ymin=-75,ymax=150,xmin=-0,xmax=100,
ytick style={color=black},
ylabel style={align=center},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick label style = {font=\footnotesize}
]
% \draw[dotted, semithick, gray!80!black] (12,-50) -- (12,80);
% \draw[dotted, semithick, gray!80!black] (54,-50) -- (54,80);
% \draw[dotted, semithick, gray!80!black] (71,-50) -- (71,80);
% \draw[dotted, semithick, gray!80!black] (85,-50) -- (85,80);
% \node[draw, scale=0.7] at (33,4) {$\leftarrow\rightarrow$};
% \node[draw, scale = 0.7] at (62,4) {$\rightarrow\leftarrow$};
% \node[draw,scale=0.7] at (78,4) {$\leftarrow\rightarrow$};
\input{plots/thermo/sl/mc}

\end{groupplot}

\end{tikzpicture}
